Adapting Behaviors via Reactive Synthesis

In the \emph{Adapter Design Pattern}, a programmer implements a \emph{Target} interface by constructing an \emph{Adapter} that accesses an existing \emph{Adaptee} code. In this work, we present a reactive synthesis interpretation to the adapter design pattern, wherein an algorithm takes an \emph{Adaptee} and a \emph{Target} transducers, and the aim is to synthesize an \emph{Adapter} transducer that, when composed with the {\em Adaptee}, generates a behavior that is equivalent to the behavior of the {\em Target}. One use of such an algorithm is to synthesize controllers that achieve similar goals on different hardware platforms. While this problem can be solved with existing synthesis algorithms, current state-of-the-art tools fail to scale. To cope with the computational complexity of the problem, we introduce a special form of specification format, called {\em Separated GR($k$)}, which can be solved with a scalable synthesis algorithm but still allows for a large set of realistic specifications. We solve the realizability and the synthesis problems for Separated GR($k$), and show how to exploit the separated nature of our specification to construct better algorithms, in terms of time complexity, than known algorithms for GR($k$) synthesis. We then describe a tool, called SGR($k$), that we have implemented based on the above approach and show, by experimental evaluation, how our tool outperforms current state-of-the-art tools on various benchmarks and test-cases.

==> Abstract_old.tex <==
%
%  \begin{abstract}
% (Dror 1) Reactive systems are systems that iteratively receive input and respond by emitting output. $GR(k)$ is a specific Linear Temporal (LTL) specification for reactive systems that is combined of $k$ constraints, each in an assume-guarantee form, over input and output variables. In this work we define and reason on \textit{Separated-$GR(k)$}. That is, a $GR(k)$ system in which the assumptions in every constraints are only of the environment variables and the guarantees of every constraints are only over the output variables.
% We first argue that although seems too specific, these separated specification can model scenarios of interest to the community. For example adapting or ``transferring" behaviors between two systems. As a specific example we give a reactive synthesis approach to the Adapter design pattern. We then solve the realizability and synthesis problem for Separated-$GR(k)$ and show how to exploit the separated specification structure to construct algorithms for realizability and synthesis that are better -complexity wise - than known algorithms for GR(k) synthesis.
% We finally implement these algorithms to a tool called $S{-}GR(k)$ and show by experimental evaluation how our tool beats current state-of-the-art tools on various benchmarks and test-cases.
% \keywords{Reactive Systems  \and Synthesis \and $GR(k)$}
%  \end{abstract}


% \begin{abstract}
% (Dror 2) The Adapter design pattern can be modeled in reactive systems settings as follows. 
% %We consider a variant of the adapter design pattern as follows. 
% Given two transducers: an $adaptee$ and a $target$, synthesize a third transducer called $adapter$ 
% such that the composition of $adaptee$ with $adapter$ produces the $target$. While this problem can be solved with reactive synthesis, general synthesis algorithms fail to scale even on small instances.
% In this work we introduce a special form of GR(k), called separated GR(k), for which we can propose much more efficient algorithms.
% In our model the transition graph turns out to be naturally separated into an input ``target'' component and an output ``adaptee'' component. In addition, we synthesize the adapter from a specification that is separated in nature and matches assumption on the target side to guarantees on the adaptee size. This format of a specification enables the synthesized adapter to ``transfer'' required behaviors, as specified by the user, between the target and the adaptee. 
% We solve the realizability and the synthesis problems for our model, termed Separated-$GR(k)$, and show how to exploit the separated nature of our structure to construct algorithms that are better -complexity wise - than known algorithms for GR(k) synthesis.
% We then implement these algorithms to a tool called $SGR(k)$ and show by experimental evaluation how our tool compares to current state-of-the-art tools on various benchmarks and test-cases.
    
    
% \end{abstract}


% \begin{abstract}
%     (Gal and Gera) Reactive synthesis is an automated procedure to obtain a correct-by-construction controller from its temporal specification. We propose a technique for a non-standard usage of reactive synthesis, inspired by the well-known \emph{Adapter design pattern}. 
%     In this design pattern, a programmer implements a \emph{Target} interface by constructing an \emph{Adapter} that accesses an existing \emph{Adaptee} code.
%     In our reactive interpretation to the adapter design pattern, we consider an existing \emph{Adaptee} active controller, and aim to synthesize an \emph{Adapter} controller that synchronizes with the adaptee controller, to achieve some \emph{Target} specification. This allows, e.g., to synthesize a controller that achieves same goals as the adapter on a different hardware, achieves goals that have not been covered by the adaptee controller execution, corrects safety violations of the adaptee controller etc.
    
%     Since reactive synthesis is infeasible (runs in $\Omega(2^N)$ time) in general, we  focus on GR($k$) specifications that link between possible behaviours of the Adaptee and Adapter controllers. Our framework, specifically the separation between the running components, enable us to improve synthesis of GR($k$) games from exponential to $O(N\log N)$ symbolic steps. We have implemented our technique into a tool SepGR($k$). Experiments we performed support the efficiency of our technique.
% \end{abstract}

\begin{abstract}
In the \emph{Adapter Design Pattern}, a programmer implements a \emph{Target} interface by constructing an \emph{Adapter} that accesses an existing \emph{Adaptee} code.  In this work, we present a reactive synthesis interpretation to the adapter design pattern wherein an algorithm takes an \emph{Adaptee} and a \emph{Target} transducers, and the aim is to synthesize an \emph{Adapter} transducer that, when composed with the {\em Adaptee}, generates a behavior that is equivalent to the behavior of the {\em Target}. One use of such an algorithm is to synthesize controllers that achieves similar goals on different hardware platforms.  While this problem can be solved with existing synthesis algorithms, existing state-of-the-art tools fail to scale.  
To cope with the computational complexity of the problem, we introduce a special form of specification format, called {\em Separated-GR($k$)}, that can be solved with scalable synthesis algorithm but still allows for a large set of realistic specifications. 
%In our model the transition graph turns out to be naturally separated into an input ``target'' component and an output ``adaptee'' component. In addition, we synthesize the adapter from a specification that is separated in nature and matches assumption on the target side to guarantees on the adaptee size. 
We solve the realizability and the synthesis problems for Separated-$GR(k)$, and show how to exploit the separated nature of our specification to construct algorithms that are better -complexity wise - than known algorithms for GR($k$) synthesis. We then describe a tool, called $SGR(k)$, that we have implemented based on the above approach and show, by experimental evaluation, how the tool outperforms current state-of-the-art tools on various benchmarks and test-cases.
\end{abstract}


% \begin{abstract}
%Gal version:
% In the \emph{Adapter Design Pattern}, a programmer implements a \emph{Target} interface by constructing an \emph{Adapter} that accesses an existing \emph{Adaptee} code.  In this work, we present a reactive synthesis interpretation to the adapter design pattern wherein the input is an \emph{Adaptee} and a \emph{Target} specification, and the aim is to synthesize an \emph{Adapter} transducer that, when composed with the {\em Adaptee}, generates a correct {\em Target} transducer. This interpretation allows e.g. to synthesize a controller that achieves same goals as the adaptee transducer on a different hardware, satisfy goals have not been covered by an adaptee execution, corrects safety violations of the adaptee etc.  While this problem can be solved with existing synthesis algorithms, existing state-of-the-art tools fail to scale even on small instances. To this end, we introduce a special form of GR($k$), called {\em Separated-GR($k$)} that connects behaviors of the adaptee and adapter transducers. We solve the realizability and the synthesis problems for Separated-GR($k$), and show how to exploit the separated nature of our structure to construct efficient algorithms, in terms of time complexity and performance, for GR($k$) synthesis. We then implement these algorithms to a tool called SGR($k$) and show by experimental evaluation how our tool compares to current state-of-the-art tools on various benchmarks and test-cases. 
% \end{abstract}


==> ConcRelated.tex <==
\section{Conclusion and related work}\label{sec:ConcRelated} \dftodo{Add further applications and ideas}
 
In this paper, we explored a reactive systems-based model of the adapter design pattern. We formalized the pattern to composition of transducers, reduced the problem of finding an adapter to synthesis of Separated-GR($k$) games, and used to the separation nature of the game to utilize a synthesis algorithm and tool that our performed current state-of-the-art tools.
 
 
The Adapter design pattern is designed... \dftodo{complete}



Reactive synthesis of LTL winning conditions was proved to be 2EXPTIME complete (in the size of the formula)~\cite{PnueliR89a}. To overcome this high-complexity lower bound, researchers identified fragments and variants for which more efficient reactive synthesis techniques exist, e.g. \cite{BloemJPPS12,AmramMP19,Ehlers11,Zielonka98,de2013linear}.
A specific fragment called GR($k$) which we exstensivley discuss in this work, and offers a balance between efficiency and expressiveness, was suggested by Bloem et al.~\cite{BloemJPPS12}. For efficiency, Piterman et al. noted that GR($k$) games are solved in time exponential in $k$ \dftodo{what is $k$} (rather than exponential in the state-space)~\cite{PitermanP06}. For expressivness, it is noted e.g. in~\cite{Ehlers11,MaozR16} that Globally-in-the-Future ($\ltlG \ltlF$) requirements allow to synthesize Deterministic B\"uchi properties (DBA properties). Dwyer et al.~\cite{DwyerAC99} identified 55  common LTL specification patterns, and Maoz et al.~\cite{MaozR16} noted that 53 out of those 55 patterns are DBA properties, and the addition of each pattern  to a specification adds, at most, three fresh Boolean variables to the game structure. Menghi et al.~\cite{MenghiTPGB19} identified common (parametric) robotic patterns, each is a DBA property as well. 


The idea of synthesizing a controller to compose to an existing system has been studied before, with different motivations and within different frameworks, e.g.~\cite{bansal2019synthesis,d2013synthesizing,ciolek2016interaction,berardi2003automatic,alur2016compositional,FLOV18}. Our work differs from these works in its variable separation feature that allows to efficiently synthesize controllers that achieve expressive requirements, i.e. GR($k$) winning conditions. In some sense, our work is analogous to K{\"{o}}nighofer et al.~\cite{KonighoferABHKT17}, who suggested to synthesize a \emph{shield} that corrects safety violations of the existing controller. Our approach, however, is mostly concerned about liveness adaptation of the existing controller behavior.


Separation of specifications to input and output component for better synthesis also found ground in Boolean Functional Synthesis. There \cite{CFTV18} showed a technique that makes use of separating every CNF clause into input and output components. Our work lies of course in the temporal logic setting. As observed, a key component in our work relies on a linear-time strategy to win weak B\"uchi games. This result can be derived from the literature. Loding and Thomas show how to reduce weak B\"uchi to weak parity~\cite{LodingT00}, and Chatterjee gave a linear time weak parity solution~\cite{Chatterjee08}. In fact, our weak B\"uchi solution can be seen as a symbolic variant of~\cite{Chatterjee08}.
Another major component in our work, that we call the \textit{delay property}, is that the system can still win by delaying any finite time and ignore the environment, before ``catching up" with the environment. In some sense this is reminiscent to the asynchronous model of reactive systems as described in~\cite{BNS18,PnueliR89,ScheweF06}, in which the algorithmic can be viewed as some form of our delay property. Preliminary work of ours however showed non-equivalence of the models.


 This work has opened several lines of explorations that we consider. As we mentioned, there is more than one way to reason on the concept of ``adapter", thus various formal models could differ. It is interesting to explore these variants, and also those that do not adhere the separated nature all the way through. That is to say, variants that translate to more general GR($k$) specification in which the separation appears in the transition problem, but not in the specification itself. 
 
 Another line of work is to consider LTL with separation of variables as a concept. Specifically consider general LTL specifications in form of conjuncts of $\phi\rightarrow\psi$ constraints where $\phi$ is only over the input variables and $\psi$ is only over the output variables. Proving whether such specifications are 2EXPTIME complete can highlight more on the nature of separated specifications.
 
 
 In our setting, the input and output systems are independent and each cannot restrict the actions of the other. Alternatively, one may suggest that the output system will take into account the $\I$-assignments. i.e, to take $\rho_\O$ to be an assertion over $\I \cup \O \cup \O'$ (rather than over $\O \cup \O'$). We do not know if such specifications can be synthesized efficiently, say in time polynomial in $N$.\dftodo{move this somewhere or merge}
 
 
 


%The idea of synthesizing a controller to compose to an existing system was proposed in K\"{o}nighofer et al.~\cite{KonighoferABHKT17}.
%\sbtodo{"proposed" is an incorrect word. There are lots of papers from FM/AI/PL/Robotics/SE which synthesize a (reactive) controller from LTL or GR($k$) specifications to compose into an existing set of systems. To name a few: My own POPL paper~\cite{bansal2019synthesis} and few others are ~\cite{kress2010automatic,d2013synthesizing,ciolek2016interaction,berardi2003automatic,alur2016compositional}. Research groups of Kress-Gazi, Richard Murray, George Pappas, etc have a lot of work on synthesis of compositional controllers in robotics and automation. In these works, the variables of the individual systems may or may not be separated. The way we differ from these works is that in all of these approaches the specification is not separated. In our work, we recognize that for a large class of scenarios, the specification can be separated. By doing so, we obtain algorithmic benefits, eventually leading to improved scalability - an issue most prior approaches encounter.}
%They suggested to synthesize a \emph{shield} that corrects safety violations of the existing controller and recovers to give the back control to the existing controller.  In sense, our approach is mostly about liveness adaptations, while shield synthesis is solely about safety corrections.
 

==> Experiments_old.tex <==
\section{Implementation and Evaluation}
\label{sec:experiments}



We have implemented our realizability check and synthesis techniques
%, given in Algorithm~\ref{algo:winning-strategy} (see Lemma~\ref{lem:win})
%and our synthesis technique, given in Algorithm~\ref{algo:winning-strategy}
into a prototype tool called \tool{}. The tool receives a game structure and a GR($k$) formula that separate variables as an input, and can check the realizability of the specification, following Algorithm~\ref{algo:sym-weak-buchi} (see Lemma~\ref{lem:win}), and further synthesize a winning strategy, following Algorithm~\ref{algo:winning-strategy}. This strategy combines the winning strategy of the Weak-B\"uchi game with a strategy for satisfying as many guarantees as possible within a winning SCC. 
%Although the latter could be implemented as a memory-less strategy, it includes memory in order to simplify the implementation\gatodo{I think we decided to reach the guarantees also in the theoretical presentation. To check later and change accordingly if needed}.
The winning strategy is represented by a collection of BDDs that compute the assignment of the primed output variables given the value of the unprimed inputs, unprimed outputs and primed inputs. The tool manipulates BDDs via the CUDD 3.0 package~\cite{CUDD}. 
%Our tool code is available open-source on (reference currently hidden for double-blind review) %\url{https://github.com/lucasmt/spectra-synt}.
%\sbtodo{Removed github repo link. Non-anonymous submissions will be desk rejected.}

%To validate our tool we \ganote{to complete...}

To evaluate our technique, we set the next research question.

\begin{description}
\item[RQ.]\label{research-qn} Is our technique efficient, in terms of running time?
\end{description}
%\gatodo{What about space consumption? since synthesis tome complexity id higher, do we need a second RQ? }
In the remainder of the section, we present experiments we performed to answer \hyperref[research-qn]{\textbf{RQ}}.

\subsubsection{Corpus}
We created a corpus that includes specifications created according to the three examples we discuss in Section~\ref{sec:modeling}.

\noindent\textbf{Toy Example.} We consider a parametric version of the toy example given in Section~\ref{sec:modeling} as follows. The input system controls variables $\mathcal T=\{t_1,\dots,t_n\}$, and the output system controls $\mathcal A=\{a_1,\dots,a_n\}$. We denote by $t_i$ (respectively, $a_i$) the state over $\mathcal T$ (respectively, $\mathcal A$)  that binary encodes the decimal value $i$. The input transitions are of the form $(t_0,t_i)$ and $(t_i,t_i)$, where $i>0$.  The output transitions are of the form $(a_0,a_{2i+1})$, $(a_{2i},a_{2i+1})$, $(a_{2i+1},a_{2i})$, and a single transition $(a_1,a_0)$ (see Section~\ref{sec:modeling} for $n=2$). We construct such toy example specifications for $n=1,\dots,10$, each we denote by $\sf{TE(\text{$n$})}$, a specification over $2n$ variables. Hence, our corpus includes 10 $\sf{TE}$ specifications.

\noindent\textbf{Cleaning Robots.} For $n=1,\dots,10$ we created a cleaning robots specification with $n$ rooms which we denote  by $\sf{CR({\text{$n$}})}$, a specification over $4n + 1$ variables. Hence, our corpus includes $10$ cleaning robots specifications. 

%\noindent\textbf{Rubik Cube.} Consider a broken cube that cannot be rotated to the left. We aim to transform instructions to a correct Rubik cube and to accordingly rotate the broken cube. Hence, the input system generates a sequence of configuration, each configuration is obtained by some rotation of the former configuration. We consider the case in which each of the cubes is rotated until one of its faces is solved. The controller we aim to synthesize rotates the broken cube, to arrange the same color solved in the correct cube. That is, the GR($k$) winning condition includes components e.g.: $F(\text{the correct cube's green face is solved})\rightarrow F(\text{the broken cube's green face is solved})$. For $n=2,3$, $\sf{Cube(\text{$n$})}$ denotes the specification for an $n\times n$-faces cube, a specification over ?? variables. Hence, our corpus includes 2 Rubik cube specifications.




\noindent\textbf{Railway Signalling.}
For $n=2,\dots,10$ and $m=2,3$, we created a railways specification denoted by $\sf{Railways(\text{$n,m$})}$, a specification over $(2+2\lceil \log m\rceil)n$ variables. Hence, our corpus includes 18 railway signalling specifications.

Overall, our corpus includes 38 specifications, all realizable.

\subsubsection{Experiment Setup and Results}
To address \hyperref[research-qn]{\textbf{RQ}}, we  compare the performance of our tool to the performance of a state-of-the-art synthesis tool. To this end, we chose the LTL synthesizer Strix as a reference~\cite{Strix}. Recently, Strix won first place in three out of four tracks of the reactive synthesis competition SYNTCOMP 2020. 

We apply both our tool and Strix to check the realizability of each specification in our corpus. We executed 10 iterations of each experiment with a timeout of 10 min.\footnote{Although our algorithm is deterministic, the automatic variable reordering of CUDD adds variance to the running times} To apply Strix over our specifications, we use the strict semantics from~\cite{Jacobs016} to transform a game structure and a winning condition into a corresponding LTL formula that characterizes the exact same winning plays.  
%We repeated each experiment 10 times,\footnote{Although our implemented method is deterministic, the default automatic variable reordering of CUDD adds variance to the running time} 
%with a timeout of ?? minutes. 

\begin{table}
    \centering
    \begin{tabular}{|c|c||c|c|c|c|c|c|c|c|c|c|}
    \hline
         \multicolumn{2}{|c||}{$n$} & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10   \\ \hline \hline

        \multirow{2}{*}{$\sf{TE(\text{$n$})}$} & \tool{} & 0.06 & 0.05 & 0.05 & 0.06 & 0.06 & 0.08 & 0.1 & 0.19 & 0.46 & 1.07 \\
         \cline{2-12}
         & Strix & 0.13 & 0.29 & TO & TO & TO & TO & TO & TO & TO & TO \\ \hline \hline

         \multirow{2}{*}{$\sf{CR(\text{$n$})}$} & \tool{} & 0.05 & 0.05 & 0.07 & 0.09 & 0.16 & 0.26 & 0.63 & 1.16 & 1.78 & 2.43 \\
         \cline{2-12}
         & Strix & 0.31 & 0.75 & 58.3 & TO & TO & TO & TO & TO & TO & TO \\
         \hline
         
         \hline \hline
         
        \multirow{2}{*}{$\sf{Railways(\text{$n,2$})}$} & \tool{} & - & 0.11 & 0.17 & 0.71 & 3.88 & 11.8 & 15.1 & 40.8 & 219 & TO  \\
         \cline{2-12}
         & Strix & - & 382 & TO & TO & TO & TO & TO & TO & TO & TO \\
         \hline
         
        \multirow{2}{*}{$\sf{Railways(\text{$n,3$})}$} & \tool{} & - & 0.07 & 0.36 & 1.67 & 8.39 & 29.8 & 50.3 & 102 & TO & TO \\
         \cline{2-12}
         & Strix & - & 381 & TO & TO & TO & TO & TO & TO & TO & TO \\
         \hline
         

         

 
    \end{tabular}
    
    \caption{Median Realizability Check Running Times (sec.)}
    \label{tbl:results}
\end{table}


% \begin{table}
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%          \multicolumn{2}{|c|}{$n$} & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10   \\ \hline \hline
%          \multirow{2}{*}{$\sf{CR(\text{$n$})}$} & \tool{} & 0.12 & 0.07 & 0.06 & 0.13 & 0.24 & 0.31 & 0.76 & 1.37 & 1.67 & 2.64 \\
%          \cline{2-12}
%          & Strix & 0.77 & 0.82 & 45 & 8594 & TO & TO & TO & TO & TO & TO \\
%          \hline
         
%         %  \hline \hline
%         %  \multirow{2}{*}{$\sf{Cube(\text{$n$})}$} & SGR($k$) & & & & & & & & & & \\
%         %  \cline{2-12}
%         %  & Strix & & & & & & & & & & \\
%         %  \hline
         
%                   \hline \hline
%          \multirow{2}{*}{$\sf{IE(\text{$n$})}$} & \tool{} & 0.07 & 0.1 & 0.07 & 0.1 & 0.08 & 0.09 & 0.12 & 0.2 & 0.47 & 1.07 \\
%          \cline{2-12}
%          & Strix & 0.21 & 0.31 & TO & TO & TO & TO & TO & TO & TO & TO \\
%          \hline
         
%          \hline \hline
         
%         \multirow{2}{*}{$\sf{Railways(\text{$n,2$})}$} & \tool{} & - & 0.05 & 0.16 & 0.82 & 4.28 & 10 & 18 & 39 & 275 & 421  \\
%          \cline{2-12}
%          & Strix & - & 91 & TO & TO & TO & TO & TO & TO & TO & TO \\
%          \hline
         
%         \multirow{2}{*}{$\sf{Railways(\text{$n,3$})}$} & \tool{} & - & - & 0.43 & 1.76 & 10 & 32 & 60 & 123 & TO & TO \\
%          \cline{2-12}
%          & Strix & - & - & TO & TO & TO & TO & TO & TO & TO & TO \\
%          \hline
         

         

 
%     \end{tabular}
    
%     \caption{Realizability Check Running Times (sec.)}
%     \label{tbl:results}
% \end{table}



\begin{figure}[b!]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[height=1in]{figures/cleaning-robots.pdf}
         \caption{Cleaning Robots}
         \label{fig:cleaning-robots}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[height=1in]{figures/intro-demo.pdf}
         \caption{Introduction Example} 
    \end{subfigure}
     ~ 
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[height=1in]{figures/railway-signalling.pdf}
         \caption{Railway Signalling}
         \label{fig:railway-signaling}
    \end{subfigure}
        \caption{Running time for the different classes of specifications.}
        \label{fig:running-time}
\end{figure}




In Table~\ref{tbl:results}, we present median running time results obtained for each specification and each tool (in sec.). The table rows refer to the benchmarks we examine, and the columns refer to the value of the parameter $n$. As an example, for the specification $\sf{CR(\text{3})}$, \tool{}'s median running time is 0.07 sec. (row titled $\sf{CR(\text{n})}$;\tool{}, column titled 3) and Strix's median realizability check running time is 58.3 sec. (row titled $\sf{CR(\text{n})}$;Strix), column titled 4). Cells reading `TO' indicate experiments reached a timeout. For every timed-out experiment, all 10 executions did not terminated, with a single exception: \tool{} successfully verified the realizability of $\sf{Railway(\text{10,2})}$ in 2 out 10 attempts.  Figure~\ref{fig:running-time} shows plots for the data in Table~\ref{tbl:results}. All experiments were executed on a single node of a high-performance computer cluster consisting of an Intel Xeon processor running at 2.6 GHz with 32GB of memory.
%We provide all raw results and means to reproduce the experiments in the paper's supporting materials~\cite{}.

We see that \tool{} performs and scales well. \tool{} reached a timeout only over rather complex specifications: $\sf{Railway(\text{10,2})}$ (2 out of 10 terminated), $\sf{Railway(\text{9,3})}$, and $\sf{Railway(\text{10,3})}$, over 40, 54 and 60 variables, respectively. For all other specifications, \tool{} returned in less than 4 min. Importantly, \tool{} enables to handle specifications that Strix failed to process. \tool{} successfully verified the realizability of 36 out of the 38 specifications we consider, and coped with 35 in all its 10 attempts. Strix managed to cope with only 7 of the specifications. Since these results might depend on the timeout we chose, we decided to explore better this key attribute. We applied Strix and \tool{} over the specifications they failed to process in all their 10 attempts again, with higher timeouts: 8 hours for Strix, and 1 hour for \tool{}. All those executions reached the higher timeout we set, and did not return.  We conclude that our technique is efficient for specifications in the {\em Separated-GR($k$)} format.











%\begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.8\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/cleaning-robots.pdf}
%         \caption{Cleaning Robots}
%         \label{fig:cleaning-robots}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.8\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/intro-demo.pdf}
%         \caption{Introduction Example}
%         \label{fig:intro-demo}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.8\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/railway-signaling.pdf}
%         \caption{Railway Signalling}
%         \label{fig:railway-signaling}
%     \end{subfigure}
%        \caption{Running time for the different classes of specifications.}
%        \label{fig:running-time}
%\end{figure}


==> Explicit.tex <==
\section{Algorithms for Solving Separated GR($k$) Games}
\label{sec:algorithmsWeakBuchi}

Following our central result of  reduction of separated GR($k$) games to weak B\"uchi games presented in Section~\ref{sec:reduction}, this section presents a complete algorithm to solve separated GR($k$) games. By now, we know that the algorithm involves two steps: First, to obtain a weak B\"uchi game from the input separated GR($k$) by identifying  the SCCs. Second, to solve the resulting weak B\"uchi game. Since the input separated GR($k$) game is represented symbolically, the central requirement of our algorithm is to solve the above two steps symbolically. 
To this end, this section begins with an algorithm for separated GR($k$) games when they are  represented in an explicit-state representation in Section~\ref{sec:explicitweakbuchi}. 
%To this end, we begin with this sections begins by reviewing a linear-time algorithm to solve weak B\"uchi games when represented with explicit states in Section~\ref{sec:explicitweakbuchi}. 
Later, Section~\ref{sec:symbolicweakbuchi} will adapt the explicit-state algorithm to the desired symbolic state representation. 



\subsection{Explicit State Representation}
\label{sec:explicitweakbuchi}



For sake of exposition, we present the algorithm when the separated GR($k$) game is represented explicitly. We observe that the algorithm is only {\em linear} in the size of the game when it is represented explicitly. 
%This is an improvement over GR($k$) games, which are solved in quadratic time in the state 

%Weak B\"uchi games have previously been studied when the states of the game are represented explicitly. Under this state representation, weak B\"uchi games can be solved in linear-time to the size of the explicit graph underlying the game~\cite{Chatterjee08}). 
%(use the reduction from weak B\"uchi to weak parity~\cite{LodingT00}, and apply an algorithm by  Chatterjee~\cite{Chatterjee08}). 
%This section reviews that algorithm.

\subsubsection{Game description in explicit-state representation.} 

A game with game structure $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and a winning condition can be equivalently represented by a game between the system and environment player on  directed graph $ (V,E)$. The states on the graph are given by states over $\I\cup\O$ and there is a directed edge from state $s$ to state $t$ in the graph if $(s,t')\models \rho_\I\wedge\rho_\O$. Recall, we assume that all states of a game structures are deadlock-free. Thus, there is at least one outgoing edge from every state in directed graph $(V,E)$.
States that satisfy $\theta_\I\wedge\theta_\O$ are the initial states of the graph. 
The game proceeds by the environment player assigning values to the input variables $\I$ and the system player assigning values to the output variables $\O$.  
The game starts at one of the initial states of the graph. 
In every round of the game, first the  environment chooses an assignment to the $\I$ variables, and then the system will choose an assignment $O$ to the $\O$ variables.
The combined assignment $I \cup O$ determines the unique state  the game moves to. \gatodo{to review the previous sentences}
The notions of plays, strategies, winning conditions, and so on naturally transfer to the explicit-state representation. 





%For readability, we also consider an explicit representation of the game between the environment and the system. Given a game structure  $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$, we define a graph that serves as a ``game-board" as follows. $G^{\mathit{GS}}=(V^\mathit{GS},E^\mathit{GS})$, where $V^\mathit{GS}=2^{\I\cup\O}$, and $(\inp_0,\out_0)E(\inp_1,\out_1)$ if $\big((\inp_0,\out_0),(\inp_1',\out_1')\big)\models \rho_\I\wedge \rho_\O$.
%At the beginning of a play, the environment chooses $\inp\in 2^\I$, the system then responds with $\out\in 2^\O$, and thus the first state of the play is $(\inp,\out)\in V^{\mathit{GS}}$. Afterwards, the payers repeatedly choose the next state of the play: form state $(\inp_0,\out_0)$ the environment chooses $\inp_1\in 2^\I$ such that $(\inp_0,\out_0,\inp_1')\models \rho^e$, the system replies with $\out_1$ such that $(\inp_0,\out_0,\inp_1',\out_1')\models \rho_\O$, and the play traverses to state $(\inp_1,\out_1)$.  Note that the notions of plays, strategies etc. naturally transfer to the explicit representation. We omit the straightforward adaptation of those notions in the explicit context. 

A {\em strongly connected component} (SCC) of a directed graph $(V,E)$ is a maximal set of states within which every state is reachable from every other state.  It is well known that SCCs partition the states of a directed graph. 

Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
Then, the defining feature of a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$ is as follows: Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all of its states are contained in $\F$ or  {\em non-accepting components} meaning none of its states is present in $\F$. 
Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a play in the directed graph is winning for the system if the play ultimately never exits an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every play will ultimately remain inside an accepting component.

%A \textit{subgraph} $G_0$ of a directed graph $G=(V,E)$ is a graph $(V_0,E_0)$ where $V_0\subseteq V$ and $E_0= E\cap (V_0\times V_0)$. 
%\textit{A path} in a graph $G=(V,E)$ is a sequence $(v_0,\cdots v_i)$ such that for all $0\leq j<i$, $(v_j,v_{j+1})\in V$. Note that a single vertex is also considered as a path.
%A \textit{strongly connected component} (SCC) in a graph $G=(V,E)$, is a maximal subset $V_0\subseteq V$ such that for every vertices $v,v' \in V_0$, there exists a path from $v$ to $v'$ in $G$. Note that the set of all SCCs forms a partition of the graph-vertices.
%An SCC, $S$ is a \emph{terminal SCC} if for every $s\in S$ the next holds: if a state $t$ is reachable from $s$, then $t\in S$.

%We exploit the special structure of the weak B\"uchi automaton to solve this game more efficiently than a typical Parity game or B\"uchi game. 


\subsubsection{Algorithm in explicit-state representation.} 


Given a separated GR($k$) game $(\GS, \psi)$, we have already proven that the weak B\"uchi game over $(\GS, \ltlG\ltlF\varphi)$ where $\ltlG\ltlF\varphi= $ is such that the two games are equirealizable (Section~\ref{}). 
Let the separated GR($k$) game be explicitly represented over the directed game $(V,E)$. Then, in this section, we prove that separated GR($k$) game over directed graph $G = (V,E)$ is solved in $\O(|V|+|E|)$.

The first step is to generate the underlying weak B\"uchi game on $G=(V,E)$. The SCCs of $G$ can be identified in  $\O (|V|+|E|)$ time using the standard DFS-based algorithm. The challenge, however, is to identify which of these SCCs are accepting and which are non-accepting. 
The naive approach would be to generate the set $\F$ from $\varphi$, where $\ltlG\ltlF\varphi$ is the winning condition of the weak B\"uchi game, and determine whether $S_i\cap \F = \emptyset$ or $S_i\subseteq \F$ for every SCC $S_i$. This step is, however, expensive as the construction of $\F$ is exponential in the number of variables in $\I\cup\O$. 
To this end, we observe that a sufficient condition for an SCC to be accepting or non-accepting is for any one of its states to be accepting or non-accepting, respectively. Thus, for each SCC $S_i$, choose any one state $s_i \in S_i$. Since $s_i$ also represents an assignment over the $\I\cup\O$, evaluate $s_i \models \varphi$.  
Then the SCC $S_i$ is accepting if $s_i \models \varphi$ and non-accepting, otherwise. Since there are at most $|V|$ SCCs in graph $G$, the complexity of this step is $\O (|V|)$ (assuming the evaluation of $s_i\models \varphi$ is a constant time operation). Therefore, we have identified all the accepting and non-accepting SCCs of $G = (V,E)$ in $\O (|V|+|E|)$ time.

The next step is to solve realizability and synthesis on the weak B\"uchi game generated in the previous step. For this we use an exisiting linear-time algorithm for weak B\"uchi games~\cite{Chatterjee08}. For sake of completeness, we review the algorithm here:

\begin{theorem}[\cite{Chatterjee08}]
\label{Thrm:WeakBuchi}
Let a weak B\"uchi game be explicitly defined over directed graph $G = (V, E)$ with winning condition $\ltlG\ltlF\varphi$ where $\varphi$ is an assertion over input variables $\I$ and output variables $\O$ . 
The realizability and synthesis of the weak B\"uchi game are solved $\O(|V|+|E|)$ time. 
\end{theorem}

\paragraph{Algorithm description.}
We are given a weak B\"uchi game over $(V,E)$ with winning condition $\ltlG\ltlF\varphi$ in explicit state representation. As described earlier, the accepting and non-accepting SCCs can be identified in $\O(|V| + |E|)$.


Let $\Statess_0, \dots \Statess_m$ be the SCCs partitioning the directed graph $(V,E)$. W.l.o.g.,  let $\Statess_1>\Statess_2>\dots >\Statess_m$ with respect to the partial order $>$ induced by the topological sorting of the SCCs. 



\begin{description}
    \item[Base case:] %\gatodo{currently, the inductive process constructs the winning region. We also need to construct a memory-less strategy. A minor modification is needed for that...}
    $\Statess_m$ is a {\em terminal partition}, i.e., are no outgoing edges from $\Statess_m$. 
    
    By definition, plays beginning in any state of $\Statess_m$  will never leave it and be of infinite length. 
    Thus, if $\Statess_m$ is an accepting component, every state is a winning state for the system, while if $\Statess_m$ is a non-accepting component every state is a winning state for the environment.
    
    \item[Induction step:]
    Suppose all states in 
    $\Statess_{i+1}, \ldots, \Statess_m$ have been classified as winning for the system and environment, we determine which states in $\Statess_i$ are winning for each player.
    Due to the DAG-like structure induced by SCCs, the states in $\Statess_{i+1}$ to $\Statess_m$
    can be collapsed into two sink states, one winning for the system and the other winning for the environment. Then, all states in $\Statess_i$ can only reach other states in $\Statess_i$ or one of the two sink states. 
    
    Suppose, $\Statess_i$ is an accepting component. 
    Then, a state in $\Statess_i$ is winning for the system if it can either force plays to stay inside $\Statess_i$, or force the play to reach the accepting sink. 
    Alternately, a state is losing for the system if the environment can force plays into the losing sink. The losing states for the system can, thus, be computed by playing a reachability game with the losing sink as the reachability objective. Due to determinacy, the remaining states in $\Statess_i$ will be winning for the system. The strategy for the system from these winning states would be the one that enables it to remain inside these newly discovered winning states of go to the accepting sink.  
    
    %\gatodo{Since we also aim to construct a strategy, and not just to identify the winning region, it makes things simpler if we analyse the case (also) from the system perspective. We can add e.g.: Hence, in the accepting partition case, the system wins from its winning region w.r.t. $\mathit{safe}(Q_i\cup W)$, where $W$ are the winning states identified so far. Note that the system player can apply the following memory-less strategy. Play to win w.r.t. $\mathit{safe}(Q_i\cup W)$. If the play reaches $W$, apply the memory-less strategy from $W$.}
    
    Suppose, $\Statess_i$ is a non-accepting component. 
    Then, a state is winning for the system if it can force plays into the winning sink. 
    These states can be computed by playing a reachability game with the winning sink as the reachability objective. This will also determine the winning strategy for the system from these states.  
\end{description}

    Recall, reachability games can be solved in linear time. Thus, the complexity of the induction step on $\Statess_i$ is $\O(|\Statess_i|+|E_i|)$, where $E_i$ is the set of edges in $\Statess_i$. Furthermore, the identification of accepting and non-accepting SCCs and topological ordering of SCCs can be determined in $\O(|V|+|E|)$. 
    Thus, realizability and synthesis in weak B\"uchi games is solved in  $\O(|V|+|E|)$ where $(V,E)$ is the directed graph.

\begin{theorem}
\label{thrm:explicitalgorithm}
Realizability and synthesis on a separated GR($k$) game explicitly defined over a directed graph $G=(V,E)$ with winning condition $\psi$ is solved in $\O(|V|+|E|)$.
\end{theorem}
\begin{proof}
The proof is already present in the description of the two steps to solve separated GR($k$) games. Since each steps takes $\O(|V|+|E|)$ time to complete, the total complexity for synthesis and realizability is $\O(|V|+|E|)$.
\end{proof}

%There are a few interesting observations to weak B\"uchi games. First, note that not all states of an accepting partition are winning for the system and analogously not all states in a non-accepting partition are losing for the system. Note, additionally, that the algorithm described in Theorem~\ref{Thrm:WeakBuchi} necessarily need to be processed linearly. For example, if $Q_1$ only has transitions to $Q_3$ and $Q_4$, then the reachability game on $Q_1$ can be solved as soon as $Q_3$ and $Q_4$ are partitioned, even if $Q_2$ has not been partitioned yet. This allows for some degree of parallelism determined by the topology of the graph induced by the SCCs. In this case, for example, the reachability games for $Q_1$ and $Q_2$ could be solved in parallel. This may lead to significant speedups depending on the structure of the state space. \gatodo{I like the first observation. It helps the reader to see the full-picture. Not sure about the second... it is nice, but maybe too much... }

\begin{comment}
\subsubsection{Connected partition problem to weak B\"uchi games \gatodo{to omit?}}

We begin by describing the the connected partition problem under explicit state representation. 
Let $G$ be the product of the graphs $G_\I$ and $G_\O$, induced by the inputs $(I, \rho_\O)$ and $(\O,\rho_\O)$, as described in Section~\ref{Sec:graphdescription}. By abuse of notation, let $X$ also be an explicit state representation of the union of the SCCs. Then the winning condition for the system is $FG(X)$, i.e., the objective of the system is to  ensure that all plays of the game will eventually never leave the set $X$.
A state $q$ in the graph $G$ is said to be {\em winning for the system} if there exists a strategy for the system such that all plays beginning in $q$ 
satisfy the winning condition. A state $q$ is said to be {\em losing for the system} if for all strategies of the system, the environment can ensure that the winning condition is not satisfied.
Then, solving the connected partition problem is equivalent to determining whether there exist initial states of $G$ that are also winning states for the system.


The core insight of our solution is that the connected partition problem induces a weak B\"uchi game. 
To see how, recall that SCCs partition a graph and induce a DAG-like structure on it. Specifically, the graph $G$ can be interpret as a weak B\"uchi automaton as follows: Let $Q_1$,\dots $Q_m$ be the partitioning of the states of graph $G$ where every $Q_i$ is a distinct SCC. Then, due to the partitioning of the states in $G$ by SCCs, a partial order $>$ gets induced between the $Q_i$s due to the underlying DAG-like structure. In particular, for all $i$,$j$, $Q_i > Q_j$ if there exists a transition 
%Addressed. Having a transition is sufficient since if transiton exists then paths will also exist \gatodo{path, right?} 
from a state $q_i\in Q_i$ to state $q_j\in Q_j$.
Now, define the accepting states be the states in $X$. Since $X$ is a union of SCCs, by virtue of our assignment of accepting states, either all states in a given partition are accepting or all are non-accepting. Hence, the partitioning induced by the SCCs and assignment of states in $X$ as accepting, we obtain  a weak B\"uchi automaton. 
The connected partition problem is, therefore, equivalent to solving a game on a weak B\"uchi automaton in which the winning condition for the system is to eventually-globally visit its accepting states.

\begin{theorem}
\label{thrm:connectedpartitionexplicit}
In explicit state representation, the connected partition problem is solvable in linear time in size of the graph.
\end{theorem}
\begin{proof}
Each step of solving the connected partition problem, namely, computation of SCCs, topological sorting of the partitions, and solving the weak B\"uchi game are linear in the size of the underlying graph. Thus, connected partition problem is solved in linear time in size of the graph. 
\qed
\end{proof}

\end{comment}

\subsection{Symbolic State Representation}
\label{sec:symbolicweakbuchi}

This section presents an algorithm to solve separated GR($k$) games when represented symbolically as in Definition~\ref{def:separatedGRk}. From Theorem~\ref{}, we know it trivially reduces to a weak B\"uchi game. The task, therefore, is to present an algorithm for weak B\"uchi games when presented symbolically. More specifically, we design a BDD based algorithm to solve a weak B\"uchi game $(\GS,\ltlG\ltlF \varphi)$ where the assertions in the game structure $\GS = (\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and the assertion $\varphi$ are given in the form of a BDDs. 

\subsubsection{Realizability}
To solve realizability, the goal is to compute a BDD for the winning region of the weak B\"uchi game and then to determine whether the initial states of the game intersects with the winning region. The construction of the winning region follows a fixed-point computation that adapts the inductive algorithm presented in  Section~\ref{sec:explicitweakbuchi}: In the basis of the fixed point computation, the winning region is the set of accepting and terminal SCCs; In the inductive step, the winning region includes winning states by examining SCCs that are higher in the topological ordering on SCCs. %There are several challenges in executing the fixed-point algorithm outlined here.  

\newcommand{\SCC}{\mathsf{\mathsf{SCC}}}
\newcommand{\Reach}{\mathsf{\mathsf{Reach}}}
\newcommand{\Reachinverse}{\mathsf{\mathsf{Reach}^{-1}}}
\newcommand{\Path}{\mathsf{\mathsf{Path}}}
\newcommand{\terminal}{\mathsf{\mathsf{Terminal}}}
\newcommand{\C}{\mathsf{\mathsf{DC}}}
\newcommand{\pre}{\mathsf{\mathsf{pre}}}
\newcommand{\winning}{\mathsf{\mathsf{Win}}}
\newcommand{\winningAux}{\mathsf{\mathsf{Win\_Aux}}}
\newcommand{\Reachability}{\mathsf{\mathsf{Reachability}}}
\newcommand{\Safety}{\mathsf{\mathsf{Safety}}}



\newcommand{\X}{\mathit{X}}
We begin with introducing necessary notation.
Let $B(\V)$ be a BDD defined over the ordered set of variables $\V = \{v_1, \ldots, v_n\}$. Let $W = \{w_1, \ldots, w_n\}$ be a new, ordered set of variables of the same cardinality. We use $B(W)$ to denote the BDD in which every variable $v_i$ is replaced with the corresponding variable $w_i$. We can extend this to a BDD $B(\V_1, \ldots, \V_m)$ over multiple sets $ \V_1, \ldots \V_m$ of variables in the natural way. 
Given an ordered set of variables $\V = \{v_1, \ldots, v_n\}$, we use $\V'$ to denote the ordered set of new variables $\V' = \{v'_1, \ldots, v'_n\}$.
We use the notation $\X$ to denote an ordered set of variables over $\I\cup\O$. 


\paragraph{BDD for SCCs.} We want to construct a predicate which indicates when two states in a game structure are present in the same SCC. Let us begin with predicate $\Reach(s,t')$ that holds if there is a path from state $s$ over $\I\cup\O$ to state $t$ over $\I\cup\O$ in the game structure $\GS$. Then, $\Reach$ is the fixed point computed iteratively as follows:


\begin{itemize}
    \item $\Path^{0}(\X, \X'):= (\I = \I') \wedge (\O = \O') $
    \item $\Path^{i+1} (\X,\X') := \exists  X'': (\rho_I\wedge \rho_O)(X,X'') \wedge \Path^{i} (X'',X')$
\end{itemize} 

Thus, a BDD for predicate  $\Reach$ is computed in $O(N)$ symbolic operations.
Similarly, let predicate 
$\Reachinverse(s,t')$ hold if there is a path from state $t$ over $\I\cup\O$ to state $s$ over $\I\cup\O$. Then  $\Reachinverse(s,t')$ holds iff $\Reach(t,s')$ holds. By a similar construction, a BDD for $\Reachinverse$ is constructed in $\O(N)$ symbolic operations. 

Then, define predicate $\SCC(s,t')$ to hold if states $s,t$ over $\I\cup\O$ are present in the same SCC in the game structure $\GS$. It is easy to see the following:  \[\SCC(\X,\X') := \Reach(\X,\X') \wedge \Reachinverse(\X,\X')\]

Therefore, a BDD for $\mathsf{SCC}$ is constructed in  $\O(N)$ symbolic operations. 




\paragraph{BDD for Terminal SCC.}
The induction basis for the construction of a winning region requires us to know what the terminal SCCs are. Let predicate $\terminal (s)$ hold if state $s$ over $\I\cup\O$ is present in a terminal SCC. Then
\[\terminal(\X) := \forall \X': \Reach(\X,\X')\rightarrow \SCC(\X,\X')
\]

Therefore, given BDDs for $\mathsf{Reach}$ and $\mathsf{SCC}$, the construction of $\mathsf{Terminal}$ requires $\O(1)$ symbolic operations. 

\paragraph{BDD to obtain SCCs higher in the topological ordering.}   
The induction step in the construction of the winning region requires us to know how to compute the {\em predecessor} SCCs w.r.t. to the topological ordering on the SCC.


Let $C$ be a set of SCCs over the game structure. For a state $s$ over $\I\cup\O$, let $s\models C$ be the shorthand for ``there exists an SCC $S\in C$ such that $s\models S $".
A set of SCCs $C$ is said to be {\em closed downwards} if for every state $s \models C$, for every state $t$ that is reachable from $s$, $t\models C$. If $C$ is closed downwards, then its predecessor, denoted $\mathit{pre}(C)\supseteq C$,  is  a set of SCCs  such that if $S$ is an SCC in $\mathit{pre}(C)$, states $s\models S$ and there exists a path from $s$ to  state $t$, then either $t\models S$ or $t\models C$. Note that $\mathit{pre}(C)$ is also closed downwards.
Observe that predicate $\terminal$ denotes a downward closed set of SCCs. 

Let predicate $\C$ over $\X$ denote a downward closed set of SCCs. Then, from the definition, we see that its predecessor $\pre(\C)$ can be obtained as follows:
\[
\pre(\C) := \forall \X': \Reach(\X,\X') \rightarrow (\SCC(\X,\X') \vee \C(X'))
\]

Then, a BDD for the predecessor of a $\pre(\C)$ is computed in $\O(1)$ symbolic operations, given a BDD for $\Reach$, $\SCC$, and the downward closed set $\C$.

\paragraph{Computing the Winning Region.}
Equipped with BDDs for $\SCC$, $\terminal$, and $\pre(\C)$ for a downward closed set of SCCs $\C$, we can finally describe the fixed-point computation to construct a BDD for the winning region in  a weak B\"uchi game. Recall, the game is defined over game structure $\GS=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and has a winning condition is given by $\ltlG\ltlF\varphi$. We assume, all assertions in $\GS$ and assertion $\varphi$ are given as a BDD in the input. 

Let $\Reachability(A,B)(\X)$ denote a BDD that takes as input a set of source states $A$ and target states $B$, and outputs those states in $A$ from which the system can guarantee to move into $B$. The BDD  for $\Reachability(A,B)$ is generated by solving a reachability game. Details can be found in ~\cite[Chapter~20]{2001automata}.


Let $\Safety(A,B)(\X)$ denote a BDD that takes as input a set of source states $A$ and target states $B$, and outputs those states in $A$ from which the system can guarantee that all plays remain inside the set $B$. $\Safety(A,B)(\X)$ is  generated by solving a safety game. 
Details can be found in ~\cite[Chapter~20]{2001automata}.


Then, let  $\winning(s)$ denote that state $s$ over $\I\cup\O$ is in the winning region. Then, $\winning$ is the fixed point of $\winningAux$ which is defined below. The construction essentially follows the algorithm presented in Section~\ref{sec:explicitweakbuchi}:
\begin{description}
    \item{\textbf{Base Case.}} $\winningAux^0(\X) := \terminal(\X) \wedge \varphi(X)$ and
    $\C^0(\X) := \terminal(\X)$
    
    \item {\textbf{Inductive Step.}} $\C^{i+1}(\X) := \pre(\C^i(\X))$.
    
    Then, a state in $\C^{i+1}(\X)$ is winning if the system can force to move into the region $\winningAux^i(\X)$. This set of states can be obtained from $\Reachability(\C^{i+1}(\X), \winningAux^i(\X))$. 
    
    Otherwise, a state in   $\C^{i+1}(\X)$ is winning if the system can force all plays in  $\C^{i+1}(\X)$ to remain in states in $A(\X) = \C^{i+1}(\X)\setminus\C^i(\X)$ that accept $\varphi$ or satisfy $\winningAux^i(\X)$. This set of states can be obtained from $\Safety(\C^{i+1}(\X), \winningAux^i(\X) \vee (\C^{i+1}(\X)\wedge \neg \C^{i}(\X)\wedge\varphi(\X)))$. 
    
    Finally, every state in $\winningAux^i(\X)$ is also winning.  Then, 
    \begin{align*}
    \winningAux^{i+1}(\X) & :=        \winningAux^i(\X) \\
    & \vee \Reachability(\C^{i+1}(\X), \winningAux^i(\X)) \\
    &  \vee  
    \Safety(\C^{i+1}(\X), \winningAux^i(\X) \vee (\C^{i+1}(\X)\wedge \neg \C^{i}(\X)\wedge\varphi(\X)))
    \end{align*}
  
\end{description}


Finally, we prove Theorem~\ref{Thrm:WeakBuchi}.
\begin{proof}[Proof Sketch of Theorem~\ref{Thrm:WeakBuchi}]
The proposed construction symbolically implements the inductive procedure from Section~\ref{sec:explicitweakbuchi}. Hence, it correctly identifies the system's winning region. 

It remains to show that the algorithm performs $O(N)$ symbolic operations. First, of all, the constructions of $\SCC$ and $\terminal$ take $\O(N)$ symbolic operations collectively. Give a downward closed set $\pre$ takes a $\O(1)$ symbolic operations. Hence, it sufficient to show that in the $i$-th induction step, solving the reachability and safety games  performs  $O(|\pre(\C^{i+1})\setminus\C^i|)$ operations. This can be proven by a careful analysis of the operations and the sizes of resulting BDDs using standard results on safety and reachability games. Details have been deferred to the Appendix.\qed 
\end{proof}

\subsubsection{Winning Strategy Extraction.} Since the algorithm solves reachability and safety games internally, the winning strategies of those games can be composed to generate a winning strategy to the weak B\"uchi game. Details have been deferred to the Appendix.

\begin{comment}
We are ready to modify the explicit strategy construction depicted in Section~\ref{subsec:dfa-game} into a symbolic one. The idea is to follow the outlined inductive procedure, while representing the relevant SCCs symbolically. 

We start with a technical construction that allows to replace variables with their primed version (or vice-versa).


Let $\beta$ be a BDD whose domain includes the the variable-sets $\V_1,\dots,\V_n$. We denote the BDD obtained from $\beta$ by replacing each $\V_i$ with $\V'_i$ by $R_{(\V_1\rightarrow\V_1',\dots,\V_n\rightarrow\V_n')}(\beta)$.
Our first goal is to show how to determine, symbolically, that two states belong to the same SCC.

\begin{lemma}
\label{lem:beta_SCC}
Let $\mathit{GS}= (\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ be a game structure.  There exists a BDD $\beta_{\mathit{SCC}}$ over $\I,\O,\I',\O'$ such that $\beta_{\mathit{SCC}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $(\inp_0,\out_0)$ and $(\inp_1,\out_1)$ belong to the same SCC. Moreover, $\beta_{\mathit{SCC}}$ can be computed in $O(N)$ symbolic operations. 
\end{lemma}

\begin{proof}
We construct a BDD $\beta_{\mathit{Reach}}$ over $\I,\O,\I',\O'$ such that $\beta_{\mathit{Reach}}(\inp_0,\out_0,\inp_1',\out_1')$ if there exists a path from $(\inp_0,\out_0)$ to $(\inp_1,\out_1)$ in $G^\mathit{GS}$. To this end, we repeatedly construct BDDs $\beta^0,\beta^1,\dots$ over $\I,\O,\I',\O'$ such that $\beta^i(\inp_0,\out_0,\inp_1,\out_1)$ if  there exists a path of length at most $i$ from $(\inp_0,\out_0)$ to $(\inp_1,\out_1)$. This process ends when $\beta^i = \beta^{i+1}$, and then we have $\beta_{\mathit{Reach}}=\beta^i$. Those are computed as follows:
\begin{itemize}
    
    \item $\beta^0$ is defined by $(\I=\I') \wedge (\O=\O')$.
    
    
    %\item $\beta^{i+1}(\inp_0,\out_0,\inp_1,\out_1) \Longleftrightarrow  (\exists \inp_2,\out_2\in \I\times\O\big( \beta^i(\inp_0,\out_0,\inp_2',\out_2') \wedge (\inp_2,\out_2,\inp_1',\out_1')\models (\rho_\I\wedge\rho_\O)\big))\vee \beta^i$.
    
    %\item To construct $\beta^1,\beta^2\dots$, we construct BDD $\rho$ over $\I',\O',\I'',\O''$ such that $\rho_{\mathit{copy}}(\inp_0',\out_0',\inp_1'',\out_1'')$ if $(\inp_0,\out_0',\inp_1',\out_1')\models \rho_\I\wedge \rho_\O$.
    
    %Now, Construct a BDD $\gamma^i$ over $\I',\O',\I'',\O''$ such that $\gamma(\inp_0',\out_0',\inp_1'',\out_1'')$ if $\beta(\inp_0,\out_0,\inp_1',\out_1')$. Construct a BDD $\delta^{i+1}$ over $??$ by   $\beta^i\wedge \I=\I''$ 
    
    \item $\beta^{i+1}$ is constructed as follows. Use replacement to construct a BDD $\rho$ over $\I,\O,\I'',\O''$ such that $\rho(\inp_0,\out_0,\inp_1'',\out_1'')\Longleftrightarrow (\inp_0,\out_0,\inp_1'\out_1')\models\rho_\I\wedge \rho_\O$. Construct a BDD $\gamma$ over $\I,\O,\I',\O',\I'',\O''$ by $\beta^i \wedge \rho$, and a BDD $\delta$ over $\I,\O,\I'',\O''$ by $\exists\I',\O'(\gamma)$. Note that $\delta(\inp_0,\out_0,\inp_1'',\out_1'')$ iff there exists a path from $(\inp_0,\out_0)$ to $(\inp_1,\out_1)$ of length $\l\in\{1,\dots,i+1\}$.
    Finally, $\beta^{i+1}$ is constructed by $R_{(\I''\rightarrow \I',\O''\rightarrow \O')}(\delta)\vee \beta^0$.
    
\end{itemize}

Hence, $\beta_{\mathit{Reach}}$ is computed in $O(N)$ symbolic operations. Likewise, we compute in $O(N)$ symbolic operations a BDD $\beta_{\mathit{Reach}^{-1}}$ over $\I,\O,\I',\O'$, satisfying $\beta_{\mathit{Reach}^{-1}}(\inp_0,\out_0,\inp_1',\out_1')$ if there exists a path in $G^\mathit{GS}$ from $(\inp_1,\out_1)$ to $(\inp_0,\out_0)$. Clearly, $\beta_{\mathit{SCC}} = \beta_{\mathit{Reach}} \wedge \beta_{\mathit{Reach}^{-1}}$.\qed
\end{proof}

To perform the induction basis, we identify all terminal SCCs in $O(1)$ symbolic operations.


\begin{lemma}
\label{lem:beta_ter}
Let $\mathit{GS}= (\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ be a game structure.
Then, given the BDDs constructed above we can construct a BDD $\beta_{\mathit{ter}}$ over $\I,\O$ in $O(1)$ symbolic operations such that $\beta_{\mathit{ter}}(\inp,\out)$ iff $(\inp,\out)$ belongs to a terminal SCC.
\end{lemma}
\begin{proof}
During the construction of $\beta_{\mathit{SCC}}$, we constructed a BDD $\beta_{\mathit{Reach}}$ over $\I,\O,\I',\O'$ that satisfies $\beta_{\mathit{Reach}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $(\inp_1,\out_1)$ is reachable from $(\inp_0,\out_0)$. Then, $\beta_{\mathit{ter}}$ is constructed by $\forall \I',\O' (\beta_\mathit{Reach}\rightarrow \beta_\mathit{SCC})$.\qed
\end{proof}





To apply the induction step our next goal is to compute the ``predecessor" SCCs of a downwards closed set of  SCCs.

\begin{definition}
Let $X$ be a set of SCCs.
\begin{enumerate}
    \item $X$ is closed downwards if for any $s\in X$, every state reachable from $s$ is also a member of $X$.
    
    \item If $X$ is closed downwards, then its predecessor is  a set of SCCs $\mathit{pre}(X)\supseteq X$  that satisfies: if $S\subseteq \mathit{pre}(X)$ is an SCC, $s\in S$, and there exists a path from $s$ to  state $t$, then $t\in S$ or $t\in X$. Note that $\mathit{pre}(X)$ is closed downwards.
\end{enumerate}\gatodo{Perhaps this def. should appear in the previous subsection}
\end{definition}



\begin{lemma}
\label{lem:pre-beta}
Let $\mathit{GS}= (\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ be a game structure,
and $\beta$ be a BDD over $\I,\O$ that characterizes a closed downwards  set of SCCs, $X$.
Then, given the BDDs constructed above, a BDD $\mathit{pre}(\beta)$ for $\mathit{pre}(X)$ is computed in $O(1)$ symbolic operations.
\end{lemma}

\begin{proof}
Construct a BDD $\gamma$ by $R_{(\I\rightarrow \I', \O\rightarrow \O')}(\beta)$. Hence, $\mathit{pre}(\beta)$ is construct by $\forall \I',\O' (\beta_\mathit{Reach} \rightarrow (\beta_\mathit{SCC} \vee \gamma) )$.\qed
\end{proof}

Now we can finally present, in Algo~\ref{algo:sym-weak-buchi}, the symbolic modification of the inductive procedure from Section~\ref{subsec:dfa-game}. The algorithm returns the system's winning region ($W$) and a memory-less winning strategy ($f^s$). %We naturally model regions, i.e. sets of states, by BDDs over $\I,\O$. A memory-less strategy is modeled by a BDD over $\I,\O,\I',\O$ that relate a state and an input to a possible output. That is, for such BDD $\sigma$, $\sigma(\inp_0,\out_0,\inp_1',\out_1')$ means that from state $(\inp_0,\out_0)$ and input $(\inp_1)$, if the input is legal, then the strategy responds with $\out_1$. 
For the simplicity of the construction, we construct a strategy that is not necessarily deterministic. That is, we allow several possible responses for given state and input, and require that a resulting play is winning for the system, regardless of the non-deterministic choices made during the play. 

The algorithm employs two sub-procedures. (1) $\mathit{reach}(\beta,W)$ receives a BDD of a closed downwards set of SCCs, $\beta$, and a BDD of target states $W\subseteq \beta$. The procedure solves reachability in the subgame $\beta$ and target set $W$ and thus outputs a pair $(W_1,f^s_1)$: $W_1$ is the winning region of the system, and $f^s_1$ is a memory-less winning strategy. 
(2) $\mathit{safe}(\beta,W)$ receives a BDD of a closed downwards set of SCCs, $\beta$, 
and a BDD of safe states $W\subseteq \beta$. The procedure solves safety in the subgame $\beta$ and safe region $W$ and thus outputs a pair $(W_2,f^s_2)$: $W_1$ is the wining region of the system, and $f^s_2$ is a memory-less winning strategy. 

Lines~\ref{line:terminal}-\ref{line:winning-terminal-states} form the induction basis. We identify the terminal states (line~\ref{line:terminal}), identify the winning terminal states - the accepting SCCs (line~\ref{line:winning-variable}), and compute a winning strategy from those SCCs - a strategy that merely finds a legal input, as we cannot leave a terminal SCC (line~\ref{line:winning-terminal-states}).

Lines~\ref{line:while-loop}-\ref{line:end-while} form the induction step. After identifying the winning states $W$ in the subgame $\beta$ along with a matching memory-less strategy $f^s$, we wish to extend $W$ and $f^s$ to $\mathit{pre}(\beta)$. The additional winning states are those from which we can reach $W$ (line~\ref{line:reach}), denoted $W_1$, and the added accepting states (say, $A$) from which can force staying in $A$ or reaching $W$ (line~\ref{line:safe}),\footnote{see Section~\ref{subsec:dfa-game} for an explanation why we can use safety-game to identify this set of states} denoted $W_2$. In line~\ref{line:extend-strategy}, we extend the winning strategy over $W_1$ and $W_2$. We extend $f^s$ to $W_1\setminus W$: a strategy to reach $W$ from which we apply $f^s$. In addition, we extend the strategy to new discovered states from $W_2$: we play a safety strategy, and if the play reaches $W$, we switch to the already constructed strategy $f^s$.
We further update the set of discovered winning states (line~\ref{line:extend-region}).



\begin{algorithm}[t]
	\caption{Weak-B\"uchi winning strategy construction}
	\label{algo:sym-weak-buchi}
	\begin{algorithmic}[1]
	    
	    \Statex \textbf{input:} A weak B\"uchi game $((\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O),GF\mathit{(acc)})$ 
	    
	    %\State construct $\beta_\mathit{SCC},\beta_\mathit{ter}$
	    
	    \State $\beta = \beta_\mathit{ter}$\label{line:terminal}
	    
	    \State $W=\beta\wedge \mathit{acc}$\label{line:winning-variable}
	    
	    \State $\sigma = W\wedge (\rho_\I\rightarrow \rho_\O)$\label{line:winning-terminal-states}
    
        \While{$\beta \neq 2^{\I\cup\O}$}\label{line:while-loop}
        
        \State $\gamma =\mathit{pre}(\beta)$\label{line:pre}
        
        \State $(W_1,f^s_1)=\mathit{reach}(\gamma,W)$\label{line:reach}
        
        \State $(W_2,f^s_2)=\mathit{safe}(\gamma,W\vee (  (\gamma\setminus \beta)\wedge \mathit{acc}))$\label{line:safe}
        
        \State $f^s = f^s \vee 
        ( (W_1\setminus W) \wedge f^s_1) \vee 
        ( (W_2\setminus (W\vee W_1)) \wedge f^s_2)$\label{line:extend-strategy}
        
        \State $W=W\vee W_1 \vee W_2$\label{line:extend-region}
        
        \State $\beta= \gamma$
        
        \EndWhile\label{line:end-while}
		
		\State\Return $(W,f^s)$
	\end{algorithmic}
\end{algorithm}


We turn to prove Theorem~\ref{Thrm:WeakBuchi}.
\begin{proof}[proof of Theorem~\ref{Thrm:WeakBuchi}]
Algorithm~\ref{algo:sym-weak-buchi} symbolically implements the inductive procedure from Section~\ref{subsec:dfa-game}. Hence, it correctly identifies the system's winning region, and constructs a winning strategy. It remains to show that it performs $O(N)$ symbolic operations. First, by Lemmas~\ref{lem:beta_SCC},~\ref{lem:beta_ter}, $\beta_\mathit{ter}$ is constructed in $O(N)$ operations. Hence, it sufficient to show that each loop execution consumes $O(|\mathit{pre}(\beta)\setminus\beta|)$ operations.   

By Lemma~\ref{lem:pre-beta}, each execution of line~\ref{line:pre} consumes $O(1)$ operations. Therefore, to prove the required, we show that the sub procedures perform  $O(|\mathit{pre}(\beta)\setminus\beta|)$ operations. We start with $\mathit{reach}(\gamma, W)$. This sub-procedure performs the next fixed point computation: $Z_0=W$, and $Z_{i+1}=\mathit{pre}_s(Z_i)\cup Z_i$, where $\mathit{pre}_s(X)$ is the set of states from which the system can force reaching $X$ in a single step. Thus, $Z_0\subseteq Z_1\subseteq \cdots$, and the winning region is $Z_i$ that satisfies $Z_i=Z_{i+1}$. We refer the reader to~\cite[Chapter~20]{2001automata} for a comprehensive discussion. Now, at each step $j< i$, at least one state is added to $Z_{j}$ thus there are at most $|\gamma\setminus W|$ steps, each is performed in $O(1)$ operations. Furthermore, if $s\in \beta\setminus W$, then we never add $s$ to a set $Z_j$. This claim is argued is follows. If we add $s$ to some $Z_j$, then the system can force reaching $W$ from $s$, and then it can win w.r.t. the B\"uchi condition. This contradicts the fact that $W$ is the system's winning region w.r.t. the B\"uchi condition  in the subgame $\beta$. Hence, an upper bound of $O(|\gamma\setminus\beta|)$ operations is established. 

Similarly, write $U=W\vee (\gamma\setminus \beta)\wedge \mathit{acc})$. $\mathit{safe}(\gamma,U)$ performs the next fixed point computation: $Z_0=U$, and $Z_{i+1}=Z_i \cap \mathit{pre}_s(Z_i)$. Thus, $Z_0\supseteq Z_1\supseteq \cdots$, and the winning region is $Z_i$ that satisfies $Z_i=Z_{i+1}$. See~\cite[Chapter~20]{2001automata} for a comprehensive discussion. As before, at each step $j<i$ at least a single state is removed from $Z_j$ and hence, an upper bound of $O(U)$ steps hold. Furthermore, a state $s\in W$ is never removed from $U$. This claim is argued as follows. Take $s\in W$, and assume that $s\in Z_j\setminus Z_{j+1}$. Consequently, the system cannot win $\mathit{safe}(W)$ from $s$ in the subgame $\beta$. Hence, the environment has a strategy to reach $\beta\setminus W$ form $s$, from which it can win w.r.t. the B\"uchi objective, in contradiction to $s\in W$. Therefore, the computation terminates after at most $O( |(\gamma\setminus\beta) \wedge \mathit{acc}|)$ steps, and an upper bound of $O(|\gamma\setminus\beta|)$ operation is established, which completes the proof.\qed 
\end{proof}

\end{comment}




%%    commented out from here
\begin{comment}
\gatodo{I have few concerns about the weak-Buchi automata debate:\\
     {\large 1.} (somewhat minor) The advantages of mentioning weak-Buchi hare are clear - we want to prepare the reader for a (sort of) generalization of our solution to the connected-partition problem. The disadvantage is that we add "noise". More definitions that are distracting the reader, and may prevent her from understanding the solution to the connected partition problem. I wonder if the advantages justify the debate.\\
   {\large 2.} (somewhat minor) You gave the classical definition from the weak-Buchi paper. As Lucas noted, this def. is equivalent to: every SCC is either accepting or rejecting (right?) Wouldn't it be better to give that def.? It is simpler to grasp, and then there is no need to explain why the connected-partition problem is weak-Buchi.\\
   {\large 3.} (major) I disagree that connected-partition is a special case of Weak-Buchi. The problem is with the game rules. In the connected partition problem, the players choose the next state together: env chooses an input $\inp$, and sys chooses an output $\out$, and the play traverses to $(\inp,\out)$. In a weak-Buchi game, following standard definitions, the states are partitioned into player 0 and player 1 states. This is a huge difference. For example, it is possible that player i will play twice... Note that we can reduce the connected partition to weak Buchi as follows: we declare all states as env-states, and add "intermediate" sys-states of the form $(\inp_0,\out_0,\inp_1)$. This works but we do not benefit from it - We get a quadratic time complexity rather than linear. \\ \\
   My suggestion: I think it is better not to mention here weak-Buchi. Instead, in a spearte sect. to define a weak buchi game precisely and to mention that a straightforward adaptation of our algorithm works for weak-Buchi. Maybe we can even leave the proof for the reader/give it in an appx./ refer to an arxiv version that includes the proof.
}


\end{comment}

\begin{comment}
\subsection{Reduction to Finally-Globally (FG) winning condition}

Assume that each $\alpha_i$ and $\beta_i$ can be represented by a deterministic B\"{u}chi word automaton (DBW). Let $A_i$ be the the DBW for $\alpha_i$ and $B_i$ the DBW for $\beta_i$. Let $S_i$ be the set of states of $A_i$ and $T_i$ the set of states of $B_i$. Let $A = A_1 \times \ldots \times A_k$ be an automaton with state space $S = S_1 \times \ldots \times S_k$ and $B = B_1 \times \ldots \times B_k$ be an automaton with state space $T = T_1 \times \ldots \times T_k$. We say that a state $s = (s_1, \ldots, s_k)$ of $A$ is \emph{accepting for component $i$} if $s_i$ is an accepting state, and similarly for a state $t = (t_1, \ldots, t_k)$ of $B$.

For convenience, we assume that each player controls a single multi-valued variable, where each value corresponds to an assignment of the propositions controlled by that player. Let $x$ be the variable controlled by the environment, and $y$ the variable controlled by the system. We can write $A=(Q^A,\Sigma^A,q_0^A,\delta^A,F_1^A,\dots,F_k^A)$ and $B=(Q^B,\Sigma^B,q_0^B,\delta^B,F_1^B,\dots,F_k^B)$, where $\Sigma^A$ (resp. $\Sigma^B$) is the set of evaluations of $x$ (resp. $y$). For a word $w$ over $\Sigma^A$ (resp. $\Sigma^B$), $w\in L(\alpha_i)$ (resp. $w\in L(\beta_i)$) iff the run of $A$ (resp. $B$) on $w$ from $q_0^A$ (resp. $q_0^B$) traverses $F_i^A$ (resp. $F_i^B$) infinitely many times. 
 
We now define a game $D$ with $Q^A\times Q^B$ as the arena. From state $(q_i^A,q_j^B)$, the players choose together the ensuing state: the environment plays first, and it chooses a ``$\delta^A$-successor" of $q_i^A$, $q_{i'}^A$. In response, the system chooses a ``$\delta^B$-successor" of $q_j^B$, $q_{j'}^B$, and the ensuing state is $(q_{i'}^A,q_{i'}^B)$. A play is an infinite sequence of states, constructed according to the described procedure.\footnote{We assume that $A$ and $B$ are `complete', in the sense that $\mathit{Dom}(\delta^A)=Q^A\times \Sigma^A$ and $\mathit{Dom}(\delta^B)=Q^B\times \Sigma^B$.} 

Every trace in the original formula $\varphi$ can be lifted to a unique play in $D$ as follows. For a trace $(x_0,y_0),\dots,(x_m,y_m),\dots$, we take the play $(s_0^A,s_0^B),\dots ,(s_m^A,s_m^A),\dots$ where $(s_0^A,s_0^B)=(q_0^A,q_0^B)$ (the initial states), and $(s_{n+1}^A,s_{n+1}^B)=(\delta^A(s_n^A,x_n),\delta^B(s_n^B,y_n))$. Here, $x_n$ and $y_n$ are assignments to variables $x$ and $y$, respectively.

We say that a trace $\tau$ for $\varphi$ \emph{corresponds} to a play $\sigma$ in $D$, if $\tau$ is \emph{lifted} to $\sigma$, as described. Although $\tau$ corresponds to a unique play $\sigma$ in $D$, there are possibly many (yet, at least one) traces that correspond to a play $\sigma$ in $D$. The following observation is straightforward.

\begin{observation} \label{obs:streett}
If $\tau$ corresponds to $\sigma$, then $\tau$ satisfies $\varphi$ iff $\sigma$ satisfies the Streett condition: $(F_1^A,F_1^B),\dots,(F_k^A,F_k^B)$.
\end{observation}

\subsubsection{Defining a Winning Condition} \label{sec:fg-condition}

Following Observation~\ref{obs:streett}, we could solve the synthesis problem by solving a Streett game. In this section, however, we describe how we can simplify the winning condition to something of the form Finally-Globally (FG), which is easier to solve.

A state $q$ of $A$ (resp. of $B$) is an \emph{$i$-cycle} if there exists an $F_i^A$-state (resp. $F_i^B$-state) in its (strongly) connected component. A state $(q^A,q^B)$ of $D$ \emph{covers cycles} if for every $i\leq k$, if $q^A$ is an $i$-cycle, then $q^B$ is an $i$-cycle as well. Let $CC$ be the set of all states of $D$ that cover cycles.

We can also speak about connected component in $D$. Naturally, $(q^A,q^B)$ and $(q'^A,q'^B)$ are in the same connected component iff $q^A$ and $q'^A$ are in the same connected component in $A$, and $q^B$ and $q'^B$ are in the same connected component in $B$. Note that $CC$ is a property of a connected component. That is, $(q^A,q^B)\in CC$ iff all states in $(q^A,q^B)$'s connected component belong to $CC$.

Now, we turn to analyse the game $D$ w.r.t. the winning condition $FG(CC)$. Let $W_s$ and $W_e$ be the winning regions of the system and the environment in $D$ w.r.t. the winning condition $FG(CC)$, respectively. Standard determinacy arguments reveal that $W_s$ and $W_e$ partition the state space of $D$. 

\begin{lemma} \label{lemma:w_e}
$W_e$ is the set of states from which the environment has a strategy to force $FG(\overline{CC})$.
\end{lemma}
\begin{proof}
Let $\sigma=(p_0^A,p_0^A),\dots$ be a play in $D$. Since the play converges to a single connected component, we have $\sigma\models \neg FG(CC)\Longleftrightarrow \sigma\models FG(\overline{CC})$. Note that this proves a stronger property: it also proves that the a spoiling strategy for the environment w.r.t. the winning condition $FG(CC)$, also forces $FG(\overline{CC})$.
\end{proof}

\subsection{The Delay Property}

One of the crucial features of the game we have defined in this section is what we call the \emph{delay property}. Intuitively, this property says that the plays by the environment and the system need not be synchronized. That is, if a player can win from a state $(q^A, q^B)$, then the same player has a strategy to win even if the two players reach $q^A$ and $q^B$ at different times.
{\color{red} GaL: This is incorrect, the delay property means that the player can wait for awhile, letting the other player take several steps. For illustration, assume that sys has a strategy from $(q_A,q_B)$, sys reaches $q_B$ at time $t$, and at time $t+l$ the configuration is $(q_A,q_B')$. But, sys cannot win from $(q_A,q_B')$ (it is not difficult to construct such an example.) }

More formally, let $f_s : Q^A \times Q^B \rightarrow Q^B$ be a strategy for the system that wins from state $(q^A,q^B)$, and let $q'^B$ be a system state such that $\delta^B(q'^B,y_i)=q^B$ for some evaluation $y_i$ of $y$. Then, we can define a strategy $g_s : (Q^A \times Q^B) \times Q^A \rightarrow Q^B$ for the system that wins from state $(q^A, q'^B)$. This $g_s$ is a function from the current state $(p^A_1, p^B_1) \in Q^A \times Q^B$ and the previous environment state $p^A_0 \in Q^A$ to the next system state $p^B_2$. Note that, as $g_s$ needs to remember the previous environment state, it is not a memoryless strategy. 

Given $f_s$, $(q^A,q^B)$ and $q'^B$, we construct $g_s$ as follows. Assume that when we start from state $(q^A, q'^B)$ the previous environment state is $\epsilon$, indicating the lack of a predecessor. {\color{red} Gal: I don't understand the $\varepsilon$ here. But, It seems that it is not that important... } Then:
\begin{align*}
    &g_s((q^A, q'^B), \epsilon) = q^B \\
    &g_s((p^A, p^B), p'^A) = f(p'^A, p^B)
\end{align*}

Intuitively, $g_s$ first moves from $q'^B$ to $q^B$. Note that at this point the environment has also moved to another state $q'^A$. Afterwards, $g_s$ simply simulates $f_s$, but using the previous environment state instead of the current one. For example, after the game moves from $(q^A, q'^B)$ to $(q'^A, q^B)$, $g_s$ should make the same move from $(q'^A, q^B)$ as $f_s$ would make from $(q^A, q^B)$. In other words, after the first move, $g_s$ acts exactly like $f_s$, but with a delay of a single step.

The following lemma then follows directly from the definition of $g_s$:

\begin{lemma}
If $(p_0^A,p_0^B),\dots,(p_i^A,p_i^B)$ is a sequence from $(q^A,q'^B)$ that is consistent with $g_s$, then $(p_0^A,p_1^B),\dots, (p_{i-1}^A,p_i^B)$ is a sequence from $(q^A,q^B)$ that is consistent with $f_s$.
\end{lemma}

We now prove that $g_s$ is indeed a winning strategy from $(q^A, q'^B)$.

\begin{lemma}
$g_s$ is winning from $(q^A, q'^B)$.
\end{lemma}
\begin{proof}
Consider a play $\sigma_g=(p_0^A,p_0^B),\dots$ from $(q^A,q'^B)$, consistent with $g_s$. By the construction, $\sigma_f=(p_0^A,p_1^A),(p_1^A,p_2^B),\dots$ is a play, consistent with $f_s$, from $(q^A,q^B)$. Since $f_s$ is winning from $(q^A,q^B)$, $\sigma_f\models FG(CC)$. Therefore, after a finite amount of time $\sigma_f$ gets stuck in a $CC$ connected component. Since the environment and system states visited after this point in $\sigma_g$ are the same, $\sigma_g$ must get stuck in the same connected component. Hence, $g_s\models FG(CC)$.
\end{proof}

\begin{lemma} \label{lemma:delay}
The following hold.
\begin{itemize}

    
    \item[(1)] If $(q^A,q^B)\in W_s$ and $\delta^B(q'^B,y_i)=q^B$ for some evaluation of $y$, $y_i$, then $(q^A,q'^B)\in W_s$.
    
    \item[(2)] If $(q^A,q^B)\in W_e$ and $\delta^A(q'^A,x_i)=q^A$ for some evaluation of $x$, $x_i$, then $(q'^A,q^B)\in W^e$.
\end{itemize}

\end{lemma}
\begin{proof}
(1) follows directly from the construction of $g_s$ from $f_s$. For (2), we can invoke Lemma~\ref{lemma:w_e} to choose a strategy $f_e$ for the environment that forces $FG(\overline{CC})$. Then, with a similar construction we can get a strategy $g_e$ that forces $FG(\overline{CC})$ from $(q'^A, q^B)$.
\end{proof}

We can then obtain the following corollary by iterating Lemma~\ref{lemma:delay}.

\begin{corollary} The following hold.
\begin{itemize}
    \item[(1)] If $(q^A,q^B)\in W_s$ and $q^B$ is reachable in $B$ from $q'^B$, then $(q^A,q'^B)\in W_s$.
    
    \item[(2)] If $(q^A,q^B)\in W_e$ and $q^A$ is reachable in $A$ from $q'^A$, then $(q'^A,q^B)\in W_e$.
\end{itemize}
\end{corollary}

\begin{corollary} The following hold.
\begin{itemize}
    \item[(1)] If $(q^A,q^B)\in W_s$ and $q'^A$ is an $A$-successor of $q^A$, then $(q'^A,q^B)\in W_s$.
    
    \item[(2)] If $(q^A,q^B)\in W_e$ and $q'^B$ is a $B$-successor of $q^B$, then $(q^A,q'^B)\in W_e$.
\end{itemize}
\end{corollary}
\begin{proof}
To prove (1), take $(q^A,q^B)\in W_s$, and assume towards a contradiction that $(q'^A,q^B)\notin W_s$. Hence, $(q'^A,q^B)\in W_e$, and by the previous lemma $(q^A,q^B)\in W_e$ as well, in contradiction to the assumption. Claim (2) is implied by the same argument. 
\end{proof}

\subsection{Correctness of the Reduction}

We now prove the correctness of the reduction of the Streett winning condition from Observation~\ref{obs:streett} to the FG(CC) winning condition defined in Section~\ref{sec:fg-condition}.

Assume that $(q_A,q_B)\in W_s$, and let $f_s$ be a winning strategy for the system w.r.t. $FG(CC)$.\footnote{We can take a memoryless strategy $f^s$. Otherwise, some small technical changes are required.} Let $g_s:Q^B\rightarrow Q^B$ be a partial function such that:
\begin{enumerate}
    
    \item For each $q^B\in Q^B$, if $q^B$ has a successor in its connected component, then $g_s(q^B)$ is such a successor.
    
    \item Let $p_0^B,\dots,p_n^B,\dots$ be an infinite sequence over $Q^B$ such that for each $i$ $p_i^B=g^i(p_0^B)$. Thus, each state in $p_0^B$'s connected component appears in that sequence infinitely often.
\end{enumerate}
We set the following strategy $h_s$ for the system that is winning w.r.t. the Streett condition. From state $(q^A,q^B)$ and input $q'^A$:
\begin{itemize}
    \item If $(q'_A,q_B)\in CC$ and $g_s(q_B)$ is defined, then return $g_s(q^B)$.
    \item Otherwise, return $f_s((q^A,q^B),q'^A)$.
\end{itemize}

The following claim that the strategy is indeed well-defined
\begin{claim} \label{claim:h_s}
Take $(p_0^A,p_0^B)\in W_s$.
If $(p_0^A,p_0^B),\dots,(p_n^A,p_n^B)$ is consistent with $h_s$, and $p_{n+1}^A$ is an $A$-successor of $p_n^A$, then $h((p_n^A,p_n^B),p_{n+1}^A)$ is defined, and for $p_{n+1}^B=h((p_n^A,p_n^B),p_{n+1})$, it holds that $(p_{n+1}^A,p_{n+1}^B)\in W_s$. 
\end{claim}
\begin{proof}
We prove the claim by induction on $n$.
First, note that $(p_n^A,p_{n}^B)\in W^s$.
If $n=0$ this holds by assumption, and otherwise it holds by the induction hypothesis. Now, if $q_{n+1}^B$ is chosen according to the first item, then Corollaries 1 and 2 ensure that $(q_{n+1}^A,q_{n+1}^B)\in W_s$. Otherwise, $h$ returns $f_s((q_{n}^A,q_n^B),q_{n+1}^A)$. Since $(q_n^A,q_n^B)\in W_s$, $q_{n+1}^B$ is well-defined. Since the sequence $(q_{n}^A,q_n^B),(q_{n+1}^A,q_{n+1}^B)$ is consistent with $f_s$, $(q_{n+1}^A,q_{n+1}^B)\in W_s$, as required.
\end{proof}

We can now use the construction of $h_s$ to prove the following lemma.

\begin{lemma}
$(q^A,q^B)\in W_s$ iff the system player can win from $(q^A,q^B)$ w.r.t. the Streett condition $(F_1^A,F_1^B),\dots,(F_k^A,F_k^B)$. 
\end{lemma}

\begin{proof}
($\rightarrow$) Let $f_s$ be a winning strategy for the system w.r.t. $FG(CC)$ and construct $h_s$ as above. Now, we show that $h_s$ is winning w.r.t. the Streett condition. Take a play from $W_s$, $(p_0^A,p_0^B),\dots$ consistent with $h_s$. Hence, some suffix of the play, $(p_i^A,p_i^B),\dots$ never leaves a certain connected component. We consider two cases:
\begin{enumerate}
    \item The suffix stays in a $CC$-component. Then, at that suffix, $h_s$ consistently applies $g_s$ to choose the next output. It follows that the play satisfies the Streett condition.
    
    \item The suffix stays in a $\overline{CC}$-component. Then, at that suffix, $h_s$ consistently applies $f_s$ to provide the next output. Therefore, the play $(p_i^A,p_i^B),\dots$ is a losing play for the system w.r.t. $FG(CC)$, and it is consistent with $f_s$. Consequently, $(p_i^A,p_i^B)\notin W_s$. However, this conclusion contradicts Claim~\ref{claim:h_s} thus this case cannot occur. 
\end{enumerate}
As a result, it follows that $h_s$ is a winning strategy from $W_s$ w.r.t. the Streett condition $(F_1^A,F_1^B),\dots,(F_n^A,F_n^B)$, as required.

($\leftarrow$) We show that the environment has a spoiling strategy w.r.t. the street condition from $W_e$. Take a (memoryless) strategy for the environment $f_e$ from $W_e$, that forces $FG(\overline{CC})$. By Lemma~\ref{lemma:w_e}, such a strategy exists. Let $g_e:Q^A\rightarrow Q^A$ be a partial function that satisfies the analogous requirements as for $g_s$.  

We set the following strategy $h_e$ for the system. From state $(q^A,q^B)$:
\begin{itemize}
    \item If $(q_A,q_B)\in \overline{CC}$ and $g_e(q_A)$ is defined, then return $g_e(q^A)$.
    \item Otherwise, return $f_e((q^A,q^B))$.
\end{itemize}
By similar arguments as before, the claim follows.
\end{proof}

By the previous lemma, we have:
\begin{theorem} \label{thm:win}
System has a winning strategy iff $(q_0^A,q_0^B)\in W_s$. Such a strategy can be constructed from the strategy $h_s$.
\end{theorem}

\subsection{Solving the $FG(CC)$ Game}

Note that the $FG(CC)$ winning condition makes the game we have described a co-Büchi game where $CC$ is the set of accepting states. As noted in Section~\ref{sec:fg-condition}, $CC$ is a property of a connected component, meaning that for each connected component, either all states are in $CC$ or none are. This matches the definition of a weak automaton:

\begin{definition}
A co-Büchi automaton is said to be \emph{weak} if there is a partitioning of its state space $Q$ into $Q_1, \ldots, Q_m$ such that:

\begin{enumerate}
    \item For every $i$, either all states in $Q_i$ are accepting or all states are non-accepting.
    \item For every $i$ and $j$, if there exists a transition from state $q \in Q_i$ to state $q' \in Q_j$, then $i \leq j$.
\end{enumerate}
\end{definition}

$Q_1, \ldots, Q_m$ can be defined appropriately as the connected components of the state space, sorted topologically. Note that weak automata are more commonly defined with a Büchi acceptance condition, but since a play can never return to a previous connected component, Büchi and co-Büchi acceptance conditions are equivalent for weak automata.

We can therefore use the special properties of a weak automaton to solve this game more efficiently than a typical Büchi or co-Büchi game. A game over a weak automaton can be solved in linear time on the number of states:

\begin{description}
    \item[Base case:] Note that a play that reaches $Q_m$ cannot ever leave $Q_m$, since it is a terminal connected component. Therefore, if $Q_m$ is an accepting component every state is a winning state, while if $Q_m$ is a non-accepting component every state is a losing state.
    \item[Induction step:] If all states in $Q_{i+1}, \ldots, Q_m$ have been classified as winning or losing, they can be collapsed into two sink states, one winning and one losing. Then, all states in $Q_i$ can only reach other states in $Q_i$ or one of the two sink states. We can now partition the states in $Q_i$ into winning and losing states by solving a reachability game, where a state is winning if the game can be forced into the winning sink from it. Since reachability games can be solved in linear time, the complexity of this step is linear on $|Q_i|$.
\end{description}

Note, additionally, that the connected components do not necessarily need to be processed linearly. For example, if $Q_1$ only has transitions to $Q_3$ and $Q_4$, then the reachability game on $Q_1$ can be solved as soon as $Q_3$ and $Q_4$ are partitioned, even if $Q_2$ has not been partitioned yet. This allows for some degree of parallelism determined by the topology of the dependence graph between the connected components. In this case, for example, the reachability games for $Q_1$ and $Q_2$ could be solved in parallel. This may lead to significant speedups depending on the structure of the state space.

\end{comment}

==> Introduction.tex <==
% \section{Introduction - Draft 1}


% Reactive systems are systems that interact with the environment through an ongoing input/output process reactions in which the system responds to the triggers emitted by the environment.
% For such systems, there is typically a system specification formalized in some logic, that describes the exact input/output reactions that the system should act upon. \gatodo{not sure about the previous sentence. Specs appear in verification and synthesis. Beyond this context, would you say that reactive systems tend to come with specs more, say, than data structures? not sure about it... I would omit that sentence...} Reactive synthesis is then the process of constructing such system from its given specification. \gatodo{something seems to be still missing before proceeding to the description of our fragment. Consider e.g. the following:\\
% While the advantages of providing  correct-by-construction systems are clear (@Suguman - a better adjective?), unfortunately, the famous double-exponential lower bound~\cite{} proves a general approach to be impractical. Therefore, identifying expressive fragments for which a feasible synthesis technique exists is of high importance. 
% }
% While reactive synthesis specifications, however, mostly reason about the interaction between the actions of the system and the environment, sometimes the objective of the specification can be to detect certain environment behaviors and respond to these with behaviors of the system. We give concrete examples in the paper, but think as a motivating example of a system A that is running on a set of specific scenarios, and the designer wishes to build a system C while using System A in a black-box manner, by designing a wrapper (called System B) that takes the behavior of system A and transforms them to System C setting. The specification that the designer writes for System B, can be then expressed as a sequence of adaptation of each System A behavior to a System B behavior. \gatodo{Really? This is what we do? I thought we construct B... What is the wrapper? I guess I need an explanation here}

% In this paper we focus on synthesis of specifications that describe such interactions between systems, in which the designer describes the in interactions between systems through their behaviors instead of interacting ``per-action". In the example above, we call System A the \textit{environment} and System B as the \textit{system}. The specifications that we are interested with, are then a conjunction of implications between a $\phi$ formula that concerns only the environment and describes the environment behavior, and a $\psi$ formula that concerns only the system and describes the required system behavior.
% %For example, if we formally consider the formulas in Linear Temporal Logic (LTL), then the specification is an LTL formula described as a conjunction of formulas of the form $\phi\rightarrow\psi$ where $\phi$ is an LTL formula only over the environment variables, and $\psi$ is an LTL formula only over the system variables.
% \gatodo{I think the description of our context should be richer. one thing that in particular seems missing to me: since A is an existing system, we an actually learn it, and not just take its "manual-specification". For example, the specification can be ?? and thus the winning condition ?? is unrealizable. But, since A is implemented such that ??, we can provide the system B: ?? that fulfils the desired w.r.t. A. }


% The formulation that in our setting is a specific type of $GR(k)$ formulation. These are a set of $k$ temporal constraints, each is of the form $\phi\rightarrow\psi$, where $\phi$ is a conjunct of Globally-Finally Boolean formulas on the \textit{environment variables only}, and $\psi$ is a conjunct of Globally-Finally Boolean formulas on the \textit{system variables only}.
%  As we see, such separation makes more efficient solution while still capture important scenarios and specifications.
% Together with the accompanied tuple that is standard in $GR(k)$ formulations [[DF: we need to clarify this]], the $GR(k)$ settings thus can be thus interpreted as a game over the state space described by the tuple, that can hint towards a route to solving $GR(k)$. Indeed, there are explicit and symbolic methods to solve such problems with an efficiency of $O(n^2)$ where $n$ is the number of states in the resulting graph game.

% However, unlike standard $GR(k)$, the environment/system variables in our formulation are separated by the $\rightarrow$ connector [[DF: say better]]. As such, our formulation describes an essential interaction between two separated games that are played: one of the environment, and one over the system. As we show in this paper, exploring this insight follows to realization that in the game played between the environment and the system, the system can always delays it's actions and wait for the environment to pick a certain path in that game. We call this property the \textit{delay property} of the game.
% We show that exploiting this property leads to decomposing the game-graph into connected component, where some of the connected component are called \textit{accepting}. Then the game between the environment and the system is reduced to a game on the connected components graphs, where the system's objective to reach an accepting connected component and to stay there (in that sense this is similar to playing game on Weak Automata). As we show, our techniques lower the complexity of solving such games over state-of-the-art techniques.

% \gatodo{I find the above discussion good, but quite unorganized. Allow me to suggest a different arrangement: 1. we focus on  GR(k) + your globally-finally description. 2. GR(k) is expressive. Mainly,  it allows to encode DBA properties (currently, I do not see anything about DBA). 3. Generally, GR(k) is inefficient - exponential in k ( certainly not $O(n^2)$!). But, our context allows a linear-time synthesis of GR(k) winning-conditions. 4. Our approach is symbolic and thus we can handle large-space systems.
% In addition: I think the delay-property, weak-automata is not in place here. This can be given afterwards, (or perhaps not at all?). In particular, my suggestion is mainly not to mix between what and how. First 'what', then 'how', if at all. }

% [[DF: from here, we need to discuss first]]

% For clarity of exposition we describe our algorithm on the explicit graph. \gatodo{not necessary for the intro, I think...} We do however implement our framework symbolically by using Binary Decision Diagrams (BDDs) to symbolically describe the game state and transitions. We evaluate our framework experimentally, comparing against state-of-the-art tools, while using elaborated and detailed problem domains that we describe. By doing that, we do not only show the strength of our framework, but also show the rich variety of problem scenarios, in which our clear-cut specifications can be used.\gatodo{I suggest to relocate  the symbolic discussion in the 'what' description (see a former comment). A par. about the evaluation is in place, of course.} 

% In Section 2 we give preliminaries and discuss related work in Section 3. In Section 4 we describe our problem formulation and describe our synthesis framework on the explicit setting, at the heart of which lies the delay-property. We then describe our symbolic implementation in Section 5. In Section 6 we elaborate on problem domains and give concrete examples, followed by running experimental evaluations on these examples and compare against state-of-the-art synthesis tools. We conclude in Section 8.

% \gatodo{I think a subsection with 2-3 examples would be nice here. }


% % \subsection{A motivating example}

% % \paragraph{Legacy Systems}
% % Suppose an existing system, which is legacy, called System A. Based on this system, the designers construct an updated System B, and would like to start running an ongoing program on System B that achieves several constraints.  Since not all properties can be achieved, the designers would settle for a plan that meet at least the same properties as executing a plan on System A will meet for System A. For that, the engineers need to monitor the plan executed on System A, and with certain modification run a similar plan on System B. The plan for System A however, is not known. We could assume for example that it is scheduled to start only ahead of time. Therefore the engineers has to come up with a strategy of what actions the updated System B should take, according to the actions that System A takes such that System B meets at least the same properties as System A.

% % Formally, System A is modeled by a graph setting $G_B$ with states and a transition system. Similarly System B has it's own graph $G_B$. The specification are in form of a formula $F$ that contains $k$ constraints of the form $varphi_k\rightarrow \psi_k$, where $\varphi_k$ is an LTL (in our case a safety) formula over only the input variables that describe possible actions over System A, and $\psi_k$ is an LTL (in our case a safety) formula over only the out variables that describe possible actions over System B. The objective is to synthesize a strategy for System B from $(G_I,G_O,F)$.



% % Rubik cube is broken.


% % \section{Introduction - Draft 1}


% % % 

% % Reactive systems are systems that interact with the environment through an on going input/output process reactions in which the system responds to the triggers emitted by the environment.
% % For such systems, there is typically a system specification formalized in some logic, that describes the exact input/output reactions that the system should act upon. Reactive synthesis, is then the process of constructing such system from it's given specification.

% % While reactive synthesis specification reasons about the interaction between the actions of the system and the environment, sometimes focusing on the action is to delicate for the specifier, and the required reasoning level is more high-level in which the specification reason on the relationship between the systems and the environment \textit{behaviors}, where the specifier is less interested in the exact action-level implementation detail, but rather just have the system's behavior to some environment specific behaviors that may occur. The environment, in that sense, can be the world, or another system that the original system needs to react to, or perhaps even just a system which the original system wants to imitate, under certain restrictions.
% % We give examples.

% % \begin{enumerate}
% % \item \textbf{Transmitter station.} Consider an intermediate transmitter station (called System $B$) that receives transmission from a the main distributer unit (called System $A$) and then sends the transmissions to a receiver unit. Due to certain constraints (e.g. limited bandwith of the transmitter station, handling many distributer stations), the tramsitter station adjusts the transmissions before sending them to the receiver. While doing so, however, certain properties of the 
% % original transmission are to be maintained. For example, some transmissions may have urgency sense in them, while other more relaxed. It is then natural for the designer of the transmitter station to specify the required behavior of the transmitter for every type of behavior received by the distributer.

% % \item \textbf{Systems modification} Consider an original system $A$ that is running a set of specific scenarios, each is a sequence of actions. The designer wishes to build a system $C$, but to use system $A$ in a black-box manner. Therefore the designer constructs System $C$ by taking system $C$, with an additional \textit{wrapper} (called System $B$) that is needed to be synthesized. The specification for the wrapper then naturally designed as required behavior adjustment, rather than for every specific action. For example,  
% % the designer may try to build a system $C$ that imitates the behavior of System $A$ as much as possible under the restriction that system $C$ has additional behavioral constraints which the designer should consider. Note that in this example, there is no actual reactivity between System $A$ and the wrapper: the wrapper observes the behavior of System $A$ and adjust it to meet the overall specification that the designer has specified.

% % \item \textbf{Traffic Controller.}
% % As another example of behavior control, consider the following example given from Shield Synthesis \cite{}.
% % Assume we have a controller for a traffic light at an intersection (let's call this controller $System A$).
% % We'll call the output of this controller a and assign it one of four values: $rr$, $rg$, $gr$ and $gg$, which indicate for each of the two lights whether that light is red ($r$) or green ($g$). The problem is that we have no guarantees about the behavior of this controller. In particular, there are two guarantees that we want to ensure: the two lights don't turn green at the same time, and the lights don't switch from $rg$ to $gr$ or vice-versa without passing through $rr$ in between. The solution in ~\cite{} is to add a \textit{shield} (which we refer to as System $B$) between the controller and the actual traffic lights. This shield takes the output a of the controller as input and outputs a new signal $b$. If $A$ would at any point violate our guarantees, System $B$ alters the output to something that would satisfy $A$. Ideally, we would also like to change the output as little as possible.
% % \end{enumerate}


% % The examples above demonstrate a large variety of problems that can be thoughts as "synthesis of behaviors" [[DF: does such term exists already?]].
% % Towards formalizing these example into computational models, we choose to use Linear Temporal Logic (LTL), commonly used to describe specifications for reactive synthesis \cite{}. In our setting however the specifications must not be written as general LTL formula, but take a specific form that we can use for our advantage. [[DF: I am not happy with the order of telling, we'll discuss]].
% % Indeed, such specification can take a special form of a collection of assume-guarantee constraints in a form of $\phi\rightarrow\psi$. However while every "assume" constraint $\phi$ is an LTL formula of the environment variables only, Every $\psi$ "guarantee" constraint is an LTL formula over system variables \textit{only}.
% % Note that this setting is different than the typical assume-guarantee constraints in which the "guarantee" constraints are set over both environment and system variables. 

% % For example, in the \textit{Transmitter station} problem, let $\{r\}$ be the alphabet of the transmissions System $A$ (the transmitter station) receives, and let $\{r'\}$ be the alphabet of the transmissions System $A$ (the transmitter station) sends. Then an example of a specification can be thought as a conjunction of constraints:

% % \begin{itemize}
% % \item $A$ is urgent, and $B$ has to address the urgency in some specific way:
% % $$ G(\neg r r)\rightarrow (FG((\neg r)^3r \vee (\neg r)^2 r \vee (\neg r)r)$$
% % (here $x^k$ means $x$ is repeated $k$ times)
% % \item $A$ is suspiciously relaxed:
% % $$GF((\neg r)^5 \wedge GF(\neg r r) \rightarrow (FG((\neg r)^8r U \neg r r))$$
% % \item Else $\rightarrow FG((\neg r)^3 r)$
% % \end{itemize}


% % Or as another example in the \textit{Traffic Controller} example, the specification can be thought of as a conjunction of the following constraints.

% % \begin{itemize}
% %     \item $GF(a= rr)\rightarrow GF(b=rr)$
% %     \item $GF(a= rg)\rightarrow GF(b=rg)$
% %     \item $GF(a= gr)\rightarrow GF(b=gr)$
% %     \item $true\rightarrow G(\neg (b=gg))$
% %     \item $true\rightarrow (G(X(b=gr))\rightarrow (\neg b=rg)$
% %     \item $true\rightarrow (G(X(b=rg))\rightarrow (\neg b=gr)$
% % \end{itemize}

% % We note that in these examples, an advantage of writing specifications as in this way, is the comfort in writing such specifications that describe behavior, as well as the readability of such terms. This was also noted in the $GR(k)$ formulation \cite{} [[DF: how are we compared to that?]].
% % Another advantage that we next show however, is that for certain settings there is also an efficiency advantage in solving such techniques.


% % \vspace{2mm}

% % We next discuss our technical advantages. [[DF: this shoud be expanded much further]]

% % \begin{itemize}
% % \item We show that for LTL assume and guarantee formulas that can be captured as a DBA, there is a techinque that is complexity-wise more efficient than the state-of-art techniques. Indeed, our methods is invoked on the so called delay property. that we explain in details and use. Note that DBA can use a variety of specification (such as all the examples above) as also noted in \cite{}.

% % \item We start by giving an explicit description of our technique, following by a symbolic description.

% % \item Since delay property can be thought of a special case of asynchrony between the environment and the system, we also discuss this relation.

% % \item Finally, we build our tool which makes use of this technique and we compare it to standard LTL synthesis approaches to see the gain of our delay technique.
% % \end{itemize}


% % In our systems Assumptions only on the environment, and the guarantee are only on the system.

% % Motivation - which system have these properties



% % Add restrictions 



% % Streetlights

% % tic tac toe

% % reduction between systems.

% % Technical - what can we syntehsize.

% % LTL synthesis in general 

% % In some cases we offer a procedure that is highly efficient 


% % %




% % %




% % %

% On going example:

% Street lights

% Tic Tac Toe


\section{Introduction}
\label{sec:intro}

The field of reactive synthesis has produced various techniques for automatic generation of  controllers that react to inputs under given constraints in a way that satisfies required specifications. These techniques have been shown to be practical in providing effective tools for the design of correct-by-construction systems. 

Inspired by the well known adapter design pattern~\cite{gamma1995design}, we study the use of reactive synthesis for synthesizing adapters that translate inputs meant for a target transducer to inputs of an adaptee transducer. Think, for example, of the task of adding a layer to an operating to adapt for a hardware vulnerability that we need to avoid.

Formally, we propose the following synthesis problem: given two finite state transducers called $Target$ and $Adaptee$, synthesize a finite state transducers called $Adaper$ such that
\[    Adaptee \circ Adapter \eqsim Target.\]
Where $\circ$ represents transducer composition, i.e., we are comparing the target with a composition of the adaptee with an adapter. Since, it is not always reasonable to require full equality, we only require that they are equivalent. The $\eqsim$ symbol represent an equivalence relation specified by  the user of the synthesis algorithm. In this work we consider specifications consisting of sets of required $\omega$-regular properties over the possible outputs of the transducer $(Adaptee \circ Adapter) \cdot Target$ where $\cdot$ represents transducer concatenation.
 To this end, we assume, without loss of generality, that the output of the $Target$ and $Adaptee$ transducers are sequences of truth assignments of two disjoint sets of, respectively, input and output atomic propositions.

Consider, for example, the transducers depicted in Figure~\ref{fig:transducers}. As common in the literature, we represent truth assignments to atomic propositions as elements in $(0+1)^*$ where 0 or 1 at the $i$th letter means assigning the $i$th variable with False or True, respectively. In this example, both transducers produce truth assignment of two (different) sets of atomic propositions of size two, so the length of all these words is two. The requirement is that, for any given input,  if an output is repeated infinitely often $Target$, it must also repeat infinitely often in $Adaptee \circ Adapter$. The transducers achieves this by circling  in the $s_0 \leftrightarrow s_1$  loop of the $Adaptee$ when the $Target$ circles in $s_1$.

\begin{figure}
    \centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.5cm,initial text=,
  thick,node/.style={fill=blue!20,draw,
  font=\sffamily\footnotesize, circle}]

\node[initial,node] (00) {$s_0$};

\node[node] (01) [above of=00] {$s_1$};
\node[node] (10) [below of=00] {$s_2$};
\node [above=0.3cm of 01] {Target};

\draw [->] (00) -- node {$U|10$} (01);
\draw [->] (00) -- node {$D|01$} (10);
\draw [->] (01) edge [loop left] node {$S|01$} (01);
\draw [->] (10) edge [loop left] node {$S|10$} (10);

\node[initial,node] (_00) [left=7cm of 00] {$s_0$};
\node[node] (_01) [above of=_00]    {$s_1$};
\node[node] (_10) [below of=_00]    {$s_2$};
\node [above=0.3cm of _01] {Adaptee};

\draw [->] (_00) edge [bend right] node [right] {$U|01$} (_01);
\draw [->] (_00) -- node {$D|10$} (_10);
\draw [->] (_01) edge [bend right] node [left] {$D|00$} (_00);
\draw [->] (_10) edge [loop left] node {$S|10$} (_10);
 
%%%
    \node[initial,circle,node,minimum width=0mm] (0) [left=4cm of 01] {$s_0$};
    
    \node[circle,node,minimum width=0mm] (1) [below of= 0] {$s_1$};
        
    \draw [->] (0) edge [bend right] 
            node [left] (A)     {$U | U$}     (1);
    
        \draw [->] (1) edge [bend right] 
            node [right]{$S | D$} (0);
    
        \draw [->] (0) edge [loop right] 
            node [right,text width=1cm ]{$S|S$ \\ $D|D$} (0);
    
    \node (adapter)  [above=0.3 cm of 0] {Adapter};

\node[] () [left=.5cm of adapter] {$\circ$};
\node[] () [right=1.5cm of adapter] {$\eqsim$};

\end{tikzpicture}
    \caption{An example of target and adaptee transducers and an adapter  that guarantees, for example, $GF(t_i) \to GF(a_i)$   for $i=1,2$  where $\{t_1, t_2\}$ and $\{a_1,a_2\}$ are the atomic propositions of the target and of the adaptee, respectively.}
    \label{fig:transducers}
\end{figure}



While most of the work on software synthesis focuses on synthesizing complete systems from their specifications, our focus is on using reactive synthesis for reusing existing components. The $Target$ transducer can model, for example, a standard Rubik cube and the $Adaptee$ can model a Rubik cube with some hardware failure. Since we know how to operate the normal cube, we could use an $Adapter$ that translates commands that we planed to send to the normal cube to commands that we can send to faulty one. The equivalence relation can say, for example, that if a side of the normal cube would have been completed infinitely often in the expected run of the normal cube it should also be completed infinitely often in the generated run of the faulty cube.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Dror will add a paragraph saying that the problem is very hard and that current state of the art tools cannot handle even small instances. Accordingly, we propose to use GR(K) formulas instead of just any $\omega$-regular properties.

Generally, synthesizing a transducer is complicated - complexity wise. Indeed, Even when equality is required, synthesizing is a non trivial task. \dftodo{write much better and explain the hardness, as a step towards GRk}


\dftodo{Now we mention GR(k) and how to utilize GR(k) that balance between expressiveness and efficiency. Mention the term "reactive synthesis".}


To allow direct use of the language of reactive synthesis, and to allow more generality, the input to our synthesis algorithm and to the tool that implements it is a representation of $Adpatee$ and $Target$  as transition systems, as depicted in Figure~\ref{fig:example}. The $Input$ transition is a representation of the $Target$ and the $Output$ transition system is a representation of the $Adatpee$ where we ignore the inputs to the systems and the state and consider only their outputs.

\begin{figure}
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,initial text=,
      thick,node/.style={fill=blue!20,draw,
      font=\sffamily\footnotesize,minimum width=15mm}]

    \node[initial,node] (00) {$\neg t_1  \wedge \neg t_2$};
    \node[node] (01) [above of=00] {$\neg t_1  \wedge t_2$};
    \node[node] (10) [below of=00] {$t_1  \wedge \neg t_2$};
    \node [above= 0.2 cm of 01] {Input};

    \draw [->] (00) --  (01);
    \draw [->] (00) --  (10);
    \draw [->] (01) edge [loop left] (01);
    \draw [->] (10) edge [loop left] (10);

    \node[initial,node] (_00) [right=2cm of 00] {$\neg a_1  \wedge \neg a_2$};
    \node[node] (_01) [above of=_00]    {$\neg a_1  \wedge a_2$};
    \node[node] (_10) [below of=_00]    {$a_1  \wedge \neg a_2$};
    \node [above= 0.2 cm of _01] {Output};

    \draw [->] (_00) edge [bend right]  (_01);
    \draw [->] (_00) --  (_10);
    \draw [->] (_01) edge [bend right]  (_00);
    \draw [->] (_10) edge [loop left] (_10);
     
    \node[node] (00) {$\neg t_1  \wedge \neg t_2$};
     
    \node[initial,circle,node,minimum width=0mm] (0) [below=2cm of 10] {$s_0$};
    
    \node[circle,node,minimum width=0mm] (1) [right=2cm of 0] {$s_1$};
    
    
    \draw [->] (0) edge [bend right] 
            node [below,text width=1cm ] (A)     {$00 | 01$ \\ $01 | 01$}     (1);
    
        \draw [->] (1) edge [bend right] 
            node [above,text width=1cm ]{$00 | 00$ \\ $01 | 00$ \\ $10 | 00$} (0);
    
        \draw [->] (0) edge [loop above] 
            node [above,text width=1cm ]{$10 | 10$} (0);
    
    \node [above of=A] {Controller};
    
    
    \end{tikzpicture}
    \caption{An example of target and adaptee transition systems and a transducer that guarantees, for example, the implications $\phi_i \to \psi_i$ for $i=1,2$ and $\phi_1=GF(\neg t_1 \wedge t_2)$, $\psi_1=GF(\neg a_1 \wedge a_2)$, $\phi_2=GF(t_1 \wedge \neg t_2)$, and $\psi_2=GF(a_1 \wedge \neg a_2)$.}
    \label{fig:example}
\end{figure}

From this point on, we will only talk about this representation of the problem, i.e., we will synthesize a controller that reads a run  of an input transition system and produces a run of an output transition system such that the combined run always satisfies a set of $GR(k)$ properties. 
%Note that it is usually not possible to ignore the input system by generating a controller that ignores its inputs and just satisfy all the $\psi$ properties. 

% In this paper we propose to use reactive synthesis in a nontraditional way: 
% we propose to apply a reactive synthesis based algorithm for generating strategies that read the actions of a controller on input systems and reacts by producing actions on output systems. 
% There is no interaction, in our setting, between the input and the output systems. 
% The only connection between the systems is formed by the synthesized strategy that observes the input system and adapts actions on the input system to actions on the output system.
% %\gatodo{"No interaction" is imprecise and thus may confuse. Consider instead e.g.: "rather then interacting with its environment, the output system merely observes the actions taken by the input system, and acts accordingly."}
% The specification to the synthesizer consists of: (1) transition systems for the input and for the output systems; (2) a temporal logic formula of a specific form
% that maps properties
% %\gatodo{I am not sure that it is "state properties". Maybe "liveness properties"? Also, I think that the footnote should appear at the end of the sentence (after the period) since it relates also to the "state property to state property".}
% of states of the  input system to properties of states of the output system.\footnote{$GR(k)$ formulas where all the left hand side variables are from the input system and all the right hand side variables are from the output system, as elaborated later in the paper.} 
% Based on this data, our strategy generates actions for the output system in reaction to actions on the input system such that if a property repeats infinitely often in the input, its related property in the output system must also repeat infinitely often.  

% Imagine, as a simple example for demonstration purposes, that we have a Rubik cube and a controller that keeps turning the cube sides in order to achieve goals that are not known to us (possibly because this is a legacy system).
% Imagine further, that there is a defect in our cube requiring us to transfer the actions that the controller planned for the normal cube to actions on the cube with the defect.
% Think, for example, of a defected Rubik cube in which the sides can only be turned clockwise, not counterclockwise.
% Using the tool proposed in this paper, we can apply the following steps towards transferring actions on the normal cube to actions on the faulty one:
% \begin{enumerate}
% \item Model both the transition systems of the normal cube and of the faulty one.
% \item Specify that the properties that we care about are completions of sides, i.e., ask the synthesizer to guarantee that if a side is completed infinitely often on the normal cube it must also be completed infinitely often on the faulty cube.  
% \item Invoke our synthesis algorithm to obtain a transfer strategy.
% \item Run the original controller on a virtual simulated copy of the normal cube and use the synthesized strategy to transfer actions that the controller planned to run on the virtual cube to actions that we can apply to the faulty one. 
% \end{enumerate}

% Note that we cannot, in this setting, directly synthesize a controller for the faulty cube because we do not have a specification of how it should behave (we do not even have the specifications for the controller of the normal cube). 
% Note also that it is not always possible to ignore the input system by generating a controller for the output system that just achieves all the goal states in the output system infinitely often. 
% Imagine, for example, a game where we are forced to move the cube in a way that allows to complete either the red side or the blue side infinitely often, but not both. In this case, we must synthesize a controller that follows the actions in the input system and translates them to actions in the output system in a way that the side that is completed infinitely often in the normal cube is also completed infinitely often in the faulty, without knowing, perhaps until a late point of the run, which side it is going to be. 

%The Rubik Cube example demonstrates the capability of our framework to handle what we call \textit{Automatic Fault Corrections}, in which the objective is to find a strategy that gives a plan to a faulty system that is at least as good as the plan for the original one [[DF: is that so??]].
%This however is not the only use-case for our approach that one could have in mind.
%Think for example of \textit{Adaptive systems in Automatic Decentralization}. There, constructing a distributed system from third-party components is challenging due to problems related to compatibility and communication issues. One approach for solving such problems is to start with a centralized solution and then adapt it to distributed setting by adding more general interactions between the components. The tools that we describe in this paper can be used for generating adaptors for running black-box components in a distributed setting. The distributed system is required to behave as the centralized one would but also obeying the restrictions modeled by the transition relation of the output system.
%As another example one could also think of \textit{automatic software product line development}, which is an engineering technique for creating a collection of similar software systems from a shared set of software assets. The tools that we are presenting in this paper can be used to implement software product lines with less effort. Specifically, a company can design a controller for a base system and then transfer its actions automatically to similar systems down the product line using our synthesis algorithm. These examples, of course, are only a partial list of potential applications for our tools. We are sure that readers can extend this list and think of many variants of the ideas raised above.


% To further motivate the proposed methodology, we list some abstract use-cases for which we identify how a transferring the actions of a controller to a new domain can be useful:

% \begin{description}

% \item[Automatic Fault Correction:] As demonstrated in the Rubik cube example, the output system can be a faulty version of the one that the controller was designed to handle. 
% The synthesis algorithm that generates the strategy for handling a fault can run on-the-fly when a fault is detected or off-line for commonly occurring faults.
% %\gatodo{Maybe it's just me, but I don't understand this sentence} 
% The synthesis can be simple, e.g., if the side can only be turned clockwise just turn it counterclockwise three times to simulate a single turn. It can also be more complicated, as follows. Say, for example, that the normal cube must commit to finishing either the yellow or the green side infinitely often, but it can do so at any time; however with the faulty cube we have to make this commitment at the first step. In this case, we have to wait for the commitment on the virtual cube and only then start our moves on the faulty cube. We can support this possibility by adding self-loops on the output system initial state which allow the synthesized strategy  to wait and examine several steps of the input system before it makes a move in the output system.
% %\gatodo{I understand the second case, but it is not clear why our synthesis algorithm supports it. Maybe add here: "we can support this possibility by adding self-loops on the output system transitions, which allow it to wait and examine several consecutive steps by the input system.}

% \item[Automatic Decentralization:] Constructing a distributed system from third-party components is challenging due to problems related to compatibility and communication issues. One approach for solving such problems is to start with a centralized solution and then adapt it to distributed settings by adding interactions between the components. The tools that we describe in this paper can be applied for adapting components that were not designed for it to operate in a distributed setting. In this case, the input system will be the centralized version for which we have a controller. The synthesis can then be used to transfer the actions to a transition system that only allows actions that can be implement in the distributed environment.

% \item[Automatic Generation of Software Product Lines:] Software product line development is an engineering technique for creating a collection of similar software systems from a shared set of software assets. The tools that we are presenting in this paper can be used to implement software product lines with less effort. Specifically, a company can design a controller for a base system and then transfer its actions automatically to similar systems down the product line using our synthesis algorithm.
%  \end{description}
 
% This is, of course, only a partial list of potential applications for our tools. We are sure that readers can extend this list and think of many variants of the ideas raised above. %The focus of this paper is on the core synthesis algorithm and on the analysis of its performance. The research on practical applications of the method for the above and for other application domains is left for future work.

% Our framework lies on the specific structure of our reactive synthesis $GR(k)$ settings. These consist of $G_I$ and $G_O$ that are transition systems for the input and output respectively, and a specification formula $\varphi$.




% that is a conjunct of $k$ $GR(1)$ constraints for each the left-side is only over the input variables, and the right-side is only over the output variables \dftodo{fix terminology}.
% While there are standard techniques that synthesize this kind of specifications (see related work for more), our solution exploits this specific setting to yield a more efficient solution in terms of computational complexity \dfnote{be more specific}. For that, we show how synthesis of our problem is reduced to solving a special kind of a  \textit{weak B\uchi} game.


\dftodo{Consider ditching this paragraph, that goes to too many details. But do mention the separation of variables. Say something like: note that we have separation of variables between the input  and output. This paper technically exploits this separation towards utilizing better algorithms.}
A problem formulation in our setting is a game structure that consists of two separated transition systems called  $G_\I$ and $G_\O$ respectively in a symbolic representation (with disjoint variables) and a $GR(k)$ formula $\Lambda$ of the form $\bigwedge_{i=1}^k(\phi_i\rightarrow\psi_i)$, where the $\phi_i$ are conjuncts of Globally-Finally Boolean formulas on the \textit{$\I$-variables only}, and the $\psi_i$ are conjuncts of Globally-Finally Boolean formulas on the \textit{$\O$-variables only}. Note that $GR(k)$ formulas also capture DBA properties, i.e. properties recognized by deterministic B\"uchi automata~\cite{}. The formula, $\Lambda$ represents a required connection between the runs of $G_\I$ and the runs of $G_\O$: it says that we want to generate runs in $G_\O$, based on an observing an ongoing run of $G_\I$, such that if things repeat infinitely often in the $\I$-run then their corresponding consequences must also occur infinitely often in the $\O$-run.

% specific type of $GR(k)$ formulation. These are a set of $k$ temporal constraints, each is of the form $\phi\rightarrow\psi$, where $\phi$ is a conjunct of Globally-Finally Boolean formulas on the \textit{environment variables only}, and $\psi$ is a conjunct of Globally-Finally Boolean formulas on the \textit{system variables only}.

%Together with the accompanied transitions systems of the input and output $G_I$ and $G_O$ respectively,
%that is standard in $GR(k)$ formulations, the 

% As such, our formulation can be interpreted as a game over the state space described by the tuple, that can hint towards a route to solving $GR(k)$. 

Note that unlike standard $GR(k)$ the choices of the system only affect $G_\O$ while the environment plays on a completely disconnected system $G_\I$. The only connection between the two is the formula $\Lambda$. 
%Indeed, there are explicit and symbolic methods to solve such problems with an efficiency of $O(n^2)$ where $n$ is the number of states in the resulting graph game. \dftodo{sharpen complexity result}.

%Note that unlike standard $GR(k)$, the environment/system variables in our formulation are separated by the $\rightarrow$ connector [[DF: say better]]. 

%As such, our formulation describes an  interaction between two separated games that are played: one of the environment, and one over the system.

To synthesize a winning strategy, we use the fact that each connected component of the product of the two systems is either a winning or a losing sub game for the output system, regardless of the initial state of the play. This allows us to reduce the problem into a \emph{weak-B\"uchi} game, i.e. to play a strategy to stabilize in a winning connected component. We further formulate an interesting property that both our game and the reduced weak B\"uchi game possess, the \emph{delay property}: Assume we follow a winning strategy, and, at some point, for some reason, the input system successfully manages to take several steps with no intermediate response by the output systems. Then, the reached state is still winning for the output system. This enable us to decide the realizability of the specification in $O(N)$ symbolic operations, and to synthesize a controller for a realizable specification in $O(|\varphi|N)$ symbolic operations, where $\varphi$ is the GR($k$) winning condition, and $N$ is the size of the state-space. We remark that, in general, GR($k$) games are solved in $O(N^{k+1}k!)$ operations~\cite{PitermanP06}.

In Section 2 we give preliminaries and discuss related work in Section 3.
%\gatodo{isn't it better before the conclusion}
In Section 4 we formulate our problem and provide a solution that uses a weak-B\"uchi solver as a black box.
In Section 5 we show how to solve weak B\"uchi games in linear time. First, we provide an explicit solution and then explain how to modify it into a symbolic algorithm. In Section 6 we utilize our framework into a tool, followed by running experimental evaluations on these examples and compare against state-of-the-art synthesis tools. We conclude in Section 7.




\subsection{Gal Point of Objection to Introduction}

To read the following after reading Figure 1.
There is also an alternative introduction in Appendix C that reflects the introduction.

For Gera - consider the following points while revising the intro.  First, note that in what is written the target corresponds to the input TS, and the adaptee is the output TS.
     \begin{itemize}
         \item   I think that the target should be what we want to have. If you say that you have the target transducer, then why there is a problem to solve here?
         
         
         \item On one hand you have $Adaptee\circ adapter$ which generates $\O$-valuations (the guarantees part). You say that this should be equiv to the Target (i.e. the Input System) that generates $\I$-valuations. This makes sense only when the gars are equal to the assumptions, I think. Quite narrows the discussion, isn't it?
         
         \item Likewise, calling the Input system: Target, makes sense when we want to imitate its behaviors. This is not the only application we have. What about correcting the Input system (traffic lights), covering it (cleaning robots), improving it (railways)? I am not sure why "imitating" is the main contribution we want to sell? Is it that so more important than correcting, covering and improving? 
         
         
         \item I ask myself how the user will use the adapter in practice. I think that the answer is that she will activate the Output (Adaptee) afterwards i.e. $Adaptee\circ adapter$ (right?). Hence, we get $(Adaptee) \circ (Adapter) = (Adaptee) \circ (Adaptee^{-1}\circ Controller \circ Target)$. Clearly, the latter is just $Controller\circ Target$. Isn't it weird? We synthesize a controller, change it to an Adapter we give the user, so the user will extract the controller out of the Adapter (i.e compose the $Adaptee$ to nullify the $Adapter^-1$ we composed to the controller) ?
        
        
         \item A similar comment to the previous item. Eventually, we satisfy a GR($k$) formula $\varphi$. I expect that the reader will ask: what system satisfies $\varphi$? The answer is of course the controller. Shouldn't we put more emphasis on the controller as what we are interested in?
        
        
         \item Technically, we synthesize a controller. I ask myself what we should do to construct an Adapter from it. I think that we need to add memory to remember the previous assignment to $\O$ so we can compute $Adaptee^{-1}$ (do you have a better way?). This means that, in the worst case, we increase the memory by a factor of  $2^\mathcal O$. Seems like a huge overhead considering the fact that the client will actually use $Adaptee \circ Adapter$. In other words, $Controller \circ Target$ is way more efficient than $Adaptee \circ adapter = Adaptee \circ (Adaptee^{-1}\circ Controller \circ \Target)$.
        Gera answers: what if the adaptee is some hardware, e.g. some robot. Then, we need to extract the command we need to give to the robot from the configuration.
         
         \item (minor, but perhaps the only interesting debate I can raise. Read only if you are in a philosophical mood.): We all agree that the reactive interpretation is 95\% adequate to the original Adapter design pattern. The question is what are the 5\% we give up on. According to the current intro, we insist to keep the next property: \textbf{the user speaks with the Adapter}. When I suggest to write $Adapter=Controller \circ Input$ my aim is to maintain the next property: \textbf{The Adapter accesses an existing code}. I want to try and argue that it is perfectly fine to give up on the requirement that the user speaks with the Adapter. The reason is that reactive systems are different from interfaces. When speaking about interfaces, the client initiates the process so it makes sense that the adapter will receive her requests. But, usually, in a reactive system the client lies in the end of the process and enjoys the outputs. As an example, think of an auto-land system. The aircraft sensors are the guys who initiate processes. The client enjoys the outputs by staying alive!  Hence, it makes sense to me to put the adapter just before the client - so the Adapter can process the outputs to fit the client needs. This is why I don't think it is that important to insist that the Adapter will act first - this is not the essence of the Adapter design pattern that we should keep.
     
     
    % \item the design pattern is about using an existing code (the adaptee). In my mind the \emph{only} code we have is the input system. Hence, the adaptee must be the input system.
    % \item Again - if the input is the target, then you were given the target and there is no problem to solve.  So, if you agree with the first comment, the input cannot be the target.
    % \item What we call input corresponds to the traditional "environment". The usual framework is that the controller we synthesize gets inputs from the environment (the input TS) and provide sys-var outputs. Here you do something extremely complicated: (1) You decide that both the environment and the controller we synthesize has the same input alphabet (which is unknown and not exactly part of the game-structure) (2) you decide that the controller acts first, upon inputs for the environment player (3) the controller produces an output from the mysterious alphabet that the "system" acts upon, (4) you let the environment run in parallel to that composition of the synthesized controller and the system, (5) for that, you came up with a non-standard transducer concatenation. I believe it will be very difficult for the reactive-synthesis community to grasp this conducting (at least it is for me. Not sure that I am a decent representative, but I do know what is going on here and it is not easy for me to understand how it works...) 
     %\item calling the input "target" makes sense only when we actually interested in the input system behaviors. It is extremely awkward over examples like the cleaning robots, the railways, and the traffic lights.
     %\item (minor) Seeing the output system as a transducer seems awkward to me. The output system is just about which steps are legal - it is the safety guarantees, no more than that. 
     %\item What you claim we synthesize (e.g. in Figure~\ref{fig:transducers}) is not what we say we synthesize in the preliminaries (i.e. the inputs and outputs are variables and not U/S/D) and not what our tool produces. It is also not aligned with how we model a strategy (a BDD over input and output variables such that ...)
     %\item more later...
     \end{itemize}



%As we show in this paper, when there is a separation of system as described above, the system can always delay its actions and wait for the environment to pick a certain path in that game.
%\gatodo{I really don't like this sentence. It is confusing as it delivers the feeling the we give the output system the possibility to do so - and this is not the case. Instead, I would write something like: "we prove an interesting property of the games we study, that we name the \emph{delay-property}: If, for some reason, the input system will decide to take several steps in a solo run with no intermediate response from the output system, this will not affect the possibility of the output system to win the play and satisfy the GR($k$) target condition."} 
%We call this property the \textit{delay property} of the game.
%We show that exploiting this property leads to a decomposition of the game-graph into connected component, where some of the connected component are called \textit{accepting}. Then the game between the environment and the system is reduced to a game on the connected components graphs, where the system's objective to reach an accepting connected component and to stay there (in that sense this is similar to playing game on Weak Automata). As we show, our techniques lower the complexity of solving such games over state-of-the-art techniques. \gatodo{the technical outline is incorrect. We should discuss}

%In Section 2 we give preliminaries and discuss related work in Section 3. In Section 4 we describe our problem formulation and describe our synthesis framework on the explicit setting\gatodo{no explicit setting in sect4}, at the heart of which lies the delay-property\gatodo{the dealt property is a property of the weak-b\"uchi game, not (exactly) of our game}. We then describe our symbolic implementation in Section 5\gatodo{we solve weak-b\"uchi in sect5}. In Section 6 we elaborate on problem domains and give concrete examples, followed by running experimental evaluations on these examples and compare against state-of-the-art synthesis tools. We conclude in Section 8.



%\dftodo{tie between the use cases and the experiments at the end}
%\dftodo{Add two paragraphs that explain the paper.}

%\dftodo{Move to Conclusion: "The focus of this paper is on the core synthesis algorithm and on the analysis of its performance. The research on practical applications of the method for the above and for other application domains is left for future work."}





==> Introduction_df.tex <==


 \section{Introduction}
 \label{sec:intro}


% In this paper we explore the adapter design pattern from the reactive systems perspective. Since the design pattern is a software-engineering concept rather than mathematical formulation, our first task is to offer formalism that capture the adapter "spirit". Already here we face a challenge: what is the correct conceptual way in which the adapter should be designed. While some variants would define an adapter as an interface between the adaptee and the target, others would describe it as an interface that subsumes the adaptee such that the user interacts only with the adapter. Another approach is to have the adapter before the adaptee, thus being an interface between the user input and the adaptee.



The field of reactive synthesis has produced various techniques for automatic generation of  controllers that react to inputs under given constraints in a way that satisfies required specifications. These techniques have been shown to be practical in providing effective tools for the design of correct-by-construction systems. 

Inspired by the well known adapter design pattern~\cite{gamma1995design}, we study the use of reactive synthesis for synthesizing adapters that translate inputs meant for a target transducer to inputs of an adaptee transducer. Think, for example, of the task of adding a layer to an operating to adapt for a hardware vulnerability that we need to avoid.

Formally, we propose the following synthesis problem: given two finite state transducers called $Target$ and $Adaptee$, synthesize a finite state transducers called $Adaper$ such that
\[    Adaptee \circ Adapter \eqsim Target.\]
Where $\circ$ represents transducer composition, i.e., we are comparing the target with a composition of the adaptee with an adapter, where the adapter acts before the adaptee. The $\eqsim$ symbol represent an equivalence relation specified by  the user of the synthesis algorithm. Since, it is not always reasonable to require full equality, we only require that they are equivalent. In this work we consider specifications consisting of sets of required $\omega$-regular properties over the possible outputs of the transducer $(Adaptee \circ Adapter) \cdot Target$ where $\cdot$ represents transducer concatenation.
 To this end, we assume, without loss of generality, that the output of the $Target$ and $Adaptee$ transducers are sequences of truth assignments of two disjoint sets of, respectively, input and output atomic propositions.

Consider, for example, the transducers depicted in Figure~\ref{fig:transducers}. As common in the literature, we represent truth assignments to atomic propositions as elements in $(0+1)^*$ where 0 or 1 at the $i$th letter means assigning the $i$th variable with False or True, respectively. In this example, both transducers produce truth assignment of two (different) sets of atomic propositions of size two, so the length of all these words is two. The requirement is that, for any given input,  if an output is repeated infinitely often $Target$, it must also repeat infinitely often in $Adaptee \circ Adapter$. The transducers achieves this by circling  in the $s_0 \leftrightarrow s_1$  loop of the $Adaptee$ when the $Target$ circles in $s_1$.

\begin{figure}
    \centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.5cm,initial text=,
  thick,node/.style={fill=blue!20,draw,
  font=\sffamily\footnotesize, circle}]

\node[initial,node] (00) {$s_0$};

\node[node] (01) [above of=00] {$s_1$};
\node[node] (10) [below of=00] {$s_2$};
\node [above=0.3cm of 01] {Target};

\draw [->] (00) -- node {$U|10$} (01);
\draw [->] (00) -- node {$D|01$} (10);
\draw [->] (01) edge [loop left] node {$S|01$} (01);
\draw [->] (10) edge [loop left] node {$S|10$} (10);

\node[initial,node] (_00) [left=7cm of 00] {$s_0$};
\node[node] (_01) [above of=_00]    {$s_1$};
\node[node] (_10) [below of=_00]    {$s_2$};
\node [above=0.3cm of _01] {Adaptee};

\draw [->] (_00) edge [bend right] node [right] {$U|01$} (_01);
\draw [->] (_00) -- node {$D|10$} (_10);
\draw [->] (_01) edge [bend right] node [left] {$D|00$} (_00);
\draw [->] (_10) edge [loop left] node {$S|10$} (_10);
 
%%%
    \node[initial,circle,node,minimum width=0mm] (0) [left=4cm of 01] {$s_0$};
    
    \node[circle,node,minimum width=0mm] (1) [below of= 0] {$s_1$};
        
    \draw [->] (0) edge [bend right] 
            node [left] (A)     {$U | U$}     (1);
    
        \draw [->] (1) edge [bend right] 
            node [right]{$S | D$} (0);
    
        \draw [->] (0) edge [loop right] 
            node [right,text width=1cm ]{$S|S$ \\ $D|D$} (0);
    
    \node (adapter)  [above=0.3 cm of 0] {Adapter};

\node[] () [left=.5cm of adapter] {$\circ$};
\node[] () [right=1.5cm of adapter] {$\eqsim$};

\end{tikzpicture}
    \caption{An example of target and adaptee transducers and an adapter  that guarantees, for example, $GF(t_i) \to GF(a_i)$   for $i=1,2$  where $\{t_1, t_2\}$ and $\{a_1,a_2\}$ are the atomic propositions of the target and of the adaptee, respectively.}
    \label{fig:transducers}
\end{figure}



While most of the work on software synthesis focuses on synthesizing complete systems from their specifications, our focus is on using reactive synthesis for reusing existing components. The $Target$ transducer can model, for example, a standard Rubik cube and the $Adaptee$ can model a Rubik cube with some hardware failure. Since we know how to operate the normal cube, we could use an $Adapter$ that translates commands that we planed to send to the normal cube to commands that we can send to faulty one. The equivalence relation can say, for example, that if a side of the normal cube would have been completed infinitely often in the expected run of the normal cube it should also be completed infinitely often in the generated run of the faulty cube.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Dror will add a paragraph saying that the problem is very hard and that current state of the art tools cannot handle even small instances. Accordingly, we propose to use GR(K) formulas instead of just any $\omega$-regular properties.

Generally, synthesizing a transducer is complicated - complexity wise. Indeed, Even when equality is required, synthesizing is a non trivial task. \dftodo{write much better and explain the hardness, as a step towards GRk}


\dftodo{Now we mention GR(k) and how to utilize GR(k) that balance between expressiveness and efficiency. Mention the term "reactive synthesis".}


To allow direct use of the language of reactive synthesis, and to allow more generality, the input to our synthesis algorithm and to the tool that implements it is a representation of $Adpatee$ and $Target$  as transition systems, as depicted in Figure~\ref{fig:example}. The $Input$ transition is a representation of the $Target$ and the $Output$ transition system is a representation of the $Adatpee$ where we ignore the inputs to the systems and the state and consider only their outputs.

\begin{figure}
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,initial text=,
      thick,node/.style={fill=blue!20,draw,
      font=\sffamily\footnotesize,minimum width=15mm}]

    \node[initial,node] (00) {$\neg t_1  \wedge \neg t_2$};
    \node[node] (01) [above of=00] {$\neg t_1  \wedge t_2$};
    \node[node] (10) [below of=00] {$t_1  \wedge \neg t_2$};
    \node [above= 0.2 cm of 01] {Input};

    \draw [->] (00) --  (01);
    \draw [->] (00) --  (10);
    \draw [->] (01) edge [loop left] (01);
    \draw [->] (10) edge [loop left] (10);

    \node[initial,node] (_00) [right=2cm of 00] {$\neg a_1  \wedge \neg a_2$};
    \node[node] (_01) [above of=_00]    {$\neg a_1  \wedge a_2$};
    \node[node] (_10) [below of=_00]    {$a_1  \wedge \neg a_2$};
    \node [above= 0.2 cm of _01] {Output};

    \draw [->] (_00) edge [bend right]  (_01);
    \draw [->] (_00) --  (_10);
    \draw [->] (_01) edge [bend right]  (_00);
    \draw [->] (_10) edge [loop left] (_10);
     
    \node[node] (00) {$\neg t_1  \wedge \neg t_2$};
     
    \node[initial,circle,node,minimum width=0mm] (0) [below=2cm of 10] {$s_0$};
    
    \node[circle,node,minimum width=0mm] (1) [right=2cm of 0] {$s_1$};
    
    
    \draw [->] (0) edge [bend right] 
            node [below,text width=1cm ] (A)     {$00 | 01$ \\ $01 | 01$}     (1);
    
        \draw [->] (1) edge [bend right] 
            node [above,text width=1cm ]{$00 | 00$ \\ $01 | 00$ \\ $10 | 00$} (0);
    
        \draw [->] (0) edge [loop above] 
            node [above,text width=1cm ]{$10 | 10$} (0);
    
    \node [above of=A] {Controller};
    
    
    \end{tikzpicture}
    \caption{An example of target and adaptee transition systems and a transducer that guarantees, for example, the implications $\phi_i \to \psi_i$ for $i=1,2$ and $\phi_1=GF(\neg t_1 \wedge t_2)$, $\psi_1=GF(\neg a_1 \wedge a_2)$, $\phi_2=GF(t_1 \wedge \neg t_2)$, and $\psi_2=GF(a_1 \wedge \neg a_2)$.}
    \label{fig:example}
\end{figure}

From this point on, we will only talk about this representation of the problem, i.e., we will synthesize a controller that reads a run  of an input transition system and produces a run of an output transition system such that the combined run always satisfies a set of $GR(k)$ properties. 

\dftodo{Consider ditching this paragraph, that goes to too many details. But do mention the separation of variables. Say something like: note that we have separation of variables between the input  and output. This paper technically exploits this separation towards utilizing better algorithms.}
A problem formulation in our setting is a game structure that consists of two separated transition systems called  $G_\I$ and $G_\O$ respectively in a symbolic representation (with disjoint variables) and a $GR(k)$ formula $\Lambda$ of the form $\bigwedge_{i=1}^k(\phi_i\rightarrow\psi_i)$, where the $\phi_i$ are conjuncts of Globally-Finally Boolean formulas on the \textit{$\I$-variables only}, and the $\psi_i$ are conjuncts of Globally-Finally Boolean formulas on the \textit{$\O$-variables only}. Note that $GR(k)$ formulas also capture DBA properties, i.e. properties recognized by deterministic B\"uchi automata~\cite{}. The formula, $\Lambda$ represents a required connection between the runs of $G_\I$ and the runs of $G_\O$: it says that we want to generate runs in $G_\O$, based on an observing an ongoing run of $G_\I$, such that if things repeat infinitely often in the $\I$-run then their corresponding consequences must also occur infinitely often in the $\O$-run.

% specific type of $GR(k)$ formulation. These are a set of $k$ temporal constraints, each is of the form $\phi\rightarrow\psi$, where $\phi$ is a conjunct of Globally-Finally Boolean formulas on the \textit{environment variables only}, and $\psi$ is a conjunct of Globally-Finally Boolean formulas on the \textit{system variables only}.

%Together with the accompanied transitions systems of the input and output $G_I$ and $G_O$ respectively,
%that is standard in $GR(k)$ formulations, the 

% As such, our formulation can be interpreted as a game over the state space described by the tuple, that can hint towards a route to solving $GR(k)$. 

Note that unlike standard $GR(k)$ the choices of the system only affect $G_\O$ while the environment plays on a completely disconnected system $G_\I$. The only connection between the two is the formula $\Lambda$. 
%Indeed, there are explicit and symbolic methods to solve such problems with an efficiency of $O(n^2)$ where $n$ is the number of states in the resulting graph game. \dftodo{sharpen complexity result}.

%Note that unlike standard $GR(k)$, the environment/system variables in our formulation are separated by the $\rightarrow$ connector [[DF: say better]]. 

%As such, our formulation describes an  interaction between two separated games that are played: one of the environment, and one over the system.

To synthesize a winning strategy, we use the fact that each connected component of the product of the two systems is either a winning or a losing sub game for the output system, regardless of the initial state of the play. This allows us to reduce the problem into a \emph{weak-B\"uchi} game, i.e. to play a strategy to stabilize in a winning connected component. We further formulate an interesting property that both our game and the reduced weak B\"uchi game possess, the \emph{delay property}: Assume we follow a winning strategy, and, at some point, for some reason, the input system successfully manages to take several steps with no intermediate response by the output systems. Then, the reached state is still winning for the output system. This enable us to decide the realizability of the specification in $O(N)$ symbolic operations, and to synthesize a controller for a realizable specification in $O(|\varphi|N)$ symbolic operations, where $\varphi$ is the GR($k$) winning condition, and $N$ is the size of the state-space. We remark that, in general, GR($k$) games are solved in $O(N^{k+1}k!)$ operations~\cite{PitermanP06}.

In Section 2 we give preliminaries and discuss related work in Section 3.
%\gatodo{isn't it better before the conclusion}
In Section 4 we formulate our problem and provide a solution that uses a weak-B\"uchi solver as a black box.
In Section 5 we show how to solve weak B\"uchi games in linear time. First, we provide an explicit solution and then explain how to modify it into a symbolic algorithm. In Section 6 we utilize our framework into a tool, followed by running experimental evaluations on these examples and compare against state-of-the-art synthesis tools. We conclude in Section 7.

\subsection{Gal Point of Objection to Introduction}

To read the following after reading Figure 1.
There is also an alternative introduction in Appendix C that reflects the introduction.

For Gera - consider the following points while revising the intro.  First, note that in what is written the target corresponds to the input TS, and the adaptee is the output TS.
     \begin{itemize}
         \item   I think that the target should be what we want to have. If you say that you have the target transducer, then why there is a problem to solve here?
         
         
         \item On one hand you have $Adaptee\circ Adapter$ which generates $\O$-valuations (the guarantees part). You say that this should be equiv to the Target (i.e. the Input System) that generates $\I$-valuations. This makes sense only when the gars are equal to the assumptions, I think. Quite narrows the discussion, isn't it?
         
         \item Likewise, calling the Input system: Target, makes sense when we want to imitate its behaviors. This is not the only application we have. What about correcting the Input system (traffic lights), covering it (cleaning robots), improving it (railways)? I am not sure why "imitating" is the main contribution we want to sell? Is it that so more important than correcting, covering and improving? 
         
         
         \item I ask myself how the user will use the adapter in practice. I think that the answer is that she will activate the Output (Adaptee) afterwards i.e. $Adaptee\circ adapter$ (right?). Hence, we get $(Adaptee) \circ (Adapter) = (Adaptee) \circ (Adaptee^{-1}\circ Controller \circ Target)$. Clearly, the latter is just $Controller\circ Target$. Isn't it weird? We synthesize a controller, change it into an Adapter, and give it the user so the user will extract the controller out of the Adapter (i.e compose the $Adaptee$ to nullify the $Adapter^{-1}$ we composed to the controller) ? This is one of the reasons I suggest $Adapter=Controller$.
        
        
         \item A similar comment to the previous item. Eventually, we satisfy a GR($k$) formula $\varphi$. I expect that the reader will ask: what system satisfies $\varphi$? The answer is of course the controller. Shouldn't we put more emphasis on the controller as what we are interested in?
        
        
         \item Technically, we synthesize a controller. I ask myself what we should do to construct an Adapter from it. I think that we need to add memory to remember the previous assignment to $\O$ so we can compute $Adaptee^{-1}$ (do you have a better way?). This means that, in the worst case, we increase the memory by a factor of  $2^\O$. Seems like a huge overhead considering the fact that the client will actually use $Adaptee \circ Adapter$. In other words, $Controller \circ Target$ is way more efficient than $Adaptee \circ adapter = Adaptee \circ (Adaptee^{-1}\circ Controller \circ Target)$.
        Gera answers: what if the adaptee is some hardware, e.g. some robot. Then, we need to extract the command we need to give to the robot from the configuration.
         
         \item (minor, but perhaps the only interesting debate I can raise. Read only if you are in a philosophical mood.): We all agree that the reactive interpretation is 95\% adequate to the original Adapter design pattern. The question is what are the 5\% we give up on. According to the current intro, we insist to keep the next property: \textbf{the user speaks with the Adapter}. When I suggest to write $Adapter=Controller$ my aim is to maintain the next property: \textbf{The Adapter accesses an existing code}. I want to try and argue that it is perfectly fine to give up on the requirement that the user speaks with the Adapter. The reason is that reactive systems are different from interfaces. When speaking about interfaces, the client initiates the process so it makes sense that the adapter will receive her requests. But, usually, in a reactive system the client lies in the end of the process and enjoys the outputs. As an example, think of an auto-land system. The aircraft sensors are the guys who initiate processes. The client enjoys the outputs by staying alive!  Hence, it makes sense to me to put the adapter just before the client - so the Adapter can process the outputs to fit to the client needs. This is why I don't think it is that important to insist that the Adapter will act first - this is not the essence of the Adapter design pattern that we should keep.
     
     
    % \item the design pattern is about using an existing code (the adaptee). In my mind the \emph{only} code we have is the input system. Hence, the adaptee must be the input system.
    % \item Again - if the input is the target, then you were given the target and there is no problem to solve.  So, if you agree with the first comment, the input cannot be the target.
    % \item What we call input corresponds to the traditional "environment". The usual framework is that the controller we synthesize gets inputs from the environment (the input TS) and provide sys-var outputs. Here you do something extremely complicated: (1) You decide that both the environment and the controller we synthesize has the same input alphabet (which is unknown and not exactly part of the game-structure) (2) you decide that the controller acts first, upon inputs for the environment player (3) the controller produces an output from the mysterious alphabet that the "system" acts upon, (4) you let the environment run in parallel to that composition of the synthesized controller and the system, (5) for that, you came up with a non-standard transducer concatenation. I believe it will be very difficult for the reactive-synthesis community to grasp this conducting (at least it is for me. Not sure that I am a decent representative, but I do know what is going on here and it is not easy for me to understand how it works...) 
     %\item calling the input "target" makes sense only when we actually interested in the input system behaviors. It is extremely awkward over examples like the cleaning robots, the railways, and the traffic lights.
     %\item (minor) Seeing the output system as a transducer seems awkward to me. The output system is just about which steps are legal - it is the safety guarantees, no more than that. 
     %\item What you claim we synthesize (e.g. in Figure~\ref{fig:transducers}) is not what we say we synthesize in the preliminaries (i.e. the inputs and outputs are variables and not U/S/D) and not what our tool produces. It is also not aligned with how we model a strategy (a BDD over input and output variables such that ...)
     %\item more later...
     \end{itemize}
     
     

\subsection{Illustrative Examples}

The example we gave above demonstrates how our technique enables us to fit an existing controller to an unmatched hardware. We formalize now two more illustrative examples to demonstrate additional usages of our technique.

\vspace{3pt}
\noindent\textbf{Cleaning robots}. In this example, we demonstrate how one can use our technique to fulfill tasks that have not been covered by an execution of an existing controller. We consider a cleaning robot that moves along a corridor-shaped house, from room $1$ to room $n$. The robot follows some plan, and accordingly cleans some of the rooms. Hence, the robot control variables $\{\mathit{in{:}room}_i: 1\leq i\leq n\}$ that model its location, and variables $\{\mathit{in{:}clean}_i: 1\leq i\leq n\}$, each it raises after cleaning the corresponding room. Moreover, it raises a signal $\mathit{done}$ when it finishes fulfilling its plan. Our goal is to synthesize a second cleaning robot that follows the first robot and cleans exactly those rooms that have not been cleaned by the first robot. Hence, the robot we synthesize controls variables $\{\mathit{out{:}room}_i: 1\leq i\leq n\}$ and $\{\mathit{out{:}clean}_i: 1\leq i\leq n\}$, and it is required to fulfill requirements of the form: $\ltlG\ltlF(\mathit{done}) \wedge \ltlG\ltlF(\mathit{in{:}clean}_i)\rightarrow \ltlG\ltlF(\mathit{out{:}clean}_i)$, $\ltlG\ltlF(\mathit{done}) \wedge \ltlG\ltlF(\mathit{!in{:}clean}_i)\rightarrow \ltlG\ltlF(\mathit{!out{:}clean}_i)$.

\vspace{3pt}
\noindent\textbf{Railway Signalling.} In this example, we demonstrate how one can use our technique to improve the quality of an existing controller. We consider a junction of $n$ railways, each railway is equipped with a signal that can be turned on (light in green) or off (light in red). Some railways overlap and thus their signals cannot be turned on simultaneously. We consider the next overlapping pattern. Railways 1-4 overlap, likewise 3-6, 5-8, and so on.

An existing system activates the signals by assigning values to  $\{\mathit{in{:}signal}_i: 1\leq i\leq n\}$. To avoid accidents, it was programmed to be strictly safe; it never raises two signals simultaneously. 

We are interested in a controller that performs better. The controller should read the valuations that the existing system provides, and correspondingly assign values to  $\{\mathit{out{:}signal}_i: 1\leq i\leq n\}$. We want the new controller to produce safe and \emph{maximal} valuations; $\mathit{out{:}signal}_i$ is turned on iff the signal of every rail that overlaps with the $i$th rail is off.

Furthermore, we want to maintain liveness properties of the input system: 
\begin{itemize}
    \item For every $i=1\dots n$, if  $\mathit{in{:}signal}_i$ is turned on infinitely often, then  $\mathit{out{:}signal}_i$ is turned on infinitely often as well.
    
    \item For every $i=1\dots n$, if  $\mathit{in{:}signal}_i$ is turned on at least once in every $m$ consecutive steps (where $m$ is a parameter of the specification), then the same holds for $\mathit{out{:}signal}_i$.
\end{itemize}






==> ProblemStatement_old_semt.tex <==
\section{Separated GR(k) Games}
\label{Sec:PrblmStmnt}

The core contribution of this work is to define the notion of separation of variables in the context of games and to demonstrate the algorithmic benefits of separation.


We say, a game structure {\em separates variables} if the choices of any one of the players does not restrict the choices of the other. This can be formalized by requiring that (a). the initial guarantees are not dependent on the input variables $\I$, and (b). the safety assumptions and guarantees are dependent only on the player's variables and not those of the other player. Formally,

%We consider game structures that separate variables. Roughy, a game separate variables if the choices of any of the players cannot restrict the possible choices of the other player. We formalize this requirement by demanding that (1) the initial guarantees are not dependent on the first input, and (2) the safety assumptions and guarantees consider only the corresponding player's former choice. 

\begin{definition}
A game structure  $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ {\em separates variables} over input variables $\I$ and output variables $\O$ if:
\begin{itemize}
    \item The environment's initial assumption $\theta_\I$ is an assertion over $\I$ only.
    \item The system's initial guarantees $\theta_\O$ is an assertion over $\O$ only.
    \item The environment's safety assumption $\rho_\I$ is an assertion over $\I\cup \I'$ only.
    \item The system's safety guarantee $\rho_\O$ is an assertion over $\O\cup \O'$ only.
\end{itemize} 
\end{definition}

The interpretation of a game structure which separates variables is that the underlying directed graph of the game structure is the product of two directed graphs, one over the variables $\I\cup\I'$ and the other over  the variables $\O\cup\O'$. In the graph over $\I\cup\I'$, the graph states correspond to states of $\I$, the initial states of the graph are given by $\theta_\I$, and there is a transition between graph states $s$ and $t$ if $(s,t')\models \rho_\I$.
The second graph over $\O\cup\O'$ is similarly defined with graph states over $\O$, initial states given by $\theta_\O$, and transitions between $\rho_\O$.

%We focus on the useful GR($k$) wining condition~\cite{?}. While GR($k$) wining conditions are synthesized in exponential time~\cite{} \gatodo{to add a precise expression...}, we shall prove that an efficient synthesis algorithm exists when the formula separate variables.
Similarly, the notion of separation of variables extends to games with GR(k) specifications as follows:
\begin{definition}
\label{def:separatedGRk}
A GR(k) specification $\varphi$ over $\I\cup\O$ separates variables  separates variables w.r.t. $\I$ and $\O$, if $ \varphi = \bigwedge_{l=1}^k (  
\bigwedge_{i=1}^{n_l} \ltlG\ltlF(\varphi_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG\ltlF(\psi_{l,j})
)$ such that each $\varphi_{l,i}$ is an assertion over $\I$ and each $\psi_{l,j}$ is an assertion over $\O$. 
A GR($k$) game $(GS,\varphi)$ over input variables $\I$ and output variables  $\O$ separates variables if game structure $GS$ separates variables and GR($k$) specification  $\varphi$ separates variables w.r.t. $\I$ and $\O$. 
\end{definition}

We call a GR($k$) game that separates variables a {\em separated GR($k$) game}. 

\sbtodo{Justify symbolic-state representation of the problem statement}

\sbtodo{Some related work before stating final result}

We remark that a standard technique allows to replace assertions of a GR($k$) winning condition with DBA-properties. The cost of such a replacement is adding auxiliary variables. Specifically, an $m$-state DBA adds $\log m$ fresh variables.  However, this approach was shown to be both expressive and feasible. As an example, Dwyer et al. identified 55 typical patterns that are common in industrial specifications. 54 out of those 55 patterns are DBA properties, and none adds more than 3 auxiliary variables to the specification. Similarly, the parametric robotic patterns identified by Menghi et al. can be be supported by rather small DBAs. 
\gatodo{: meanwhile, this comment is mentioned here but it should be relocated.}


\begin{theorem}\label{thm:main}
[\sbtodo{To rephrase. Clarify technical result}]
Let $(\mathit{GS},\varphi)$ be a separated GR($k$) game over the input/output variables $\I$ and $\O$. Then, the realizability and synthesis problems for $(\mathit{GS},\varphi)$ are solved in $O(|\varphi|N)$ symbolic operations, where $N=|2^{\I\cup\O}|$.
\end{theorem}

The proof of Theorem~\ref{thm:main} is combined of two major step. In the first step, presented in Section~\ref{sec:reduction}, we describe how separated $GR(k)$ games can be reduced to solving a special type of weak b\"uchi games and how to translate a winning strategy for the later, to a strategy for separated $GR(k)$. Section~\ref{sec:algorithmsWeakBuchi} is dedicated to show how weak b\"uchi games are solved. 
Since the natural presentation of the problem is symbolic, we chose to describe a symbolic presentation of a solution for both steps. Note that while some of the symbolic descriptions we next discuss are common, an efficient representation to others are not trivial.




\begin{comment}
\subsection{Describing the problem as a graph \gatodo{to omit?}}
\label{Sec:graphdescription}

Since our solution involves a graph representation of the problem, we note that we can describe the problem as two graphs $G_\I=(V_\I,E_I),G_\O=(V_\O,E_\O)$ as follows. For $\mathcal X\in\{\I,\O\}$, $V_{\mathcal X} =2^{\mathcal X}$, and $E_\mathcal X=\{(s_0,s_1) : (s_0,s_1)\models \rho_\mathit X\}$.
%The set of vertices of $G_I$ is $2^{\I}$ and an edge $(s,s')$ is in $G_\I$ iff $(s,s')\models \rho_\I$. similarly, the set of vertices of $G_\O$ is $2^{\O}$ and an edge $(t,t')$ is in $G_\O$ iff $(s,s')\models \rho_\O$.
As such, we will be mostly interested in $G=G_\I\times G_\O=(V_\I\times V_\O,E)$ That is, the product graph $G$ of $G_\I$ and $G_\O$, in which $\big((s_0,t_0),(s_1,t_1)\big)\in E$ iff $(s_0,s_1)\in E_\I$ and $(t,t')\in E_\O$.

We rephrase the interaction between the players by seeing $G$ as a game-board. The vertices $V$ are the game states. From a state $(\inp_0,\out_0)$ the players choose together the ensuing state. First, system $A$ chooses $\inp_1\in V_\I$ such that $(\inp_0,\inp_1)\in V_\I$. Then, system $B$ responds by choosing $\out_1\in V_\O$ such that $(\out_0,\out_1)\in V_\I$, and the play traverses to $(\inp_1,\out_1)$.
We further adapt and apply on $G$ the notions of \emph{plays} and \emph{strategies}, given in the preliminaries section. These are defined in a natural manner and we omit the straightforward details.

To avoid possible different terminologies, we remind some fundamental notations.
A \textit{subgraph} $G_0$ of a directed graph $G$ is a graph $(V_0,E_0)$ where $V_0\subseteq V$ and $E_0= E\cap (V_0\times V_0)$. 
\textit{A path} in a graph $G$ is a sequence $(v_0,\cdots v_i)$ s.t. for all $0\leq j<i$ $(v_j,v_{j+1})\in V$. Note that a single vertex is also considered as a path.
A \textit{strongly connected component} (SCC) in a graph $G=(V,E)$, is a maximal subset $V_0\subseteq V$ such that for every vertices $v,v' \in V_0$, there exists a path from $v$ to $v'$ in $G$. Note that the set of all SCCs forms a partition of the graph-vertices.
%A \textit{maximal strongly connected component} is a strongly connected component that is not contained in any other strongly connected component.




%Note that this presentation does not serve as an arena which explicitly implements the symbolic representation of the game between the two players; it merely represents all legal steps the players can choose cooperatively.



%We now define a list $L$ of strongly connected components over $G$.

%Later we will define strongly connected components on $G$, then define the Connected-Partition problem.

%Add a list of Good connected components and bad connected components.

%A play is winning for the system if there a connected component $C$ in the list such that $GF(C)$ is satisfied. Otherwise the play is winning for the environment.

%Definitions needed:
%\begin{enumerate}
%    \item Notations for states and transition relations for $G_{\I}$ and $G_{\O}$
    
%    \item path
%    \item Strongly connected components
%    \item Good SCCs and Bad SCCs
%    \item Play
%    \item Winning plays for system and environment players
%    \item Synthesis problem and realizability problem (if different from what is given in Definition~\ref{Def:Symbolic}). 
%\end{enumerate}

\end{comment}

==> ProblemStatemento-old.tex <==
\section{Problem Formulation}
\label{sec:problem-def}

Our work can be thought of having two parts: formal modeling of the adapter design pattern in the reactive synthesis case, and solving the realizability and synthesis problem of our technical model.
We first describe two models that derive from different interpretation of the adapter design pattern. We show, however, how our formal model can address both interpretations towards conceiving a solution. That is to say - we show how both cars can use the same engine.
Next, we describe the technical model which we solve: the separated GR($k$) games.

\subsection{Modeling the adaptive design pattern}
\label{sec:modeling}

The adaptive design pattern allows three variant that can be thought of \dftodo{Bring citations}. In the first variant, the adapter's task is to come \textit{before} the adaptee. That means, serve as an interface between the user an the adapter that translates the input from the user to an input to the adaptee.
In the second variant, the adapter comes \textit{after}  the adaptee. In the third, the adapter \textit{cover} the adaptee.
All these variants need to interface with the \textit{Target} components that receives the same input ($input1$ in our case) but has it's own output.

% \begin{figure}
%     \centering
%     \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,initial text=,
%       thick,node/.style={fill=blue!20,draw,
%       font=\sffamily\footnotesize,minimum width=15mm}]
    
%     \node[node] (01) {$input1$};
%     \node[node] (02) [below of= 01] {$Adapter$};
%      \node[node] (03) [below of= 02] {$Adaptee$};
%      \node[node] (04) [below of= 03] {$output1$};
%       \node [above=0.3cm of 01] {1st Variant};
%     \draw [->] (01) -- (02);
%     \draw [->] (02) --  (03);
%     \draw [->] (03) --  (04);

%  \node[node] (31) [right = 2cm of 01] {$input1$};
%     \node[node] (32) [below of= 31] {$Adapee$};
%      \node[node] (33) [below of= 32] {$Adapter$};
%      \node[node] (34) [below of= 33] {$output1$};
%       \node [above=0.3cm of 31] {2nd Variant};
%     \draw [->] (31) -- (32);
%     \draw [->] (32) --  (33);
%     \draw [->] (33) --  (34);

%  \node[node] (21) [right = 2cm of 31] {$input1$};
%     \node[node] (22) [below of= 21] {$Adapter (contains Adaptee)$};
%      \node[node] (24) [below of= 22] {$output1$};
%       \node [above=0.3cm of 21] {3rd Variant};
%     \draw [->] (21) -- (22);
%     \draw [->] (22) --  (24);
%     \draw [->] (22) --  (24);
    
%      \node[node] (41) [right = 2cm of 21] {$input1$};
%     \node[node] (42) [below of= 41] {$Target$};
%      \node[node] (44) [below of= 42] {$output2$};
%       \node [above=0.3cm of 41] {Target};
%     \draw [->] (41) -- (42);
%     \draw [->] (42) --  (44);
%     \draw [->] (42) --  (44);
    

%     \end{tikzpicture}
%     \caption{Three different variants of our system plus the Target component}
%     \label{fig:3ModelExample}
% \end{figure}

The model in which the Adapter is \textit{before} the adaptee was discussed in Section~\ref{sec:intro}. Another variant to consider is where the Adapter is an ``over-all" solution. i.e., the adapter gets as an input the same input as Target, and emits the same output as the Adaptee. Formally, we synthesize an Adapter transducer as:
$\Adapter\equiv \Target$. Then we can use the same Separated-GR($k$) formulation to construct a controller from $\Target$ output to $\Adaptee$ output. Note however, that here the required Adapter is $\mathit{Controller}\circ \Target$.


Another way to consider adapters, is when the the adapter comes \textit{before} the adaptee. That is, the adpater takes the output of the adaptee and converts it to an output that matchet the output of the target. As an example, think of a socket adapter that connects an electrical gadget to a socket of a system that requires different voltage. Here we show how the modeling takes a whole different form, yet can be eventually reduced to solving Separated-GR($k$) as well.

We propose the following model: given a  transducer $\Adaptee$, synthesize transducer $\Adapter$ such that
\[   \mathit{Adapter} \circ  \mathit{Adaptee}  \models \mathit{Target \ Specification},\]
\dftodo{Gal, please explain why the Target is specification}
where $\circ$ represents transducer composition. To obtain a better understanding, we provide an explicit toy example, depicted in Figure~\ref{fig:example}. The existing Adaptee transducer controls variables $t_1$ and $t_2$, and it chooses to turn on only one of them. The Adapter transducer we aim to construct controls $a_1$ and $a_2$, and it has the following limitations: if it chooses to turn on $a_1$, it cannot change the values of $a_1$ and $a_2$ anymore. But, if it turns on $a_2$, it must turn it off immediately afterwards. This \emph{safety} limitations are depicted through what we call the \emph{output} transition system. In addition to this safety property, the liveness property the composition need to satisfy is captured by the LTL, specifically GR($k$), formula: $(\ltlG \ltlF(t_1)\rightarrow \ltlG \ltlF(a_1)) \wedge (\ltlG \ltlF(t_2) \rightarrow \ltlG \ltlF(a_2))$. The output system and the GR($k$) formula constitute the target specification. We provide in Figure~\ref{fig:example} an Adapter transducer that achieves the required.


\dftodo{Gal, please motivate choosing the specification Adaptee->Target as we discussed}


\begin{figure}
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,initial text=,
      thick,node/.style={fill=blue!20,draw,
      font=\sffamily\footnotesize,minimum width=15mm}]

    \node[initial,node] (00) {$\neg t_1  \wedge \neg t_2$};
    \node[node] (01) [above of=00] {$\neg t_1  \wedge t_2$};
    \node[node] (10) [below of=00] {$t_1  \wedge \neg t_2$};
    \node [above= 0.2 cm of 01] {Adaptee (Input)};

    \draw [->] (00) --  (01);
    \draw [->] (00) --  (10);
    \draw [->] (01) edge [loop left] (01);
    \draw [->] (10) edge [loop left] (10);

    \node[initial,node] (_00) [right=2cm of 00] {$\neg a_1  \wedge \neg a_2$};
    \node[node] (_01) [above of=_00]    {$\neg a_1  \wedge a_2$};
    \node[node] (_10) [below of=_00]    {$a_1  \wedge \neg a_2$};
    \node [above= 0.2 cm of _01] {Output};

    \draw [->] (_00) edge [bend right]  (_01);
    \draw [->] (_00) --  (_10);
    \draw [->] (_01) edge [bend right]  (_00);
    \draw [->] (_10) edge [loop left] (_10);
     
    
    
    \node[node,circle,minimum width=0mm] (0n) [below=2cm of 10] {$s_0$};
    
        
    \node [above= 20pt of 0n] {Adapter (Controller)};
    
    \node[initial,circle,node,minimum width=0mm] (In) [left=2.5cm of 0n] {$ini$};
    

    

    
    \node[node,circle,minimum width=0mm] (1n) [right=3cm of 0n] {$s_1$};
    


    \draw [->] (In) edge 
            node [above,text width=2cm ]      {$\ltltt|\neg a_1\wedge \neg a_2$}     (0n);    
    
    \draw [->] (0n) edge [bend left] 
            node [above,text width=2cm ] (A)     {$\neg t_1|\neg a_1 \wedge a_2$}     (1n);
    
    \draw [->] (1n) edge [bend left] 
            node [below,text width=2cm ]{$\ltltt|\neg a_1\wedge\neg a_2$} (0n);
            
  %  \draw [->] (0n) edge [bend right] 
  %          node [left,text width=1cm ]      {$t_1 \wedge \neg t_2$}     (2n);
    
        \draw [->] (0n) edge [loop below] 
            node [below,text width=2.5cm ]{$t_1|a_1\wedge \neg a_2$} (0n);
    
    
    \end{tikzpicture}
    \caption{An example of an adpatee and adapter transducers. The adapter respects the output limitations, and the composition of the adaptee with the adaptor satisfies $(\ltlG \ltlF(t_1)\rightarrow \ltlG \ltlF(a_1)) \wedge (\ltlG \ltlF(t_2) \rightarrow \ltlG \ltlF(a_2))$}
    \label{fig:example}
\end{figure}

Thus, in this variant, the $input$ transition is the Adapter, the $Output$ Transition is the Target and the specification is from the Adapter to the Target!
As such, unlike the 1st variant, the synthesized controller is a transducer from the Adapter output to the Target output.
We note that here the controller is already the required Adapter, so no further constructions are required.



% \subsubsection{Illustrative Examples}

% The example we gave above demonstrates how our technique enables us to fit an existing controller to an unmatched hardware. We formalize now two more illustrative examples to demonstrate additional usages of our technique.

% \vspace{3pt}
% \noindent\textbf{Cleaning robots}. In this example, we demonstrate how one can use our technique to fulfill tasks that have not been covered by an execution of an existing controller. We consider a cleaning robot that moves along a corridor-shaped house, from room $1$ to room $n$. The robot follows some plan, and accordingly cleans some of the rooms. Hence, the robot control variables $\{\mathit{in{:}room}_i: 1\leq i\leq n\}$ that model its location, and variables $\{\mathit{in{:}clean}_i: 1\leq i\leq n\}$, each it raises after cleaning the corresponding room. Moreover, it raises a signal $\mathit{done}$ when it finishes fulfilling its plan. Our goal is to synthesize a second cleaning robot that follows the first robot and cleans exactly those rooms that have not been cleaned by the first robot. Hence, the robot we synthesize controls variables $\{\mathit{out{:}room}_i: 1\leq i\leq n\}$ and $\{\mathit{out{:}clean}_i: 1\leq i\leq n\}$, and it is required to fulfill requirements of the form: $\ltlG\ltlF(\mathit{done}) \wedge \ltlG\ltlF(\mathit{in{:}clean}_i)\rightarrow \ltlG\ltlF(\mathit{out{:}clean}_i)$, $\ltlG\ltlF(\mathit{done}) \wedge \ltlG\ltlF(\mathit{!in{:}clean}_i)\rightarrow \ltlG\ltlF(\mathit{!out{:}clean}_i)$.

% \vspace{3pt}
% \noindent\textbf{Railway Signalling.} In this example, we demonstrate how one can use our technique to improve the quality of an existing controller. We consider a junction of $n$ railways, each railway is equipped with a signal that can be turned on (light in green) or off (light in red). Some railways overlap and thus their signals cannot be turned on simultaneously. We consider the next overlapping pattern. Railways 1-4 overlap, likewise 3-6, 5-8, and so on.

% An existing system activates the signals by assigning values to  $\{\mathit{in{:}signal}_i: 1\leq i\leq n\}$. To avoid accidents, it was programmed to be strictly safe; it never raises two signals simultaneously. 

% We are interested in a controller that performs better. The controller should read the valuations that the existing system provides, and correspondingly assign values to  $\{\mathit{out{:}signal}_i: 1\leq i\leq n\}$. We want the new controller to produce safe and \emph{maximal} valuations; $\mathit{out{:}signal}_i$ is turned on iff the signal of every rail that overlaps with the $i$th rail is off.

% Furthermore, we want to maintain liveness properties of the input system: 
% \begin{itemize}
%     \item For every $i=1\dots n$, if  $\mathit{in{:}signal}_i$ is turned on infinitely often, then  $\mathit{out{:}signal}_i$ is turned on infinitely often as well.
    
%     \item For every $i=1\dots n$, if  $\mathit{in{:}signal}_i$ is turned on at least once in every $m$ consecutive steps (where $m$ is a parameter of the specification), then the same holds for $\mathit{out{:}signal}_i$.
% \end{itemize}






\subsection{Separated GR($k$) Games}
\label{Sec:PrblmStmnt}




The core contribution of this work is to define the notion of separation of variables in the context of games and to demonstrate the algorithmic benefits of separation.


We say that a game structure {\em separates variables} if the choices of any one of the players does not restrict the choices of the other. This can be formalized by requiring that each assumption and guarantee is dependent only on the player's variables and not those of the other player. Formally,

%We consider game structures that separate variables. Roughy, a game separate variables if the choices of any of the players cannot restrict the possible choices of the other player. We formalize this requirement by demanding that (1) the initial guarantees are not dependent on the first input, and (2) the safety assumptions and guarantees consider only the corresponding player's former choice. 

\begin{definition}
A game structure  $\mathit{\GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ {\em separates variables} over input variables $\I$ and output variables $\O$ if:
\begin{itemize}
    \item The environment's initial assumption $\theta_\I$ is an assertion over $\I$ only.
    \item The system's initial guarantees $\theta_\O$ is an assertion over $\O$ only.
    \item The environment's safety assumption $\rho_\I$ is an assertion over $\I\cup \I'$ only.
    \item The system's safety guarantee $\rho_\O$ is an assertion over $\O\cup \O'$ only.
\end{itemize} 
\end{definition}

The interpretation of a game structure which separates variables is that the underlying game graph $(V, E)$ is the product of two distinct directed graphs over disjoint sets of variables:  $G_\I$ over the variables $\I\cup\I'$, and $G_\O$ over the variables $\O\cup\O'$. For $\V \in \{\I, \O\}$, the vertices of $G_\V$ correspond to states over $\V$ and there is an edge between states $s$ and $t$ if $(s, t') \models \rho_\V$.

%In $G_\I$, the graph states correspond to states of $\I$, the initial states of the graph are given by $\theta_\I$, and there is a transition between graph states $s$ and $t$ if $(s,t')\models \rho_\I$. $G_\O$ is similarly defined with graph states over $\O$, initial states given by $\theta_\O$, and transitions between $\rho_\O$.

%We focus on the useful GR($k$) wining condition~\cite{?}. While GR($k$) wining conditions are synthesized in exponential time~\cite{} \gatodo{to add a precise expression...}, we shall prove that an efficient synthesis algorithm exists when the formula separate variables.
Similarly, the notion of separation of variables extends to games with GR(k) specifications as follows:
\begin{definition}
\label{def:separatedGRk}
A GR(k) specification $\varphi$ over $\I\cup\O$  separates variables w.r.t. $\I$ and $\O$ if $ \varphi = \bigwedge_{l=1}^k (  
\bigwedge_{i=1}^{n_l} \ltlG\ltlF(\varphi_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG\ltlF(\psi_{l,j})
)$ such that each $\varphi_{l,i}$ is an assertion over $\I$ and each $\psi_{l,j}$ is an assertion over $\O$. 
A GR($k$) game $(\GS,\varphi)$ over input variables $\I$ and output variables  $\O$ separates variables if game structure $\GS$ separates variables and GR($k$) winning condition $\varphi$ separates variables w.r.t. $\I$ and $\O$. 
\end{definition}

We call a GR($k$) game that separates variables a {\em separated GR($k$) game}. 

\gatodo{I suggest to give here few sentences that connect between the var-sep definition, and the problem description in the intro}

\sbtodo{Justify symbolic-state representation of the problem statement}

\sbtodo{Some related work before stating final result}

We remark that a standard technique allows to replace assertions of a GR($k$) winning condition with properties represented by a deterministic B\"uchi automaton (DBA)~\cite{?}. The cost of such a replacement is adding auxiliary variables. Specifically, an $m$-state DBA adds $\log m$ fresh variables.  However, this approach was shown to be both expressive and feasible. As an example, Dwyer et al. identified 55 typical patterns that are common in industrial specifications. 54 out of those 55 patterns are DBA properties, and none adds more than 3 auxiliary variables to the specification. Similarly, the parametric robotic patterns identified by Menghi et al. can be be supported by rather small DBAs. 
\gatodo{: meanwhile, this comment is mentioned here but it should be relocated.}
\dftodo{move this remark to intro or to prelims}


\begin{theorem}\label{thm:main}
[\sbtodo{To rephrase. Clarify technical result}]
Let $(\mathit{\GS},\varphi)$ be a separated GR($k$) game over the input/output variables $\I$ and $\O$. Then, the realizability and synthesis problems for $(\mathit{\GS},\varphi)$ are solved in $O(|\varphi|N)$ symbolic operations, where $N=|2^{\I\cup\O}|$.
\end{theorem}

% The proof of Theorem~\ref{thm:main} is combined of two major step. In the first step, presented in Section~\ref{sec:reduction}, we describe how separated GR($k$) games can be reduced to solving a special type of weak b\"uchi games and how to translate a winning strategy for the later, to a strategy for separated GR($k$). Section~\ref{sec:algorithmsWeakBuchi} is dedicated to show how weak b\"uchi games are solved. 
% Since the natural presentation of the problem is symbolic, we chose to describe a symbolic presentation of a solution for both steps. Note that while some of the symbolic descriptions we next discuss are common, an efficient representation to others are not trivial.

Since the construction of the strategy that proves Theorem~\ref{thm:main} is symbolic and non trivial, we choose to separate the proof into two parts. In the first part, that we discuss in Section~\ref{}, we describe the proof layout. We levarage this in Section~\ref{} to describe the symbolic solution and prove the complexity analysis of our solution.






\begin{comment}
\subsection{Describing the problem as a graph \gatodo{to omit?}}
\label{Sec:graphdescription}

Since our solution involves a graph representation of the problem, we note that we can describe the problem as two graphs $G_\I=(V_\I,E_I),G_\O=(V_\O,E_\O)$ as follows. For $\mathcal X\in\{\I,\O\}$, $V_{\mathcal X} =2^{\mathcal X}$, and $E_\mathcal X=\{(s_0,s_1) : (s_0,s_1)\models \rho_\mathit X\}$.
%The set of vertices of $G_I$ is $2^{\I}$ and an edge $(s,s')$ is in $G_\I$ iff $(s,s')\models \rho_\I$. similarly, the set of vertices of $G_\O$ is $2^{\O}$ and an edge $(t,t')$ is in $G_\O$ iff $(s,s')\models \rho_\O$.
As such, we will be mostly interested in $G=G_\I\times G_\O=(V_\I\times V_\O,E)$ That is, the product graph $G$ of $G_\I$ and $G_\O$, in which $\big((s_0,t_0),(s_1,t_1)\big)\in E$ iff $(s_0,s_1)\in E_\I$ and $(t,t')\in E_\O$.

We rephrase the interaction between the players by seeing $G$ as a game-board. The vertices $V$ are the game states. From a state $(\inp_0,\out_0)$ the players choose together the ensuing state. First, system $A$ chooses $\inp_1\in V_\I$ such that $(\inp_0,\inp_1)\in V_\I$. Then, system $B$ responds by choosing $\out_1\in V_\O$ such that $(\out_0,\out_1)\in V_\I$, and the play traverses to $(\inp_1,\out_1)$.
We further adapt and apply on $G$ the notions of \emph{plays} and \emph{strategies}, given in the preliminaries section. These are defined in a natural manner and we omit the straightforward details.

To avoid possible different terminologies, we remind some fundamental notations.
A \textit{subgraph} $G_0$ of a directed graph $G$ is a graph $(V_0,E_0)$ where $V_0\subseteq V$ and $E_0= E\cap (V_0\times V_0)$. 
\textit{A path} in a graph $G$ is a sequence $(v_0,\cdots v_i)$ s.t. for all $0\leq j<i$ $(v_j,v_{j+1})\in V$. Note that a single vertex is also considered as a path.
A \textit{strongly connected component} (SCC) in a graph $G=(V,E)$, is a maximal subset $V_0\subseteq V$ such that for every vertices $v,v' \in V_0$, there exists a path from $v$ to $v'$ in $G$. Note that the set of all SCCs forms a partition of the graph-vertices.
%A \textit{maximal strongly connected component} is a strongly connected component that is not contained in any other strongly connected component.




%Note that this presentation does not serve as an arena which explicitly implements the symbolic representation of the game between the two players; it merely represents all legal steps the players can choose cooperatively.



%We now define a list $L$ of strongly connected components over $G$.

%Later we will define strongly connected components on $G$, then define the Connected-Partition problem.

%Add a list of Good connected components and bad connected components.

%A play is winning for the system if there a connected component $C$ in the list such that $GF(C)$ is satisfied. Otherwise the play is winning for the environment.

%Definitions needed:
%\begin{enumerate}
%    \item Notations for states and transition relations for $G_{\I}$ and $G_{\O}$
    
%    \item path
%    \item Strongly connected components
%    \item Good SCCs and Bad SCCs
%    \item Play
%    \item Winning plays for system and environment players
%    \item Synthesis problem and realizability problem (if different from what is given in Definition~\ref{Def:Symbolic}). 
%\end{enumerate}

\end{comment}

==> ProofLayoutOld.tex <==

\section{Framework layout}\label{sec:reduction}

In this section we describe and prove our solution for Theorem~\ref{thm:main}. We elaborate on the symbolic construction in Section~\ref{sec:symsol}.
The separated nature of our specification allows for the following observation, upon which our solution approach is founded. Consider an infinite play $\pi$ in $\GS$. Like every infinite path on a finite graph, $\pi$ eventually ends in an SCC $S$. Since the game graph $G$ can be decomposed into an input graph $G_\I$ and an output graph $G_\O$, we have that the projection of $S$ on the inputs is an SCC $S_\I$ in $G_\I$, and the projection of $S$ on the outputs is an SCC $S_\O$ in $G_\O$. The input side of $\pi$ converges to $S_\I$ whereas the output side $\pi$ converges to $S_\O$. 
%\dftodo{perhaps better define projection. I also think we can clean proof of Lemma 5.1 with it}
%\lmttodo{Done, it's defined at the end of the first paragraph of the Preliminaries}
%Since the system can move on $G_I$ regardless of the moves that the environment makes on $G_O$, the system can visit every state of $S_I$ at will, regardless of the actions of the environment.

Now, let $S$ be an SCC with projections  $S_\I$ on $G_\I$ and $S_\O$ on $G_\O$, and let $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
\bigwedge_{i=1}^{n_l} \ltlG \ltlF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG \ltlF(g_{l,j})$.
Then $S$ is called \textit{accepting} if for \textit{every} constraint $\varphi_l$, where $l\in\{1,\dots,k\}$, one of the following hold:
\begin{description}
\item[All guarantees hold in $S$.] For every $j\in\{1,\dots,m_l\}$, there exists $\out\in S_\O$ such that $\out\models g_{l,j}$.

\item[Some assumption cannot hold in $S$.] There exists $j\in\{1,\dots,n_l\}$ such that for all $\inp\in S_\I$, $\inp\not\models a_{l,j}$. 
\end{description}

Then intuitively, if the system has a strategy $f_B$ for which every play converges to an accepting SCC, then the system has a winning strategy for Separated-GR($k$): play $f_B$ until reaching an accepting SCC $S$, then play a strategy $f_\travel$ that travels around $S$ satisfying as many of the $g_{l,j}$ guarantees as possible.
%all the vertices $o$ in $S_O$\gatodo{to touch all the guarantees} to make sure that all the $g_{l,j}$ conditions are satisfied.
If the environment moves the play to a non-accepting SCC, the system can start playing $f_B$ again to reach a different accepting SCC.

A complication arises however when switching between $f_\travel$ and $f_B$, since it is conceivable that while the system is following $f_\travel$, the environment could move to a different SCC that is outside of the winning region of $f_B$.
%performing $f_\travel$ may take the system out of the winning regions of $f_B$.
Thus, it is not clear that we can indeed combine both to make a winning strategy for the system.
To show that we can indeed combine both strategies, we need the following property that we call the \textit{delay property}: if $(\inp_1, \out_1)$ is a state in the winning region of $f_B$, and $(\inp_2, \out_0)$ is a state for which there is a path in $G_\I$ from $\inp_1$ to $\inp_2$ and a path in $G_\O$ from $\out_0$ to $\out_1$, then $(\inp_2, \out_0)$ is also in the winning region of $f_B$. We formally state and prove the delay property in Section~\ref{sec:delay}.

After proving the delay property, it remains to describe how to construct the winning strategy. Since the system can move in $G_\O$ regardless of the moves that the environment makes in $G_\I$, constructing $f_\travel$ can be done by simply finding a path in $S_\O$ that satisfies the maximum number of guarantees.
To synthesize $f_B$, we first define a weak B\"uchi game $B = (\GS, \ltlG \ltlF (\nu_{acc}))$, where $\GS$ is the game structure of the original GR($k$) game and $\nu_{acc}$ is an assertion satisfied exactly by those states that are in an accepting SCC. In Section~\ref{sec:syntstrat} we prove that a winning strategy for $B$ can be used as the strategy $f_B$, and therefore the realizability of Separated-GR($k$) can be reduced to the realizability of weak B\"uchi games. Later, in Section~\ref{sec:algorithmsWeakBuchi}, we explain how the winning strategy can be constructed symbolically.
%While $f_\travel$ can be easily constructed since the system can move on $G_\I$ regardless of the moves that the environment makes on $G_\O$, a weak \Buchi game has to be solved on $G$ in order to synthesize $f_B$.

%The rest of the section goes as follows. In Section~\ref{sec:delay} we formally state and prove the delay property. We then describe and prove the winning strategy for Separated-GR($k$) in Section~\ref{sec:syntstrat}. In Section~\ref{sec:algorithmsWeakBuchi} we explain how to construct a winning strategy symbolically.





% The main part in our solution to Theorem~\ref{thm:main} relies on a reduction to weak B\"uchi games. 
% To ease the exposition we first give an outline of the solution, followed by details.

% \subsubsection{Outline}

% We first consider our input game structure $\GS$ as a weak \Buchi game. For that we consider the SCCs of $\GS$ and mark every SCC $S$ as accepting, if the system can win the GR($k$)-game in the subgame $S$, i.e. if for every component of the GR($k$) formula,
% $\varphi_l=\bigwedge_{i=1}^{n_l} \ltlG \ltlF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG \ltlF(g_{l,j})$, either (1) the environment cannot satisfy one of $\varphi_l$'s  assumptions in the subgame $S$, or (2) the system can satisfy all $\varphi_l$' guarantees in the subgame $S$.
% \dftodo{Better write: Subgame, what is an SCC over GS, better write the conditions}

% Next, we show that realizability for separated GR($k$) games is reduced to realizability of the weak B\"uchi game, described above.
% That means: the system can win w.r.t. the GR($k$) objective iff it can win this special weak \Buchi game. That settles the the \textbf{realizability} part of Theorem~\ref{thm:main}.


% Finally, we show how to use the winning strategy obtained for the weak \Buchi game to obtain a winning strategy for weak separated games. Intuitively we mark the SCCs of $\GS$ as described above, and apply the `weak B\"uchi' strategy until reaching an accepting SCC, $S$. Then, we play another strategy that circles on $S$ to reach all possible outputs in $S$. Then, whenever the environment leads the game out of $S$, we switch back to the weak B\"uchi strategy. We repeat this process until the play eventually stabilizes in an accepting SCC, in which we win w.r.t. the GR($k$) condition. This solves the \textbf{synthesis} problem. 




% \subsection{Constructing weak B\"uchi games} 
% \label{Sec:ConversionSeparatedToWeak}

% We first show how to construct a symbolic weak \Buchi game from a separated GR($k$) game. 

% % Recall from Section~\ref{Sec:Prelims} that a game with game structure $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and a winning condition can be equivalently represented by a game between the system and environment player on  directed graph $ (V,E)$. The states set $V$ is given by states over $\I\cup\O$, and $E$ is the set of all directed edges $(s,t)$ for which $(s,t')\models \rho_\I\wedge\rho_\O$. Recall, we assume that all states of a game structures are deadlock-free\dftodo{Where do we make this assumption and why?}. Thus, there is at least one outgoing edge from every state in directed graph $(V,E)$.
% % Finally, the initial states of the graph are the states  $\theta_\I\wedge\theta_\O$.

% To meet the condition of a weak \Buchi game, we now describe how to separate the SCCs of $(V,E)$ \gatodo{what is $(V,E)$?} to accepting and non accepting SCC. 
% Let $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
% \bigwedge_{i=1}^{n_l} \ltlG \ltlF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG \ltlF(g_{l,j})$.
% Then an SCC $S$ at $(V,E)$ is called \textit{accepting} if for \textit{every} constraint $\varphi_l$, where $l\in\{1,\dots,k\}$, one of the following hold:
% \begin{description}
% \item[All guarantees hold in $S$.] For every $j\in\{1,\dots,m_l\}$, there exists $(\inp,\out)\in S$ such that $\out\models g_{l,j}$.

% \item[Some assumption cannot hold in $S$.] There exists $i\in\{1,\dots,n_l\}$ such that for all $(\inp,\out)\in S$, $\inp\not\models a_{l,i}$. 
% \end{description}


% Intuitively, every winning play for the game structure $\GS$ must converge to an accepting SCC \gatodo{I don't understand this sentence. This is a sufficient and necessary condition to win a play, right? Why "intuitively"?} (every infinite play at every graph based game must eventually converge to a single SCC). To see that the special form of separated specification $\varphi$ that we have requires from a winning strategy that for every constraint $\varphi_l$ either: all guarantees hold; there is an assumption that does not hold
% \dftodo{clean assume/guarantee terminology, clean that paragraph}. We formalize this intuition in Section \ref{sec:syntstrat}. We call the strategy that solves weak \Buchi $f_{B}$.

% It is interesting to observe what action should the system do when reaching an accepting SCC. Intuitively, while in an accepting SCC $S$, making sure that every \textit{system vertex} \dftodo{change terminology} of $S$ is visited infinitely often, should suffice for the system meet the specification conditions and to win \dftodo{better explain?}, \textit{no matter what actions the environment performs}. Indeed note that in our specification, the system can indeed keep visiting any system-vertex regardless of the actions of the environment \dftodo{this is a key observation, say it much before and highlight!}. We call this strategy $f_{travel}$. \gatodo{This is not what we do. For each guarantee $g_{l,i}$ we play a reachability game inside $S$. If S has no $g_{l,i}$-state, the play immediately terminates. B.t.w. this is why we get time complexity $O(|\varphi|N)$: $O(|\varphi|)$ reachability games.}


% A complication rises however when combining both $f_B$ \gatodo{$f_B$ was not defined} and $f_{travel}$ while in $f_B$, performing $f_{travel}$ may take the system out of the winning regions of $f_B$. Thus it is not clear that we can indeed combine both to make winning strategy for the system.
% To overcome that we show the following the following property that we call the \textit{delay property}: if $(x,y)$ is a state in the winning region of $f_B$, and $(a,b)$ is a state for which there is a path in $G_I$ \dftodo{change font} from $x$ to $a$ and a path in $G_O$ from $b$ to $y$, then $(a,b)$ is also in the winning region of $f_B$.

% Note that under this property the system can  "delay" within an SCC and still win the separation game. 

% % since $S$ is defined according to \textit{both} environment and system graphs. Therefore the environment can choose an action that make the play depart from $S$. In this case, the system must find it's way and chase the environment, but how can it do it from every state in $S$ in which it was? 
% % We answer this by showing that the system can delay in an SCC as long as it wants and still win the game. For that we need the delay property, described below \dftodo{I wrote rubbish here. Better clean!! why not just use the reachability? Why the delay at all?}.








% The game proceeds by the environment player assigning values to the input variables $\I$ and the system player assigning values to the output variables $\O$.  
% The game starts at one of the initial states of the graph. 
% In every round of the game, first the  environment chooses an assignment to the $\I$ variables, and then the system will choose an assignment $O$ to the $\O$ variables.
% The combined assignment $I \cup O$ determines the unique state  the game moves to.
% The notions of plays, strategies, winning conditions and so on naturally transfer to the explicit-state representation. 





%For readability, we also consider an explicit representation of the game between the environment and the system. Given a game structure  $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$, we define a graph that serves as a ``game-board" as follows. $G^{\mathit{GS}}=(V^\mathit{GS},E^\mathit{GS})$, where $V^\mathit{GS}=2^{\I\cup\O}$, and $(\inp_0,\out_0)E(\inp_1,\out_1)$ if $\big((\inp_0,\out_0),(\inp_1',\out_1')\big)\models \rho_\I\wedge \rho_\O$.
%At the beginning of a play, the environment chooses $\inp\in 2^\I$, the system then responds with $\out\in 2^\O$, and thus the first state of the play is $(\inp,\out)\in V^{\mathit{GS}}$. Afterwards, the payers repeatedly choose the next state of the play: form state $(\inp_0,\out_0)$ the environment chooses $\inp_1\in 2^\I$ such that $(\inp_0,\out_0,\inp_1')\models \rho^e$, the system replies with $\out_1$ such that $(\inp_0,\out_0,\inp_1',\out_1')\models \rho_\O$, and the play traverses to state $(\inp_1,\out_1)$.  Note that the notions of plays, strategies etc. naturally transfer to the explicit representation. We omit the straightforward adaptation of those notions in the explicit context. 

% A {\em strongly connected component} (SCC) of a directed graph $(V,E)$ is a maximal set of states within which every state is reachable from every other state.  It is well known that SCCs partition the states of a directed graph.

% Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
% Then, these SCCs hold a special property in a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$. Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
% Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all their states are contained in $\F$ or  {\em non-accepting components} mean none of their states is present in $\F$. 
% Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a path is winning for the system if the path ultimately never exist an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every path will ultimately remain inside an accepting component.

%A \textit{subgraph} $G_0$ of a directed graph $G=(V,E)$ is a graph $(V_0,E_0)$ where $V_0\subseteq V$ and $E_0= E\cap (V_0\times V_0)$. 
%\textit{A path} in a graph $G=(V,E)$ is a sequence $(v_0,\cdots v_i)$ such that for all $0\leq j<i$, $(v_j,v_{j+1})\in V$. Note that a single vertex is also considered as a path.
%A \textit{strongly connected component} (SCC) in a graph $G=(V,E)$, is a maximal subset $V_0\subseteq V$ such that for every vertices $v,v' \in V_0$, there exists a path from $v$ to $v'$ in $G$. Note that the set of all SCCs forms a partition of the graph-vertices.
%An SCC, $S$ is a \emph{terminal SCC} if for every $s\in S$ the next holds: if a state $t$ is reachable from $s$, then $t\in S$.

%We exploit the special structure of the weak B\"uchi automaton to solve this game more efficiently than a typical Parity game or B\"uchi game. 

\begin{comment}

Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
Then, these SCCs hold a special property in a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$. Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all their states are contained in $\F$ or  {\em non-accepting components} mean none of their states is present in $\F$. 
Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a path is winning for the system if the path ultimately never exist an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every path will ultimately remain inside an accepting component.

% \subsection{Explicit State Representation}
% \label{sec:explicitweakbuchi}


Weak B\"uchi games have previously been studied when the states of the game are represented explicitly. Under this state representation, weak B\"uchi games can be solved in linear-time to the size of the explicit graph underlying the game~\cite{krish'spaper}. This section reviews that algorithm. 
\end{comment}


% \subsection{Name Name Name}

% We can now state the main theorem of the section that essentially describes the reduction statement. \dftodo{change my writing, this is awful}

% \begin{theorem}\label{thm:reduction}
% .....
% \end{theorem}



% In this section we prove Theorem \ref{thm:reduction}. This proof also yields an algorithm for computing a winning strategy for separated $GR(k)$ games from a 
% winning strategy on weak \Buchi games. 

\subsection{The Delay Property}\label{sec:delay}

The delay property can be used to show that combining the weak \Buchi game strategy $f_B$ and the SCC travel strategy $f_\travel$ maintains the system in the winning region. 
The Delay Property Theorem essentially says that while in an SCC $S$ contained in the winning region, if the environment moves unilaterally to a different SCC in $G_\I$, the new SCC will still be in the winning region for the system.
%that is a winning region\gatodo{contained in a winning region? from which we can win?}, the system can remain in an $S$ or the environment can leave an $S$, and the system still stays in the winning zone.\gatodo{Not sure this is clear}
It is important to note that this property does not hold for every weak \Buchi game, only for those in which the game structure separates variables as in Definition~\ref{def:separates-variables}.
%We remark that this property is unique to the game we are dealing with. It does not hold for every  weak \Buchi game.

We start with the following lemma that states that the system can still win with a single step delay.


\begin{lemma}\label{lem:1delay}
Consider a weak B\"uchi game $B$ that separates variables.
%constructed in Section~\ref{sec:accepting-SCCs}. \gatodo{High chances the reviewers will comment on this forward ref. Especially as it is an appx. If it is needed for the flow, why it is in appx? \\ Consider instead to define in the prev. overview the weak Buchi game with target $GF(acc)$ where $acc$ is a set of states (not a BDD!). i.e. to write instead "consider the weak Buchi game $(\G,\ltlG \ltlF (\mathit{acc}))$..."}
Let $\inp_0,\inp_1\in 2^\I$ such that  $(\inp_0,\inp'_1)\models \rho_\I$, and assume that the system can win from $(\inp_0,\out_0)$. Then the system can also win from $(\inp_1,\out_0)$.
\end{lemma}

\begin{proof}
Let $f$ be a winning strategy for the system from $(\inp_0,\out_0)$. 
We construct a winning strategy $f_d$ from $(\inp_1,\out_0)$. Intuitively, $f_d$ acts from state $(\inp_1, \out_0)$ as if it were following $f$ from state $(\inp_0, \out_0)$, with a delay of a single step: the input in the current step is used to choose the output in the next step.
%it ignores the final input, and shifts the sequence of outputs one step backwards \dftodo{clarify}.
%Since a strategy is deterministic, to simplify notation we denote a strategy $f((\inp_1,\out_0),\dots,(\inp_m,\out_{m-1}))$ as $f(\inp_1,\dots,\inp_m)$.\gatodo{I suggest not to do that. If we gave some notation, use it as is} 



% Recall that the strategy $f^s$ is played as follows. In a state $(i,j)$ the environment makes an action $i'$, and the strategy makes an action $o'$ for which $o'=f^s((i_0,O_0),\cdots (i,o))$ is a result of applying the strategy on previous states so far. Thus the next state reached is $(i',o')$ \dftodo{clarify, but remove or move to prelims}.

We use $f$ to define $f_d$ inductively over play prefixes of length $m\geq 1$, by setting $f_d((\inp_1, \out_0), \ldots, (\inp_m, \out_{m-1}), \inp_{m+1}) = f((\inp_0, \out_0), \ldots, (\inp_{m-1}, \out_{m-1}), \inp_m)$.
%$f_d(\inp_1,\dots,\inp_{m+1})=f(\inp_0,\dots,\inp_m)$. 
Note that $f_d$ is well defined since the game separate variables: from state $(\inp, \out)$, the outputs that can be chosen for the successor state depend only on $\out$, and not on $\inp$.
%for all $\inp,\hat{\inp}\in\I$, $\out \in \O$, the actions that the system can do from state $(i,o)$ and from state  $(\hat{i},o)$ are the same \dftodo{clarify}.
Note that by this definition, for every play $(\inp_1,\out_0),(\inp_2,\out_1),\dots, (\inp_{m+1},\out_m),\dots$ consistent with $f_d$, there is a play $(\inp_0,\out_0),(\inp_1,\out_1),\dots, (\inp_m,\out_m),\dots$ consistent with $f$.

Even if $f$ is memory-less, note that $f_d$ is not. We remark that \textbf{we define $f_d$ only for proving the lemma, and it is not part of our solution.} We shall provide a memory-less winning weak B\"uchi strategy later. 

Next, we show that $f_d$ is winning if $f$ is winning.
Take a play $(\inp_1,\out_0),(\inp_2,\out_1),\dots$, consistent with $f_d$. By the construction, $(\inp_0,\out_0),(\inp_1,\out_1),\dots$ is consistent with $f$. Since this is a play on a weak \Buchi game, after some point it must remain in a single SCC $S$, say from state $(\inp_j,\out_j)$. Since $f$ is a winning strategy the SCC $S$ must be accepting. %and thus stabilizes in an accepting SCC $S$, say from state $(\inp_j,\out_j)$.
Then $\out_j,\out_{j+1},\dots$ is an infinite path in the SCC $S|_\O$, and $\inp_j,\inp_{j+1},\dots$ is an infinite path in the SCC $S|_\I$. %Specifically, it means that $\inp_{j+1}$ is a path in $S\uparrow\I$. 
Consequently, $(\inp_1,\out_0),(\inp_2,\out_1),\dots $ converges to an SCC $\hat{S}$ in which $\hat{S}|_\I = S|_\I$ and $\hat{S}|_\O = S|_\O$. Since the conditions for an SCC $D$ to be accepting depend only on the relation between $D|_\I$ and $D|_\O$, we have that $\hat{S}$ is accepting since $S$ is accepting as well.\qed




% Define a \textit{standard SCC} as an SCC that is result of a product of input-SCC and output-SCC (in our setting, an SCC can have a singleton in the input or output, thus it is not always like this.\dftodo{Is this so? anyhow clean and move definition to prelims}).

% Now, assume that $f^s$ is winning, and let $((\inp_1,\out_0),(\inp_2,\out_1),\cdots (\inp_{m+1},\out_m),\cdots)$ be a play in $f^s_d$. Then there is \dftodo{There is a glitch here, check old proof (commented out after this one) and fix accordingly}
% $((\inp_0,\out_0),(\inp_1,\out_1),\cdots (\inp_m,\out_m),\cdots)$ is a play in $f^s$ that ends in an accepting SCC $S$ since $f^s$ is winning. Specifically there is an input SCC $S_\I$ and output SCC $S_\O$ such that $S=S_\I\times S_\O$ and such that $(\inp_0, \inp_1, \inp_2,\cdots)$ ends up in $S_I$, and $(\out_0, \out_1,\out_2,\cdots)$ ends in $S_\O$.\gatodo{is it that clear?} Therefore $(\inp_1, \inp_2,\cdots)$ also ends up in $S_\I$, and as a result, the play $((\inp_1,\out_0),(\inp_2,\out_1),\cdots (\inp_{m+1},\out_m),\cdots)$ also ends up in the winning SCC $S$ as required.




% Now, we claim that $S_d$ is an accepting SCC. To prove this claim, take a component $\varphi_l  =
% \bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$.  
% First, assume that for every guarantee $GF(g_{l,j})$, $S$ includes a state $s$ such that $s\models g_{l,j}$.  Hence, there exists a path in $S$ from $(\inp_i,\out_i)$ to a state $(\inp,\out)$ such that $\out\models g_{l_j}$. Use Observation~\ref{obs:shift} to conclude that the same holds for $S_d$: there exists a path in $S_d$ from $(\inp_{i+1},\out_i)$ to a state $(\widehat\inp,\out)$, and $\out\models g_{l,j}$. 

% Second, assume that for some assumption $a_{l,j}$, $S$ does not include a state $s\models a_{l,j}$. Assume, towards a contradiction, that there exists $s_d=(\inp^d,\out^d)\in S_d$ such that $\out_d \models a_{l,j}$. Hence, there exists a path in $S_d$ from $(\inp_{i+1},\out_i)$ to $(\inp^d,\out^d)$. Use Observation~\ref{obs:shift} to conclude that $S$ includes an $a_{l,j}$-state as well, in contradiction to the assumption.
% Consequently, $S_d$ is an accepting SCC and thus $f^s_d$ wins w.r.t. the B\"uchi objective, as required.\gatodo{to read again...}\qed


\end{proof}








% \begin{theorem}\label{thm:delay}[The Delay Property Theorem]
% Consider the weak B\"uchi game constructed in Section~\ref{sec:accepting-SCCs}. Let $\inp_0,\dots,\inp_n\in (2^\I)^+$ be a sequence such that for all $i\in\{0,\dots,n\}$, $(\inp_i,\inp_{i+1})\models \rho_\I$. Moreover, let $\out_{-m},\dots,\out_0\in (2^\O)^+$ be a sequence such that for all $i\in\{-m,\dots,-1\}$, $(\out_i,\out_{i+1})\models \rho_\O$.
% If the system can win from $(\inp_0,\out_0)$, then it can also win from $(\inp_n,\out_{-m})$.
% \end{theorem}


We can now prove the delay property, following by straightforward induction from Lemma~\ref{lem:1delay}.


\begin{theorem}[Delay Property Theorem]\label{thm:delay}
Consider a weak B\"uchi game $B$ that separates variables.
%constructed in Section~\ref{sec:accepting-SCCs}.
Let $\inp_0,\dots,\inp_n\in (2^\I)^+$ be a path in $G_\I$, and for $m\geq 0$, let $\out_{-m},\dots,\out_0\in (2^\O)^+$ be a path in $G_\O$. Assume that the system can win from $(\inp_0,\out_0)$. Then the system can also win from $(\inp_n,\out_{-m})$.
\end{theorem}

\begin{proof}
From $(\inp_n,\out_{-m})$, the system can simply ignore the inputs and follow the path in $G_\O$ to $\out_0$. Let $(\inp_{n+m}, \out_0)$ be the state at that point in the play. Note that there is a path between $\inp_n$ and $\inp_{n+m}$, and therefore there is a path between $\inp_0$ and $\inp_{n+m}$. If the system can win from $(\inp_0, \out_0)$ then by induction on Lemma~\ref{lem:1delay} it can win from $(\inp, \out_0)$ for all $\inp$ such that there is a path in between $\inp_0$ and $\inp$. Therefore, the system can win from $(\inp_{n+m}, \out_0)$, and by consequence from $(\inp_n,\out_{-m})$.
% \dftodo{write better, perhaps clarify}
% To show that the system can win from $(\inp_n,\out_{-m})$ for every $m\geq 0$, it is sufficient to show that the system can win from $(\inp_0,\out_{-1})$. The system applies the following strategy: first, for any legal input $\inp$ the system responds with $\out_0$. Then, by the previous lemma, the system has a winning strategy from $(\inp,\out_0)$. \dftodo{Do we need to elaborate? Perhaps write it a bit more precise.} \qed
\end{proof}

A corollary of Theorem~\ref{thm:delay} is the following statement about the structure of the winning region of a weak \Buchi game that separates variables.

\begin{corollary}\label{cor:delay}
The winning region of a weak \Buchi game $B$ that separates variables is a union of SCCs.
\end{corollary}

\begin{proof}
Let $(\inp,\out)$ be a state in the winning region of $B$, let $(\hat\inp,\hat\out)$ be a state in the same SCC $S$ of $(\inp,\out)$, and let $S|_\I$ and $S|_\O$ be the projections of $S$ on $G_\I$ and $G_\O$, respectively.
Then there is a path $\inp_0,\ldots, \inp_n$ for some $n\geq 0$ in $S|_\I$ such that $\inp_0=\inp$ and $\hat\inp=\inp_n$. Similarly, there is a path $\out_{-m},\ldots, \out_0$ for some $m\geq 0$ in $S|_\O$ such that $\hat\out_0=\out$ and $\hat\out=\out_{-m}$. Then by the delay property of Theorem~\ref{thm:delay}, the vertex $(\hat\inp,\hat\out)=(\inp_n,\out_{-m})$ is also in the winning region of $B$. \qed
\end{proof}








\subsection{Synthesizing a Winning Strategy}\label{sec:syntstrat}

We now present a solution outline to the realizability and synthesis problem for separated GR($k$) games. We analyze construction time in the symbolic construction that follows in Section~\ref{sec:algorithmsWeakBuchi}.

Given a separated GR($k$) game $(\GS, \varphi)$, we first find all accepting SCCs, and denote their union by $V_{acc}$. Let $\nu_{acc}$ be the assertion that accepts exactly those states in $V_{acc}$. Next, we construct the following:
\begin{description}
\item[$f_B$:] A memory-less strategy that wins the weak \Buchi game  $(\GS,\ltlG \ltlF(\nu_{acc}))$. An explicit algorithm that solves weak \Buchi games is described in~\cite{Chatterjee08}, and is given in Appendix~\ref{}\gatodo{we don't give it, right?}. In section~\ref{sec:algorithmsWeakBuchi} we describe in detail a symbolic algorithm.
Note that $f_B$ is \textit{not} the strategy constructed in the delay-property lemma.\gatodo{redundant, I think. We say that it is memory-less and we added a comment in the proof. }

\item[$f_\travel$:] A strategy for the system that, when played inside of an SCC $S_\O$ in $G_\O$, (a) always remains inside $S_\O$, and (b) for every guarantee $g_{l,j}$ in $\varphi$, visits a state that satisfies $g_{l,j}$ infinitely often as long as such a state exists in $S_\O$. Note that such a strategy always exists and can entirely ignore the inputs. 
%A memory-less strategy for the system that reaches every state in a given SCC infinitely often. \dftodo{perhaps be more precise} \gatodo{I wonder how to construct such a strategy, symbolically, in $O(N)$ steps.}
\item [$f$:] A strategy that combines $f_B$ and $f_\travel$ as follows: given a state $s$ and an input $i$, if $s$ is in an accepting SCC, apply $f_\travel$; else apply $f_B$.

% That is, $f^s_\mathit{travel}$ satisfies the next property. Let $S$ be an SCC, and consider the subgame induced by $S$. Then, for every $(\inp,\out)\in S$, when the system applies $f^s_\mathit{travel}$, the play will traverse infinitely often states of the form $(\widehat{\inp},\out)$. 
\end{description}


Overall, the strategy depicted in Algorithm~\ref{algo:winning-strategy} is constructed  in $O(|\varphi|N)$ symbolic operations.\dftodo{expand more} \lmttodo{Should this be here instead of in the next section?}


%   \begin{algorithm}[t!]
%   	\caption{A winning strategy (Input: Separated Game}
%   	\label{algo:winning-strategy}
%   	\begin{algorithmic}[1]
		
% 		\Statex{\begin{center}
%   				/*\quad\quad  From state $s$ and input $\inp$ \quad\quad*/
%  		\end{center}}
	
%   	    \State construct $\beta_\mathit{SCC}$ \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
	
%   	    \State $\gamma = \exists\O'(\beta)$ 
	    
%   		\State if $\beta_\mathit{acc}(s)$ and $\gamma(s,\inp')$ \Return $f^s_\mathit{travel}(s,\inp)$
		
%   		\State \Return $f^s_\mathit{wb}(s,\inp)$
%   	\end{algorithmic}
  	
  	
%   	\begin{algorithmic}[1]
		
% 		\Statex{\begin{center}
%   				/*\quad\quad  Implementation of $f_{\mathit{travel}}(s,i)$ \quad\quad*/
%  		\end{center}}
% 	\setcounter{ALG@line}{-1}
	
% 	\State \textbf{initialization}: $\mathit{mem}\leftarrow 0$
%   	    \For{$i=0$ to $m-1$}
	    
% 	    \State $\mathit{target}=\mathit{mem}+i \mod m$
	    
%   	    \State $\out= f_{r(\mathit{target})}(s,i)$
%   	    \State if $\out\neq \bot$ \Return $\out$ 
%   		\EndFor
% 		\State \Return $\out$ such that $\beta_{\mathit{SCC}}(s,\inp',\out')$

%   	\end{algorithmic}
  	
  	
  	
  	
%   \end{algorithm}



\begin{lemma}\label{lem:win}\gatodo{1. We cannot give this lemma her since we haven't defined precisely the strategies it is about. 2. We need (somewhere) to prove the correctness of the $f$. Then, lemma 2 follows almost immediately- no need in the proof we give here.}
If a winning strategy $f_B$ exists for the weak \Buchi game $B = (\GS,\ltlG \ltlF(\nu_{acc}))$, then $f$ is a winning strategy for the separated GR($k$) game $A = (\GS, \varphi)$.
\end{lemma}

\begin{proof}
Since $B$ has a winning strategy, then for every initial input $\inp_0 \models \theta_\I$ there is an initial output $\out_0 \models \theta_\O$ such that $(i_0,o_0)$ is in the winning region of $B$.
We will show that playing $f$ always keeps the play in the winning region of $B$, and therefore the play eventually converges to an accepting SCC $S$. Once this happens, following $f_\travel$ guarantees that $\varphi$ is satisfied.\dftodo{put in a separate lemma}

We know that as long as the play is in the winning region of $B$, following $f_B$ will keep it inside the winning region. Therefore, when we switch from $f_B$ to $f_\travel$ we must be inside the winning region and, by definition of $f$, in an accepting SCC $S$. By Corollary~\ref{cor:delay}, as long as we remain inside $S$, which is guaranteed by $f_\travel$, the play will remain in the winning region. Therefore, the only way that the play can leave the winning region is if, while the system is following $f_\travel$, the environment chooses an input that takes the play to a different, non-winning SCC. We now prove that this cannot happen.

Assume that from state $(\inp_0, \out_0)$ in the accepting SCC $S$, the system chooses output $\out_{-m}$ according to $f_\travel$ and the environment chooses input $\inp_n$ such that $(\inp_n, \out_{-m})$ is in a different SCC. Note that $(\inp_0, \out_0)$ is in the winning region, there is a path from $\inp_0$ to $\inp_n$ and there is a path from $\out_{-m}$ to $\out_0$ (since by construction $f_\travel$ remains in the same SCC in $G_\O$). Therefore, by Theorem~\ref{thm:delay} $(\inp_n, \out_{-m})$ is in the winning region as well. 
\qed
\end{proof}

% \begin{proof}
% Since $B$ has a winning strategy, then for every initial input $\inp_0 \models \theta_\I$ there is an initial output $\out_0 \models \theta_\O$ such that $(i_0,o_0)$ is in the winning region of $B$.
% We will show that playing $f$ always keeps the play in the winning region of $B$. Therefore, the play eventually converges to an accepting SCC $S$, and by following $f_\travel$ the GR($k$) winning condition is satisfied.\dftodo{put in a separate lemma}

% To see that, we use the delay property corollary (about the winning region). Therefore as long $f^s_{wb}$ is switched to $f^s_{\mathit{travel}}$ and $f^s_{\mathit{travel}}$ is being played, the system remains in the winning region.

% Now assume that the strategy switched to $f^s_{wb}$ from $f^s_{\mathit{travel}}$. Then we have a state $s$ in an accepting $SCC$, i.e. in the winning region of $f^s_{wb}$,\gatodo{I have no idea what is a winning region of a strategy. Perhaps you mean that $f^s_{wb}$ wins from $s$?} and we need to see that $f^s_{wb}(s,i)$ is in the winning region of $f^s_{wb}$ as well \dftodo{why isn't it obvious???}. For that we use the delay property lemma \dftodo{I don't think we need to use it again} to show that we are still in the winning region \dftodo{clean!!!}.

% For the other side, note that if $(i_0,o_0)$ is not in the winning region of $f^s_{wb}$, then an accepting SCC cannot be reached by the system. Thus, every SCC that is reached does not meet the GR($k$) conditions. 

% \qed
% \end{proof}

Lemma~\ref{lem:win} shows that we can use weak \Buchi games to synthesize a winning strategy for separated GR($k$) games, allowing us to prove the following theorem.

\begin{theorem}\label{thm:realiizability}\gatodo{we can't give it here}
Realizability for separated GR($k$) games can be reduced to realizability of weak \Buchi games.
\end{theorem}

\begin{proof}
Given a separated GR($k$) game, if the corresponding weak \Buchi game is realizable the winning strategy $f_B$ can be used to compute $f$. If it is not realizable, then the environment can force every play to converge to a non-accepting SCC. Since the GR($k$) winning condition cannot be satisfied from a non-accepting SCC, the separated GR($k$) game is also not realizable.
% Given separated GR($k$) games $G$, construct the weak \Buchi game $G'$ by constructing the $\nu_{acc}$..
% Then check realizability for $G'$. By Lemma~\ref{lem:win}, we have that $G$ is realizable if and only if the initial state $(i_0,o_0)$ is in the winning region of a strategy for $G'$, i.e. iff $G'$ is realizable. \qed
\end{proof}


In Section~\ref{sec:algorithmsWeakBuchi} we show in detail how to do\gatodo{to do?} symbolic synthesis for weak \Buchi games.

%  \subsection{Synthesizing a Winning Strategy}\label{sec:syntstrat}

%  We are ready to present a solution to the realizability and synthesis problem. We construct two strategies, each is constructed by $O(N)$ symbolic operations:
%  \begin{description}
%  \item[$f^s_{wb}$.] A memory-less strategy that wins the weak-B\"uchi game  $((\I,\O,\theta_\I,\theta_\O,\rho_{\I},\rho_{\O}),GF(\beta_{\mathit{acc}}))$.

%  \item[$f^s_{\mathit{travel}}$.] a memory-less strategy for the system to reach all possible inputs in a given SCC. That is, $f^s_\mathit{travel}$ satisfies the next property. Let $S$ be an SCC, and consider the subgame induced by $S$. Then, for every $(\inp,\out)\in S$, when the system applies $f^s_\mathit{travel}$, the play will traverse infinitely often states of the form $(\widehat{\inp},\out)$. \gatodo{I wonder how to construct such a strategy, symbolically, in $O(N)$ steps.}
%  \end{description}

%  Let $W$ be a winning region of $f^s_{wb}$. In Algorithm~\ref{algo:winning-strategy}, we present a strategy that wins for the system from $W$.




%  \begin{algorithm}[t]
%  	\caption{A winning strategy}
%  	\label{algo:winning-strategy}
%  	\begin{algorithmic}[1]
		
%  		\Statex{\begin{center}
%  				/*\quad\quad  From state $s$ and input $\inp$ \quad\quad*/
% 		\end{center}}
	
%  	    \State construct $\beta_\mathit{SCC}$ \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
	
%  	    \State $\gamma = \exists\O'(\beta)$ 
	    
%  		\State if $\beta_\mathit{acc}(s)$ and $\gamma(s,\inp')$ \Return $f^s_\mathit{travel}(s,\inp)$
		
%  		\State \Return $f^s_\mathit{wb}(s,\inp)$
%  	\end{algorithmic}
%  \end{algorithm}

%  We can now prove Theorem~\ref{thm:win}.
%  \begin{proof}
%  We show that $W$ is the system's winning region, and further that Algorithm~\ref{algo:winning-strategy} correctly constructs a strategy that wins from $W$.

%  First, we prove that Algorithm~\ref{} construct a strategy that wins from $W$. ...

% \end{proof}


==> StrategyConstruction_gal.tex <==
\section{Strategy Construction (Gal's suggestion)}
\label{sec:algorithmsWeakBuchi}


In this section we describe how to implement the framework of Section~\ref{sec:delay} to solve realizability and synthesis for separated GR($k$) games. We start by describing a construction of a strategy $f_B$ that wins weak \Buchi games. Then we explain how to construct an overall strategy. Since our construction is BDD-based, we refer the reader to Appendix~\ref{} for the fine technical details.


% Following our central result of  reduction of separated GR($k$) games to weak B\"uchi games presented in Section~\ref{sec:reduction}, this section presents a complete algorithm to solve separated GR($k$) games. By now, we know that the algorithm involves two steps: First, to obtain a weak B\"uchi game from the input separated GR($k$) by identifying  the SCCs. Second, to solve the resulting weak B\"uchi game. Since the input separated GR($k$) game is represented symbolically, the central requirement of our algorithm is to solve the above two steps symbolically. 
% To this end, this section begins with an algorithm for separated GR($k$) games when they are  represented in an explicit-state representation in Section~\ref{sec:explicitweakbuchi}. 
% %To this end, we begin with this sections begins by reviewing a linear-time algorithm to solve weak B\"uchi games when represented with explicit states in Section~\ref{sec:explicitweakbuchi}. 
% Later, Section~\ref{sec:symbolicweakbuchi} will adapt the explicit-state algorithm to the desired symbolic state representation. 



\subsection{Constructing weak \Buchi game symbolic strategy}
\label{sec:accepting-SCCs}

We now describe a symbolic algorithm for weak \Buchi game synthesis. We remark that \textbf{our algorithm fits every weak \Buchi game; we do not assume that the underlying game structure separates variables}.
 First, we explain the algorithm in guidelines, and later provide a symbolic construction (Algorithm~\ref{}). In Appendix~\ref{}, we provide a correctness proof and further constructions of BDDs that our algorithm employs.



\paragraph{High-level algorithm description.} 
We are given a weak B\"uchi game $(\GS,\ltlG\ltlF( \mathit{acc}))$.
%with game graph $(V,E)$ and winning condition $\ltlG\ltlF\varphi$. %in explicit state representation.
%As described earlier, the accepting and non-accepting SCCs can be identified in $O(|V| + |E|)$.\gatodo{redundant. We don't want to identify them in the graph}
Let $(\Statess_0, \dots \Statess_m)$ be a topoloigical sort of the SCCs in the game graph of $\GS$. %partitioning the directed graph $(V,E)$. W.l.o.g.\gatodo{no need in wlog since we describe, not construct},  let $\Statess_1>\Statess_2>\dots >\Statess_m$ with respect to the partial order $>$ induced by the topological sorting of the SCCs.  
The algorithm works in backward induction.
In the \textbf{base case}, we take all  {\em terminal partitions} $S_j,\dots,\Statess_m$. That is, each SCC $S_i$ such that no other SCC is reachable from $S_i$. 
In this case, plays beginning in $\Statess_i$  will never leave it and be of infinite length. Thus, if a terminal $\Statess_i$ is an accepting component, every state of $S_i$ is a winning state for the system, while if $\Statess_i$ is a non-accepting component, every state of $S_i$ is a winning state for the environment.

For the \textbf{induction step}, let $\vec{S}=(S_{i+1},\dots,S_m)$, and
suppose that the set $\bigcup \vec{S}$ has been classified into winning states  for the system $W_{i+1}^s$, and winning states for the environment $W_{i+1}^e$. 
 Let $\vec{S_0}=(\Statess_j,\Statess_{j+1}, \ldots, \Statess_{i})$ be the SCCs from which all edges leaving the SCC lead to an SCC in $\vec{S}$. Let $A$ be the union of all accepting SCCs in $\vec{S_0}$, and let $N$ be the union of all non-accepting SCCs in $\vec{S_0}$. Now, if $s\in N$, the system can win from $s$ iff it can force $\ltlF(W_{i+1}^s)$ from $s$. Analogously, the system can win from $s\in A$ iff it can force  $\ltlG(A\cup W_{i+1}^s)$. Hence, by solving these reachability and safety games, we can update $W_{i+1}^s$ and $W_{i+1}^e$ into $W_{j}^s$ and $W_j^s$ that partition $\bigcup(S_j,\dots,S_m)$ into winning states for the system and winning states for the environment.
 
 
\begin{algorithm}[t!]
	\caption{Weak-B\"uchi winning strategy construction}
	\label{algo:sym-weak-buchi}
	\begin{algorithmic}[1]
	    
	    \Statex \textbf{input:} A weak B\"uchi game $((\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O),GF\mathit{(acc)})$ 
	    
	    %\State construct $\beta_\mathit{SCC},\beta_\mathit{ter}$
	    
	    \State $\beta = \beta_\mathit{ter}$\label{line:terminal}
	    
	    \State $W=\beta\wedge \mathit{acc}$\label{line:winning-variable}
	    
	    \State $\sigma = W\wedge (\rho_\I\rightarrow \rho_\O)$\label{line:winning-terminal-states}
    
        \While{$\beta \neq 2^{\I\cup\O}$}\label{line:while-loop}
        
        \State $\gamma =\mathit{pre}(\beta)$\label{line:pre}
        
        \State $(W_1,f^s_1)=\mathit{reach}(\gamma,W)$\label{line:reach}
        
        \State $(W_2,f^s_2)=\mathit{safe}(\gamma,W\vee (  (\gamma\setminus \beta)\wedge \mathit{acc}))$\label{line:safe}
        
        \State $f^s = f^s \vee 
        ( (W_1\setminus W) \wedge f^s_1) \vee 
        ( (W_2\setminus (W\vee W_1)) \wedge f^s_2)$\label{line:extend-strategy}
        
        \State $W=W\vee W_1 \vee W_2$\label{line:extend-region}
        
        \State $\beta= \gamma$
        
        \EndWhile\label{line:end-while}
		
		\State\Return $(W,f^s)$
	\end{algorithmic}
\end{algorithm}
 
\paragraph{Weak B\"uchi algorithm.} Algorithm~\ref{} is  a linear time realizability and synthesis algorithm for weak B\"uchi games. The algorithm gets as an input a B\"uchi game $(\GS,\ltlG \ltlF (\mathit{acc}))$, and computes the system's winning region $W$ and a memory-less strategy $f$ in a form of a BDD. That is, $f$ is a BDD $f(\I,\O,\I',\O')$ such that $f(s,i)=o$ if $(s,i,o)\models f$. The algorithm assumes intactness of the input, i.e. that the B\"uchi game is indeed weak.


The algorithm employs several BDDs, all constructed in linear time.
\begin{itemize}
    \item $\beta_{\mathit{ter}}$. a BDD for all terminal SCCs.
    \item If $\beta$ characterizes a set $\mathcal S_0$ of ``closed-downwards" SCCs (i.e. a suffix of some topological sort) $pre(\beta)$ identifies all SCCs  from which only SCCs in $\beta$ are reachable. Computed in time $O(|pre(\beta)\setminus \beta|)$.
    
    \item $\mathit{reach}(\gamma,\beta)$. Synthesizes a reachability strategy in the subgame $\gamma$ with target $\beta$.
    
        \item $\mathit{reach}(\gamma,\beta)$. Synthesizes a safety strategy in the subgame $\gamma$ with target $\beta$.
\end{itemize}

We prove in Appendix~\ref{} the correctness of the algorithm and thus establish the next result.

\begin{theorem}\label{thm:weakbuchi}
Realizability and Synthesis for weak \Buchi games can be done in $O(N)$ symbolic steps.
\end{theorem}


\subsection{Symbolically solving Separated-GR($k$) games}\label{sec:symsol}


  \begin{algorithm}[t!]
  	\caption{A winning strategy}
  	\label{algo:winning-strategy}
  	\begin{algorithmic}[1]
		
		\setcounter{ALG@line}{-1}
		
		\State \textbf{initialization:} construct $\beta_\mathit{SCC}$, $\gamma{=}\exists\O'(\beta)$  \quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
		\Statex
		\Statex{\begin{center}
  				/*\quad\quad  From state $s$ and input $\inp$ \quad\quad*/
 		\end{center}}
	
  	    %\State construct $\beta_\mathit{SCC}$ \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
	
  	    %\State $\gamma = \exists\O'(\beta)$ 
	    
  		\State if $\beta_\mathit{acc}(s)$ and $\gamma(s,\inp')$ \Return $f_\travel(s,\inp)$
		
  		\State \Return $f_B(s,\inp)$
  	\end{algorithmic}
  	
  	
  	\begin{algorithmic}[1]
		
		\Statex{\begin{center}
  				/*\quad\quad  Implementation of $f_\travel(s,i)$ \quad\quad*/
 		\end{center}}
	\setcounter{ALG@line}{-1}
	
	\State \textbf{initialization}: $\mathit{mem}\leftarrow 0$
  	    \For{$i=0$ to $m-1$}
	    
	    \State $\mathit{target}=\mathit{mem}+i \mod m$
	    
  	    \State $\out= f_{r(\mathit{target})}(s,i)$
  	    \State if $\out\neq \bot$ \Return $\out$ 
  		\EndFor
		\State \Return $\out$ such that $\beta_{\mathit{SCC}}(s,\inp',\out')$

  	\end{algorithmic}
  	
  	
  	
  	
  \end{algorithm}

Having a symbolic strategy for weak \Buchi, we can finally show how to solve realizability and synthesis for Separated-GR($k$) games. 
Algorithm~\ref{} merely follows the outline we gave in Section~\ref{}. 

The algorithm constcuts a BDD $\beta_{\mathit{scc}}(\I,\O,\I',\O')$ such that $(s,t)\models \beta_{\mathit{scc}}$ iff $s$ and $t$ belong to the same SCC. It further implements the strategy $f_\travel$ discussed in Section~\ref{sec:reduction} as follows. We arbitrarily order all guarantees that appear in our GR($k$) formula: ${\gar}_0,\dots,{\gar}_{m-1}$. For each guarantee $\gar_j$, we take a reachability strategy $f_{r(j)}$ that never leaves the SCC it is applied from. If  $s\in S$, an SCC that includes no $\gar_j$-state, then $f_{r(j)}$ returns a distinguished value $\bot$. We equip $f_\travel$ with a memory variable $\mathit{mem}\in\{0,\dots,m-1\}$. $f_\travel(s,i)$ is computed as follows: for $\mathit{mem},\mathit{mem}+1,\dots$ we find the first $t=\mathit{mem}+j\mod m$ such that the SCC of $s$ includes a $\gar_j$ state, and   activates $f_{r(t)}$ to reach such state (loop in line 1). If no guarantees can be satisfied in $S$, we just return an arbitrary output to stay in $S$ (line 6). The reachability strategies and  $\beta{\mathit{scc}}$ are constructed in time $O(N)$. Hence, as we show in Appendix~\ref{}, Algorithm~\ref{} constructs a winning strategy in time $O(|\varphi|N)$, which implies Theorem~\ref{thm:main}. In addition, we see that a state $s$ wins for the system iff it wins w.r.t. to the B\"uchi objective we defined, and thus the next follows.

\begin{theorem}\label{thm:realiizability}
Realizability for separated GR($k$) games can be reduced to realizability of weak \Buchi games and thus is solved in time $O(N)$.
\end{theorem}









==> StrategyConstruction_old.tex <==
\section{Strategy construction-old}
\label{sec:algorithmsWeakBuchi}


% In this section we describe how to implement the framework of Section~\ref{sec:delay} to solve realizability and synthesis for separated GR($k$) games. We describe our symbolic construction, followed by a complexity analysis.
% Following our framework, we start by describing a symbolic construction of a strategy $f^{sym}_B$ that wins weak \Buchi games. Then we explain how to construct an overall strategy. Since our construction is BDD-based, we refer the reader to the appendix\gatodo{to Appendix~\ref{}. We will have 1 or 2 appxs? } for the fine technical details.


% % Following our central result of  reduction of separated GR($k$) games to weak B\"uchi games presented in Section~\ref{sec:reduction}, this section presents a complete algorithm to solve separated GR($k$) games. By now, we know that the algorithm involves two steps: First, to obtain a weak B\"uchi game from the input separated GR($k$) by identifying  the SCCs. Second, to solve the resulting weak B\"uchi game. Since the input separated GR($k$) game is represented symbolically, the central requirement of our algorithm is to solve the above two steps symbolically. 
% % To this end, this section begins with an algorithm for separated GR($k$) games when they are  represented in an explicit-state representation in Section~\ref{sec:explicitweakbuchi}. 
% % %To this end, we begin with this sections begins by reviewing a linear-time algorithm to solve weak B\"uchi games when represented with explicit states in Section~\ref{sec:explicitweakbuchi}. 
% % Later, Section~\ref{sec:symbolicweakbuchi} will adapt the explicit-state algorithm to the desired symbolic state representation. 



% \subsection{Constructing weak \Buchi game symbolic strategy}
% \label{sec:accepting-SCCs}
% \gatodo{time complexity is $O()$ and not $\O()$. $\O$ is something else in the paper...}
% We now describe a symbolic algorithm for weak \Buchi game synthesis. We note that this algorithm fits every weak \Buchi game, and not only those that are resulted from our specifications.\gatodo{To be more explicit: we do not assume var-separation}
%  We build on top of an existing explicit linear-time algorithm for weak B\"uchi games~\cite{Chatterjee08} that runs in $O(|V|+|E|)$ time, where $(V,E)$ is the underlying game graph. We explain the algorithm briefly, with a detailed description appearing in the appendix.\gatodo{which appx?}\gatodo{1. I (briefly) looked at~\cite{Chatterjee08}. Although you can possibly link between computations of our algo and~\cite{Chatterjee08}, I am not sure it is "on top". We deal with a topological sort and~\cite{Chatterjee08} with attractors to 'colors'.  Maybe we just mention that linear-time algo can be derived form the litruture and take full ownership on the algo we give?\\
% 2. I suggest to omit the V+E analysis. 
% we are not interested in time complexity of the algo variant on the graph representation}


% \paragraph{High-level algorithm description.} \dftodo{think of writing it symbolically}
% We are given a weak B\"uchi game with game graph $(V,E)$ and winning condition $\ltlG\ltlF\varphi$. %in explicit state representation.
% As described earlier, the accepting and non-accepting SCCs can be identified in $O(|V| + |E|)$.\gatodo{redundant. We don't want to identify them in the graph}
% Let $\Statess_0, \dots \Statess_m$ be the SCCs partitioning the directed graph $(V,E)$. W.l.o.g.\gatodo{no need in wlog since we describe, not construct},  let $\Statess_1>\Statess_2>\dots >\Statess_m$ with respect to the partial order $>$ induced by the topological sorting of the SCCs.  The algorithm works in backward induction.
% In the \textit{base case}, we take all  {\em terminal partitions} $S_j,\dots,\Statess_m$. That is, each SCC $S_i$ such that no other SCC is reachable from $S_i$. 
% In this case, plays beginning in any state of $\Statess_i$ in the list  will never leave it and be of infinite length. Thus, if a terminal $\Statess_i$ is an accepting component, every state of $S_i$ is a winning state for the system, while if $\Statess_i$ is a non-accepting component, every state of $S_i$ is a winning state for the environment.\gatodo{maybe recall here that there are no deadlocks? Otherwise $S_m$ can be a deadlock... }

% For the induction step, suppose that $\vec{S} =\{\Statess_{i+1}, \ldots, \Statess_m\}$ have been classified as winning for the system or the environment,\gatodo{the description is incorrect. It is possible that some states in an SCC S are winning, an some are not} and partition $\vec{S}$ into a set of accepting SCCs $\vec{S}_{\mathit{acc}}$ and non accepting SCCs $\vec{S}_{\mathit{rej}}$. Let $\vec{S'}=\{\Statess_j,\Statess_{j+1}, \ldots, \Statess_{i}\}$ be the SCCs from which all edges leaving the SCC lead to an SCC in $\vec{S}$, and take $S_i\in \vec{S}'$.
% %Then, note that a state in $\Statess_i$ is winning for the system if and only if it can either force plays to stay inside $\Statess_i$, or force the play to reach the $\vec{S}_{acc}$, a safety game on with winning condition $\vec{S}_{acc}$ with a  reachability game  with winning condition $\vec{S}_{rej}$ can determine the accepting SCCs from $\vec{S'}$. \lmttodo{This paragraph is confusing, there seems to be something missing.}
% If $S_i$ is a non accepting SCC, the system can win from $s\in S_i$ iff it can force reaching $S\vec{S_{\mathit{acc}}}$ from $s$. Otherwise, if $S_i$ is an accepting SCC, the system can win from $s\in S_i$ iff it can win w.r.t. the safety winning condition  $\ltl G (S_i\cup \vec{S_{\mathit{acc}}})$. 
% \dftodo{I cut the complexity analysis to appendix. I think we should adjust that once we have it clean.}


% \ganote{up here}
In this section we describe how to implement the framework of Section~\ref{sec:delay} to solve realizability and synthesis for separated GR($k$) games. We start by describing a construction of a strategy $f_B$ that wins weak \Buchi games. Then we explain how to construct an overall strategy. Since our construction is BDD-based, we refer the reader to Appendix~\ref{} for the fine technical details.


% Following our central result of  reduction of separated GR($k$) games to weak B\"uchi games presented in Section~\ref{sec:reduction}, this section presents a complete algorithm to solve separated GR($k$) games. By now, we know that the algorithm involves two steps: First, to obtain a weak B\"uchi game from the input separated GR($k$) by identifying  the SCCs. Second, to solve the resulting weak B\"uchi game. Since the input separated GR($k$) game is represented symbolically, the central requirement of our algorithm is to solve the above two steps symbolically. 
% To this end, this section begins with an algorithm for separated GR($k$) games when they are  represented in an explicit-state representation in Section~\ref{sec:explicitweakbuchi}. 
% %To this end, we begin with this sections begins by reviewing a linear-time algorithm to solve weak B\"uchi games when represented with explicit states in Section~\ref{sec:explicitweakbuchi}. 
% Later, Section~\ref{sec:symbolicweakbuchi} will adapt the explicit-state algorithm to the desired symbolic state representation. 



\subsection{Constructing weak \Buchi game symbolic strategy}
\label{sec:accepting-SCCs}

We now describe a symbolic algorithm for weak \Buchi game synthesis. We remark that \textbf{our algorithm fits every weak \Buchi game; we do not assume that the underlying game structure separates variables}.
 First, we explain the algorithm in guidelines, and later provide a symbolic construction (Algorithm~\ref{}). In Appendix~\ref{}, we provide a correctness proof and further constructions of BDDs that our algorithm employs.



\paragraph{High-level algorithm description.} 
We are given a weak B\"uchi game $(\GS,\ltlG\ltlF( \mathit{acc}))$.
%with game graph $(V,E)$ and winning condition $\ltlG\ltlF\varphi$. %in explicit state representation.
%As described earlier, the accepting and non-accepting SCCs can be identified in $O(|V| + |E|)$.\gatodo{redundant. We don't want to identify them in the graph}
Let $(\Statess_0, \dots \Statess_m)$ be a topoloigical sort of the SCCs in the game graph of $\GS$. %partitioning the directed graph $(V,E)$. W.l.o.g.\gatodo{no need in wlog since we describe, not construct},  let $\Statess_1>\Statess_2>\dots >\Statess_m$ with respect to the partial order $>$ induced by the topological sorting of the SCCs.  
The algorithm works in backward induction.
In the \textbf{base case}, we take all  {\em terminal partitions} $S_j,\dots,\Statess_m$. That is, each SCC $S_i$ such that no other SCC is reachable from $S_i$. 
In this case, plays beginning in $\Statess_i$  will never leave it and be of infinite length. Thus, if a terminal $\Statess_i$ is an accepting component, every state of $S_i$ is a winning state for the system, while if $\Statess_i$ is a non-accepting component, every state of $S_i$ is a winning state for the environment.

For the \textbf{induction step}, let $\vec{S}=(S_{i+1},\dots,S_m)$, and
suppose that the set $\bigcup \vec{S}$ has been classified into winning states  for the system $W_{i+1}^s$, and winning states for the environment $W_{i+1}^e$. 
 Let $\vec{S_0}=(\Statess_j,\Statess_{j+1}, \ldots, \Statess_{i})$ be the SCCs from which all edges leaving the SCC lead to an SCC in $\vec{S}$. Let $A$ be the union of all accepting SCCs in $\vec{S_0}$, and let $N$ be the union of all non-accepting SCCs in $\vec{S_0}$. Now, if $s\in N$, the system can win from $s$ iff it can force $\ltlF(W_{i+1}^s)$ from $s$. Analogously, the system can win from $s\in A$ iff it can force  $\ltlG(A\cup W_{i+1}^s)$. Hence, by solving these reachability and safety games, we can update $W_{i+1}^s$ and $W_{i+1}^e$ into $W_{j}^s$ and $W_j^s$ that partition $\bigcup(S_j,\dots,S_m)$ into winning states for the system and winning states for the environment.
 
\subsubsection{ Weak \Buchi algorithm construction}


We are given a weak \Buchi game $((\I, \O, \theta_\I, \theta_\O, \rho_\I, \rho_\O), \ltlG \ltlF \varphi)$ with BDDs representing $\theta_\I$, $\theta_\O$, $\rho_\I$, $\rho_\O$ and $\varphi$.
The goal is to compute a BDD for the winning region of the weak B\"uchi game and then to determine whether the initial states of the game intersect with the winning region. The construction of the winning region follows a fixed-point computation that adapts the inductive algorithm presented in  Section~\ref{sec:explicitweakbuchi}: in the basis of the fixed point computation, the winning region is the set of accepting and terminal SCCs; in the inductive step, the winning region includes winning states by examining SCCs that are higher in the topological ordering on SCCs.
%There are several challenges in executing the fixed-point algorithm outlined here. 
In what follows we describe a sequence of BDDs that we construct towards constructing the overall BDD.
We use the notation $\X$\gatodo{not a big issue at all, but maybe $\V$ is more standard?} to denote an ordered set of variables over $\I\cup\O$. 



% We begin with introducing necessary notation.
% Let $B(\V)$ be a BDD defined over the ordered set of variables $\V = \{v_1, \ldots, v_n\}$. Let $W = \{w_1, \ldots, w_n\}$ be a new, ordered set of variables of the same cardinality. We use $B(W)$ to denote the BDD in which every variable $v_i$ is replaced with the corresponding variable $w_i$. We can extend this to a BDD $B(\V_1, \ldots, \V_m)$ over multiple sets $ \V_1, \ldots \V_m$ of variables in the natural way. 
% Given an ordered set of variables $\V = \{v_1, \ldots, v_n\}$, we use $\V'$ to denote the ordered set of new variables $\V' = \{v'_1, \ldots, v'_n\}$.


\paragraph{BDD for SCCs.} We want to construct a predicate which indicates when two states in a game structure are present in the same SCC. Let predicate $\Reach(s,t')$ hold if there is a path from state $s$ over $\I\cup\O$ to state $t$ over $\I\cup\O$ in the game structure $\GS$.
Similarly, a predicate $\Reachinverse(s,t')$ holds if and only if  $\Reach(t,s')$ holds.
BDDs for   $\Reach$  and $\Reachinverse$  can be computed in $\O(N)$ symbolic operations, see appendix for details.
Then, a BDD for an SCC is constructed in  $\O(N)$ symbolic operations as $\SCC(\X,\X') := \Reach(\X,\X') \wedge \Reachinverse(\X,\X')$. \lmttodo{Need to decide whether to use $\Reach(s,t')$ or $\Reach(\X,\X')$. }






\paragraph{BDD for Terminal SCC.}
The induction basis for the construction of a winning region requires us to know what the terminal SCCs are. Let predicate $\terminal (s)$ hold if state $s$ over $\I\cup\O$ is present in a terminal SCC. Then
$\terminal(\X) := \forall \X': \Reach(\X,\X')\rightarrow \SCC(\X,\X')$.
Therefore, given BDDs for $\mathsf{Reach}$ and $\mathsf{SCC}$, the construction of $\mathsf{Terminal}$ requires $\O(1)$ symbolic operations. 

% \paragraph{BDD to obtain SCCs higher in the topological ordering.}   
% The induction step in the construction of the winning region requires us to know how to compute the {\em predecessor} SCCs w.r.t. to the topological ordering on the SCC.


% Let $C$ be a set of SCCs over the game structure. For a state $s$ over $\I\cup\O$, let $s\models C$ be the shorthand for ``there exists an SCC $S\in C$ such that $s\models S $".
% A set of SCCs $C$ is said to be {\em closed downwards} if for every state $s \models C$, for every state $t$ that is reachable from $s$, $t\models C$. If $C$ is closed downwards, then its predecessor, denoted $\mathit{pre}(C)\supseteq C$,  is  a set of SCCs  such that if $S$ is an SCC in $\mathit{pre}(C)$, states $s\models S$ and there exists a path from $s$ to  state $t$, then either $t\models S$ or $t\models C$. Note that $\mathit{pre}(C)$ is also closed downwards.
% Observe that predicate $\terminal$ denotes a downward closed set of SCCs. 

% Let predicate $\C$ over $\X$ denote a downward closed set of SCCs. Then, from the definition, we see that its predecessor $\pre(\C)$ can be obtained as follows:
% \[
% \pre(\C) := \forall \X': \Reach(\X,\X') \rightarrow (\SCC(\X,\X') \vee \C(X'))
% \]

% Then, a BDD for the predecessor of a $\pre(\C)$ is computed in $\O(1)$ symbolic operations, given a BDD for $\Reach$, $\SCC$, and the downward closed set $\C$.

\paragraph{Computing the Winning Region.}

We can finally describe the fixed-point computation to construct a BDD for the winning region in  a weak \Buchi game. 
Let $\Reachability(A,B)(\X)$\gatodo{I suggest to change the notation so it would be clear that A and B are parameters and X are vars. e.g. $\mathit{A-Reachabilty_B(X)}$ } denote a BDD, generated by solving a reachability game, that takes as input a set of source states $A$ and target states $B$, and outputs those states in $A$ from which the system can guarantee to move into $B$.
Same. let $\Safety(A,B)(\X)$ denote a BDD, generated by solving a safety game, that takes as input a set of source states $A$ and target states $B$, and outputs those states in $A$ from which the system can guarantee that all plays remain inside the set $B$.
Details can be found in ~\cite[Chapter~20]{2001automata}.\gatodo{Wrong chapter...}


Then, let  $\winning(s)$ denote that state $s$ over $\I\cup\O$ is in the winning region. Then, $\winning$ is the fixed point of $\winningAux$ which is defined below, where the construction essentially follows the explicit algorithm:
\begin{description}
    \item{\textbf{Base Case.}} $\winningAux^0(\X) := \terminal(\X) \wedge \varphi(X)$ and
    $\C^0(\X) := \terminal(\X)$
    
    \item {\textbf{Inductive Step.}} Define:
    
    $$\C^{i+1}(\X) :=  \forall \X': \Reach(\X,\X') \rightarrow (\SCC(\X,\X') \vee \C(X'))$$
    
    \begin{align*}
    \winningAux^{i+1}(\X) & :=        \winningAux^i(\X) \\
    & \vee \Reachability(\C^{i+1}(\X), \winningAux^i(\X)) \\
    &  \vee  
    \Safety(\C^{i+1}(\X), \winningAux^i(\X)\\
    &\vee (\C^{i+1}(\X)\wedge \neg \C^{i}(\X)\wedge\varphi(\X)))
    \end{align*}
  
\end{description}


To explain the construction of $\winning$, note that a state in $\C^{i+1}(\X)$ is winning in one of these cases:
(i) Every state in $\winningAux^i(\X)$ is also winning.  
(ii) The system can force to move into the region $\winningAux^i(\X)$. This set of states can be obtained from $\Reachability(\C^{i+1}(\X), \winningAux^i(\X))$. 
(iii) %state in   $\C^{i+1}(\X)$ is winning if
the system can force all plays in  $\C^{i+1}(\X)$ to remain in states in $A(\X) = \C^{i+1}(\X)\setminus\C^i(\X)$ that accept $\varphi$ or satisfy $\winningAux^i(\X)$. This set of states can be obtained from $\Safety(\C^{i+1}(\X), \winningAux^i(\X) \vee (\C^{i+1}(\X)\wedge \neg \C^{i}(\X)\wedge\varphi(\X)))$. 
    

Finally, we prove the following theorem.

\begin{theorem}\label{thm:weakbuchi}
Realizability and Synthesis for weak \Buchi games can be done in $O(N)$ symbolic steps.
\end{theorem}

\paragraph{Proof Outline.}
The proposed construction symbolically implements the inductive procedure of the explicit algorithm. Hence, it correctly identifies the system's winning region. 
It remains to show that the algorithm performs $O(N)$ symbolic operations. First, of all, the constructions of $\SCC$ and $\terminal$ take $\O(N)$ symbolic operations collectively. It suffices to show that in the $i$-th induction step, solving the reachability and safety games  performs  $O(|\pre(\C^{i+1})\setminus\C^i|)$ operations. This can be proven by a careful analysis of the operations and the sizes of resulting BDDs using standard results on safety and reachability games. Details have been deferred to the Appendix\gatodo{this high-level description explains realizability check, but I think it fails to explain the strategy construction}.\qed 


\subsection{Symbolically solving Separated-GR($k$) games}\label{sec:symsol}

Having a symbolic strategy for weak \Buchi, we can finally show how to symbolically solve realizability and synthesis for Separated-GR($k$) games. followed by a time complexity analysis.
Our construction mainly follows our framework. Our current solution for $f_t$ is a strategy with memory $|\varphi|$ as we define below in details.

\paragraph{Defining accepting states}

We are given a Separated-GR($k$) game structure $\GS = (\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and an assertion $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j}))$. We first need to represent $\GS$ and $\varphi$ as BDDs.\gatodo{??}, These symbolic representations are standard in common in the literature e.g. \cite{} \dftodo{complete}. Next, we describe the set of accepting states symbolically. That is, we provide a linear-time construction of a BDD that recognizes all accepting states.


% This section presents an algorithm to solve separated GR($k$) games when represented symbolically as in Definition~\ref{def:separatedGRk}. From Theorem~\ref{}, we know it trivially reduces to a weak B\"uchi game. The task, therefore, is to present an algorithm for weak B\"uchi games when presented symbolically. More specifically, we design a BDD based algorithm to solve a weak B\"uchi game $(\GS,\ltlG\ltlF \varphi)$ where the assertions in the game structure $\GS = (\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and the assertion $\varphi$ are given in the form of a BDDs.



We first define every state in an accepting SCC as an \textit{accepting state}. We next turn to show that all accepting states can be identified efficiently. \dftodo{move lemma to 6.2}

\begin{lemma}
A BDD $\beta_\mathit{acc}$ over $\I,\O$ such that $\beta_\mathit{acc}(\inp,\out)$ if $(\inp,\out)$ is accepting, can be constructed in $O(|\varphi|+N)$ symbolic operations.
\end{lemma}
\begin{proof}
Consider the BDD $\beta_\mathit{SCC}$ \dftodo{see that $B_{SCC}$ is defined oenly later, fix that} \lmttodo{Should this be $\SCC(X, X')$? Unify notation.}, constructed in $O(N)$ operations (see Lemma~\ref{lem:beta_SCC}). Take a component $\varphi_l= 
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$. First, we identify all states such that their SCC includes a $g_{j,l}$-state. For $j\in\{1,\dots,m_l\}$, let $\beta_{g_{l,j}}$ be a BDD over $\I,\O,\I',\O'$ such that $\beta_{g_{l,j}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $\out_1\models g_{l,j}$. Hence, the BDD $\gamma_{l,j}$ over $\I,\O$, defined by $\exists \I',\O'(\beta_\mathit{SCC} \wedge \beta_{g_{l,j}})$, accepts a state $(\inp,\out)$ if its SCC includes a state $s\models g_{l,j}$.

Now, we focus on the assumptions. Similarly to the former case, for $i\in\{1,\dots,n_i\}$, let $\beta_{a_{l,j}}$ be a BDD over $\I,\O,\I',\O'$ such that $\beta_{a_{l,j}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $\inp_1\models a_{l,i}$. Hence, the BDD $\alpha_{l,i}$ over $\I,\O$, defined by $\forall \I',\O'(\beta_\mathit{SCC}\rightarrow \neg\beta_{a_{l,i}})$,
accepts a state $(\inp,\out)$ if its SCC does not includes a state $s$ such that $s\models a_{l,j}$.

Therefore, the BDD $\beta_\mathit{acc}$ is constructed by $\bigwedge_{l=1}^k(  (\bigwedge_{j=1}^{m_l}\gamma_{l,j}) \vee (\bigvee_{i=1}^{n_l} \alpha_{l,i}))$ \lmttodo{Should this be $\neg \alpha_{l,i}$?}. The construction is performed by $O(|\varphi|+N)$ operations. \qed
\end{proof}


\paragraph{Constructing $f_{B}$.}

Next, we use Theorem~\ref{} to construct a symbolic strategy as a BDD for our weak \Buchi game.

\paragraph{Constructing $f_{\travel}$.}


  For the presentation of $f_{\travel}$ we arbitrarily order all guarantees that appear in our GR($k$) formula: ${\gar}_0,\dots,{\gar}_{m-1}$. For each guarantee $\gar_j$, we take a reachability strategy $f_{r(j)}$ that never leaves the SCC it is applied from. For the sake of presentation, we assume that if  $s\in S$, an SCC that includes no $\gar_j$-state, then $f_{r(j)}$ returns a distinguished value $\bot$. We equip $f_\travel$ with a memory variable $\mathit{mem}\in\{0,\dots,m-1\}$. $f_\travel(s,i)$ is computed as follows: for $\mathit{mem},\mathit{mem}+1,\dots$ we find the first $\mathit{mem}+j$ such that the SCC of $s$ includes a $\gar_j$ state, and   activates $f_{r(\mathit{mem}+j)}$ to reach such state (loop in line 1). If no guarantees can be satisfied in $S$, we just return an arbitrary output to stay in $S$ (line 6). We remark that we chose a loop-based algorithmic presentation for readability purposes. However, $f_\travel$ can be implemented by BDD operations (without the distinguished value $\bot$) with memory of size $m$. The construction of $f_\travel$ requires $O(|\varphi|N)$ symbolic BDD-operations as we need to construct $m$ reachability strategies (clearly, $m\leq |\varphi|$). 


\paragraph{Combining the strategies}

Finally, we invoke the framework and interleave the strategies. The following algorithm \label{algo:winning-strategy} describes our flow. Correctness follows from the framework correctness.

%Overall, the strategy depicted in Algorithm~\ref{algo:winning-strategy} is constructed  in $O(|\varphi|N)$ symbolic operations.\dftodo{expand more}


  \begin{algorithm}[t!]
  	\caption{A winning strategy}
  	\label{algo:winning-strategy}
  	\begin{algorithmic}[1]
		
		\setcounter{ALG@line}{-1}
		
		\State \textbf{initialization:} construct $\beta_\mathit{SCC}$, $\gamma{=}\exists\O'(\beta)$  \quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
		\Statex
		\Statex{\begin{center}
  				/*\quad\quad  From state $s$ and input $\inp$ \quad\quad*/
 		\end{center}}
	
  	    %\State construct $\beta_\mathit{SCC}$ \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
	
  	    %\State $\gamma = \exists\O'(\beta)$ 
	    
  		\State if $\beta_\mathit{acc}(s)$ and $\gamma(s,\inp')$ \Return $f_\travel(s,\inp)$
		
  		\State \Return $f_B(s,\inp)$
  	\end{algorithmic}
  	
  	
  	\begin{algorithmic}[1]
		
		\Statex{\begin{center}
  				/*\quad\quad  Implementation of $f_\travel(s,i)$ \quad\quad*/
 		\end{center}}
	\setcounter{ALG@line}{-1}
	
	\State \textbf{initialization}: $\mathit{mem}\leftarrow 0$
  	    \For{$i=0$ to $m-1$}
	    
	    \State $\mathit{target}=\mathit{mem}+i \mod m$
	    
  	    \State $\out= f_{r(\mathit{target})}(s,i)$
  	    \State if $\out\neq \bot$ \Return $\out$ 
  		\EndFor
		\State \Return $\out$ such that $\beta_{\mathit{SCC}}(s,\inp',\out')$

  	\end{algorithmic}
  	
  	
  	
  	
  \end{algorithm}


==> StrategySolution.tex <==
\section{Synthesis for Separated-GR($k$)}\label{sec:solution}


The problem of synthesizing a controller in our formulation, is therefore reduced to the problem of realizability and synthesis of separated games.\gatodo{isn't it the same problem? I don't understand... } Thus our main result of this paper is as follows.

\begin{theorem}\label{thm:main}
Let $(\mathit{\GS},\varphi)$ be a separated GR($k$) game over the input/output variables $\I$ and $\O$. Then, the realizability and synthesis problems for $(\mathit{\GS},\varphi)$ are solved in $O(|\varphi|N)$ symbolic operations, where $N=|2^{\I\cup\O}|$.\gatodo{realizability in $O(N)$}
\end{theorem}

% In Sections~\ref{} we prove Theorem~\ref{thm:main} that resulted in an algorithm to  synthesize a strategy \dftodo{say better}. Since the construction is symbolic and non trivial, we choose to separate the proof into two parts. In the first part, that we discuss in Section~\ref{}, we describe the proof layout. We leverage this in Section~\ref{} to describe the symbolic solution and prove the complexity analysis of our solution.

 \gatodo{I actually liked better the separation between the problem and solution}

\subsection{Solution layout}\label{sec:reduction}

In this section we describe and prove our solution for Theorem~\ref{thm:main}. We elaborate on the symbolic construction in Section~\ref{sec:symsol}.
The separated nature of our specification allows for the following observation, upon which our solution approach is founded. Consider an infinite play $\pi$ in $\GS$. Like every infinite path on a finite graph, $\pi$ eventually ends in an SCC $S$. Since the game graph $G$ can be decomposed into an input graph $G_\I$ and an output graph $G_\O$, we have that the projection of $S$ on the inputs is an SCC $S_\I$ in $G_\I$, and the projection of $S$ on the outputs is an SCC $S_\O$ in $G_\O$. The input side of $\pi$ converges to $S_\I$ whereas the output side $\pi$ converges to $S_\O$. 
%\dftodo{perhaps better define projection. I also think we can clean proof of Lemma 5.1 with it}
%\lmttodo{Done, it's defined at the end of the first paragraph of the Preliminaries}
%Since the system can move on $G_I$ regardless of the moves that the environment makes on $G_O$, the system can visit every state of $S_I$ at will, regardless of the actions of the environment.

Now, let $S$ be an SCC with projections  $S_\I$ on $G_\I$ and $S_\O$ on $G_\O$, and let $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
\bigwedge_{i=1}^{n_l} \ltlG \ltlF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG \ltlF(g_{l,j})$.
Then $S$ is called \textit{accepting} if for \textit{every} constraint $\varphi_l$, where $l\in\{1,\dots,k\}$, one of the following hold:
\begin{description}
\item[All guarantees hold in $S$.] For every $j\in\{1,\dots,m_l\}$, there exists $\out\in S_\O$ such that $\out\models g_{l,j}$.

\item[Some assumption cannot hold in $S$.] There exists $j\in\{1,\dots,n_l\}$ such that for all $\inp\in S_\I$, $\inp\not\models a_{l,j}$. 
\end{description}

Then intuitively, if the system has a strategy $f_B$ for which every play converges to an accepting SCC, then the system has a winning strategy for Separated-GR($k$): play $f_B$ until reaching an accepting SCC $S$, then play a strategy $f_\travel$ that travels around $S$ satisfying as many of the $g_{l,j}$ guarantees as possible.
%all the vertices $o$ in $S_O$\gatodo{to touch all the guarantees} to make sure that all the $g_{l,j}$ conditions are satisfied.
If the environment moves the play to a non-accepting SCC, the system can start playing $f_B$ again to reach a different accepting SCC.

A complication arises however when switching between $f_\travel$ and $f_B$, since it is conceivable that while the system is following $f_\travel$, the environment could move to a different SCC that is outside of the winning region of $f_B$.
%performing $f_\travel$ may take the system out of the winning regions of $f_B$.
Thus, it is not clear that we can indeed combine both to make a winning strategy for the system.
To show that we can indeed combine both strategies, we need the following property that we call the \textit{delay property}: if $(\inp_1, \out_1)$ is a state in the winning region of $f_B$, and $(\inp_2, \out_0)$ is a state for which there is a path in $G_\I$ from $\inp_1$ to $\inp_2$ and a path in $G_\O$ from $\out_0$ to $\out_1$, then $(\inp_2, \out_0)$ is also in the winning region of $f_B$. We formally state and prove the delay property in Section~\ref{sec:delay}.

After proving the delay property, it remains to describe how to construct the winning strategy. Since the system can move in $G_\O$ regardless of the moves that the environment makes in $G_\I$, constructing $f_\travel$ can be done by simply finding a path in $S_\O$ that satisfies the maximum number of guarantees.
To synthesize $f_B$, we first define a weak B\"uchi game $B = (\GS, \ltlG \ltlF (\nu_{acc}))$, where $\GS$ is the game structure of the original GR($k$) game and $\nu_{acc}$ is an assertion satisfied exactly by those states that are in an accepting SCC. In Section~\ref{sec:syntstrat} we prove that a winning strategy for $B$ can be used as the strategy $f_B$, and therefore the realizability of Separated-GR($k$) can be reduced to the realizability of weak B\"uchi games. Later, in Section~\ref{sec:algorithmsWeakBuchi}, we explain how the winning strategy can be constructed symbolically.

\dftodo{merge these two}
We now present a solution outline to the realizability and synthesis problem for separated GR($k$) games. We analyze construction time in the symbolic construction that follows in Section~\ref{sec:algorithmsWeakBuchi}.

Given a separated GR($k$) game $(\GS, \varphi)$, we first find all accepting SCCs, and denote their union by $V_{acc}$. Let $\nu_{acc}$ be the assertion that accepts exactly those states in $V_{acc}$. Next, we construct the following:
\begin{description}
\item[$f_B$:] A memory-less strategy that wins the weak \Buchi game  $(\GS,\ltlG \ltlF(\nu_{acc}))$. An explicit algorithm that solves weak \Buchi games is described in~\cite{Chatterjee08}, and is given in Appendix~\ref{}\gatodo{we don't give it, right?}. In section~\ref{sec:algorithmsWeakBuchi} we describe in detail a symbolic algorithm.
Note that $f_B$ is \textit{not} the strategy constructed in the delay-property lemma.\gatodo{redundant, I think. We say that it is memory-less and we added a comment in the proof. }

\item[$f_\travel$:] A strategy for the system that, when played inside of an SCC $S_\O$ in $G_\O$, (a) always remains inside $S_\O$, and (b) for every guarantee $g_{l,j}$ in $\varphi$, visits a state that satisfies $g_{l,j}$ infinitely often as long as such a state exists in $S_\O$. Note that such a strategy always exists and can entirely ignore the inputs. 
%A memory-less strategy for the system that reaches every state in a given SCC infinitely often. \dftodo{perhaps be more precise} \gatodo{I wonder how to construct such a strategy, symbolically, in $O(N)$ steps.}
\item [$f$:] A strategy that combines $f_B$ and $f_\travel$ as follows: given a state $s$ and an input $i$, if $s$ is in an accepting SCC, apply $f_\travel$; else apply $f_B$.


%While $f_\travel$ can be easily constructed since the system can move on $G_\I$ regardless of the moves that the environment makes on $G_\O$, a weak \Buchi game has to be solved on $G$ in order to synthesize $f_B$.

%The rest of the section goes as follows. In Section~\ref{sec:delay} we formally state and prove the delay property. We then describe and prove the winning strategy for Separated-GR($k$) in Section~\ref{sec:syntstrat}. In Section~\ref{sec:algorithmsWeakBuchi} we explain how to construct a winning strategy symbolically.





% The main part in our solution to Theorem~\ref{thm:main} relies on a reduction to weak B\"uchi games. 
% To ease the exposition we first give an outline of the solution, followed by details.

% \subsubsection{Outline}

% We first consider our input game structure $\GS$ as a weak \Buchi game. For that we consider the SCCs of $\GS$ and mark every SCC $S$ as accepting, if the system can win the GR($k$)-game in the subgame $S$, i.e. if for every component of the GR($k$) formula,
% $\varphi_l=\bigwedge_{i=1}^{n_l} \ltlG \ltlF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG \ltlF(g_{l,j})$, either (1) the environment cannot satisfy one of $\varphi_l$'s  assumptions in the subgame $S$, or (2) the system can satisfy all $\varphi_l$' guarantees in the subgame $S$.
% \dftodo{Better write: Subgame, what is an SCC over GS, better write the conditions}

% Next, we show that realizability for separated GR($k$) games is reduced to realizability of the weak B\"uchi game, described above.
% That means: the system can win w.r.t. the GR($k$) objective iff it can win this special weak \Buchi game. That settles the the \textbf{realizability} part of Theorem~\ref{thm:main}.


% Finally, we show how to use the winning strategy obtained for the weak \Buchi game to obtain a winning strategy for weak separated games. Intuitively we mark the SCCs of $\GS$ as described above, and apply the `weak B\"uchi' strategy until reaching an accepting SCC, $S$. Then, we play another strategy that circles on $S$ to reach all possible outputs in $S$. Then, whenever the environment leads the game out of $S$, we switch back to the weak B\"uchi strategy. We repeat this process until the play eventually stabilizes in an accepting SCC, in which we win w.r.t. the GR($k$) condition. This solves the \textbf{synthesis} problem. 




% \subsection{Constructing weak B\"uchi games} 
% \label{Sec:ConversionSeparatedToWeak}

% We first show how to construct a symbolic weak \Buchi game from a separated GR($k$) game. 

% % Recall from Section~\ref{Sec:Prelims} that a game with game structure $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and a winning condition can be equivalently represented by a game between the system and environment player on  directed graph $ (V,E)$. The states set $V$ is given by states over $\I\cup\O$, and $E$ is the set of all directed edges $(s,t)$ for which $(s,t')\models \rho_\I\wedge\rho_\O$. Recall, we assume that all states of a game structures are deadlock-free\dftodo{Where do we make this assumption and why?}. Thus, there is at least one outgoing edge from every state in directed graph $(V,E)$.
% % Finally, the initial states of the graph are the states  $\theta_\I\wedge\theta_\O$.

% To meet the condition of a weak \Buchi game, we now describe how to separate the SCCs of $(V,E)$ \gatodo{what is $(V,E)$?} to accepting and non accepting SCC. 
% Let $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
% \bigwedge_{i=1}^{n_l} \ltlG \ltlF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG \ltlF(g_{l,j})$.
% Then an SCC $S$ at $(V,E)$ is called \textit{accepting} if for \textit{every} constraint $\varphi_l$, where $l\in\{1,\dots,k\}$, one of the following hold:
% \begin{description}
% \item[All guarantees hold in $S$.] For every $j\in\{1,\dots,m_l\}$, there exists $(\inp,\out)\in S$ such that $\out\models g_{l,j}$.

% \item[Some assumption cannot hold in $S$.] There exists $i\in\{1,\dots,n_l\}$ such that for all $(\inp,\out)\in S$, $\inp\not\models a_{l,i}$. 
% \end{description}


% Intuitively, every winning play for the game structure $\GS$ must converge to an accepting SCC \gatodo{I don't understand this sentence. This is a sufficient and necessary condition to win a play, right? Why "intuitively"?} (every infinite play at every graph based game must eventually converge to a single SCC). To see that the special form of separated specification $\varphi$ that we have requires from a winning strategy that for every constraint $\varphi_l$ either: all guarantees hold; there is an assumption that does not hold
% \dftodo{clean assume/guarantee terminology, clean that paragraph}. We formalize this intuition in Section \ref{sec:syntstrat}. We call the strategy that solves weak \Buchi $f_{B}$.

% It is interesting to observe what action should the system do when reaching an accepting SCC. Intuitively, while in an accepting SCC $S$, making sure that every \textit{system vertex} \dftodo{change terminology} of $S$ is visited infinitely often, should suffice for the system meet the specification conditions and to win \dftodo{better explain?}, \textit{no matter what actions the environment performs}. Indeed note that in our specification, the system can indeed keep visiting any system-vertex regardless of the actions of the environment \dftodo{this is a key observation, say it much before and highlight!}. We call this strategy $f_{travel}$. \gatodo{This is not what we do. For each guarantee $g_{l,i}$ we play a reachability game inside $S$. If S has no $g_{l,i}$-state, the play immediately terminates. B.t.w. this is why we get time complexity $O(|\varphi|N)$: $O(|\varphi|)$ reachability games.}


% A complication rises however when combining both $f_B$ \gatodo{$f_B$ was not defined} and $f_{travel}$ while in $f_B$, performing $f_{travel}$ may take the system out of the winning regions of $f_B$. Thus it is not clear that we can indeed combine both to make winning strategy for the system.
% To overcome that we show the following the following property that we call the \textit{delay property}: if $(x,y)$ is a state in the winning region of $f_B$, and $(a,b)$ is a state for which there is a path in $G_I$ \dftodo{change font} from $x$ to $a$ and a path in $G_O$ from $b$ to $y$, then $(a,b)$ is also in the winning region of $f_B$.

% Note that under this property the system can  "delay" within an SCC and still win the separation game. 

% % since $S$ is defined according to \textit{both} environment and system graphs. Therefore the environment can choose an action that make the play depart from $S$. In this case, the system must find it's way and chase the environment, but how can it do it from every state in $S$ in which it was? 
% % We answer this by showing that the system can delay in an SCC as long as it wants and still win the game. For that we need the delay property, described below \dftodo{I wrote rubbish here. Better clean!! why not just use the reachability? Why the delay at all?}.








% The game proceeds by the environment player assigning values to the input variables $\I$ and the system player assigning values to the output variables $\O$.  
% The game starts at one of the initial states of the graph. 
% In every round of the game, first the  environment chooses an assignment to the $\I$ variables, and then the system will choose an assignment $O$ to the $\O$ variables.
% The combined assignment $I \cup O$ determines the unique state  the game moves to.
% The notions of plays, strategies, winning conditions and so on naturally transfer to the explicit-state representation. 





%For readability, we also consider an explicit representation of the game between the environment and the system. Given a game structure  $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$, we define a graph that serves as a ``game-board" as follows. $G^{\mathit{GS}}=(V^\mathit{GS},E^\mathit{GS})$, where $V^\mathit{GS}=2^{\I\cup\O}$, and $(\inp_0,\out_0)E(\inp_1,\out_1)$ if $\big((\inp_0,\out_0),(\inp_1',\out_1')\big)\models \rho_\I\wedge \rho_\O$.
%At the beginning of a play, the environment chooses $\inp\in 2^\I$, the system then responds with $\out\in 2^\O$, and thus the first state of the play is $(\inp,\out)\in V^{\mathit{GS}}$. Afterwards, the payers repeatedly choose the next state of the play: form state $(\inp_0,\out_0)$ the environment chooses $\inp_1\in 2^\I$ such that $(\inp_0,\out_0,\inp_1')\models \rho^e$, the system replies with $\out_1$ such that $(\inp_0,\out_0,\inp_1',\out_1')\models \rho_\O$, and the play traverses to state $(\inp_1,\out_1)$.  Note that the notions of plays, strategies etc. naturally transfer to the explicit representation. We omit the straightforward adaptation of those notions in the explicit context. 

% A {\em strongly connected component} (SCC) of a directed graph $(V,E)$ is a maximal set of states within which every state is reachable from every other state.  It is well known that SCCs partition the states of a directed graph.

% Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
% Then, these SCCs hold a special property in a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$. Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
% Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all their states are contained in $\F$ or  {\em non-accepting components} mean none of their states is present in $\F$. 
% Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a path is winning for the system if the path ultimately never exist an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every path will ultimately remain inside an accepting component.

%A \textit{subgraph} $G_0$ of a directed graph $G=(V,E)$ is a graph $(V_0,E_0)$ where $V_0\subseteq V$ and $E_0= E\cap (V_0\times V_0)$. 
%\textit{A path} in a graph $G=(V,E)$ is a sequence $(v_0,\cdots v_i)$ such that for all $0\leq j<i$, $(v_j,v_{j+1})\in V$. Note that a single vertex is also considered as a path.
%A \textit{strongly connected component} (SCC) in a graph $G=(V,E)$, is a maximal subset $V_0\subseteq V$ such that for every vertices $v,v' \in V_0$, there exists a path from $v$ to $v'$ in $G$. Note that the set of all SCCs forms a partition of the graph-vertices.
%An SCC, $S$ is a \emph{terminal SCC} if for every $s\in S$ the next holds: if a state $t$ is reachable from $s$, then $t\in S$.

%We exploit the special structure of the weak B\"uchi automaton to solve this game more efficiently than a typical Parity game or B\"uchi game. 

\begin{comment}

Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
Then, these SCCs hold a special property in a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$. Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all their states are contained in $\F$ or  {\em non-accepting components} mean none of their states is present in $\F$. 
Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a path is winning for the system if the path ultimately never exist an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every path will ultimately remain inside an accepting component.

% \subsection{Explicit State Representation}
% \label{sec:explicitweakbuchi}


Weak B\"uchi games have previously been studied when the states of the game are represented explicitly. Under this state representation, weak B\"uchi games can be solved in linear-time to the size of the explicit graph underlying the game~\cite{krish'spaper}. This section reviews that algorithm. 
\end{comment}


% \subsection{Name Name Name}

% We can now state the main theorem of the section that essentially describes the reduction statement. \dftodo{change my writing, this is awful}

% \begin{theorem}\label{thm:reduction}
% .....
% \end{theorem}



% In this section we prove Theorem \ref{thm:reduction}. This proof also yields an algorithm for computing a winning strategy for separated $GR(k)$ games from a 
% winning strategy on weak \Buchi games. 

\subsection{The Delay Property}\label{sec:delay}

The delay property can be used to show that combining the weak \Buchi game strategy $f_B$ and the SCC travel strategy $f_\travel$ maintains the system in the winning region. 
The Delay Property Theorem essentially says that while in an SCC $S$ contained in the winning region, if the environment moves unilaterally to a different SCC in $G_\I$, the new SCC will still be in the winning region for the system.
%that is a winning region\gatodo{contained in a winning region? from which we can win?}, the system can remain in an $S$ or the environment can leave an $S$, and the system still stays in the winning zone.\gatodo{Not sure this is clear}
It is important to note that this property does not hold for every weak \Buchi game, only for those in which the game structure separates variables as in Definition~\ref{def:separates-variables}.
%We remark that this property is unique to the game we are dealing with. It does not hold for every  weak \Buchi game.

We start with the following lemma that states that the system can still win with a single step delay.


\begin{lemma}\label{lem:1delay}
Consider a weak B\"uchi game $B$ that separates variables.
%constructed in Section~\ref{sec:accepting-SCCs}. \gatodo{High chances the reviewers will comment on this forward ref. Especially as it is an appx. If it is needed for the flow, why it is in appx? \\ Consider instead to define in the prev. overview the weak Buchi game with target $GF(acc)$ where $acc$ is a set of states (not a BDD!). i.e. to write instead "consider the weak Buchi game $(\G,\ltlG \ltlF (\mathit{acc}))$..."}
Let $\inp_0,\inp_1\in 2^\I$ such that  $(\inp_0,\inp'_1)\models \rho_\I$, and assume that the system can win from $(\inp_0,\out_0)$. Then the system can also win from $(\inp_1,\out_0)$.
\end{lemma}

\begin{proof}
Let $f$ be a winning strategy for the system from $(\inp_0,\out_0)$. 
We construct a winning strategy $f_d$ from $(\inp_1,\out_0)$. Intuitively, $f_d$ acts from state $(\inp_1, \out_0)$ as if it were following $f$ from state $(\inp_0, \out_0)$, with a delay of a single step: the input in the current step is used to choose the output in the next step.
%it ignores the final input, and shifts the sequence of outputs one step backwards \dftodo{clarify}.
%Since a strategy is deterministic, to simplify notation we denote a strategy $f((\inp_1,\out_0),\dots,(\inp_m,\out_{m-1}))$ as $f(\inp_1,\dots,\inp_m)$.\gatodo{I suggest not to do that. If we gave some notation, use it as is} 



% Recall that the strategy $f^s$ is played as follows. In a state $(i,j)$ the environment makes an action $i'$, and the strategy makes an action $o'$ for which $o'=f^s((i_0,O_0),\cdots (i,o))$ is a result of applying the strategy on previous states so far. Thus the next state reached is $(i',o')$ \dftodo{clarify, but remove or move to prelims}.

We use $f$ to define $f_d$ inductively over play prefixes of length $m\geq 1$, by setting $f_d((\inp_1, \out_0), \ldots, (\inp_m, \out_{m-1}), \inp_{m+1}) = f((\inp_0, \out_0), \ldots, (\inp_{m-1}, \out_{m-1}), \inp_m)$.
%$f_d(\inp_1,\dots,\inp_{m+1})=f(\inp_0,\dots,\inp_m)$. 
Note that $f_d$ is well defined since the game separate variables: from state $(\inp, \out)$, the outputs that can be chosen for the successor state depend only on $\out$, and not on $\inp$.
%for all $\inp,\hat{\inp}\in\I$, $\out \in \O$, the actions that the system can do from state $(i,o)$ and from state  $(\hat{i},o)$ are the same \dftodo{clarify}.
Note that by this definition, for every play $(\inp_1,\out_0),(\inp_2,\out_1),\dots, (\inp_{m+1},\out_m),\dots$ consistent with $f_d$, there is a play $(\inp_0,\out_0),(\inp_1,\out_1),\dots, (\inp_m,\out_m),\dots$ consistent with $f$.

Even if $f$ is memory-less, note that $f_d$ is not. We remark that \textbf{we define $f_d$ only for proving the lemma, and it is not part of our solution.} We shall provide a memory-less winning weak B\"uchi strategy later. 

Next, we show that $f_d$ is winning if $f$ is winning.
Take a play $(\inp_1,\out_0),(\inp_2,\out_1),\dots$, consistent with $f_d$. By the construction, $(\inp_0,\out_0),(\inp_1,\out_1),\dots$ is consistent with $f$. Since this is a play on a weak \Buchi game, after some point it must remain in a single SCC $S$, say from state $(\inp_j,\out_j)$. Since $f$ is a winning strategy the SCC $S$ must be accepting. %and thus stabilizes in an accepting SCC $S$, say from state $(\inp_j,\out_j)$.
Then $\out_j,\out_{j+1},\dots$ is an infinite path in the SCC $S|_\O$, and $\inp_j,\inp_{j+1},\dots$ is an infinite path in the SCC $S|_\I$. %Specifically, it means that $\inp_{j+1}$ is a path in $S\uparrow\I$. 
Consequently, $(\inp_1,\out_0),(\inp_2,\out_1),\dots $ converges to an SCC $\hat{S}$ in which $\hat{S}|_\I = S|_\I$ and $\hat{S}|_\O = S|_\O$. Since the conditions for an SCC $D$ to be accepting depend only on the relation between $D|_\I$ and $D|_\O$, we have that $\hat{S}$ is accepting since $S$ is accepting as well.\qed




% Define a \textit{standard SCC} as an SCC that is result of a product of input-SCC and output-SCC (in our setting, an SCC can have a singleton in the input or output, thus it is not always like this.\dftodo{Is this so? anyhow clean and move definition to prelims}).

% Now, assume that $f^s$ is winning, and let $((\inp_1,\out_0),(\inp_2,\out_1),\cdots (\inp_{m+1},\out_m),\cdots)$ be a play in $f^s_d$. Then there is \dftodo{There is a glitch here, check old proof (commented out after this one) and fix accordingly}
% $((\inp_0,\out_0),(\inp_1,\out_1),\cdots (\inp_m,\out_m),\cdots)$ is a play in $f^s$ that ends in an accepting SCC $S$ since $f^s$ is winning. Specifically there is an input SCC $S_\I$ and output SCC $S_\O$ such that $S=S_\I\times S_\O$ and such that $(\inp_0, \inp_1, \inp_2,\cdots)$ ends up in $S_I$, and $(\out_0, \out_1,\out_2,\cdots)$ ends in $S_\O$.\gatodo{is it that clear?} Therefore $(\inp_1, \inp_2,\cdots)$ also ends up in $S_\I$, and as a result, the play $((\inp_1,\out_0),(\inp_2,\out_1),\cdots (\inp_{m+1},\out_m),\cdots)$ also ends up in the winning SCC $S$ as required.




% Now, we claim that $S_d$ is an accepting SCC. To prove this claim, take a component $\varphi_l  =
% \bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$.  
% First, assume that for every guarantee $GF(g_{l,j})$, $S$ includes a state $s$ such that $s\models g_{l,j}$.  Hence, there exists a path in $S$ from $(\inp_i,\out_i)$ to a state $(\inp,\out)$ such that $\out\models g_{l_j}$. Use Observation~\ref{obs:shift} to conclude that the same holds for $S_d$: there exists a path in $S_d$ from $(\inp_{i+1},\out_i)$ to a state $(\widehat\inp,\out)$, and $\out\models g_{l,j}$. 

% Second, assume that for some assumption $a_{l,j}$, $S$ does not include a state $s\models a_{l,j}$. Assume, towards a contradiction, that there exists $s_d=(\inp^d,\out^d)\in S_d$ such that $\out_d \models a_{l,j}$. Hence, there exists a path in $S_d$ from $(\inp_{i+1},\out_i)$ to $(\inp^d,\out^d)$. Use Observation~\ref{obs:shift} to conclude that $S$ includes an $a_{l,j}$-state as well, in contradiction to the assumption.
% Consequently, $S_d$ is an accepting SCC and thus $f^s_d$ wins w.r.t. the B\"uchi objective, as required.\gatodo{to read again...}\qed


\end{proof}








% \begin{theorem}\label{thm:delay}[The Delay Property Theorem]
% Consider the weak B\"uchi game constructed in Section~\ref{sec:accepting-SCCs}. Let $\inp_0,\dots,\inp_n\in (2^\I)^+$ be a sequence such that for all $i\in\{0,\dots,n\}$, $(\inp_i,\inp_{i+1})\models \rho_\I$. Moreover, let $\out_{-m},\dots,\out_0\in (2^\O)^+$ be a sequence such that for all $i\in\{-m,\dots,-1\}$, $(\out_i,\out_{i+1})\models \rho_\O$.
% If the system can win from $(\inp_0,\out_0)$, then it can also win from $(\inp_n,\out_{-m})$.
% \end{theorem}


We can now prove the delay property, following by straightforward induction from Lemma~\ref{lem:1delay}.


\begin{theorem}[Delay Property Theorem]\label{thm:delay}
Consider a weak B\"uchi game $B$ that separates variables.
%constructed in Section~\ref{sec:accepting-SCCs}.
Let $\inp_0,\dots,\inp_n\in (2^\I)^+$ be a path in $G_\I$, and for $m\geq 0$, let $\out_{-m},\dots,\out_0\in (2^\O)^+$ be a path in $G_\O$. Assume that the system can win from $(\inp_0,\out_0)$. Then the system can also win from $(\inp_n,\out_{-m})$.
\end{theorem}

\begin{proof}
From $(\inp_n,\out_{-m})$, the system can simply ignore the inputs and follow the path in $G_\O$ to $\out_0$. Let $(\inp_{n+m}, \out_0)$ be the state at that point in the play. Note that there is a path between $\inp_n$ and $\inp_{n+m}$, and therefore there is a path between $\inp_0$ and $\inp_{n+m}$. If the system can win from $(\inp_0, \out_0)$ then by induction on Lemma~\ref{lem:1delay} it can win from $(\inp, \out_0)$ for all $\inp$ such that there is a path in between $\inp_0$ and $\inp$. Therefore, the system can win from $(\inp_{n+m}, \out_0)$, and by consequence from $(\inp_n,\out_{-m})$.
% \dftodo{write better, perhaps clarify}
% To show that the system can win from $(\inp_n,\out_{-m})$ for every $m\geq 0$, it is sufficient to show that the system can win from $(\inp_0,\out_{-1})$. The system applies the following strategy: first, for any legal input $\inp$ the system responds with $\out_0$. Then, by the previous lemma, the system has a winning strategy from $(\inp,\out_0)$. \dftodo{Do we need to elaborate? Perhaps write it a bit more precise.} \qed
\end{proof}

A corollary of Theorem~\ref{thm:delay} is the following statement about the structure of the winning region of a weak \Buchi game that separates variables.

\begin{corollary}\label{cor:delay}
The winning region of a weak \Buchi game $B$ that separates variables is a union of SCCs.
\end{corollary}

\begin{proof}
Let $(\inp,\out)$ be a state in the winning region of $B$, let $(\hat\inp,\hat\out)$ be a state in the same SCC $S$ of $(\inp,\out)$, and let $S|_\I$ and $S|_\O$ be the projections of $S$ on $G_\I$ and $G_\O$, respectively.
Then there is a path $\inp_0,\ldots, \inp_n$ for some $n\geq 0$ in $S|_\I$ such that $\inp_0=\inp$ and $\hat\inp=\inp_n$. Similarly, there is a path $\out_{-m},\ldots, \out_0$ for some $m\geq 0$ in $S|_\O$ such that $\hat\out_0=\out$ and $\hat\out=\out_{-m}$. Then by the delay property of Theorem~\ref{thm:delay}, the vertex $(\hat\inp,\hat\out)=(\inp_n,\out_{-m})$ is also in the winning region of $B$. \qed
\end{proof}





\subsection{Constructing weak \Buchi game strategy}
\label{sec:accepting-SCCs}
\gatodo{time complexity is $O()$ and not $\O()$. $\O$ is something else in the paper...}
We now describe a symbolic algorithm for weak \Buchi game synthesis. We note that this algorithm fits every weak \Buchi game, and not only those that are resulted from our specifications.\gatodo{To be more explicit: we do not assume var-separation}
 We build on top of an existing explicit linear-time algorithm for weak B\"uchi games~\cite{Chatterjee08} that runs in $O(|V|+|E|)$ time, where $(V,E)$ is the underlying game graph. We explain the algorithm briefly, with a detailed description appearing in the appendix.\gatodo{which appx?}\gatodo{1. I (briefly) looked at~\cite{Chatterjee08}. Although you can possibly link between computations of our algo and~\cite{Chatterjee08}, I am not sure it is "on top". We deal with a topological sort and~\cite{Chatterjee08} with attractors to 'colors'.  Maybe we just mention that linear-time algo can be derived form the litruture and take full ownership on the algo we give?\\
2. I suggest to omit the V+E analysis. 
we are not interested in time complexity of the algo variant on the graph representation}


\subsubsection{High-level algorithm description.} \dftodo{think of writing it symbolically}
We are given a weak B\"uchi game with game graph $(V,E)$ and winning condition $\ltlG\ltlF\varphi$. %in explicit state representation.
As described earlier, the accepting and non-accepting SCCs can be identified in $O(|V| + |E|)$.\gatodo{redundant. We don't want to identify them in the graph}
Let $\Statess_0, \dots \Statess_m$ be the SCCs partitioning the directed graph $(V,E)$. W.l.o.g.\gatodo{no need in wlog since we describe, not construct},  let $\Statess_1>\Statess_2>\dots >\Statess_m$ with respect to the partial order $>$ induced by the topological sorting of the SCCs.  The algorithm works in backward induction.
In the \textit{base case}, we take all  {\em terminal partitions} $S_j,\dots,\Statess_m$. That is, each SCC $S_i$ such that no other SCC is reachable from $S_i$. 
In this case, plays beginning in any state of $\Statess_i$ in the list  will never leave it and be of infinite length. Thus, if a terminal $\Statess_i$ is an accepting component, every state of $S_i$ is a winning state for the system, while if $\Statess_i$ is a non-accepting component, every state of $S_i$ is a winning state for the environment.\gatodo{maybe recall here that there are no deadlocks? Otherwise $S_m$ can be a deadlock... }

For the induction step, suppose that $\vec{S} =\{\Statess_{i+1}, \ldots, \Statess_m\}$ have been classified as winning for the system or the environment,\gatodo{the description is incorrect. It is possible that some states in an SCC S are winning, an some are not} and partition $\vec{S}$ into a set of accepting SCCs $\vec{S}_{\mathit{acc}}$ and non accepting SCCs $\vec{S}_{\mathit{rej}}$. Let $\vec{S'}=\{\Statess_j,\Statess_{j+1}, \ldots, \Statess_{i}\}$ be the SCCs from which all edges leaving the SCC lead to an SCC in $\vec{S}$, and take $S_i\in \vec{S}'$.
%Then, note that a state in $\Statess_i$ is winning for the system if and only if it can either force plays to stay inside $\Statess_i$, or force the play to reach the $\vec{S}_{acc}$, a safety game on with winning condition $\vec{S}_{acc}$ with a  reachability game  with winning condition $\vec{S}_{rej}$ can determine the accepting SCCs from $\vec{S'}$. \lmttodo{This paragraph is confusing, there seems to be something missing.}
If $S_i$ is a non accepting SCC, the system can win from $s\in S_i$ iff it can force reaching $S\vec{S_{\mathit{acc}}}$ from $s$. Otherwise, if $S_i$ is an accepting SCC, the system can win from $s\in S_i$ iff it can win w.r.t. the safety winning condition  $\ltl G (S_i\cup \vec{S_{\mathit{acc}}})$. 
\dftodo{I cut the complexity analysis to appendix. I think we should adjust that once we have it clean.}


\subsubsection{Symbolic algorithm description.}


We are given a weak \Buchi game $((\I, \O, \theta_\I, \theta_\O, \rho_\I, \rho_\O), \ltlG \ltlF \varphi)$ with BDDs representing $\theta_\I$, $\theta_\O$, $\rho_\I$, $\rho_\O$ and $\varphi$.
The goal is to compute a BDD for the winning region of the weak B\"uchi game and then to determine whether the initial states of the game intersect with the winning region. The construction of the winning region follows a fixed-point computation that adapts the inductive algorithm presented in  Section~\ref{sec:explicitweakbuchi}: in the basis of the fixed point computation, the winning region is the set of accepting and terminal SCCs; in the inductive step, the winning region includes winning states by examining SCCs that are higher in the topological ordering on SCCs.
%There are several challenges in executing the fixed-point algorithm outlined here. 
In what follows we describe a sequence of BDDs that we construct towards constructing the overall BDD.
We use the notation $\X$\gatodo{not a big issue at all, but maybe $\V$ is more standard?} to denote an ordered set of variables over $\I\cup\O$. 



% We begin with introducing necessary notation.
% Let $B(\V)$ be a BDD defined over the ordered set of variables $\V = \{v_1, \ldots, v_n\}$. Let $W = \{w_1, \ldots, w_n\}$ be a new, ordered set of variables of the same cardinality. We use $B(W)$ to denote the BDD in which every variable $v_i$ is replaced with the corresponding variable $w_i$. We can extend this to a BDD $B(\V_1, \ldots, \V_m)$ over multiple sets $ \V_1, \ldots \V_m$ of variables in the natural way. 
% Given an ordered set of variables $\V = \{v_1, \ldots, v_n\}$, we use $\V'$ to denote the ordered set of new variables $\V' = \{v'_1, \ldots, v'_n\}$.


\paragraph{BDD for SCCs.} We want to construct a predicate which indicates when two states in a game structure are present in the same SCC. Let predicate $\Reach(s,t')$ hold if there is a path from state $s$ over $\I\cup\O$ to state $t$ over $\I\cup\O$ in the game structure $\GS$.
Similarly, a predicate $\Reachinverse(s,t')$ holds if and only if  $\Reach(t,s')$ holds.
BDDs for   $\Reach$  and $\Reachinverse$  can be computed in $\O(N)$ symbolic operations, see appendix for details.
Then, a BDD for an SCC is constructed in  $\O(N)$ symbolic operations as $\SCC(\X,\X') := \Reach(\X,\X') \wedge \Reachinverse(\X,\X')$. \lmttodo{Need to decide whether to use $\Reach(s,t')$ or $\Reach(\X,\X')$. }






\paragraph{BDD for Terminal SCC.}
The induction basis for the construction of a winning region requires us to know what the terminal SCCs are. Let predicate $\terminal (s)$ hold if state $s$ over $\I\cup\O$ is present in a terminal SCC. Then
$\terminal(\X) := \forall \X': \Reach(\X,\X')\rightarrow \SCC(\X,\X')$.
Therefore, given BDDs for $\mathsf{Reach}$ and $\mathsf{SCC}$, the construction of $\mathsf{Terminal}$ requires $\O(1)$ symbolic operations. 

% \paragraph{BDD to obtain SCCs higher in the topological ordering.}   
% The induction step in the construction of the winning region requires us to know how to compute the {\em predecessor} SCCs w.r.t. to the topological ordering on the SCC.


% Let $C$ be a set of SCCs over the game structure. For a state $s$ over $\I\cup\O$, let $s\models C$ be the shorthand for ``there exists an SCC $S\in C$ such that $s\models S $".
% A set of SCCs $C$ is said to be {\em closed downwards} if for every state $s \models C$, for every state $t$ that is reachable from $s$, $t\models C$. If $C$ is closed downwards, then its predecessor, denoted $\mathit{pre}(C)\supseteq C$,  is  a set of SCCs  such that if $S$ is an SCC in $\mathit{pre}(C)$, states $s\models S$ and there exists a path from $s$ to  state $t$, then either $t\models S$ or $t\models C$. Note that $\mathit{pre}(C)$ is also closed downwards.
% Observe that predicate $\terminal$ denotes a downward closed set of SCCs. 

% Let predicate $\C$ over $\X$ denote a downward closed set of SCCs. Then, from the definition, we see that its predecessor $\pre(\C)$ can be obtained as follows:
% \[
% \pre(\C) := \forall \X': \Reach(\X,\X') \rightarrow (\SCC(\X,\X') \vee \C(X'))
% \]

% Then, a BDD for the predecessor of a $\pre(\C)$ is computed in $\O(1)$ symbolic operations, given a BDD for $\Reach$, $\SCC$, and the downward closed set $\C$.

\paragraph{Computing the Winning Region.}

We can finally describe the fixed-point computation to construct a BDD for the winning region in  a weak \Buchi game. 
Let $\Reachability(A,B)(\X)$\gatodo{I suggest to change the notation so it would be clear that A and B are parameters and X are vars. e.g. $\mathit{A-Reachabilty_B(X)}$ } denote a BDD, generated by solving a reachability game, that takes as input a set of source states $A$ and target states $B$, and outputs those states in $A$ from which the system can guarantee to move into $B$.
Same. let $\Safety(A,B)(\X)$ denote a BDD, generated by solving a safety game, that takes as input a set of source states $A$ and target states $B$, and outputs those states in $A$ from which the system can guarantee that all plays remain inside the set $B$.
Details can be found in ~\cite[Chapter~20]{2001automata}.\gatodo{Wrong chapter...}


Then, let  $\winning(s)$ denote that state $s$ over $\I\cup\O$ is in the winning region. Then, $\winning$ is the fixed point of $\winningAux$ which is defined below, where the construction essentially follows the explicit algorithm:
\begin{description}
    \item{\textbf{Base Case.}} $\winningAux^0(\X) := \terminal(\X) \wedge \varphi(X)$ and
    $\C^0(\X) := \terminal(\X)$
    
    \item {\textbf{Inductive Step.}} Define:
    
    $$\C^{i+1}(\X) :=  \forall \X': \Reach(\X,\X') \rightarrow (\SCC(\X,\X') \vee \C(X'))$$
    
    \begin{align*}
    \winningAux^{i+1}(\X) & :=        \winningAux^i(\X) \\
    & \vee \Reachability(\C^{i+1}(\X), \winningAux^i(\X)) \\
    &  \vee  
    \Safety(\C^{i+1}(\X), \winningAux^i(\X)\\
    &\vee (\C^{i+1}(\X)\wedge \neg \C^{i}(\X)\wedge\varphi(\X)))
    \end{align*}
  
\end{description}


To explain the construction of $\winning$, note that a state in $\C^{i+1}(\X)$ is winning in one of these cases:
(i) Every state in $\winningAux^i(\X)$ is also winning.  
(ii) The system can force to move into the region $\winningAux^i(\X)$. This set of states can be obtained from $\Reachability(\C^{i+1}(\X), \winningAux^i(\X))$. 
(iii) %state in   $\C^{i+1}(\X)$ is winning if
the system can force all plays in  $\C^{i+1}(\X)$ to remain in states in $A(\X) = \C^{i+1}(\X)\setminus\C^i(\X)$ that accept $\varphi$ or satisfy $\winningAux^i(\X)$. This set of states can be obtained from $\Safety(\C^{i+1}(\X), \winningAux^i(\X) \vee (\C^{i+1}(\X)\wedge \neg \C^{i}(\X)\wedge\varphi(\X)))$. 
    

Finally, we prove the following theorem.

\begin{theorem}\label{thm:weakbuchi}
Realizability and Synthesis for weak \Buchi games can be done in $O(N)$ symbolic steps.
\end{theorem}

\paragraph{Proof Outline.}
The proposed construction symbolically implements the inductive procedure of the explicit algorithm. Hence, it correctly identifies the system's winning region. 
It remains to show that the algorithm performs $O(N)$ symbolic operations. First, of all, the constructions of $\SCC$ and $\terminal$ take $\O(N)$ symbolic operations collectively. It suffices to show that in the $i$-th induction step, solving the reachability and safety games  performs  $O(|\pre(\C^{i+1})\setminus\C^i|)$ operations. This can be proven by a careful analysis of the operations and the sizes of resulting BDDs using standard results on safety and reachability games. Details have been deferred to the Appendix\gatodo{this high-level description explains realizability check, but I think it fails to explain the strategy construction}.\qed 































































\subsection{Solving Separated-GR($k$) games}\label{sec:syntstrat}


Having a symbolic strategy for weak \Buchi, we can finally show how to symbolically solve realizability and synthesis for Separated-GR($k$) games. followed by a time complexity analysis.
Our construction mainly follows our framework. Our current solution for $f_t$ is a strategy with memory $|\varphi|$ as we define below in details.

\paragraph{Defining accepting states}

We are given a Separated-GR($k$) game structure $\GS = (\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and an assertion $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j}))$. We first need to represent $\GS$ and $\varphi$ as BDDs.\gatodo{??}, These symbolic representations are standard in common in the literature e.g. \cite{} \dftodo{complete}. Next, we describe the set of accepting states symbolically. That is, we provide a linear-time construction of a BDD that recognizes all accepting states.


% This section presents an algorithm to solve separated GR($k$) games when represented symbolically as in Definition~\ref{def:separatedGRk}. From Theorem~\ref{}, we know it trivially reduces to a weak B\"uchi game. The task, therefore, is to present an algorithm for weak B\"uchi games when presented symbolically. More specifically, we design a BDD based algorithm to solve a weak B\"uchi game $(\GS,\ltlG\ltlF \varphi)$ where the assertions in the game structure $\GS = (\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and the assertion $\varphi$ are given in the form of a BDDs.



We first define every state in an accepting SCC as an \textit{accepting state}. We next turn to show that all accepting states can be identified efficiently. \dftodo{move lemma to 6.2}

\begin{lemma}
A BDD $\beta_\mathit{acc}$ over $\I,\O$ such that $\beta_\mathit{acc}(\inp,\out)$ if $(\inp,\out)$ is accepting, can be constructed in $O(|\varphi|+N)$ symbolic operations.
\end{lemma}
\begin{proof}
Consider the BDD $\beta_\mathit{SCC}$ \dftodo{see that $B_{SCC}$ is defined oenly later, fix that} \lmttodo{Should this be $\SCC(X, X')$? Unify notation.}, constructed in $O(N)$ operations (see Lemma~\ref{lem:beta_SCC}). Take a component $\varphi_l= 
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$. First, we identify all states such that their SCC includes a $g_{j,l}$-state. For $j\in\{1,\dots,m_l\}$, let $\beta_{g_{l,j}}$ be a BDD over $\I,\O,\I',\O'$ such that $\beta_{g_{l,j}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $\out_1\models g_{l,j}$. Hence, the BDD $\gamma_{l,j}$ over $\I,\O$, defined by $\exists \I',\O'(\beta_\mathit{SCC} \wedge \beta_{g_{l,j}})$, accepts a state $(\inp,\out)$ if its SCC includes a state $s\models g_{l,j}$.

Now, we focus on the assumptions. Similarly to the former case, for $i\in\{1,\dots,n_i\}$, let $\beta_{a_{l,j}}$ be a BDD over $\I,\O,\I',\O'$ such that $\beta_{a_{l,j}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $\inp_1\models a_{l,i}$. Hence, the BDD $\alpha_{l,i}$ over $\I,\O$, defined by $\forall \I',\O'(\beta_\mathit{SCC}\rightarrow \neg\beta_{a_{l,i}})$,
accepts a state $(\inp,\out)$ if its SCC does not includes a state $s$ such that $s\models a_{l,j}$.

Therefore, the BDD $\beta_\mathit{acc}$ is constructed by $\bigwedge_{l=1}^k(  (\bigwedge_{j=1}^{m_l}\gamma_{l,j}) \vee (\bigvee_{i=1}^{n_l} \alpha_{l,i}))$ \lmttodo{Should this be $\neg \alpha_{l,i}$?}. The construction is performed by $O(|\varphi|+N)$ operations. \qed
\end{proof}


\paragraph{Constructing $f_{B}$.}

Next, we use Theorem~\ref{} to construct a symbolic strategy as a BDD for our weak \Buchi game.

\paragraph{Constructing $f_{\travel}$.}


  For the presentation of $f_{\travel}$ we arbitrarily order all guarantees that appear in our GR($k$) formula: ${\gar}_0,\dots,{\gar}_{m-1}$. For each guarantee $\gar_j$, we take a reachability strategy $f_{r(j)}$ that never leaves the SCC it is applied from. For the sake of presentation, we assume that if  $s\in S$, an SCC that includes no $\gar_j$-state, then $f_{r(j)}$ returns a distinguished value $\bot$. We equip $f_\travel$ with a memory variable $\mathit{mem}\in\{0,\dots,m-1\}$. $f_\travel(s,i)$ is computed as follows: for $\mathit{mem},\mathit{mem}+1,\dots$ we find the first $\mathit{mem}+j$ such that the SCC of $s$ includes a $\gar_j$ state, and   activates $f_{r(\mathit{mem}+j)}$ to reach such state (loop in line 1). If no guarantees can be satisfied in $S$, we just return an arbitrary output to stay in $S$ (line 6). We remark that we chose a loop-based algorithmic presentation for readability purposes. However, $f_\travel$ can be implemented by BDD operations (without the distinguished value $\bot$) with memory of size $m$. The construction of $f_\travel$ requires $O(|\varphi|N)$ symbolic BDD-operations as we need to construct $m$ reachability strategies (clearly, $m\leq |\varphi|$). 


\paragraph{Combining the strategies}

Finally, we invoke the framework and interleave the strategies. The following algorithm \label{algo:winning-strategy} describes our flow. Correctness follows from the framework correctness.

%Overall, the strategy depicted in Algorithm~\ref{algo:winning-strategy} is constructed  in $O(|\varphi|N)$ symbolic operations.\dftodo{expand more}


  \begin{algorithm}[t!]
  	\caption{A winning strategy}
  	\label{algo:winning-strategy}
  	\begin{algorithmic}[1]
		
		\setcounter{ALG@line}{-1}
		
		\State \textbf{initialization:} construct $\beta_\mathit{SCC}$, $\gamma{=}\exists\O'(\beta)$  \quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
		\Statex
		\Statex{\begin{center}
  				/*\quad\quad  From state $s$ and input $\inp$ \quad\quad*/
 		\end{center}}
	
  	    %\State construct $\beta_\mathit{SCC}$ \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
	
  	    %\State $\gamma = \exists\O'(\beta)$ 
	    
  		\State if $\beta_\mathit{acc}(s)$ and $\gamma(s,\inp')$ \Return $f_\travel(s,\inp)$
		
  		\State \Return $f_B(s,\inp)$
  	\end{algorithmic}
  	
  	
  	\begin{algorithmic}[1]
		
		\Statex{\begin{center}
  				/*\quad\quad  Implementation of $f_\travel(s,i)$ \quad\quad*/
 		\end{center}}
	\setcounter{ALG@line}{-1}
	
	\State \textbf{initialization}: $\mathit{mem}\leftarrow 0$
  	    \For{$i=0$ to $m-1$}
	    
	    \State $\mathit{target}=\mathit{mem}+i \mod m$
	    
  	    \State $\out= f_{r(\mathit{target})}(s,i)$
  	    \State if $\out\neq \bot$ \Return $\out$ 
  		\EndFor
		\State \Return $\out$ such that $\beta_{\mathit{SCC}}(s,\inp',\out')$

  	\end{algorithmic}
  	
  	
  	
  	
  \end{algorithm}

















% That is, $f^s_\mathit{travel}$ satisfies the next property. Let $S$ be an SCC, and consider the subgame induced by $S$. Then, for every $(\inp,\out)\in S$, when the system applies $f^s_\mathit{travel}$, the play will traverse infinitely often states of the form $(\widehat{\inp},\out)$. 
\end{description}


Overall, the strategy depicted in Algorithm~\ref{algo:winning-strategy} is constructed  in $O(|\varphi|N)$ symbolic operations.\dftodo{expand more} \lmttodo{Should this be here instead of in the next section?}


\subsubsection{Correctness of construction}





\begin{lemma}\label{lem:win}\gatodo{1. We cannot give this lemma her since we haven't defined precisely the strategies it is about. 2. We need (somewhere) to prove the correctness of the $f$. Then, lemma 2 follows almost immediately- no need in the proof we give here.}
If a winning strategy $f_B$ exists for the weak \Buchi game $B = (\GS,\ltlG \ltlF(\nu_{acc}))$, then $f$ is a winning strategy for the separated GR($k$) game $A = (\GS, \varphi)$.
\end{lemma}

\begin{proof}
Since $B$ has a winning strategy, then for every initial input $\inp_0 \models \theta_\I$ there is an initial output $\out_0 \models \theta_\O$ such that $(i_0,o_0)$ is in the winning region of $B$.
We will show that playing $f$ always keeps the play in the winning region of $B$, and therefore the play eventually converges to an accepting SCC $S$. Once this happens, following $f_\travel$ guarantees that $\varphi$ is satisfied.\dftodo{put in a separate lemma}

We know that as long as the play is in the winning region of $B$, following $f_B$ will keep it inside the winning region. Therefore, when we switch from $f_B$ to $f_\travel$ we must be inside the winning region and, by definition of $f$, in an accepting SCC $S$. By Corollary~\ref{cor:delay}, as long as we remain inside $S$, which is guaranteed by $f_\travel$, the play will remain in the winning region. Therefore, the only way that the play can leave the winning region is if, while the system is following $f_\travel$, the environment chooses an input that takes the play to a different, non-winning SCC. We now prove that this cannot happen.

Assume that from state $(\inp_0, \out_0)$ in the accepting SCC $S$, the system chooses output $\out_{-m}$ according to $f_\travel$ and the environment chooses input $\inp_n$ such that $(\inp_n, \out_{-m})$ is in a different SCC. Note that $(\inp_0, \out_0)$ is in the winning region, there is a path from $\inp_0$ to $\inp_n$ and there is a path from $\out_{-m}$ to $\out_0$ (since by construction $f_\travel$ remains in the same SCC in $G_\O$). Therefore, by Theorem~\ref{thm:delay} $(\inp_n, \out_{-m})$ is in the winning region as well. 
\qed
\end{proof}

% \begin{proof}
% Since $B$ has a winning strategy, then for every initial input $\inp_0 \models \theta_\I$ there is an initial output $\out_0 \models \theta_\O$ such that $(i_0,o_0)$ is in the winning region of $B$.
% We will show that playing $f$ always keeps the play in the winning region of $B$. Therefore, the play eventually converges to an accepting SCC $S$, and by following $f_\travel$ the GR($k$) winning condition is satisfied.\dftodo{put in a separate lemma}

% To see that, we use the delay property corollary (about the winning region). Therefore as long $f^s_{wb}$ is switched to $f^s_{\mathit{travel}}$ and $f^s_{\mathit{travel}}$ is being played, the system remains in the winning region.

% Now assume that the strategy switched to $f^s_{wb}$ from $f^s_{\mathit{travel}}$. Then we have a state $s$ in an accepting $SCC$, i.e. in the winning region of $f^s_{wb}$,\gatodo{I have no idea what is a winning region of a strategy. Perhaps you mean that $f^s_{wb}$ wins from $s$?} and we need to see that $f^s_{wb}(s,i)$ is in the winning region of $f^s_{wb}$ as well \dftodo{why isn't it obvious???}. For that we use the delay property lemma \dftodo{I don't think we need to use it again} to show that we are still in the winning region \dftodo{clean!!!}.

% For the other side, note that if $(i_0,o_0)$ is not in the winning region of $f^s_{wb}$, then an accepting SCC cannot be reached by the system. Thus, every SCC that is reached does not meet the GR($k$) conditions. 

% \qed
% \end{proof}

Lemma~\ref{lem:win} shows that we can use weak \Buchi games to synthesize a winning strategy for separated GR($k$) games, allowing us to prove the following theorem.

\begin{theorem}\label{thm:realiizability}\gatodo{we can't give it here}
Realizability for separated GR($k$) games can be reduced to realizability of weak \Buchi games.
\end{theorem}

\begin{proof}
Given a separated GR($k$) game, if the corresponding weak \Buchi game is realizable the winning strategy $f_B$ can be used to compute $f$. If it is not realizable, then the environment can force every play to converge to a non-accepting SCC. Since the GR($k$) winning condition cannot be satisfied from a non-accepting SCC, the separated GR($k$) game is also not realizable.
% Given separated GR($k$) games $G$, construct the weak \Buchi game $G'$ by constructing the $\nu_{acc}$..
% Then check realizability for $G'$. By Lemma~\ref{lem:win}, we have that $G$ is realizable if and only if the initial state $(i_0,o_0)$ is in the winning region of a strategy for $G'$, i.e. iff $G'$ is realizable. \qed
\end{proof}


In Section~\ref{sec:algorithmsWeakBuchi} we show in detail how to do\gatodo{to do?} symbolic synthesis for weak \Buchi games.






==> Symbolic_old.tex <==

\section{Realizability and synthesis for separated GR(k)}\label{sec:reduction}


The main part in our solution to Theorem~\ref{thm:main} relies on a reduction to weak B\"uchi games. 
To ease the exposition we first give an outline of the solution, followed by details.

\subsubsection{Outline}

We first consider our input game structure $\GS$ as a weak \Buchi game. For that we consider the SCCs of $\GS$ and mark every SCC $S$ as accepting, if the system can win the GR($k$)-game in the subgame $S$, i.e. if for every component of the GR($k$) formula,
$\varphi_l=\bigwedge_{i=1}^{n_l} \ltlG \ltlF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG \ltlF(g_{l,j})$, either (1) the environment cannot satisfy one of $\varphi_l$'s  assumptions in the subgame $S$, or (2) the system can satisfy all $\varphi_l$' guarantees in the subgame $S$.
\dftodo{Better write: Subgame, what is an SCC over GS, better write the conditions}

Next, we show that realizability for separated GR($k$) games is reduced to realizability of the weak B\"uchi game, described above.
That means: the system can win w.r.t. the GR($k$) objective iff it can win this special weak \Buchi game. That settles the the \textbf{realizability} part of Theorem~\ref{thm:main}.


Finally, we show how to use the winning strategy obtained for the weak \Buchi game to obtain a winning strategy for weak separated games. Intuitively we mark the SCCs of $\GS$ as described above, and apply the `weak B\"uchi' strategy until reaching an accepting SCC, $S$. Then, we play another strategy that circles on $S$ to reach all possible outputs in $S$. Then, whenever the environment leads the game out of $S$, we switch back to the weak B\"uchi strategy. We repeat this process until the play eventually stabilizes in an accepting SCC, in which we win w.r.t. the GR($k$) condition. This solves the \textbf{synthesis} problem. 








\subsection{Constructing weak B\"uchi games} 
\label{Sec:ConversionSeparatedToWeak}

We first show how to construct a symbolic weak \Buchi game from a separated GR($k$) game. 

% Recall from Section~\ref{Sec:Prelims} that a game with game structure $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and a winning condition can be equivalently represented by a game between the system and environment player on  directed graph $ (V,E)$. The states set $V$ is given by states over $\I\cup\O$, and $E$ is the set of all directed edges $(s,t)$ for which $(s,t')\models \rho_\I\wedge\rho_\O$. Recall, we assume that all states of a game structures are deadlock-free\dftodo{Where do we make this assumption and why?}. Thus, there is at least one outgoing edge from every state in directed graph $(V,E)$.
% Finally, the initial states of the graph are the states  $\theta_\I\wedge\theta_\O$.

To meet the condition of a weak \Buchi game, we now describe how to separate the SCCs of $(V,E)$ \gatodo{what is $(V,E)$?} to accepting and non accepting SCC. 
Let $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
\bigwedge_{i=1}^{n_l} \ltlG \ltlF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG \ltlF(g_{l,j})$.
Then an SCC $S$ at $(V,E)$ is called \textit{accepting} if for \textit{every} constraint $\varphi_l$, where $l\in\{1,\dots,k\}$, one of the following hold:
\begin{description}
\item[All guarantees hold in $S$.] For every $j\in\{1,\dots,m_l\}$, there exists $(\inp,\out)\in S$ such that $\out\models g_{l,j}$.

\item[Some assumption cannot hold in $S$.] There exists $i\in\{1,\dots,n_l\}$ such that for all $(\inp,\out)\in S$, $\inp\not\models a_{l,i}$. 
\end{description}


Intuitively, every winning play for the game structure $\GS$ must converge to an accepting SCC \gatodo{I don't understand this sentence. This is a sufficient and necessary condition to win a play, right? Why "intuitively"?} (every infinite play at every graph based game must eventually converge to a single SCC). To see that the special form of separated specification $\varphi$ that we have requires from a winning strategy that for every constraint $\varphi_l$ either: all guarantees hold; there is an assumption that does not hold
\dftodo{clean assume/guarantee terminology, clean that paragraph}. We formalize this intuition in Section \ref{sec:syntstrat}. We call the strategy that solves weak \Buchi $f_{B}$.

It is interesting to observe what action should the system do when reaching an accepting SCC. Intuitively, while in an accepting SCC $S$, making sure that every \textit{system vertex} \dftodo{change terminology} of $S$ is visited infinitely often, should suffice for the system meet the specification conditions and to win \dftodo{better explain?}, \textit{no matter what actions the environment performs}. Indeed note that in our specification, the system can indeed keep visiting any system-vertex regardless of the actions of the environment \dftodo{this is a key observation, say it much before and highlight!}. We call this strategy $f_{travel}$. \gatodo{This is not what we do. For each guarantee $g_{l,i}$ we play a reachability game inside $S$. If S has no $g_{l,i}$-state, the play immediately terminates. B.t.w. this is why we get time complexity $O(|\varphi|N)$: $O(|\varphi|)$ reachability games.}


A complication rises however when combining both $f_B$ \gatodo{$f_B$ was not defined} and $f_{travel}$ while in $f_B$, performing $f_{travel}$ may take the system out of the winning regions of $f_B$. Thus it is not clear that we can indeed combine both to make winning strategy for the system.
To overcome that we show the following the following property that we call the \textit{delay property}: if $(x,y)$ is a state in the winning region of $f_B$, and $(a,b)$ is a state for which there is a path in $G_I$ \dftodo{change font} from $x$ to $a$ and a path in $G_O$ from $b$ to $y$, then $(a,b)$ is also in the winning region of $f_B$.

Note that under this property the system can  "delay" within an SCC and still win the separation game. 

% since $S$ is defined according to \textit{both} environment and system graphs. Therefore the environment can choose an action that make the play depart from $S$. In this case, the system must find it's way and chase the environment, but how can it do it from every state in $S$ in which it was? 
% We answer this by showing that the system can delay in an SCC as long as it wants and still win the game. For that we need the delay property, described below \dftodo{I wrote rubbish here. Better clean!! why not just use the reachability? Why the delay at all?}.








% The game proceeds by the environment player assigning values to the input variables $\I$ and the system player assigning values to the output variables $\O$.  
% The game starts at one of the initial states of the graph. 
% In every round of the game, first the  environment chooses an assignment to the $\I$ variables, and then the system will choose an assignment $O$ to the $\O$ variables.
% The combined assignment $I \cup O$ determines the unique state  the game moves to.
% The notions of plays, strategies, winning conditions and so on naturally transfer to the explicit-state representation. 





%For readability, we also consider an explicit representation of the game between the environment and the system. Given a game structure  $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$, we define a graph that serves as a ``game-board" as follows. $G^{\mathit{GS}}=(V^\mathit{GS},E^\mathit{GS})$, where $V^\mathit{GS}=2^{\I\cup\O}$, and $(\inp_0,\out_0)E(\inp_1,\out_1)$ if $\big((\inp_0,\out_0),(\inp_1',\out_1')\big)\models \rho_\I\wedge \rho_\O$.
%At the beginning of a play, the environment chooses $\inp\in 2^\I$, the system then responds with $\out\in 2^\O$, and thus the first state of the play is $(\inp,\out)\in V^{\mathit{GS}}$. Afterwards, the payers repeatedly choose the next state of the play: form state $(\inp_0,\out_0)$ the environment chooses $\inp_1\in 2^\I$ such that $(\inp_0,\out_0,\inp_1')\models \rho^e$, the system replies with $\out_1$ such that $(\inp_0,\out_0,\inp_1',\out_1')\models \rho_\O$, and the play traverses to state $(\inp_1,\out_1)$.  Note that the notions of plays, strategies etc. naturally transfer to the explicit representation. We omit the straightforward adaptation of those notions in the explicit context. 

% A {\em strongly connected component} (SCC) of a directed graph $(V,E)$ is a maximal set of states within which every state is reachable from every other state.  It is well known that SCCs partition the states of a directed graph.

% Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
% Then, these SCCs hold a special property in a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$. Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
% Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all their states are contained in $\F$ or  {\em non-accepting components} mean none of their states is present in $\F$. 
% Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a path is winning for the system if the path ultimately never exist an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every path will ultimately remain inside an accepting component.

%A \textit{subgraph} $G_0$ of a directed graph $G=(V,E)$ is a graph $(V_0,E_0)$ where $V_0\subseteq V$ and $E_0= E\cap (V_0\times V_0)$. 
%\textit{A path} in a graph $G=(V,E)$ is a sequence $(v_0,\cdots v_i)$ such that for all $0\leq j<i$, $(v_j,v_{j+1})\in V$. Note that a single vertex is also considered as a path.
%A \textit{strongly connected component} (SCC) in a graph $G=(V,E)$, is a maximal subset $V_0\subseteq V$ such that for every vertices $v,v' \in V_0$, there exists a path from $v$ to $v'$ in $G$. Note that the set of all SCCs forms a partition of the graph-vertices.
%An SCC, $S$ is a \emph{terminal SCC} if for every $s\in S$ the next holds: if a state $t$ is reachable from $s$, then $t\in S$.

%We exploit the special structure of the weak B\"uchi automaton to solve this game more efficiently than a typical Parity game or B\"uchi game. 

\begin{comment}

Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
Then, these SCCs hold a special property in a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$. Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all their states are contained in $\F$ or  {\em non-accepting components} mean none of their states is present in $\F$. 
Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a path is winning for the system if the path ultimately never exist an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every path will ultimately remain inside an accepting component.

% \subsection{Explicit State Representation}
% \label{sec:explicitweakbuchi}


Weak B\"uchi games have previously been studied when the states of the game are represented explicitly. Under this state representation, weak B\"uchi games can be solved in linear-time to the size of the explicit graph underlying the game~\cite{krish'spaper}. This section reviews that algorithm. 
\end{comment}

\subsubsection{Symbolically identifying the accepting SCCs}
\label{sec:accepting-SCCs}

Since our algorithms are symbolic, we now turn to give a symbolic definitions of the weak \Buchi game and its components. While most of the symbolic representations are standard in common in the literature, we nevertheless describe below how to symbolically identify the accepting SCC. That is,  to provide a linear-time construction of a BDD that recognizes all accepting states.

% \begin{definition}
% Let $(\mathit{GS},\varphi)$ be a GR($k$) that separates variables, over the input/output variables, $\I$ and $\O$. Write $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
% \bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j}))$. 
% Take a state $s\in 2^{\I\cup\O}$, and let $S$ be its SCC. Then, $s$ is accepting if for every $l\in\{1,\dots,k\}$ one of the following hold:
% \begin{description}
% \item[All guarantees hold in $S$.] For every $j\in\{1,\dots,m_l\}$, there exists $(\inp,\out)\in S$ such that $\out\models g_{l,j}$.

% \item[Some assumption cannot hold in $S$.] There exists $i\in\{1,\dots,n_l\}$ such that for all $(\inp,\out)\in S$, $\inp\not\models a_{l,i}$. 
% \end{description}
% \end{definition}

We first define every state in an accepting SCC as an \textit{accepting state}.
We next turn to show that all accepting states can be identified efficiently.

\begin{lemma}Let $(\mathit{GS},\varphi)$ be a GR($k$)-game that separates variables, over the input/output variables, $\I$ and $\O$. Write $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})
)$.
Then, a BDD $\beta_\mathit{acc}$ over $\I,\O$ such that $\beta_\mathit{acc}(\inp,\out)$ if $(\inp,\out)$ is accepting, can be constructed in $O(|\varphi|+N)$ symbolic operations.
\end{lemma}
\begin{proof}
Consider the BDD $\beta_\mathit{SCC}$, constructed in $O(N)$ operations (see Lemma~\ref{lem:beta_SCC}). Take a component $\varphi_l= 
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$. First, we identify all states that their SCC includes a $g_{j,l}$-state. For $j\in\{1,\dots,m_l\}$, let $\beta_{g_{l,j}}$ be a BDD over $\I,\O,\I',\O'$ such that $\beta_{g_{l,j}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $\out_1\models g_{l,j}$. Hence, the BDD $\gamma_{l,j}$ over $\I,\O$, defined by $\exists \I',\O'(\beta_\mathit{SCC} \wedge \beta_{g_{l,j}})$, accepts a state $(\inp,\out)$ if its SCC includes a state $s\models g_{l,j}$.

Now, we focus on the assumptions. In similar to the former case, for $i\in\{1,\dots,n_i\}$, let $\beta_{a_{l,j}}$ be a BDD over $\I,\O,\I',\O'$ such that $\beta_{a_{l,j}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $\inp_1\models a_{l,i}$. Hence, the BDD $\alpha_{l,i}$ over $\I,\O$, defined by $\forall \I',\O'(\beta_\mathit{SCC}\rightarrow \neg\beta_{a_{l,i}})$,
accepts a state $(\inp,\out)$ if its SCC does not includes a state $s$ such that $s\models a_{l,j}$.

Therefore, the BDD $\beta_\mathit{acc}$ is constructed by $\bigwedge_{l=1}^k(  (\bigwedge_{j=1}^{m_l}\gamma_{l,j}) \vee (\bigvee_{i=1}^{n_l} \alpha_{l,i}))$. The construction is performed by $O(|\varphi|+N)$ operations. \qed
\end{proof}




% \subsection{Name Name Name}

% We can now state the main theorem of the section that essentially describes the reduction statement. \dftodo{change my writing, this is awful}

% \begin{theorem}\label{thm:reduction}
% .....
% \end{theorem}



% In this section we prove Theorem \ref{thm:reduction}. This proof also yields an algorithm for computing a winning strategy for separated $GR(k)$ games from a 
% winning strategy on weak \Buchi games. 

\subsection{The Delay Property}

At the heart of our strategy lies the delay property that makes sure that combining the weak \Buchi game strategy $f_B$ and the SCC travel strategy $f_{travel}$ can maintain winning regions for the system.

% \begin{theorem}\label{thm:delay}[The Delay Property Theorem]
% Consider the weak B\"uchi game constructed in Section~\ref{sec:accepting-SCCs}. Let $\inp_0,\dots,\inp_n\in (2^\I)^+$ be a sequence such that for all $i\in\{0,\dots,n\}$, $(\inp_i,\inp_{i+1})\models \rho_\I$. Moreover, let $\out_{-m},\dots,\out_0\in (2^\O)^+$ be a sequence such that for all $i\in\{-m,\dots,-1\}$, $(\out_i,\out_{i+1})\models \rho_\O$.
% If the system can win from $(\inp_0,\out_0)$, then it can also win from $(\inp_n,\out_{-m})$.
% \end{theorem}

\begin{theorem}\label{thm:delay}[The Delay Property Theorem]
Consider the weak B\"uchi game constructed in Section~\ref{sec:accepting-SCCs}. Let $\inp_0,\dots,\inp_n\in (2^\I)^+$ be a path in $G_\I$, and for $m\geq 0$, let $\out_{-m},\dots,\out_0\in (2^\O)^+$ a path in $G_\O$. Assume that the system can win from $(\inp_0,\out_0)$. Then the system can also win from $(\inp_n,\out_{-m})$.
\end{theorem}

The Delay Property Theorem essentially says that while in an SCC $S$ that is a winning region, the system can remain in an $S$ or the environment can leave an $S$, and the system still stays in the winning zone.  We remark that this property is unique to the game we are dealing with. It does not hold for every  weak \Buchi game.

A corollary of Theorem~\ref{thm:delay} is the following statement about the structure of the winning region of the winning weak \Buchi game strategy $f_B$.

\begin{corollary}\label{cor:delay}
The winning region of $f_B$ is a union of SCCs in the weak \Buchi game graph.
\end{corollary}


We next prove Theorem~\ref{thm:delay}. For that we start by proving the following lemma.

\begin{lemma}\label{lem:1delay}
Consider the weak B\"uchi game constructed in Section~\ref{sec:accepting-SCCs}. Let $\inp_0,\inp_1\in (2^\I)^+$ such that  $(\inp_0,\inp_1)\models \rho_\I$, and assume that the system can win from $(\inp_0,\out_0)$. Then the system can also win from $(\inp_1,\out_0)$.
\end{lemma}

\begin{proof}
Let $f^s$ be a winning strategy for the system from $(\inp_0,\out_0)$. 
We construct a winning strategy $f^s_d$ from $(\inp_1,\out_0)$. Intuitively, $f^s_d$ acts like $f^s$ with a delay of a single step: it ignores the final input, and shifts the sequence of outputs one step backwards \dftodo{clarify}.
Since a strategy is deterministic, to ease the notation we denote a strategy $f((\inp_1,\out_0),\dots,(\inp_m,\out_{m-1}))$ as $f(\inp_1,\dots,\inp_m)$.



% Recall that the strategy $f^s$ is played as follows. In a state $(i,j)$ the environment makes an action $i'$, and the strategy makes an action $o'$ for which $o'=f^s((i_0,O_0),\cdots (i,o))$ is a result of applying the strategy on previous states so far. Thus the next state reached is $(i',o')$ \dftodo{clarify, but remove or move to prelims}.

We use $f^s$ to define $f^s_d$ inductively over play-prefixes of length $m\geq 1$ and set $f^s_d(\inp_1,\dots,\inp_{m+1})=f^s(\inp_0,\dots,\inp_m)$. 
Note that $f^s_d$ is well defined since the games are separated, then for $(i,i')\models \rho_\I$ we have that for every $o$, the actions that the system can do from state $(i,o)$ and from state  $(i',o)$ are the same \dftodo{clarify}. 
Note that by this definition, for every play $((\inp_1,\out_0),(\inp_2,\out_1),\cdots (\inp_{m+1},\out_m),\cdots)$ in $f^s_d$, there is a play $((\inp_0,\out_0),(\inp_1,\out_1),\cdots (\inp_m,\out_m),\cdots)$ in $f^s$.

While $f^s$ is memory-less, note that $f^s_d$ is not memory-less. We do define however $f^s_d$ for the proof only. In Section \ref{} we show how to construct a memory-less strategy that replaces $f^s_d$ \dftodo{clean}.

Next, we show that $f^s_d$ is winning if $f^s$.
Define a \textit{standard SCC} as an SCC that is result of a product of input-SCC and output-SCC (in our setting, an SCC can have a singleton in the input or output, thus it is not always like this.\dftodo{Is this so? anyhow clean and move definition to prelims}).

Now, assume that $f^s$ is winning, and let $((\inp_1,\out_0),(\inp_2,\out_1),\cdots (\inp_{m+1},\out_m),\cdots)$ be a play in $f^s_d$. Then there is 
$((\inp_0,\out_0),(\inp_1,\out_1),\cdots (\inp_m,\out_m),\cdots)$ is a play in $f^s$ that ends in an accepting SCC $S$ since $f^s$ is winning. Specifically there is an input SCC $S_I$ and output SCC $S_O$ such that $S=S_I\times S_O$ and such that $(\inp_0, \inp_1, \inp_2,\cdots)$ ends up in $S_I$, and $(\out_0, \out_1,\out_2,\cdots)$ ends in $S_O$. Therefore $(\inp_1, \inp_2,\cdots)$ also ends up in $S_I$, and as a result, the play $((\inp_1,\out_0),(\inp_2,\out_1),\cdots (\inp_{m+1},\out_m),\cdots)$ also ends up in the winning SCC $S$ as required. \qed
\end{proof}


Theorem \ref{thm:delay} now follows by straightforward induction from Lemma \ref{lem:1delay}. To show that the system can win from $(\inp_n,\out_{-m})$ for every $m\geq 0$,  it is sufficient to show that the system can win from $(\inp_0,\out_{-1})$. The system applies the following strategy: first, for any legal input $\inp$ the system responds with $\out_0$. Then, by the previous lemma, the system has a winning strategy from $(\inp,\out_0)$. \dftodo{Do we need to elaborate? Perhaps write it a bit more precise.}







\subsection{Synthesizing a Winning Strategy}\label{sec:syntstrat}

We now present a solution to the realizability and synthesis problem for separated GR($k$) games. For that, we first construct two strategies, each is constructed by $O(N)$ \dftodo{clarify $O(N)$ steps} symbolic operations:
\begin{description}
\item[$f^s_{wb}$.] A memory-less strategy that wins the weak-B\"uchi game  $((\I,\O,\theta_\I,\theta_\O,\rho_{\I},\rho_{\O}),GF(\beta_{\mathit{acc}}))$. We show how to construct $f^s_{wb}$ in Section \ref{}. Note that this is \textit{not} the strategy constructed in the delay-property lemma.

\item[$f^s_{\mathit{travel}}$.] a memory-less strategy for the system that reaches every state in a given SCC infinitely often. \dftodo{perhaps be more precise}
\gatodo{I wonder how to construct such a strategy, symbolically, in $O(N)$ steps.}


% That is, $f^s_\mathit{travel}$ satisfies the next property. Let $S$ be an SCC, and consider the subgame induced by $S$. Then, for every $(\inp,\out)\in S$, when the system applies $f^s_\mathit{travel}$, the play will traverse infinitely often states of the form $(\widehat{\inp},\out)$. 
\end{description}


Now, let $f^s_{wb}$ and $f^s_{\mathit{travel}}$ be the strategies defined above. Then  strategy $f$ for separated GR($k$) games is defined as follows.
Given a state $s$ and an environment action $i$: if $s$ is in an accepting SCC, return $f^s_{\mathit{travel}}(s,i)$; else return $f^s_{wb}(s,i)$.

\begin{lemma}\label{lem:win}
$f$ is winning for our separated GR($k$) game if and only if $f^s_{wb}$ is winning for the weak \Buchi game that we described \dftodo{clean!!!}.
\end{lemma}

\begin{proof}
Assume that the initial state $(i_0,o_0)$ is in the winning region of $f^s_{wb}$. Then we show that playing $f$ always keeps the system in the winning region of $f^s_{wb}$. Then we have that playing $f$ always keeps reaching accepting SCC and then travesring all of them meets the GR($k$) conditions.\dftodo{put in a separate lemma}

To see that, we use the delay property corollary (about the winning region). Therefore as long $f^s_{wb}$ is switched to $f^s_{\mathit{travel}}$ and $f^s_{\mathit{travel}}$ is being played, the system remains in the winning region.

Now assume that the strategy switched to $f^s_{wb}$ from $f^s_{\mathit{travel}}$. Then we have a state $s$ in an accepting $SCC$, i.e. in the winning region of $f^s_{wb}$, and we need to see that $f^s_{wb}(s,i)$ is in the winning region of $f^s_{wb}$ as well \dftodo{why isn't it obvious???}. For that we use the delay property lemma \dftodo{I don't think we need to use it again} to show that we are still in the winning region \dftodo{clean!!!}.

For the other side, note that if $(i_0,o_0)$ is not in the winning region of $f^s_{wb}$, then an accepting SCC cannot be reached by the system. Thus, every SCC that is reached does not meet the GR($k$) conditions. 





\qed
\end{proof}

Lemma~\ref{lem:win} shows how synthesis can be done by using synthesis for weak \Buchi games. 
For realizability, we can now get the following theorem that is immediate from Lemma~\ref{lem:win}.

\begin{theorem}\label{thm:realiizability}
Realizability for separated GR($k$) games can be reduced to realizability of weak \Buchi games in $O(N)$ (to the size of the input etc.)
\end{theorem}

\begin{proof}
Given separated GR($k$) games $G$, construct the weak \Buchi game $G'$ by constructing the SCCs (symbolically?) in $O(N)$ steps.
Then check realizability for $G'$. By Lemma~\ref{lem:win}, we have that $G$ is realizable iff the initial state $(i_0,o_0)$ is in the winning region of a strategy for $G'$, i.e. iff $G'$ is realizable.
\end{proof}


In Section~\ref{sec:algorithmsWeakBuchi} we show in detail how to do symbolic synthesis for weak \Buchi games.

% \subsection{Synthesizing a Winning Strategy}\label{sec:syntstrat}

% We are ready to present a solution to the realizability and synthesis problem. We construct two strategies, each is constructed by $O(N)$ symbolic operations:
% \begin{description}
% \item[$f^s_{wb}$.] A memory-less strategy that wins the weak-B\"uchi game  $((\I,\O,\theta_\I,\theta_\O,\rho_{\I},\rho_{\O}),GF(\beta_{\mathit{acc}}))$.

% \item[$f^s_{\mathit{travel}}$.] a memory-less strategy for the system to reach all possible inputs in a given SCC. That is, $f^s_\mathit{travel}$ satisfies the next property. Let $S$ be an SCC, and consider the subgame induced by $S$. Then, for every $(\inp,\out)\in S$, when the system applies $f^s_\mathit{travel}$, the play will traverse infinitely often states of the form $(\widehat{\inp},\out)$. \gatodo{I wonder how to construct such a strategy, symbolically, in $O(N)$ steps.}
% \end{description}

% Let $W$ be a winning region of $f^s_{wb}$. In Algorithm~\ref{algo:winning-strategy}, we present a strategy that wins for the system from $W$.




% \begin{algorithm}[t]
% 	\caption{A winning strategy}
% 	\label{algo:winning-strategy}
% 	\begin{algorithmic}[1]
		
% 		\Statex{\begin{center}
% 				/*\quad\quad  From state $s$ and input $\inp$ \quad\quad*/
% 		\end{center}}
	
% 	    \State construct $\beta_\mathit{SCC}$ \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
	
% 	    \State $\gamma = \exists\O'(\beta)$ 
	    
% 		\State if $\beta_\mathit{acc}(s)$ and $\gamma(s,\inp')$ \Return $f^s_\mathit{travel}(s,\inp)$
		
% 		\State \Return $f^s_\mathit{wb}(s,\inp)$
% 	\end{algorithmic}
% \end{algorithm}

% We can now prove Theorem~\ref{thm:win}.
% \begin{proof}
% We show that $W$ is the system's winning region, and further that Algorithm~\ref{algo:winning-strategy} correctly constructs a strategy that wins from $W$.

% First, we prove that Algorithm 2 construct a strategy that wins from $W$. ...

% \end{proof}


==> Symbolic_old_semi.tex <==
\section{Reduction of Separated GR($k$) to Weak B\"uchi Games}\label{sec:reduction}

We turn to solve our main problem. The solution relies on a reduction to weak B\"uchi games. 
The idea is to mark an SCC, $S$ as accepting, if the system can win the GR($k$)-game in the subgame $S$. This holds if for every component of the GR($k$) formula,
$\varphi_l=\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$, either (1) the environment cannot satisfy one of $\varphi_l$'s  assumptions in the subgame $S$, or (2) the system can satisfy all $\varphi_l$' guarantees in the subgame $S$.

We argue that the system can win w.r.t. the GR($k$) objective iff it can win the weak B\"uchi game, described above. This solves the \textbf{realizability} problem. Moreover, the following strategy is winning for the system: we apply the `weak B\"uchi' strategy until reaching an accepting SCC, $S$ in which we merely play a strategy to reach all possible outputs in $S$. If the environment leads the game out of $S$, we switch back to the weak B\"uchi strategy. We repeat this process until the play eventually stabilizes in an accepting SCC, in which we win w.r.t. the GR($k$) condition. This solves the \textbf{synthesis} problem. 

Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
Then, these SCCs hold a special property in a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$. Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all their states are contained in $\F$ or  {\em non-accepting components} mean none of their states is present in $\F$. 
Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a path is winning for the system if the path ultimately never exist an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every path will ultimately remain inside an accepting component.

% \subsection{Explicit State Representation}
% \label{sec:explicitweakbuchi}


Weak B\"uchi games have previously been studied when the states of the game are represented explicitly. Under this state representation, weak B\"uchi games can be solved in linear-time to the size of the explicit graph underlying the game~\cite{krish'spaper}. This section reviews that algorithm. 



\subsubsection{Weak B\"uchi games representation.} 

Recall from Section~\ref{Sec:Prelims}, a game with game structure $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and a winning condition can be equivalently represented by a game between the system and environment player on  directed graph $ (V,E)$. The states on the graph are given by states over $\I\cup\O$ and there is a directed edge from state $s$ to state $t$ in the graph if $(s,t')\models \rho_\I\wedge\rho_\O$. Recall, we assume that all states of a game structures are deadlock-free. Thus, there is at least one outgoing edge from every state in directed graph $(V,E)$.
States which $\theta_\I\wedge\theta_\O$ are the initial states of the graph. 
% The game proceeds by the environment player assigning values to the input variables $\I$ and the system player assigning values to the output variables $\O$.  
% The game starts at one of the initial states of the graph. 
% In every round of the game, first the  environment chooses an assignment to the $\I$ variables, and then the system will choose an assignment $O$ to the $\O$ variables.
% The combined assignment $I \cup O$ determines the unique state  the game moves to.
% The notions of plays, strategies, winning conditions and so on naturally transfer to the explicit-state representation. 





%For readability, we also consider an explicit representation of the game between the environment and the system. Given a game structure  $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$, we define a graph that serves as a ``game-board" as follows. $G^{\mathit{GS}}=(V^\mathit{GS},E^\mathit{GS})$, where $V^\mathit{GS}=2^{\I\cup\O}$, and $(\inp_0,\out_0)E(\inp_1,\out_1)$ if $\big((\inp_0,\out_0),(\inp_1',\out_1')\big)\models \rho_\I\wedge \rho_\O$.
%At the beginning of a play, the environment chooses $\inp\in 2^\I$, the system then responds with $\out\in 2^\O$, and thus the first state of the play is $(\inp,\out)\in V^{\mathit{GS}}$. Afterwards, the payers repeatedly choose the next state of the play: form state $(\inp_0,\out_0)$ the environment chooses $\inp_1\in 2^\I$ such that $(\inp_0,\out_0,\inp_1')\models \rho^e$, the system replies with $\out_1$ such that $(\inp_0,\out_0,\inp_1',\out_1')\models \rho_\O$, and the play traverses to state $(\inp_1,\out_1)$.  Note that the notions of plays, strategies etc. naturally transfer to the explicit representation. We omit the straightforward adaptation of those notions in the explicit context. 

% A {\em strongly connected component} (SCC) of a directed graph $(V,E)$ is a maximal set of states within which every state is reachable from every other state.  It is well known that SCCs partition the states of a directed graph.

% Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
% Then, these SCCs hold a special property in a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$. Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
% Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all their states are contained in $\F$ or  {\em non-accepting components} mean none of their states is present in $\F$. 
% Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a path is winning for the system if the path ultimately never exist an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every path will ultimately remain inside an accepting component.

%A \textit{subgraph} $G_0$ of a directed graph $G=(V,E)$ is a graph $(V_0,E_0)$ where $V_0\subseteq V$ and $E_0= E\cap (V_0\times V_0)$. 
%\textit{A path} in a graph $G=(V,E)$ is a sequence $(v_0,\cdots v_i)$ such that for all $0\leq j<i$, $(v_j,v_{j+1})\in V$. Note that a single vertex is also considered as a path.
%A \textit{strongly connected component} (SCC) in a graph $G=(V,E)$, is a maximal subset $V_0\subseteq V$ such that for every vertices $v,v' \in V_0$, there exists a path from $v$ to $v'$ in $G$. Note that the set of all SCCs forms a partition of the graph-vertices.
%An SCC, $S$ is a \emph{terminal SCC} if for every $s\in S$ the next holds: if a state $t$ is reachable from $s$, then $t\in S$.

%We exploit the special structure of the weak B\"uchi automaton to solve this game more efficiently than a typical Parity game or B\"uchi game. 




% \subsection{Identifying the accepting SCCs}
% \label{sec:accepting-SCCs}

Our first goal is to identify the accepting SCCs, efficiently. That is, to provide a linear-time construction of a BDD that recognizes all accepting states.

\begin{definition}
Let $(\mathit{GS},\varphi)$ be a GR($k$) that separates variables, over the input/output variables, $\I$ and $\O$. Write $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j}))$. 
Take a state $s\in 2^{\I\cup\O}$, and let $S$ be its SCC. Then, $s$ is accepting if for every $l\in\{1,\dots,k\}$ one of the following hold:
\begin{description}
\item[All guarantees hold in $S$.] For every $j\in\{1,\dots,m_l\}$, there exists $(\inp,\out)\in S$ such that $\out\models g_{l,j}$.

\item[Some assumption cannot hold in $S$.] There exists $i\in\{1,\dots,n_l\}$ such that for all $(\inp,\out)\in S$, $\inp\not\models a_{l,i}$. 
\end{description}
\end{definition}

We turn to show that all accepting states can be identified efficiently.

\begin{lemma}Let $(\mathit{GS},\varphi)$ be a GR($k$)-game that separates variables, over the input/output variables, $\I$ and $\O$. Write $\varphi=\bigwedge_{l=1}^k \varphi_l$, where  $\varphi_l  =
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})
)$.
Then, a BDD $\beta_\mathit{acc}$ over $\I,\O$ such that $\beta_\mathit{acc}(\inp,\out)$ if $(\inp,\out)$ is accepting, can be constructed in $O(|\varphi|+N)$ symbolic operations.
\end{lemma}
\begin{proof}
Consider the BDD $\beta_\mathit{SCC}$, constructed in $O(N)$ operations (see Lemma~\ref{lem:beta_SCC}). Take a component $\varphi_l= 
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$. First, we identify all states that their SCC includes a $g_{j,l}$-state. For $j\in\{1,\dots,m_l\}$, let $\beta_{g_{l,j}}$ be a BDD over $\I,\O,\I',\O'$ such that $\beta_{g_{l,j}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $\out_1\models g_{l,j}$. Hence, the BDD $\gamma_{l,j}$ over $\I,\O$, defined by $\exists \I',\O'(\beta_\mathit{SCC} \wedge \beta_{g_{l,j}})$, accepts a state $(\inp,\out)$ if its SCC includes a state $s\models g_{l,j}$.

Now, we focus on the assumptions. In similar to the former case, for $i\in\{1,\dots,n_i\}$, let $\beta_{a_{l,j}}$ be a BDD over $\I,\O,\I',\O'$ such that $\beta_{a_{l,j}}(\inp_0,\out_0,\inp_1',\out_1')$ iff $\inp_1\models a_{l,i}$. Hence, the BDD $\alpha_{l,i}$ over $\I,\O$, defined by $\forall \I',\O'(\beta_\mathit{SCC}\rightarrow \neg\beta_{a_{l,i}})$,
accepts a state $(\inp,\out)$ if its SCC does not includes a state $s$ such that $s\models a_{l,j}$.

Therefore, the BDD $\beta_\mathit{acc}$ is constructed by $\bigwedge_{l=1}^k(  (\bigwedge_{j=1}^{m_l}\gamma_{l,j}) \vee (\bigvee_{i=1}^{n_l} \alpha_{l,i})$. The construction is performed by $O(|\varphi|+N)$ operations. \qed
\end{proof}






\subsection{The Delay Property}

Recall that we aim to alternate between two strategies. One that wins w.r.t. the B\"uchi objective, and one that satisfies the GR($k$) objective within an accepting SCC. This technique works since our weak B\"uchi game satisfies the ``\emph{delay property}"; it is safe for the system to halt the B\"uchi strategy for a while, and allow the environment to take several steps instead of a single step. We remark that this property is unique to the game we are dealing with. It does not hold for every  weak B\"uchi game.
 
 %For illustration, assume that the system follows a winning strategy, and the play reaches a state $(\inp_0,\out_0)$. Now, the environment chooses an input $\inp_1$ such that $(\inp_0,\inp_1')\models \rho_\I$. Assume that, for some reason, the system was not fast enough and failed to reply. As a result, the play's state is now $(\inp_1,\out_0)$. We claim that the system can still win w.r.t. the B\"uchi objective. Moreover, this statement remains correct even if the system will fail to reply to several ensuing steps by the environment, and thus the play will reach a state  $(\inp_n,\out_0)$. We remark that this delay property is unique to weak B\"uchi games that separate variables, and do not hold in general.

\begin{lemma}[the delay property]
\label{lem:delay} Consider the weak B\"uchi game constructed in Section~\ref{sec:accepting-SCCs}. Consider a sequence $\inp_0,\dots,\inp_n\in (2^\I)^+$ such that for all $i<n$, $(\inp_i,\inp_{i+1})\models \rho_\I$. If the system can win from $(\inp_0,\out_0)$, then it can also win from $(\inp_n,\out_0)$.
\end{lemma}

\begin{proof} It suffices to show that the system can win from $(\inp_1,\out_0)$. Let $f^s$ be a winning strategy for the system from $(\inp_0,\out_0)$. 
We construct a winning strategy $f^s_d$ from $(\inp_1,\out_0)$. Intuitively, $f^s_d$ acts like $f^s$ with a delay of a single step: it ignores the final input, and shifts the sequence of outputs one step backwards.

We inductively define $f^s_d$ over play-prefixes of length $m$, such that the following hold: if $(\inp_1,\out_0),\dots,(\inp_m,\out_{m-1})$ is consistent with $f^s_d$, then $(\inp_0,\out_0),\dots,(\inp_{m-1},\out_{m-1})$ is consistent with $f^s$.
Assume that $f^s_d$ has been defined over sequences of length smaller than $m$ such that the induction hypothesis hold. 
Let $(\inp_1,\out_0),\dots,(\inp_m,\out_{m-1})$ be a sequence of states from $(\inp_1,\out_0)$, consistent with $f^s_d$, and take $\inp_{m+1}\in 2^\I$ such that $(\inp_m,\inp_{m+1}')\models \rho_\I$. By the induction hypothesis, $(\inp_0,\out_0),\dots,(\inp_{m-1},\out_{m-1})$ is consistent with $f^s$. As $(\inp_{m-1},\inp_m')\models \rho_\I$, $\inp_m$ is a legal input from $(\inp_{m-1},\out_{m-1})$. Hence, $f^s((\inp_0,\out_0),\dots,(\inp_{m-1}',\out_{m-1}),\inp_{m})$ is defined. Write $f^s((\inp_0,\out_0),\dots,(\inp_{m-1}',\out_{m-1}),\inp_{m})=\out_m$, and set $f^s_d((\inp_1,\out_0),\dots,(\inp_m,\out_{m-1}),\inp_{m+1})=\out_{m}$. Since $f^s$ is a strategy, $(\out_{m-1},\out_m)\models\rho_\O$ thus the definition is valid, and it is not difficult to see that the induction hypothesis hold.

We turn to show that $f^s_d$ wins the weak B\"uchi game, and we start with the formulation of the next observation. The observation immediately follows from the fact that $\mathit{GS}$ separates variables. 

\begin{observation}
\label{obs:shift}
Let $(\inp_0,\out_0),\dots,(\inp_n,\out_n)$ be a sequence of states such that for every $i<n$, $(\inp_i,\out_i,\inp_{i+1}',\out_{i+1}')\models \rho_\I\wedge\rho_\O$. Then, the sequences $(\inp_1,\out_0),\dots,(\inp_n,\out_{n-1})$ and $(\inp_0,\out_1),\dots,(\inp_{n-1},\out_n)$ are also consistent with $\rho_\I$ and $\rho_\O$: for every $i<n-1$, $(\inp_{i+1},\out_i,\inp_{i+2}',\out_{i+1}')\models \rho_\I\wedge \rho_\O$ and $(\inp_i,\out_{i+1},\inp_{i+1}',\out_{i+2}')\models \rho_\I\wedge \rho_\O$.
\end{observation}

Take a play $(\inp_1,\out_0),(\inp_2,\out_1),\dots $, consistent with $f^s_d$. We shall prove that it stabilizes in an accepting SCC. By the construction, $(\inp_0,\out_0),(\inp_1,\out_1),\dots$ is consistent with $f^s$ and thus stabilizes in an accepting SCC, $S$, say from state $(\inp_i,\out_i)$. We start by proving that our play stabilizes in an SCC, $S_d$, form state $(\inp_{i+1},out_i)$. Indeed, by Observation~\ref{obs:shift}, the existence of a path form $(\inp_j,\out_j)$ to $(\inp_i,\out_i)$, for $j>i$, implies the existence of a path from $(\inp_{j+1},\out_j)$ to $(\inp_{i+1},\out_i)$.

Now, we claim that $S_d$ is an accepting SCC. To prove this claim, take a component $\varphi_l  =
\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$.  
First, assume that for every guarantee $GF(g_{l,j})$, $S$ includes a state $s$ such that $s\models g_{l,j}$.  Hence, there exists a path in $S$ from $(\inp_i,\out_i)$ to a state $(\inp,\out)$ such that $\out\models g_{l_j}$. Use Observation~\ref{obs:shift} to conclude that the same holds for $S_d$: there exists a path in $S_d$ from $(\inp_{i+1},\out_i)$ to a state $(\widehat\inp,\out)$, and $\out\models g_{l,j}$. 

Second, assume that for some assumption $a_{l,j}$, $S$ does not include a state $s\models a_{l,j}$. Assume, towards a contradiction, that there exists $s_d=(\inp^d,\out^d)\in S_d$ such that $\out_d \models a_{l,j}$. Hence, there exists a path in $S_d$ from $(\inp_{i+1},\out_i)$ to $(\inp^d,\out^d)$. Use Observation~\ref{obs:shift} to conclude that $S$ includes an $a_{l,j}$-state as well, in contradiction to the assumption.
Consequently, $S_d$ is an accepting SCC and thus $f^s_d$ wins w.r.t. the B\"uchi objective, as required.\gatodo{to read again...}\qed
\end{proof}

The delay property implies the next consequence. It is not only the case that the system can halt for a while, it can also move backward.

\begin{lemma}[forward-backward delay]
Consider the weak B\"uchi game constructed in Section~\ref{sec:accepting-SCCs}. Let $\inp_0,\dots,\inp_n\in (2^\I)^+$ be a sequence such that for all $i\in\{0,\dots,n\}$, $(\inp_i,\inp_{i+1})\models \rho_\I$. Moreover, let $\out_{-m},\dots,\out_0\in (2^\O)^+$ be a sequence such that for all $i\in\{-m,\dots,-1\}$, $(\out_i,\out_{i+1})\models \rho_\O$.
If the system can win from $(\inp_0,\out_0)$, then it can also win from $(\inp_n,\out_{-m})$.
\end{lemma}
\begin{proof}
By the previous lemma, using a standard inductive argument, it sufficient to show that the system can win from $(\inp_0,\out_{-1})$. The system applies the following strategy: first, for any legal input $\inp$ the system responds with $\out_0$. Then, by the previous lemma, the system has a winning strategy from $(\inp,\out_0)$.\qed 
\end{proof}























%Second, we employ the identified good SCCs to solve the realizability and synthesis problem ({\color{red} add cross-ref}). Let $X$ be the union of all good SCCs, $W$ be system $B$'s wining region w.r.t. $FG(X)$ (i.e. w.r.t. the connected partition problem over $G,X$), and $g^B$ a matching (memory-less) strategy. \textbf{Realizability}: $W$ is system $B$'s wining region. \textbf{Synthesis}: the following strategy $f^B$ wins for system $B$ from $W$. From state $(i_0,o_0)$ and input $i_1$, if $(i_1,o_0)$ belongs to a good SCC, $C$, go to a state in $C$, striving to eventually reach all states in $C$. Otherwise, return $g^B((i_0,o_0),i_1)$. Note that we are using the delay-property. As long we stay in the same connected component, $g^B$ can be applied.

%\subsection{Identifying the Good Components}

%We turn to describe the first stage of the construction outlined above; identifying all good SCCs.

%\begin{lemma}
%There exists a BDD $\beta_{\mathit{SCC}}$ over $\I,\O,\I',\O'$ s.t. $\beta_{\mathit{SCC}}(i_0,o_0,i_1,o_1)$ iff $(i_0,o_0)$ and $(i_1,o_1)$ belong to the same SCC. Moreover, $\beta_{\mathit{SCC}}$ can be computed in $O(N)$ symbolic operations. 
%\end{lemma}

%\begin{proof}
%We construct a BDD $\beta_{\mathit{Reach}}$ s.t. $\beta_{\mathit{Reach}}(i_0,o_0,i_1,o_1)$ if there exists a path from $(i_0,o_0)$ to $(i_1,o_1)$ in $G$. We repeatedly construct BDDS $\beta^0,\beta^1,\dots$ over $\I,\O,\I',\O'$ s.t. $\beta^i(i_0,o_0,i_1,o_1)$ if  there exists a path of length at most $i$ from $(i_0,o_0)$ to $(i_1,o_1)$. This process ends when $\beta^i = \beta^{i+1}$, and then we have $\beta_{\mathit{Reach}}=\beta^i$. We have,

%\begin{equation*}
%    \beta^0(i_0,o_0,i_1',o_1')\Longleftrightarrow (i_0=i_1)\wedge (o_0=o_1)
%\end{equation*}
%\begin{equation*}
%    \beta^{i+1}(i_0,o_0,i_1,o_1) \Longleftrightarrow \exists i_2,o_2\in \I\times\O\big( \beta^i(i_0,o_0,i_2',o_2') \wedge (i_2,o_2,i_1',o_1')\models (\rho_I\wedge\rho_O)\big)
%\end{equation*}

%Hence, $\beta_{\mathit{Reach}}$ is computed in $O(N)$ symbolic operations. Likewise, we compute in $O(N)$ symbolic operations a BDD $\beta_{\mathit{Reach}^{-1}}$ over $\I,\O,I',\O'$, defined by: $\beta_{\mathit{Reach}^{-1}}(i_0,o_0,i_1,o_1)$ if there exists a path in $G$ from $(i_1,o_1)$ to $(i_0,o_0)$. Clearly, $\beta_{\mathit{SCC}} = \beta_{\mathit{Reach}} \wedge \beta_{\mathit{Reach}^{-1}}$.\qed
%\end{proof}

%As explained, we mark an SCC, $C$, as ``good" if it induces a subgame in which the system has a winning strategy w.r.t. the given GR($k$) winning condition.

%\begin{definition}
%An SCC, $C$ is a corridor, if it is a singleton $C=\{i,o\}$, and it has no self-loop.
%\end{definition}

%\begin{definition}
%\label{def:good_SCC}
%An SCC, C is good w.r.t. a GR($k$) formula $\varphi = \bigwedge_{l=1}^k (  \bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j}))$ if for every component $ \bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$ one of the following hold
%\begin{itemize}
%    \item $\exists i\in\{1,\dots,n_l\}\forall (i,o)\in C((i,o)\not\models a_{l,i})$, or
    
%    \item $\forall j\in\{1,\dots,m_l\}\exists (i,o)\in C((i,o)\models g_{j,l})$.
%\end{itemize}
%\end{definition}

%\begin{remark}
%Note that Definition~\ref{def:good_SCC} also marks some singleton SCCs with no self-loops as ``good". This is not problematic since we construct a winning strategy for system $B$ w.r.t. $FG(\text{good SCC})$. As a play may only traverse no-self-loop-singleton SCCs, marking such SCCs as good is immaterial.
%\end{remark}

%We are ready to show that good SCCs can be computed efficiently. 

%\begin{lemma}
%There exists a BDD $\beta_{\mathit{good}}$ over $\I\cup\O$, computed in $O(N)$ symbolic operations, such that $\beta_{\mathit{good}}(i,o)$ iff the SCC of $(i,o)$ is good.
%\end{lemma}

%\begin{proof}
%Let $\varphi_l=\bigwedge_{i=1}^{n_l} GF(a_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} GF(g_{l,j})$ be the $l$-th component of $\varphi$. First, we focus on $\varphi_l$'s antecedents. We construct a BDD $\beta_l$ over $\I,\O$ by the formula $\vee_{i=1}^{n_l}(\forall i_1,o_1 (\beta_{\mathit{SCC}}(i_0,o_0,i_1,o_1) \rightarrow (i_1,o_1)\models \neg a_{i,l})))$. That is, $\beta$ accepts a state $(i,o)$ if its SCC does not include an $a_{l,i}$-state for some $i$. 

%Second, we turn to deal with $\varphi_l$'s consequences.  We construct a BDD $\gamma_l$ over $\I,\O$ by the formula $\wedge_{j=1}^{m_l}\exists i_1,o_1(\beta_{\mathit{SCC}}(i_0,o_0,i_1,o_1) \wedge (i_1,o_1)\models g_{j,l})$. That is, $\gamma_l$ accepts $(i,o)$ if for every $j\in\{1,\dots,m_l\}$, $(i,o)$'s SCC includes a $g_{j,l}$-state.
 
% Finally, we construct a BDD $\beta_{\mathit{good}}$ over $\I,\O$, via the formula $\wedge_{l=1}^k(\beta_l\vee \gamma_l)$. Note that, given the BDD $\beta_{\mathit{SCC}}$, each $\beta_l$ and each $\gamma_l$ is constructed by $O(\varphi_l)$ symbolic operations. Therefore, overall, $\beta_{\mathit{good}}$ is constructed by $O(N+|\varphi|)$ symbolic operations. As we assume that $N>|\varphi|$, $\beta_{\mathit{good}}$ is constructed by $O(N)$ symbolic operations.
%\end{proof}




\subsection{Synthesizing a Winning Strategy}

We are ready to present a solution to the realizability and synthesis problem. We construct two strategies, each is constructed by $O(N)$ symbolic operations:
\begin{description}
\item[$f^s_{wb}$.] A memory-less strategy that wins the weak-B\"uchi game  $((\I,\O,\theta_\I,\theta_\O,\rho_{\I},\rho_{\O}),GF(\beta_{\mathit{acc}}))$.

\item[$f^s_{\mathit{travel}}$.] a memory-less strategy for the system to reach all possible inputs in a given SCC. That is, $f^s_\mathit{travel}$ satisfies the next property. Let $S$ be an SCC, and consider the subgame induced by $S$. Then, for every $(\inp,\out)\in S$, when the system applies $f^s_\mathit{travel}$, the play will traverse infinitely often states of the form $(\widehat{\inp},\out)$. \gatodo{I wonder how to construct such a strategy, symbolically, in $O(N)$ steps.}
\end{description}

Let $W$ be a winning region of $f^s_{wb}$. In Algorithm~\ref{algo:winning-strategy}, we present a strategy that wins for the system from $W$.




\begin{algorithm}[t]
	\caption{A winning strategy}
	\label{algo:winning-strategy}
	\begin{algorithmic}[1]
		
		\Statex{\begin{center}
				/*\quad\quad  From state $s$ and input $\inp$ \quad\quad*/
		\end{center}}
	
	    \State construct $\beta_\mathit{SCC}$ \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad {//  see Lemma~\ref{lem:beta_SCC}} 
	
	    \State $\gamma = \exists\O'(\beta)$ 
	    
		\State if $\beta_\mathit{acc}(s)$ and $\gamma(s,\inp')$ \Return $f^s_\mathit{travel}(s,\inp)$
		
		\State \Return $f^s_\mathit{wb}(s,\inp)$
	\end{algorithmic}
\end{algorithm}

We can now prove Theorem~\ref{thm:win}.
\begin{proof}
We show that $W$ is the system's winning region, and further that Algorithm~\ref{algo:winning-strategy} correctly constructs a strategy that wins from $W$.

First, we prove that Algorithm 2 construct a strategy that wins from $W$. ...

\end{proof}


==> explicitprelims.tex <==
\subsection{Definitions in explicit state representation}

A {\em weak \Buchi game} is a game in which in every SCC $S$ all the states are either accepting (then $S$ is called an \textit{accepting SCC}) or rejecting (then $S$ is called a \textit{rejecting SCC}).



==> intro_df_2.tex <==


\section{Introduction}
\label{sec:intro}

The field of reactive synthesis has produced various techniques for automatic generation of  controllers that react to inputs under given constraints in a way that satisfies required specifications. These techniques have been shown to be practical in providing effective tools for the design of correct-by-construction systems. 

Inspired by the well known adapter design pattern~\cite{gamma1995design}, we study the use of reactive synthesis for synthesizing adapters that translate inputs meant for a target transducer to inputs of an adaptee transducer. Think, for example, of the task of adding a layer to an operating to adapt for a hardware vulnerability that we need to avoid.


In what follows, we describe the steps of the modeling: from the Adapter design patterns to transducers, and from there to GR($k$) specification.

\subsubsection{The Adapter Design Pattern}


In the adapter design approach, the programmer implements a \emph{Target} interface by writing a code for an \emph{Adapter} that calls existing methods of an \emph{Adaptee} interface. 

Citing Wikipedia, the Adapter Design Pattern meets challenges such as how can a class be reused that does not have an interface that a client requires?

The suggested solution by the adapter design pattern describes is therefore:
Define a separate \textit{adapter} class that converts the incompatible interface of a class, called \textit{adaptee} into another interface, called \textit{target}, that is the interface that the clients require.

\dftodo{Should we put an example???}

% For illustration, consider a class that rotates a Rubik cube and thus implements the methods {\sf rot\_left}, {\sf rot\_right}, {\sf rot\_up}, {\sf rot\_down}. Now, assume that we have a broken cube that cannot be rotated to the left. Hence, we implement {\sf broken\_rot\_left} by calling {\sf rot\_right} three times. In this example, the interface for the broken cube is
% the \textit{adaptee}, the interface for the correct cube is the \textit{target}. The \textit{adapter} converts the broken cube into correct moves. \dftodo{Gera, please fix - I think I got this example wrong}.



\subsubsection{From Design Pattern to Transducers}

Formally, we propose the following synthesis problem: given two finite state transducers called $Target$ and $Adaptee$, synthesize a finite state transducers called $Adaper$ such that
\[    Adaptee \circ Adapter \eqsim Target.\]
Where $\circ$ represents transducer composition, i.e., we are comparing the target with a composition of the adaptee with an adapter, where the adapter acts before the adaptee. The $\eqsim$ symbol represent an equivalence relation specified by  the user of the synthesis algorithm. Since, it is not always reasonable to require full equality, we only require that they are equivalent. In this work we consider specifications consisting of sets of required $\omega$-regular properties over the possible outputs of the transducer $(Adaptee \circ Adapter) \cdot Target$ where $\cdot$ represents transducer concatenation.
 To this end, we assume, without loss of generality, that the output of the $Target$ and $Adaptee$ transducers are sequences of truth assignments of two disjoint sets of, respectively, input and output atomic propositions.

The following Figure~\ref{fig:ModelExample} demonstrates our modeling.  The adapter that we synthesize however receives $input1$ that is also the input to $target$ and emits $input'$ that fits the adaptee. Together, $Adaptee \circ Adapter$ receives $input$ that $target$ also obtains, and emit $output1$, while $target$ emits $output2$. In an ideal world we would ask that $output1$ and $output2$ are equal, so $Adaptee \circ Adapter$ and $target$ are indistinguishable to the user, so to speak. A more realistic approach that we adopt asks that $Adapter$ is synthesized such that $output1$ and $output2$ meet certain specifications described by the specifier.

\begin{figure}
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,initial text=,
      thick,node/.style={fill=blue!20,draw,
      font=\sffamily\footnotesize,minimum width=15mm}]

    \node[node] (21) {$input1$};
    \node[node] (24) [below of= 21] {$input1$};
    
    \node[node] (00) [right = 1cm of 21] {$Adapter$};
    \node[node] (01) [right = 1cm of 00] {$Adaptee$};
    \node[node] (22) [right = 1cm of 01] {$output1$};
    \node[node] (10) [below of= 00] {$Target$};
    \node[node] (23) [below of= 22] {$output2$};
    
    
    \draw [->] (21) --  (00);
    \draw [->] (24) -- (10);
    \draw [->] (00) --  (01);
    \draw [->] (01) --  (22);
    \draw [->] (10) --  (23);
    
    
   % \draw [->] (00) --  (10);
    % \draw [->] (01) edge [loop left] (01);
    % \draw [->] (10) edge [loop left] (10);

    % \node[initial,node] (_00) [right=2cm of 00] {$\neg a_1  \wedge \neg a_2$};
    % \node[node] (_01) [above of=_00]    {$\neg a_1  \wedge a_2$};
    % \node[node] (_10) [below of=_00]    {$a_1  \wedge \neg a_2$};
    % \node [above= 0.2 cm of _01] {Output};

    % \draw [->] (_00) edge [bend right]  (_01);
    % \draw [->] (_00) --  (_10);
    % \draw [->] (_01) edge [bend right]  (_00);
    % \draw [->] (_10) edge [loop left] (_10);
     
    % \node[node] (00) {$\neg t_1  \wedge \neg t_2$};
     
    
    \end{tikzpicture}
    \caption{A model of our system}
    \label{fig:ModelExample}
\end{figure}

As an example of our model system, consider the transducers depicted in Figure~\ref{fig:transducers}. As common in the literature, we represent truth assignments to atomic propositions as elements in $(0+1)^*$ where 0 or 1 at the $i$th letter means assigning the $i$th variable with False or True, respectively. In this example, both transducers produce truth assignment of two (different) sets of atomic propositions of size two, so the length of all these words is two. The requirement is that, for any given input,  if an output is repeated infinitely often $Target$, it must also repeat infinitely often in $Adaptee \circ Adapter$. The transducers achieves this by circling  in the $s_0 \leftrightarrow s_1$  loop of the $Adaptee$ when the $Target$ circles in $s_1$. The input for $Target$ and $Adaptee$ is also the same, we notated the $Adaptee$ input in prime to ease the reading.

\begin{figure}
    \centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.5cm,initial text=,
  thick,node/.style={fill=blue!20,draw,
  font=\sffamily\footnotesize, circle}]

\node[initial,node] (00) {$s_0$};

\node[node] (01) [above of=00] {$s_1$};
\node[node] (10) [below of=00] {$s_2$};
\node [above=0.3cm of 01] {Target};

\draw [->] (00) -- node {$U|10$} (01);
\draw [->] (00) -- node {$D|01$} (10);
\draw [->] (01) edge [loop left] node {$S|01$} (01);
\draw [->] (10) edge [loop left] node {$S|10$} (10);

\node[initial,node] (_00) [left=7cm of 00] {$s_0$};
\node[node] (_01) [above of=_00]    {$s_1$};
\node[node] (_10) [below of=_00]    {$s_2$};
\node [above=0.3cm of _01] {Adaptee};

\draw [->] (_00) edge [bend right] node [right] {$U'|01$} (_01);
\draw [->] (_00) -- node {$D'|10$} (_10);
\draw [->] (_01) edge [bend right] node [left] {$D'|00$} (_00);
\draw [->] (_10) edge [loop left] node {$S'|10$} (_10);
 
%%%
    \node[initial,circle,node,minimum width=0mm] (0) [left=4cm of 01] {$s_0$};
    
    \node[circle,node,minimum width=0mm] (1) [below of= 0] {$s_1$};
        
    \draw [->] (0) edge [bend right] 
            node [left] (A)     {$U | U'$}     (1);
    
        \draw [->] (1) edge [bend right] 
            node [right]{$S | D'$} (0);
    
        \draw [->] (0) edge [loop right] 
            node [right,text width=1cm ]{$S|S'$ \\ $D|D'$} (0);
    
    \node (adapter)  [above=0.3 cm of 0] {Adapter};

\node[] () [left=.5cm of adapter] {$\circ$};
\node[] () [right=1.5cm of adapter] {$\eqsim$};

\end{tikzpicture}
    \caption{An example of target and adaptee transducers and an adapter  that guarantees, for example, $GF(t_i) \to GF(a_i)$   for $i=1,2$  where $\{t_1, t_2\}$ and $\{a_1,a_2\}$ are the atomic propositions of the target and of the adaptee, respectively.}
    \label{fig:transducers}
\end{figure}



While most of the work on software synthesis focuses on synthesizing complete systems from their specifications, our focus is on using reactive synthesis for reusing existing components. The $Target$ transducer can model, for example, a standard Rubik cube and the $Adaptee$ can model a Rubik cube with some hardware failure. Since we know how to operate the normal cube, we could use an $Adapter$ that translates commands that we planed to send to the normal cube to commands that we can send to faulty one. The equivalence relation can say, for example, that if a side of the normal cube would have been completed infinitely often in the expected run of the normal cube it should also be completed infinitely often in the generated run of the faulty cube.



\subsubsection{From Transducers to Separated GR($k$)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Dror will add a paragraph saying that the problem is very hard and that current state of the art tools cannot handle even small instances. Accordingly, we propose to use GR(K) formulas instead of just any $\omega$-regular properties.

Generally, synthesizing a transducer is complicated - complexity wise. Indeed, Even when equality is required, synthesizing is a non trivial task. \dftodo{write much better and explain the hardness, as a step towards GRk}


\dftodo{Now we mention GR(k) and how to utilize GR(k) that balance between expressiveness and efficiency. Mention the term "reactive synthesis".}

We thus next explain our GR($k$) model. In order for the adapter to work properly, it must know both the $target$ transducer and the $Adapter$ transducer inside out. Therefore both are a part of our synthesis input. Since each transducer is deterministic, we can model each transducer as a transition system that contains only the outputs of each transducer.
Next we assume that the specification describes a relation that ties every output behavior of $target$ to an output behavior of the $Adaptee$. 
Therefore, we synthesize a $controller$ transducer that relates the $Target$ output to the $Adaptee$ output, that meets the specification.

Finally we note that the $Adapter$ transducer is $Adaptee^{-1}\circ Controller \circ Target$. \dftodo{Gera, how can we motivate that?}





To allow direct use of the language of reactive synthesis, and to allow more generality, the input to our synthesis algorithm and to the tool that implements it is a representation of $Adpatee$ and $Target$  as transition systems, as depicted in Figure~\ref{fig:example}. 







The $Input$ transition is a representation of the $Target$ and the $Output$ transition system is a representation of the $Adatpee$ where we ignore the inputs to the systems and the state and consider only their outputs.

\begin{figure}
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,initial text=,
      thick,node/.style={fill=blue!20,draw,
      font=\sffamily\footnotesize,minimum width=15mm}]

    \node[initial,node] (00) {$\neg t_1  \wedge \neg t_2$};
    \node[node] (01) [above of=00] {$\neg t_1  \wedge t_2$};
    \node[node] (10) [below of=00] {$t_1  \wedge \neg t_2$};
    \node [above= 0.2 cm of 01] {Input};

    \draw [->] (00) --  (01);
    \draw [->] (00) --  (10);
    \draw [->] (01) edge [loop left] (01);
    \draw [->] (10) edge [loop left] (10);

    \node[initial,node] (_00) [right=2cm of 00] {$\neg a_1  \wedge \neg a_2$};
    \node[node] (_01) [above of=_00]    {$\neg a_1  \wedge a_2$};
    \node[node] (_10) [below of=_00]    {$a_1  \wedge \neg a_2$};
    \node [above= 0.2 cm of _01] {Output};

    \draw [->] (_00) edge [bend right]  (_01);
    \draw [->] (_00) --  (_10);
    \draw [->] (_01) edge [bend right]  (_00);
    \draw [->] (_10) edge [loop left] (_10);
     
    \node[node] (00) {$\neg t_1  \wedge \neg t_2$};
     
    \node[initial,circle,node,minimum width=0mm] (0) [below=2cm of 10] {$s_0$};
    
    \node[circle,node,minimum width=0mm] (1) [right=2cm of 0] {$s_1$};
    
    
    \draw [->] (0) edge [bend right] 
            node [below,text width=1cm ] (A)     {$00 | 01$ \\ $01 | 01$}     (1);
    
        \draw [->] (1) edge [bend right] 
            node [above,text width=1cm ]{$00 | 00$ \\ $01 | 00$ \\ $10 | 00$} (0);
    
        \draw [->] (0) edge [loop above] 
            node [above,text width=1cm ]{$10 | 10$} (0);
    
    \node [above of=A] {Controller};
    
    
    \end{tikzpicture}
    \caption{An example of target and adaptee transition systems and a transducer that guarantees, for example, the implications $\phi_i \to \psi_i$ for $i=1,2$ and $\phi_1=GF(\neg t_1 \wedge t_2)$, $\psi_1=GF(\neg a_1 \wedge a_2)$, $\phi_2=GF(t_1 \wedge \neg t_2)$, and $\psi_2=GF(a_1 \wedge \neg a_2)$.}
    \label{fig:example}
\end{figure}

From this point on, we will only talk about this representation of the problem, i.e., we will synthesize a controller that reads a run  of an input transition system and produces a run of an output transition system such that the combined run always satisfies a set of $GR(k)$ properties. 
%Note that it is usually not possible to ignore the input system by generating a controller that ignores its inputs and just satisfy all the $\psi$ properties. 

% In this paper we propose to use reactive synthesis in a nontraditional way: 
% we propose to apply a reactive synthesis based algorithm for generating strategies that read the actions of a controller on input systems and reacts by producing actions on output systems. 
% There is no interaction, in our setting, between the input and the output systems. 
% The only connection between the systems is formed by the synthesized strategy that observes the input system and adapts actions on the input system to actions on the output system.
% %\gatodo{"No interaction" is imprecise and thus may confuse. Consider instead e.g.: "rather then interacting with its environment, the output system merely observes the actions taken by the input system, and acts accordingly."}
% The specification to the synthesizer consists of: (1) transition systems for the input and for the output systems; (2) a temporal logic formula of a specific form
% that maps properties
% %\gatodo{I am not sure that it is "state properties". Maybe "liveness properties"? Also, I think that the footnote should appear at the end of the sentence (after the period) since it relates also to the "state property to state property".}
% of states of the  input system to properties of states of the output system.\footnote{$GR(k)$ formulas where all the left hand side variables are from the input system and all the right hand side variables are from the output system, as elaborated later in the paper.} 
% Based on this data, our strategy generates actions for the output system in reaction to actions on the input system such that if a property repeats infinitely often in the input, its related property in the output system must also repeat infinitely often.  

% Imagine, as a simple example for demonstration purposes, that we have a Rubik cube and a controller that keeps turning the cube sides in order to achieve goals that are not known to us (possibly because this is a legacy system).
% Imagine further, that there is a defect in our cube requiring us to transfer the actions that the controller planned for the normal cube to actions on the cube with the defect.
% Think, for example, of a defected Rubik cube in which the sides can only be turned clockwise, not counterclockwise.
% Using the tool proposed in this paper, we can apply the following steps towards transferring actions on the normal cube to actions on the faulty one:
% \begin{enumerate}
% \item Model both the transition systems of the normal cube and of the faulty one.
% \item Specify that the properties that we care about are completions of sides, i.e., ask the synthesizer to guarantee that if a side is completed infinitely often on the normal cube it must also be completed infinitely often on the faulty cube.  
% \item Invoke our synthesis algorithm to obtain a transfer strategy.
% \item Run the original controller on a virtual simulated copy of the normal cube and use the synthesized strategy to transfer actions that the controller planned to run on the virtual cube to actions that we can apply to the faulty one. 
% \end{enumerate}

% Note that we cannot, in this setting, directly synthesize a controller for the faulty cube because we do not have a specification of how it should behave (we do not even have the specifications for the controller of the normal cube). 
% Note also that it is not always possible to ignore the input system by generating a controller for the output system that just achieves all the goal states in the output system infinitely often. 
% Imagine, for example, a game where we are forced to move the cube in a way that allows to complete either the red side or the blue side infinitely often, but not both. In this case, we must synthesize a controller that follows the actions in the input system and translates them to actions in the output system in a way that the side that is completed infinitely often in the normal cube is also completed infinitely often in the faulty, without knowing, perhaps until a late point of the run, which side it is going to be. 

%The Rubik Cube example demonstrates the capability of our framework to handle what we call \textit{Automatic Fault Corrections}, in which the objective is to find a strategy that gives a plan to a faulty system that is at least as good as the plan for the original one [[DF: is that so??]].
%This however is not the only use-case for our approach that one could have in mind.
%Think for example of \textit{Adaptive systems in Automatic Decentralization}. There, constructing a distributed system from third-party components is challenging due to problems related to compatibility and communication issues. One approach for solving such problems is to start with a centralized solution and then adapt it to distributed setting by adding more general interactions between the components. The tools that we describe in this paper can be used for generating adaptors for running black-box components in a distributed setting. The distributed system is required to behave as the centralized one would but also obeying the restrictions modeled by the transition relation of the output system.
%As another example one could also think of \textit{automatic software product line development}, which is an engineering technique for creating a collection of similar software systems from a shared set of software assets. The tools that we are presenting in this paper can be used to implement software product lines with less effort. Specifically, a company can design a controller for a base system and then transfer its actions automatically to similar systems down the product line using our synthesis algorithm. These examples, of course, are only a partial list of potential applications for our tools. We are sure that readers can extend this list and think of many variants of the ideas raised above.


% To further motivate the proposed methodology, we list some abstract use-cases for which we identify how a transferring the actions of a controller to a new domain can be useful:

% \begin{description}

% \item[Automatic Fault Correction:] As demonstrated in the Rubik cube example, the output system can be a faulty version of the one that the controller was designed to handle. 
% The synthesis algorithm that generates the strategy for handling a fault can run on-the-fly when a fault is detected or off-line for commonly occurring faults.
% %\gatodo{Maybe it's just me, but I don't understand this sentence} 
% The synthesis can be simple, e.g., if the side can only be turned clockwise just turn it counterclockwise three times to simulate a single turn. It can also be more complicated, as follows. Say, for example, that the normal cube must commit to finishing either the yellow or the green side infinitely often, but it can do so at any time; however with the faulty cube we have to make this commitment at the first step. In this case, we have to wait for the commitment on the virtual cube and only then start our moves on the faulty cube. We can support this possibility by adding self-loops on the output system initial state which allow the synthesized strategy  to wait and examine several steps of the input system before it makes a move in the output system.
% %\gatodo{I understand the second case, but it is not clear why our synthesis algorithm supports it. Maybe add here: "we can support this possibility by adding self-loops on the output system transitions, which allow it to wait and examine several consecutive steps by the input system.}

% \item[Automatic Decentralization:] Constructing a distributed system from third-party components is challenging due to problems related to compatibility and communication issues. One approach for solving such problems is to start with a centralized solution and then adapt it to distributed settings by adding interactions between the components. The tools that we describe in this paper can be applied for adapting components that were not designed for it to operate in a distributed setting. In this case, the input system will be the centralized version for which we have a controller. The synthesis can then be used to transfer the actions to a transition system that only allows actions that can be implement in the distributed environment.

% \item[Automatic Generation of Software Product Lines:] Software product line development is an engineering technique for creating a collection of similar software systems from a shared set of software assets. The tools that we are presenting in this paper can be used to implement software product lines with less effort. Specifically, a company can design a controller for a base system and then transfer its actions automatically to similar systems down the product line using our synthesis algorithm.
%  \end{description}
 
% This is, of course, only a partial list of potential applications for our tools. We are sure that readers can extend this list and think of many variants of the ideas raised above. %The focus of this paper is on the core synthesis algorithm and on the analysis of its performance. The research on practical applications of the method for the above and for other application domains is left for future work.

% Our framework lies on the specific structure of our reactive synthesis $GR(k)$ settings. These consist of $G_I$ and $G_O$ that are transition systems for the input and output respectively, and a specification formula $\varphi$.




% that is a conjunct of $k$ $GR(1)$ constraints for each the left-side is only over the input variables, and the right-side is only over the output variables \dftodo{fix terminology}.
% While there are standard techniques that synthesize this kind of specifications (see related work for more), our solution exploits this specific setting to yield a more efficient solution in terms of computational complexity \dfnote{be more specific}. For that, we show how synthesis of our problem is reduced to solving a special kind of a  \textit{weak B\uchi} game.


\subsubsection{The Separated GR($k$) model}

\dftodo{Consider ditching this paragraph, that goes to too many details. But do mention the separation of variables. Say something like: note that we have separation of variables between the input  and output. This paper technically exploits this separation towards utilizing better algorithms.}
A problem formulation in our setting is a game structure that consists of two separated transition systems called  $G_\I$ and $G_\O$ respectively in a symbolic representation (with disjoint variables) and a $GR(k)$ formula $\Lambda$ of the form $\bigwedge_{i=1}^k(\phi_i\rightarrow\psi_i)$, where the $\phi_i$ are conjuncts of Globally-Finally Boolean formulas on the \textit{$\I$-variables only}, and the $\psi_i$ are conjuncts of Globally-Finally Boolean formulas on the \textit{$\O$-variables only}. Note that $GR(k)$ formulas also capture DBA properties, i.e. properties recognized by deterministic B\"uchi automata~\cite{}. The formula, $\Lambda$ represents a required connection between the runs of $G_\I$ and the runs of $G_\O$: it says that we want to generate runs in $G_\O$, based on an observing an ongoing run of $G_\I$, such that if things repeat infinitely often in the $\I$-run then their corresponding consequences must also occur infinitely often in the $\O$-run.

% specific type of $GR(k)$ formulation. These are a set of $k$ temporal constraints, each is of the form $\phi\rightarrow\psi$, where $\phi$ is a conjunct of Globally-Finally Boolean formulas on the \textit{environment variables only}, and $\psi$ is a conjunct of Globally-Finally Boolean formulas on the \textit{system variables only}.

%Together with the accompanied transitions systems of the input and output $G_I$ and $G_O$ respectively,
%that is standard in $GR(k)$ formulations, the 

% As such, our formulation can be interpreted as a game over the state space described by the tuple, that can hint towards a route to solving $GR(k)$. 

Note that unlike standard $GR(k)$ the choices of the system only affect $G_\O$ while the environment plays on a completely disconnected system $G_\I$. The only connection between the two is the formula $\Lambda$. 
%Indeed, there are explicit and symbolic methods to solve such problems with an efficiency of $O(n^2)$ where $n$ is the number of states in the resulting graph game. \dftodo{sharpen complexity result}.

%Note that unlike standard $GR(k)$, the environment/system variables in our formulation are separated by the $\rightarrow$ connector [[DF: say better]]. 

%As such, our formulation describes an  interaction between two separated games that are played: one of the environment, and one over the system.

To synthesize a winning strategy, we use the fact that each connected component of the product of the two systems is either a winning or a losing sub game for the output system, regardless of the initial state of the play. This allows us to reduce the problem into a \emph{weak-B\"uchi} game, i.e. to play a strategy to stabilize in a winning connected component. We further formulate an interesting property that both our game and the reduced weak B\"uchi game possess, the \emph{delay property}: Assume we follow a winning strategy, and, at some point, for some reason, the input system successfully manages to take several steps with no intermediate response by the output systems. Then, the reached state is still winning for the output system. This enable us to decide the realizability of the specification in $O(N)$ symbolic operations, and to synthesize a controller for a realizable specification in $O(|\varphi|N)$ symbolic operations, where $\varphi$ is the GR($k$) winning condition, and $N$ is the size of the state-space. We remark that, in general, GR($k$) games are solved in $O(N^{k+1}k!)$ operations~\cite{PitermanP06}.

In Section 2 we give preliminaries and discuss related work in Section 3.
%\gatodo{isn't it better before the conclusion}
In Section 4 we formulate our problem and provide a solution that uses a weak-B\"uchi solver as a black box.
In Section 5 we show how to solve weak B\"uchi games in linear time. First, we provide an explicit solution and then explain how to modify it into a symbolic algorithm. In Section 6 we utilize our framework into a tool, followed by running experimental evaluations on these examples and compare against state-of-the-art synthesis tools. We conclude in Section 7.



\subsection{Illustrative Examples}

In addition to the example given before, we formalize two more illustrative examples to demonstrate additional usages of our technique.

\vspace{3pt}
\noindent\textbf{Cleaning robots}. We consider a cleaning robot that moves along a corridor-shape building from room 1 to room $n$. The robot follows some plan, and accordingly cleans some of the room. Our goal is to synthesize a second cleaning robot that follows the first robot and cleans exactly those rooms that have not been cleaned by the first robot. 
\ganote{to complete about vars etc.}

\vspace{3pt}
\noindent\textbf{Railway Signalling.} We consider a junction of $n$ railways, each railway is equipped with a signal that can be turned on (light in green) or off (light in red). Some railways overlap and thus their signals cannot be turned on simultaneously. We consider the next overlapping pattern. Railways 1-4 overlap, likewise 3-6, 5-8, and so on.

An existing system handles the signalling system by providing assignment over  $\{\mathit{in{:}signal}_i: 1\leq i\leq n\}$. To avoid accidents, it was programmed to be strictly safe; it never raises two signals simultaneously. We are interested in a controller that performs better, by assigning values to  as we explain below.

Formally, the input system controls variables , and ...

it is strictly safe: at each step, at most a single signal is turned on.

We aim to synthesize a safe and efficient controller that tracks the assignments that the input system produces, and accordingly activates the signalling system in an improved manner. The controller we are interested in controls variables $\{\mathit{out{:}signal}_i: 1\leq i\leq n\}$, and it produces \emph{maximal assignments} in the following sense: if the signal of every rail that overlaps with the $i$th rail is off, then $\mathit{out{:}signal}_i$ must be turned on.
Furthermore, we want to maintain liveness properties of the input system: 
\begin{itemize}
    \item For every $i=1\dots n$, if  $\mathit{in{:}signal}_i$ is turned on infinitely often, then  $\mathit{out{:}signal}_i$ is turned on infinitely often as well.
    
    \item For every $i=1\dots n$, if  $\mathit{in{:}signal}_i$ is turned on at least once in every $m$ consecutive steps (where $m$ is a parameter of the specification), then the same holds for $\mathit{out{:}signal}_i$.
\end{itemize}





\subsection{Gal Point of Objection to Introduction}

To read the following after reading Figure 1.
There is also an alternative introduction in Appendix F that reflects the introduction.

As agreed, I will explain here why I object to what written so far (and thus to what is written afterwards). First, note that in what is written the target corresponds to the input TS, and the adaptee is the output TS.
     \begin{itemize}
         \item      I think that the target should be what we want to have. If you say that you have the target transducer, then why there is a problem to solve here?
     \item the design pattern is about using an existing code (the adaptee). In my mind the \emph{only} code we have is the input system. Hence, the adaptee must be the input system.
     \item Again - if the input is the target, then you were given the target and there is no problem to solve.  So, if you agree with the first comment, the input cannot be the target.
     \item What we call input corresponds to the traditional "environment". The usual framework is that the controller we synthesize gets inputs from the environment (the input TS) and provide sys-var outputs. Here you do something extremely complicated: (1) You decide that both the environment and the controller we synthesize has the same input alphabet (which is unknown and not exactly part of the game-structure) (2) you decide that the controller acts first, upon inputs for the environment player (3) the controller produces an output from the mysterious alphabet that the "system" acts upon, (4) you let the environment run in parallel to that composition of the synthesized controller and the system, (5) for that, you came up with a non-standard transducer concatenation. I believe it will be very difficult for the reactive-synthesis community to grasp this conducting (at least it is for me. Not sure that I am a decent representative, but I do know what is going on here and it is not easy for me to understand how it works...) 
     \item calling the input "target" makes sense only when we actually interested in the input system behaviors. It is extremely awkward over examples like the cleaning robots, the railways, and the traffic lights.
     \item (minor) Seeing the output system as a transducer seems awkward to me. The output system is just about which steps are legal - it is the safety guarantees, no more than that. 
     \item What you claim we synthesize (e.g. in Figure~\ref{fig:transducers}) is not what we say we synthesize in the preliminaries (i.e. the inputs and outputs are variables and not U/S/D) and not what our tool produces. It is also not aligned with how we model a strategy (a BDD over input and output variables such that ...)
     \item more later...
     \end{itemize}



==> prelims_old.tex <==
\section{Preliminaries}
\label{Sec:Prelims}


\dftodo{clean this paragraph!!}
Given a set of Boolean variables $\V$, a {\em state over $\V$} is an assignment to the variables in $\V$. Their {\em primed versions} are defined as follows:\gatodo{I don't understand what 'their' refers to. Actually, I think that the whole sentence 'Their ...as follows:' is redundant. What is its purpose? Maybe we should remove it?} For a set of Boolean variables $\V$, $\V' = \{v' | v \in \V\}$ is the set of {\em primed variables of $\V$}. 
%\gatodo{perhaps add: $2^\V$ is the set of states over $\V$. Note, state has been defined as an assignment to $\V$, so not needed.} 
Given a state $s$ over $\V$, {\em primed state $s'$ over $\V'$} assigns $v'\in \V'$ to $\mathsf{True}$ iff $v\in\V$ is assigned to $\mathsf{True}$ in state $s$. 
An {\em assertion over $\V$} is a Boolean formula over variables $\V$.
A state $s$ satisfies an assertion $\rho$ over the same variables, denoted $s \models \rho$, if the assertion evaluates to $\mathsf{True}$ on the assignment to variables in state $s$\gatodo{This sentence makes sense if $s$ is a subset of $\V$. But, since you defined a state to be an assignment, it probably should be: ' .. to $\mathsf{True}$ by the assignment $s$'. B.t.w., throughout the paper I refereed to states as subsets of $\V$. If you decide that a state is an assignment (i.e. a function to true,false), we should align the rest of the paper with this def. }.  


%For $\mathcal U\subseteq\mathcal V$, $s|_\mathcal{U}$ is a state over $\mathcal U$ defined by $s|_\mathcal U=s\cap U$.

%Let $\mathcal{V}$ be a set of Boolean variables. A \emph{state} over $\mathcal V$ is an element of $2^\mathcal V$, i.e. an assignment to the variables in $\mathcal V$. An \emph{assertion} over $\mathcal{V}$ is a Boolean formula that includes only variables from $\mathcal V$. For a state $s$ and assertion $\rho$, we write $s\models \rho$ if $\rho$ is evaluated to $\mathit{true}$ by assigning $\mathit{true}$ to all variables in $s$, and $\mathit{false}$ to all variables in $\mathcal V\setminus s$. For $\mathcal U\subseteq\mathcal V$, $s|_\mathcal{U}$ is a state over $\mathcal U$ defined by $s|_\mathcal U=s\cap U$.$\mathcal V'$ is the \emph{primed version} of $\mathcal V$, defined by $\mathcal{V}'=\{v': v\in \mathcal{V}\}$. For a state $t$ over $\mathcal V$,  $t'$ is the state over $\mathcal V'$ defined by $t'=\{v':v\in t\}$. 


\subsubsection{Linear Temporal Logic}

Linear Temporal Logic ($\ltl$)~\cite{Pnueli77} extends propositional logic with infinite-horizon temporal operators. 
The syntax of an $\ltl$ formula over a finite set of Boolean variables  $\V$ is  defined as follows: 
$\varphi:= v\in\V \mid \ltlNeg \varphi \mid \varphi \land \varphi \mid \varphi \lor \varphi \mid \ltlX \varphi \mid \varphi \ltlU \varphi \mid \ltlF \varphi \mid \ltlG \varphi$.\gatodo{@Suguman: quite petty, but you changed $\varphi::=$ to $\varphi:=$ (right?) I think that for context-free grammar $::=$ is more common...}
Here $\ltlX$ (Next), $\ltlU$ (Until), $\ltlF$ (Eventually), $\ltlG$ (Always) are temporal operators.  
The semantics of $\ltl$ can be found in~\cite{Pnueli77}.\gatodo{wouldn't it be better to give a popular textbook here?}
\dftodo{add about GR(k)}
\gatodo{Not sure we should speak here about GR(k). Later we specify some LTL-winning conditions that we use throughout the paper. I also think it would help the reader if we present those conds as LTL wining conds rather than "just" LTL formulas }



\begin{comment}
We turn to define the semantics of an LTL formula. Let $\pi\in (2^\mathcal V)^\omega$ be an infnite sequence of states. For $i>0$, $\pi^i\in (2^\mathcal V)^\omega$ is the sequence $\pi(i),\pi(i+1),\dots$.

The satisfaction relation between an infinite sequence of states $\pi\in 2^\mathcal V$ and an LTL formula $\varphi$, $\pi\models \varphi$ is inductively defined as follows. (1) $\pi\models \mathit{asrt}$ if $\pi(0)\models \mathit{asrt}$; (2) \emph{G}lobally: $\pi\models G(\varphi)$ if $\forall i\geq 0(\pi^i\models \varphi)$; (3) \emph{F}uture: $\pi\models F(\varphi)$ if $\exists i\geq 0(\pi^i\models \varphi)$; (4) \emph{U}ntil: $\pi\models (\varphi_1)U(\varphi_2)$ if $\exists i\geq 0( \pi^i\models \varphi_2 \text{ and } \forall j\in\{0,\dots,i-1\}(\pi^j\models \varphi_1))$; (5) Boolean operators are treated in a standard manner.
\end{comment}

\subsubsection{Game structures and games} 
A game structure $\GS=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ defines a turn-based interaction between an {\em environment} and a {\em system} players over Boolean variables $\I$ and $\O$. The environment player assigns values to the input variables $\I$ and the system assigns values to the output variables $\O$.
Assertions over these variables and their primed versions define {\em initial conditions} $\theta_\I,\theta_\O$ for the environment and the system respectively, and {\em safety conditions} $\rho_\I,\rho_\O$ for the interactions.
Intuitively, $\GS$ can be viewed as a directed graph in which states of the graph are given by states over $ \I\cup\O$. A state $s$ over $\I\cup\O$ is an initial state of the graph if $s \models \theta_\I\wedge \theta_\O$. There is a transition from state $s$ to state $t$ if $(s,t') \models \rho_\I\wedge \rho_\O$.
%A play progresses by the players taking turns to assign values to their own variables till infinitum.  At the start, the players must satisfy the initial conditions and
%must satisfy the safety conditions thereafter.


Formally we define a game structure as follows. The input variables $\I$ and output variables $\O$ of $\GS$ are two disjoint sets of variables that are controlled by the environment and system, respectively. The environment's {\em  initial assumption} $\theta_\I$ is an assertion over $\I$, and the system's \emph{initial guarantees} $\theta_\O$ is an assertion over $\I\cup\O$.
The environment's \emph{safety assumptions} $\rho_\I$ is an assertion over $\I\cup\O\cup\I'$, where the interpretation of  $(\inp_0,\out_0,\inp_1')\models \rho_\I$ is that from state $(\inp_0,\out_0)$ the environment can assign $\inp_1$ to the input variables. W.l.o.g, we assume $\rho_\I$ is deadlock free, i.e., for all $(\inp_0, \out_0)$ there exists an $\inp_1$ s.t. $(\inp_0,\out_0,\inp_1')\models \rho_\I$. Similarly, the system's \emph{safety guarantees} $\rho_\O$ is an assertion over $\I\cup\O\cup\I'\cup\O'$, where the interpretation of    
     $(\inp_0,\out_0,\inp_1', \out_1')\models \rho_\O$ is that from state $(\inp_0,\out_0)$ when the environment assigns $\inp_1$ to the input variables, the system can assign $\out_1$ to the output variables. Again, w.l.o.g, we assume $\rho_\O$ is deadlock free, i.e., for all $(\inp_0, \out_0, \inp_1')$ there exists an $\out_1$ s.t. $(\inp_0,\out_0,\inp_1',\out_1')\models \rho_\O$.
    
    
    
    




%     \item The environment's \emph{safety assumptions} $\rho_\I$ is an assertion over $\I\cup\O\cup\I'$. 
    
%     The interpretation of    
%     $(\inp_0,\out_0,\inp_1')\models \rho_\I$ is that from state $(\inp_0,\out_0)$ the environment can assign $\inp_1$ to the input variables. 
    
%     W.l.o.g, we assume $\rho_\I$ is deadlock free, i.e., for all $(\inp_0, \out_0)$ there exists an $\inp_1$ s.t. $(\inp_0,\out_0,\inp_1')\models \rho_\I$. 
    
%     \item The system's \emph{safety guarantees} $\rho_\O$ is an assertion over $\I\cup\O\cup\I'\cup\O'$.
    
%     The interpretation of    
%     $(\inp_0,\out_0,\inp_1', \out_1')\models \rho_\O$ is that from state $(\inp_0,\out_0)$ when the environment assigns $\inp_1$ to the input variables, the system can assign $\out_1$ to the output variables. 
    
%     W.l.o.g, we assume $\rho_\O$ is deadlock free, i.e., for all $(\inp_0, \out_0, \inp_1')$ there exists an $\out_1$ s.t. $(\inp_0,\out_0,\inp_1',\out_1')\models \rho_\O$. 
% \end{itemize}
% \end{definition}

% Intuitively, a game structure is a directed graph in which states of the graph are given by states over $ \I\cup\O$. A state $s$ over $\I\cup\O$ is an initial state of the graph if $s \models \theta_\I\wedge \theta_\O$. There is a transition from state $s$ to state $t$ if $(s,t') \models \rho_\I\wedge \rho_\O$.


A play over $\GS$ progresses by the players taking turns to assign values to their own variables till infinitum, where at the start, the players must satisfy the initial conditions and must satisfy the safety conditions thereafter.
Formally a \emph{play} $\pi=s_0,s_1,\dots$ is an infinite sequence of states over $\I\cup\O$ such that $s_0\models \theta_\I\wedge \theta_\O$ and $(s_j,s_{j+1}')\models \rho_\I\wedge \rho_\O$  for all $j\geq 0$.
A \emph{play prefix} is either a play or a finite sequence of states that can be extended to a play.
Then a {\em strategy} is a function   $f:(2^{\I\cup\O})^+\times 2^\I\rightarrow 2^\O$ such that if $s_0,\dots,s_m$ is a play prefix, $(s_m,\inp')\models \rho_\I$ and $f(s_0,\dots,s_m,\inp)=\out$, then $(s_m,\inp',\out')\models \rho_\O$.
Intuitively, a strategy directs the system on what to assign to the output variables depending on the history of a play and the most recent assignment by the environment to the output variables. 
A play prefix is said to be {\em consistent with a strategy} $f$ if for all states $s_j = (\inp_j, \out_j)$ in the prefix $f(s_0,\dots, s_{j-1}, \inp_j) = \out_j$ for all $j \geq 0$. 
A strategy is memoryless if it only depends on the last state and the most recent assignment to the output variables. 
Formally, a {\em memoryless strategy} is a function   $f:(2^{\I\cup\O})\times 2^\I\rightarrow 2^\O$ such that if $(s_m,\inp')\models \rho_\I$ and $f(s_m,\inp')=\out$, then $(s_m,\inp',\out')\models \rho_\O$.



\begin{comment}
A strategy is a partial function   $f^s:(2^{\I\cup\O})^+\times 2^\I\rightarrow 2^\O$ such that if $\pi=s_0,\dots,s_m$ is a play-prefix, $(s_m,\inp')\models \rho_\I$ and $f^s(s_0,\dots,s_m,\inp)=\out$, then $(s_k,\inp',\out')\models \rho_\O$. 

A play-prefix $s_0,\dots$ is consistent with strategy $f^s$ if for every state $s_m$ in the sequence where $m>0$, we have $f^s(s_0,\dots,s_{m-1},{s_m|}_\I)=s_m|_\O$. 

Furthermore, we require that if a finite play-prefix $\pi=s_0,\dots,s_m$ is consistent with $f^s$ and $(s_m,\inp')\models \rho_\I$, then $f^s(s_0,\dots,s_m,\inp)$ is defined. 


A strategy is \emph{memory-less} if the value it returns depends only on the last state and the input. That is, if $f^s(\pi,s,\inp)=f^s(\sigma,s,\inp)$ for every two sequences $\pi,\sigma\in (2^{\I\cup\O})^*$, $s\in 2^{\I\cup\O}$, and $\inp\in 2^\I$ such that $(\pi,s)$ and $(\sigma,s)$ are consistent with $f^s$, and $(s,\inp')\models \rho_\I$.

\end{comment}


% A \emph{winning condition} over a set of variables $\mathcal V$ is a subset of $(2^{\mathcal V})^\omega$. 

We now describes a game over a game structure.
A {\em game} is a tuple $(\GS,\varphi)$ where $\GS$ is a game structure over inputs $\I$ and outputs $\O$ and $\varphi$ is a subset of $(2^{\mathcal V})^\omega$. $\varphi$ is called a {\em winning condition} over $\I\cup\O$.
A play $\pi$ is \emph{winning} for the system if $\pi\in \varphi$. A strategy $f$ \emph{wins from state $s$} if every play $\pi$ from $s$ that is consistent with $f$ is winning for the system. A strategy $f$ \emph{wins from  $S$} where $S$ is an assertion over $\I\cup\O$ if it wins from every $s\models S$. The \emph{winning region} of the system is the set of states  from which it has a winning strategy. 
A strategy $f$ is \emph{winning} if for every $\inp\models \theta_\I$ there exists $\out\in 2^\O$ such that $(\inp,\out)\models \theta_\O$ and $f$ wins from $(\inp,\out)$. 
In this paper, we have the following games that are defined over the following winning conditions.

\begin{itemize}
\item
{\em Reachability games}:  $\ltlF(\varphi)$ where $\varphi$ is an assertion over $\I\cup\O$. 

\item 
{\em Safety games}: $\ltlG(\varphi)$ where $\varphi$ is an assertion over $\I\cup\O$. 

%\item[B\"uchi.] $GF(\mathit{asrt})$, where $\mathit{asrt}$ is an assertion. In a B\"uchi game, the system must infinitely often reach a state $s$ such that $s\models\mathit{asrt}$.
\item{\em B\"uchi games}:
$\ltlG\ltlF(\varphi)$ where $\varphi$ is an assertion over $\I\cup\O$.

\item
{\em GR($k$) games}:  $\bigwedge_{l=1}^k (  
\bigwedge_{i=1}^{n_l} \ltlG\ltlF(\varphi_{l,i}) \rightarrow \bigwedge_{j=1}^{m_l} \ltlG\ltlF(\psi_{l,j}))$ where all $\varphi_{l,i}$ and $\psi_{l,j}$ are  assertions over $\I\cup\O$. 



%Hence,  GR($k$) is an assume-guarantee condition. For each $l\in\{1,\dots,k\}$, the system must make sure that if assertions $a_{l,1},\dots,a_{l,n_l}$ are satisfied infinitely often during a play, then $g_{l,1},\dots,g_{l,m_l}$ are satisfied infinitely often as well.
\end{itemize} \dftodo{clean this list!}


 Given a game $(\mathit{GS},\varphi)$,
 the following problems are considered in this work:
\begin{description}
\item[Realizability.] Whether a winning strategy for the system exists.

\item[Synthesis.] Construct a winning strategy for the system if possible, or announce that no such strategy exists.
\end{description}

We note that a realizability check can be reduced to the identification of the winning region, $W$: A winning strategy exists, iff for all $\inp\models \theta_\I$ there exists $\out\in2^\O$ such that $(\inp,\out)\models \theta_\O$ and $(\inp,\out)\in W$. Hence, the synthesis problem can be solved by constructing a strategy that wins from $W$.

%Let $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ be game structure, and $\varphi$ a winning condition over $\I\cup\O$.

\subsubsection{Game description in explicit-state representation.} \dftodo{merge this subsection with other parts and shorten considerably}

A game with game structure $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$ and a winning condition can be equivalently represented by a game between the system and environment player on  directed graph $ (V,E)$. The states on the graph are given by states over $\I\cup\O$ and there is a directed edge from state $s$ to state $t$ in the graph if $(s,t')\models \rho_\I\wedge\rho_\O$. Recall, we assume that all states of a game structures are deadlock-free. Thus, there is at least one outgoing edge from every state in directed graph $(V,E)$.
States that satisfy $\theta_\I\wedge\theta_\O$ are the initial states of the graph. 
The game proceeds by the environment player assigning values to the input variables $\I$ and the system player assigning values to the output variables $\O$.  
The game starts at one of the initial states of the graph. 
In every round of the game, first the  environment chooses an assignment to the $\I$ variables, and then the system will choose an assignment $O$ to the $\O$ variables.
The combined assignment $I \cup O$ determines the unique state  the game moves to. \gatodo{to review the previous sentences}
The notions of plays, strategies, winning conditions, and so on naturally transfer to the explicit-state representation. 





%For readability, we also consider an explicit representation of the game between the environment and the system. Given a game structure  $\mathit{GS}=(\I,\O,\theta_\I,\theta_\O,\rho_\I,\rho_\O)$, we define a graph that serves as a ``game-board" as follows. $G^{\mathit{GS}}=(V^\mathit{GS},E^\mathit{GS})$, where $V^\mathit{GS}=2^{\I\cup\O}$, and $(\inp_0,\out_0)E(\inp_1,\out_1)$ if $\big((\inp_0,\out_0),(\inp_1',\out_1')\big)\models \rho_\I\wedge \rho_\O$.
%At the beginning of a play, the environment chooses $\inp\in 2^\I$, the system then responds with $\out\in 2^\O$, and thus the first state of the play is $(\inp,\out)\in V^{\mathit{GS}}$. Afterwards, the payers repeatedly choose the next state of the play: form state $(\inp_0,\out_0)$ the environment chooses $\inp_1\in 2^\I$ such that $(\inp_0,\out_0,\inp_1')\models \rho^e$, the system replies with $\out_1$ such that $(\inp_0,\out_0,\inp_1',\out_1')\models \rho_\O$, and the play traverses to state $(\inp_1,\out_1)$.  Note that the notions of plays, strategies etc. naturally transfer to the explicit representation. We omit the straightforward adaptation of those notions in the explicit context. 

A {\em strongly connected component} (SCC) of a directed graph $(V,E)$ is a maximal set of states within which every state is reachable from every other state.  It is well known that SCCs partition the states of a directed graph. 



Let $\Statess_0\dots,\Statess_m$ be the set of SCCs that partition the directed graph of a game structure.
Then, the defining feature of a weak B\"uchi game with winning condition $\ltlG\ltlF \varphi$ is as follows: Let $\F$ be the set of explicit states that satisfy the assertion $\varphi$. Then, for all SCCs $\Statess_i$, either $\Statess\subseteq \F$ or $\Statess\cap\F=\emptyset$.
Thus, the SCCs of a weak B\"uchi game are either {\em accepting components} meaning all of its states are contained in $\F$ or  {\em non-accepting components} meaning none of its states is present in $\F$. 
Then, as stated by the winning condition $\ltlG\ltlF \varphi$, a play in the directed graph is winning for the system if the play ultimately never exits an accepting component. Similarly, a strategy is accepting for the system if it can guarantee that every play will ultimately remain inside an accepting component.



\subsubsection{Weak B\"uchi Games.} 
A B\"uchi game $(\GS, \ltlG\ltlF\varphi)$ is called a {\em weak B\"uchi game} if the game structure $\GS$ has the following special  structure described.

%Intuitively, the partition of the states of the directed graph induced by its {\em strongly connected components} (SCC) have a special property. A strongly connected component is the maximal set of states of a directed graph such that for all pairs of states $s$ and $t$ present in the SCC, there is a path from $s$ to $t$ and there is a path from $t$ to $s$. Then, the property of the SCCs in a weak B\"uchi game is that either all states in an SCC satisfy the assertion $\varphi$ or none of the states of an SCC satisfy the assertion $\varphi$. 


An assertion  $\Statess$ over $\I\cup\O$ is said to be a {\em strongly connected component} (SCC) in a game structure if $S \not\equiv \mathsf{False}$ and for each pair of states $s$ and $t$ over $\I\cup\O$ for which there exist finite-length play prefixes $\pi_{s\rightarrow t}$ and $\pi_{t\rightarrow s}$ such that (a) the first and final states in $\pi_{s\rightarrow t}$ are $s$ and $t$, respectively, and (b) the first and final states in $\pi_{t\rightarrow s}$ are $t$ and $s$, respectively, then $s\models \Statess$ iff $t\models \Statess$. It is easy to prove that the states of a game structure are partitioned by finitely many such components, i.e., there exist distinct SCCs $\Statess_0,\dots,\Statess_m$ such that 
$\bigvee S_j \equiv \mathsf{True}$ and $\forall i,j, \Statess_i\wedge \Statess_j \equiv \mathsf{False}$.



%for every assertion $\Statess_i$, for each pair of states $s$ and $t$ over $\I\cup\O$, if there exist finite-length play prefixes $\pi_{s\rightarrow t}$ and $\pi_{t\rightarrow s}$ such that (a) the first and final states in $\pi_{s\rightarrow t}$ are $s$ and $t$, respectively, and (b) the first and final states in $\pi_{t\rightarrow s}$ are $t$ and $s$, respectively, then $s\models \Statess_i$ and $t\models \Statess_i$.
%Furthermore, for all pairs of states $s$ and $t$ over $\I\cup\O$, if $s\models \Statess_i$ and $t\models\Statess_j$ such that $\Statess_i \neq \Statess_j$, then 
%Intuitively, each $\Statess_i$ corresponds to a {\em strongly connected component} of the induced directed graph. Recall,  a strongly connected component of a directed graph is a maximal set of states such that there is a path in each direction between each pair of states belonging to the component. Then, it is easy to show that $\bigvee S_j \equiv \mathsf{True}$ and $\forall i,j, \Statess_i\wedge \Statess_j \equiv \mathsf{False}$.

Let $\Statess_0\dots\Statess_m$ be the set of SCCs that partition the game structure. Then, these SCCs hold a special property in a weak B\"uchi game with winning condition $\ltlG\ltlF\varphi$. The property is that for all $i$, either $\Statess_i \Rightarrow \varphi$ holds or $\Statess_i \Rightarrow \neg\varphi$. 

%such that (a). for all $\Statess_i$, either for all state if $s \models \Statess_i$ then $s \models \varphi$  or for all state if $s \models \Statess_i$ then $s \models \neg\varphi$, \gatodo{since these are assertions you can just write: "either $S_i\Rightarrow \varphi$, or $S_i\Rightarrow \neg\varphi$" } and (b).  There exists a partial order $\geq$ on the collection of the $\Statess_i$ such that for every state $s \models \Statess_i$ and state $t \models \Statess_j$ for which $(s,t') \models \rho_\I\wedge \rho_\O$, $\Statess_i \geq \Statess_j$  i.e. the transition relation $\rho_I\wedge\rho_O$ is restricted so that in each transition, the graph structure either stays at the same assertion $S_i$ or moves to a assertion smaller in the partial order.



%This is an improvement over GR($k$) games, which are solved in quadratic time in the state 

%Weak B\"uchi games have previously been studied when the states of the game are represented explicitly. Under this state representation, weak B\"uchi games can be solved in linear-time to the size of the explicit graph underlying the game~\cite{Chatterjee08}). 
%(use the reduction from weak B\"uchi to weak parity~\cite{LodingT00}, and apply an algorithm by  Chatterjee~\cite{Chatterjee08}). 
%This section reviews that algorithm.




\subsubsection{BDDs and Symbolic Operations} \dftodo{Revise}

A \emph{Binary Decision Diagram}~\cite{?} (BDD) is a DAG-representation of an assertion. BDD-nodes (which are not leaves) are labeled with variables, BDD-arrows with variable-valuations, and BDD-leaves with true/false. BDDs are considered as a useful representation as they support Boolean operations and further satisfaction quarries that can be computed efficiently~\cite{?}. Various professional tools that implement BDDs exist~\cite{?}.

We say that a BDD $\beta$ is over $\mathcal V_1,\dots,\mathcal V_n$, if it represents an assertion over $\mathcal V_1\cup\cdots\cup \mathcal V_n$. For a BDD $\beta$ over $\mathcal V_1,\dots,\mathcal V_n$ and states $s_1,\dots,s_n$ over $\mathcal V_1,\dots,\mathcal{V}_n$, respectively, we write $\beta(s_1,\dots,s_n)$ if the assertion that
$\beta$ represents is evaluated to $\mathit{true}$ by the states $s_1,\dots,s_n$. For a set of variables $\mathcal V$, we write $\mathcal V=\mathcal V'$ to denote the BDD that represents the assertion $\bigwedge_{v\in \mathcal V}(v=v')$. We also employ the following \emph{symbolic operations}: (1) Boolean operations: $\neg,\vee,\wedge,\rightarrow$ with their standard meaning; (2) For a BDD $\beta$ over $\mathcal{V}_1,\dots, \mathcal V_n$, the BDD $\gamma$ defined by $\exists \mathcal V_n (\beta)$ (respectively, $\forall \mathcal V_n(\beta)$) is a BDD over $\mathcal V_1,\dots,\mathcal V_{n-1}$ that satisfies the following: For states $s_1,\dots,s_{n-1}$ over $\mathcal V_1,\dots,\mathcal V_{n-1}$, respectively, $\gamma(s_1,\dots,s_{n-1})$ if there exists (respectively, for every) state $s_n$ over $\mathcal V_n$, $\beta(s_1,\dots,s_n)$.

We use BDDs to model sets (e.g. winning regions) and memory-less strategies. A BDD $\beta$ over $\mathcal V$ represents a set $S\subseteq 2^\mathcal V$ in a natural manner: $S=\{s: \beta(s)\}$. A BDD $\beta$ over $\I,\O,\I',\O'$ represents a memory-less strategy $f^s$ as follows: $\beta(\inp_0,\out_0,\inp_1',\out_1')$ if $f^s(\pi,(\inp_0,\out_0),\inp_1)=\out_1$ for $\pi\in (2^{\I\cup\O})^*$ such that $(\pi,(\inp,\out))$ is consistent with $f^s$, and $(\inp_0,\out_0,\inp_1')\models \rho_\I$. We present symbolic constructions of strategies. That is, algorithms that construct BDDs that represent memory-less strategies. Time is measured in \#symbolic-operations performed. 


%\input{Section/explicitprelims}
